Multiplier Bootstrap-based Exploration

Despite the great interest in the bandit problem, designing efficient algorithms for complex models remains challenging, as there is typically no analytical way to quantify uncertainty. In this paper, we propose Multiplier Bootstrap-based Exploration (MBE), a novel exploration strategy that is applicable to any reward model amenable to weighted loss minimization. We prove both instance-dependent and instance-independent rate-optimal regret bounds for MBE in sub-Gaussian multi-armed bandits. With extensive simulation and real data experiments, we show the generality and adaptivity of MBE.

==> 9_Main_proof.tex <==


\section{Proof of Theorem \ref{thm.MAB}}\label{proof_thm}


Before starting our proof, we first give the definition of sub-exponential variables. To be specific, we call a \textit{zero-mean} variable $X$ sub-exponential with parameters $\lambda$ and $\alpha$ if
\[
    \E \exp \{ t X \} \leq \exp \left\{ \frac{t^2 \lambda^2}{2}\right\}, \qquad |t| \leq \frac{1}{\alpha} ,
\]
denoted as $X \sim \subE(\lambda, \alpha)$. Specially, we denote $\subE(\lambda) := \subE(\lambda, \lambda)$. 
Similar to the sub-Gaussian variables, we have the following concentration {property}
\[
    \pr (X \geq t) \leq \exp \left\{ - \frac{1}{2} \left( \frac{t^2}{\lambda^2} \wedge \frac{t}{\alpha}\right) \right\}, \qquad  {\forall} \, t \geq 0.
\]

%\red{(Move to the main text?)} 
%Now suppose each arms' rewards' setting is as follows:
%\begin{itemize}
    %\item $\{ R_{k, \ell}\}$ are sub-Gaussian independent sample such that $\mu_k = \E R_{k, \ell} \in [0, 1]$ with finite sub-Gaussian parameter $\sigma_k^2 $.
%\end{itemize}

%Recall that the quantity of what we care about is the sum of our cumulative regret:
%\[
    %\operatorname{Reg}_{T} := \E \operatorname{Reg}_{T}(Y,\mathcal{A}) = \E \sum_{t=1}^{T} [R_1 - R_{A_{t}}]=\sum_{k=2}^{K} \Delta_{k} \E \Big[\sum_{t=1}^{T} 1 \left\{A_{t}=k\right\}\Big],
%\]
%where we assume $\mu_1 = \max_{k \in [K]} \mu_k$. In other words, the first arm
%is the best arm with the {highest} expected reward. We want to show $\operatorname{Reg}_T$ can be bounded by a log regret, i.e. $C \times\log T$ for any $T \in \mathbb{N}$ under Algorithm 3. 
%Here $C$ is free of the round $T$. 
%\red{(Bounded by the order is not correct. Either "has the same order with xxx", or bounded by xxx. Any if you talk about order, there is no need to say $\forall T$, by definition.)} 



\subsection{Basic Idea}

% Here we want to use is the following lemma, which is a  decomposition of the cumulative regret as 
Our proof relies on the following decomposition of the cumulative regret from \cite{kveton2019garbage}. 
We will recap its proof in Appendix \ref{sec:proof_lemma} for completeness. Let the history of arm $k$ after $s$ pulls be a set $\his_{k, s}$ of cardinality $s$, $Q_{k, s} (\tau) := \pr \big( \overline{Y}_{k, s} > \tau \, | \his_{k, s} \big)$ be the tail probability that $\overline{Y}_{k, s}$ conditioned on history $\his_{k, s}$ is a least $\tau$ for some tunable parameter $\tau$, and $N_{k, s} (\tau) := 1 / Q_{k, s} (\tau) - 1$.
\begin{lemma}\label{lem.a.b}
% When we select arms according to the
Suppose in MAB we select arms according to the rule 
$A_t = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 
% in the MAB problem, then 
Then for any $\{ \tau_k \}_{k = 2}^K \subseteq \mathbb{R}^{K - 1}$, 
the expected $T$-round regret can be bounded above as
\[
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\]
where
\[
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] =: \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1 =: \sum_{s = 0}^{T - 1} b_{k, s} + 1.
\]
\end{lemma}
Recall the summation index $s$ is the time we pull the $k$-th arm in the total $T$ round{s}. 
%\red{[(a and b) are just numbers, and they can not control anything. They represent something, and bounding them means something is controlled.]}
The definition of $a_{k}$ and $b_{k}$ have important meaning, $a_{k}$ represents the expected number of rounds that optimal arm $1$ has been being underestimted, while $b_{k}$ is the probability that the suboptimal arm $k$ is being overestimated.
%$a_k$ represents that the  probability of pulling the optimal arm is not too small in its tails, while $b_k$ is the tail probabilities of rewards of all arms are not too large. 
%\red{[A general comment: I suggest adding more "," and prepositions such as "that" to provide a better flow. Omitting them is convenient for ourselves, but not the readers. 
Here we only need to consider the lower bound of the tail of the distribution of the rewards from the optimal arm. 
%\red{(Like commented last time, an arm does not have a tail, but its reward distribution has. As commented above, clarifying the logic will help our proof as well.)}
The intuition is: (i) we only need the rewards from the optimal arm taking a relatively large value with a probability that is not too small; (ii) we do not care about the tiny probability of a large reward from suboptimal arms. 
%\red{(this is part of the intuition; should not put a "." here. Maybe something like "the intuition is that (i) xxx and (ii) xxx.)}
% And this Lemma is valid for any algorithm in MAB problem as long as the action step is $A_{t} = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 


In the following steps, we will bound $a_k$ and $b_k$ separately up to order $\log T$. Denote $\pr_{\xi}(A)$ is the probability of event $A$ concerning the law of $\xi$ and taking other quantities as deterministic. Recall that we denote two functions $a(s, T) \lesssim b(s, T)$ if $a(s, T) \leq c \times b(s, T)$ for some constant $c$ free of $s$ and $T$. 
And we write $a(s, T) \asymp b(s, T)$ if both $a(s, T) \lesssim b(s, T)$ and $a(s, T) \gtrsim b(s, T)$. 
The proof of all lemmas can be found in Appendix \ref{sec:proof_lemma}. 

\subsection{Bounding $a_k$}
%\red{Grammar: Should be split into two sentence. "(we) recall" is one and "it is" is another.}
%Recall that our target is bounding $a_k$ and $b_k$ up to order $\log T$, it is enough to show that {this can hold}
%for 
%{any large enough} $T$. 

For bounding $a_{k}$ with $C\log T$ for some constant $C > 0$, we will need first prove a weaker statement: $a_{k, s}$ as a function of $T$ can be upper bounded by some constants free of $T$. As we can see later, this is a critical intermediate step for proving $a_{k, s}$ has an order $\log T$.
%This is a   
%\red{$a_{k,s}$ is ONE constant, and bounded by constants? I know what you want to say. Just be more careful with these wordings. }
%weaker condition for $a_{k} \lesssim \log T$. 
%\blue{And we will see later control $a_{k, s}$ with a constant is a critical intermediate step to bound 
%\[
    %\log T \gtrsim a_k = \sum_{s = 0}^{T - 1} a_{k, s} \underbrace{\lesssim T}_{\text{by bounding $a_{k, s}$ with a constant.}}.
%\]}
%\red{Why we want to do this first? Tell readers the motivation/plan.}

\subsubsection{Bounding $a_{k,s}$ by constant}
Note that if we take
%\red{If one equation will not be cited, we should not give it an index}
\begin{equation}\label{requirement_0}
    \tau_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda},
\end{equation}
then we will have
\begin{equation}\label{constant_bound}
    \begin{aligned}
    	a_{k, s} & = \E \left[ \left( \frac{1}{Q_{1, s}(\tau_k)}  - 1\right) \wedge T \right] \\
    	(\text{by } Q_{1, s}(\cdot) \text{ is decreasing})&\leq \E \frac{1}{Q_{1, s}(\tau_k)} \leq \E Q_{1, s}^{-1} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right),
    \end{aligned}
\end{equation}
Hence, we need to find a lower bound of %\red{(Maybe I am wrong): lower bound is not a verb. Bound from below or sth else.} 
the tail probability $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right) = \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right)$. And throughout the proof, we will use the choice of \eqref{requirement_0} for $\tau_k$, and we can take advantage of the bound \eqref{constant_bound}. 

For further analyzing \eqref{constant_bound}, we write it as the probability with respect to the weighted random summation of Gaussian random variable $\{ \omega_i, \omega_i', \omega_i''\}$.

%\red{
%\begin{lemma}\label{lemma:gaussian_weight}
    %Suppose $\{x_i, y_i, z_i\}_{i = 1}^n \subseteq \mathbb{R}$ and $\{ \omega_i, \omega_i', \omega_i''\}_{i = 1}^n$ i.i.d. $\mathcal{N} (1, \sigma_{\omega}^2)$ random variables, then 
    %\[
        %\begin{aligned}
            %& \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{ i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \right)\\
            %\geq & \exp \left\{-\frac{3\left(S_{x}-S_{y}-S_{z}\right)^{2}}{2 \sigma_{\omega}^{2}\left(T_{x}+T_{y}+T_{z}\right)}\right\}\times\ind \left(S_{x} \geq S_{y}+S_{z}+\sqrt{2 \pi}\right)+(1-\Phi(\sqrt{2 \pi})) \times\ind \left(S_{x} \leq S_{y}+S_{z}+\sqrt{2 \pi}\right),
    %\end{aligned}
    %\] 
    %if $T_x + T_y + T_z \neq 0$. Furthermore, if $S_x + S_y + S_z \neq 0$, we will have 
    %\[
        %\begin{aligned}
            %& \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{ i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \right)\\
            %\geq & \exp \left\{-\frac{3\left(S_{x}-S_{y}-S_{z}\right)^{2}}{2 \sigma_{\omega}^{2} / n \left(S_x + S_y + S_z\right)^2}\right\} \times\ind \left(S_{x} \geq S_{y}+S_{z}+\sqrt{2 \pi}\right)+(1-\Phi(\sqrt{2 \pi})) \times\ind \left(S_{x} \leq S_{y}+S_{z}+\sqrt{2 \pi}\right),
        %\end{aligned}
    %\] 
    %where $S_x = \sum_{i = 1}^n x_i$ and $T_x = \sum_{i = 1}^n x_i^2$. And $S_y, S_z, T_y, T_z$ are similarly defined. 
%\end{lemma}
%}

Let $x_i := (2 \lambda + 1) R_{1, i} - (\mu_1 + \lambda)$, $y_i := \lambda (\mu_1 - 1 - \lambda) $, $z_i :=  \lambda (\lambda + \mu_1) $ for $i \in [s]$, then
\[
    S_x = \sum_{i = 1}^s x_i = s \big( (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big), \quad S_y = \sum_{i = 1}^s y_i = s \lambda (\mu_1 - 1 - \lambda), \quad S_z = \sum_{i = 1}^s z_i = s \lambda (\lambda + \mu_1),
\]
with $S_x - S_y - S_z = s (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1)$ and
\[
    T_x = \sum_{i = 1}^s x_i^2 = \sum_{i = 1}^s \big[  (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big]^2, \quad T_y = \sum_{i = 1}^s y_i^2 = s \lambda^2 (\mu_1 - 1 - \lambda)^2, \quad T_z = \sum_{i = 1}^s z_i^2 = s \lambda^2 (\lambda + \mu_1)^2,
\]
with $T_x + T_y + T_z = \sum_{i = 1}^s \big[  (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big]^2  + s \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]$. Let $Z$ be the standard Gaussian variable. For a standard Gaussian variable $Z$, we have the follow lemma.
\begin{lemma}\label{lemma:gaussian_weight}
	Let $Z$ be standard Gaussian variable, then the tail probability satisfies
	\[
	    \frac{1}{4} \exp (- x^2 ) < \pr(Z > x) \leq \frac{1}{2} \exp ( - {x^2} / {2} )
	\]
	for any $x \geq 0$. 
\end{lemma}
%And we first consider the case that $\mu_1 \neq {1} / {2}$. By applying Lemma \ref{lemma:gaussian_weight}
Then we write the probability as
\[
    \begin{aligned}
        & Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) \\
        = & \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right) \\
        = & \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \big( (2 \lambda + 1) R_{1, i} - (\mu_1 + \lambda) \big)\omega_i > \lambda (\mu_1 - 1 - \lambda) \sum_{i = 1}^s \omega_i' + \lambda (\lambda + \mu_1) \sum_{i = 1}^s \omega_i'' \right).
    \end{aligned}
\]
Hence, by applying the first inequality in Lemma \ref{lemma:gaussian_weight} and use the fact that $T_x + T_y + T_z \geq T_z \geq s \lambda^4$, one cannot give a valid tuning condition.
\[
    \begin{aligned}
        & Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) \\
        = & \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s x_i \omega_i - \sum_{i = 1}^s y_i \omega_i' -   \sum_{i = 1}^s z_i \omega_i'' > 0 \right) \\
        = & \pr_{Z} \left( Z > \frac{- (S_x - S_y - S_z)}{\sigma_{\omega} \sqrt{T_x + T_y + T_z}}\right) \\
        \geq & \frac{1}{2} \times \ind \left( \frac{- (S_x - S_y - S_z)}{\sigma_{\omega} \sqrt{T_x + T_y + T_z}} < 0 \right) + \frac{1}{4} \exp \left\{ - \frac{(S_x - S_y - S_z)^2}{\sigma_{\omega}^2 (T_x + T_y + T_z)} \right\} \times  \ind \left( \frac{- (S_x - S_y - S_z)}{\sigma_{\omega} \sqrt{T_x + T_y + T_z}} > 0 \right) \\
        \geq & \frac{1}{2} \times \ind \left(S_x - S_y - S_z > 0 \right) + \frac{1}{4} \exp \left\{ - \frac{(S_x - S_y - S_z)^2}{\sigma_{\omega}^2 \cdot s \lambda^4} \right\} \times  \ind \left( S_x - S_y - S_z \leq 0 \right) \\
        = & \frac{1}{2} \ind \left( \overline{R}_{1, s} - \mu_1 > 0 \right) + \frac{1}{4} \exp \left\{ - \frac{s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1 )^2}{\sigma_{\omega}^2\lambda^4}\right\} \ind \left( \overline{R}_{1, s} - \mu_1 \leq 0 \right).
    \end{aligned}
\]
%which gives the lower bound of $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)$ in the last step.
%where the $\geq$ is by the following lemma.
%\red{1. ", by"; 2. equations are also part of the sentence. Avoid a long sentence. Try something like ". the equality/inequality is due to the following lemma."}
where $Z$ again is the standard Gaussian variable and we will use this notation through this proof. Then this result combined with the fact \eqref{constant_bound} gives the upper bound for $a_{k, s}$ as
\[
    \begin{aligned}
    	a_{k, s} & \leq 2 \pr \left( \overline{R}_{1, s} - \mu_1 > 0 \right) + 4  \E \exp \left\{ \frac{s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1 )^2}{\sigma_{\omega}^2\lambda^4}\right\} \ind \left( \overline{R}_{1, s} - \mu_1 \leq 0 \right) \\
    	& \leq 2 + 4  \E \exp \left\{ \frac{s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1 )^2}{\sigma_{\omega}^2\lambda^4}\right\} 
    \end{aligned}
\]
%\[
    %\begin{aligned}
        %a_{k, s} & \leq \E \exp \left\{\frac{3s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2} \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]}\right\}\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        % ~~~~~~~~~~~~~~~~~~~~~~~~ + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times \pr \left( \overline{R}_{1, s} - \mu_1 \leq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \\
        %\leq \E \exp \left\{\frac{3s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2} \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]}\right\}\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}
    %\end{aligned}
%\]
\iffalse
\begin{equation}\label{a_k_constant_2}
    \begin{aligned}
        a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        & ~~~~~~~~~~~~~~ + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times \pr \left( \overline{R}_{1, s} - \mu_1 \leq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \\ 
        & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \ind \left( \mu_1 > \frac{1}{2} \right) \\
        & ~~~~ + \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right)  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        & = : I + II + III, 
        %& \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \\
        %& \qquad + \E \exp \left\{ \frac{3 \pi }{\sigma_{\omega}^2 \big[ (1 + 2 \lambda) \overline{R}_{1, s} - (\mu_1 + \lambda)\big]^2}\right\} 1 \left\{ \mu_1 \leq \frac{1}{2} - \frac{\sqrt{2 \pi}}{2 s \lambda}\right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        %& \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        %& \qquad \qquad \qquad \qquad \qquad \qquad + \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < \frac{1}{2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        %& \leq  \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        %& \qquad \qquad \qquad \qquad \qquad \qquad  + \max_{s \in \mathbb{Z}} \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < \frac{1}{2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        %& \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}
    \end{aligned}
\end{equation}
where $III = \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}$ is a constant. We will bound $I$ and $II$ as follows. 
\begin{itemize}
	\item Bounding $I$: 
	\[
	    \begin{aligned}
	    	I & = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \times\ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	   \alignedoverset{\overline{R}_{1, s} > \mu_1 > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \text{ when } \mu_1 > \frac{1}{2}}{\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \mu_1 +\frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 \ind \left( \overline{R}_{1, s}  \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) }\right\} \\
	    	   %\alignedoverset{\lambda(2 \mu_1 - 1) + \sqrt{2 \pi} / s > 0 \text{ when } \mu_1 > 1 / 2}{\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \\
	    	   %& ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 + \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	  %& \overset{\text{by using both event in the first two indicators}}{=} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2 \ind \left( \overline{R}_{1, s}  > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \\
	    	  %& ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 + \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	  %& {\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \mu_1 +\frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 \ind \left( \overline{R}_{1, s}  \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) }\right\} \\
	    	  & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 > \frac{1}{2} \right)\\
	    	  \alignedoverset{\text{by using } \mu_1 > \frac{1}{2}}{\leq} \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\}  \ind \left( \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \ind \left(  \mu_1 > \frac{1}{2} \right).
	    \end{aligned}
	\]
	
	\item Bounding $II$: 
	
	%Consider two cases: 
	
	%(i) \textit{If $R_{1, s} - \mu_1$ is symmetric about $0$}, then
	%\[
	    %\begin{aligned}
	    	%II & = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%& = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \mu_1 + \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%\alignedoverset{\text{by symmetry}} = \E \exp \left\{ \frac{3 s (\mu_1 - \overline{R}_{1, s})^2}{2 \sigma_{\omega}^2 \left((\mu_1 - \overline{R}_{1, s})  +  \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)^2 }\right\} \times \ind \left( \mu_1 - \overline{R}_{1, s} > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right)  \\
	    	%\alignedoverset{\text{by } \frac{\mu_1 + \lambda}{1 + 2 \lambda} > \mu_1}{\geq} \E \exp \left\{ \frac{3 s (\mu_1 - \overline{R}_{1, s})^2}{2 \sigma_{\omega}^2 \left( \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda} + \frac{\sqrt{2\pi}}{s (2\lambda + 1)}\right)^2 }\right\} \times \ind \left( \mu_1 - \overline{R}_{1, s} > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%& = \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ - \lambda (1 - 2\mu_1) + \sqrt{2 \pi} / s\big]^2}\right\}  \ind \left( \mu_1 - \overline{R}_{1, s }\geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \ind \left(  \mu_1 < \frac{1}{2} \right).
	    %\end{aligned}
	%\]
	
	
	%(ii) \textit{If $R_{1, s} - \mu_1$ is not symmetric about $0$.} 
	We first note under the indicator $\ind\left(\overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)$, we have
	\[
	    \overline{R}_{1, s} > \mu_1 + \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} > \mu_1.
	\]
	The basic idea is the fact that $\E X = \int_0^{\infty} \pr (X > r) \, \mathrm{d} r$ for any positive $X$. Hence, for any $r > 0$,  we consider set that 
	\[
	    \begin{aligned}
	    	E(r, s) & := \left\{ \overline{R}_{1, s} - \mu_1: \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} > r \right\} \\
	    	& = \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r\right\}.
	    \end{aligned}
	\]
	We need to divide the analysis into two cases: (i) $\overline{R}_{1, s} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} $ and (ii)
	$\overline{R}_{1, s} < \frac{\mu_1 + \lambda}{1 + 2 \lambda} $ respectively. We first prove the case (i) since it is easier. Note that 
	\begin{equation}\label{a_k_constant_II_case1}
		\overline{R}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} > \mu_1
	\end{equation}
	when $\mu_1 < \frac{1}{2}$. Hence we can write $E(r, s)$ on condition \eqref{a_k_constant_II_case1} as
	\[
	    \begin{aligned}
	    	E(r, s) \alignedoverset{\text{by \eqref{a_k_constant_II_case1}}}{=} \left\{  \overline{R}_{1, s} - \mu_1 : \frac{\sqrt{3 s} (\overline{R}_{1, s} - \mu_1)}{\sqrt{2} \sigma_{\omega} \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)} > \sqrt{\log r}\right\} \\
	    	& = \left\{  \overline{R}_{1, s} - \mu_1 : \sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} > \left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right) (\overline{R}_{1, s} - \mu_1) \right\} \\
	    	& = \left\{ \begin{array}{ll}
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} > 0 >  \left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right) (\overline{R}_{1, s} - \mu_1) \right\}, & r \leq \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}, \\
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \frac{\sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}}{\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} > (\overline{R}_{1, s} - \mu_1) \right\}, & r > \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} 
	    	\end{array}\right. \\
	    	\alignedoverset{\text{by \eqref{a_k_constant_II_case1} again}}{=} \left\{ \begin{array}{ll}
	    		\left\{ \overline{R}_{1, s} - \mu_1 \in \mathbb{R} \right\}, & r \leq \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}, \\
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} > (\overline{R}_{1, s} - \mu_1) \right\}, & r > \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} 
	    	\end{array} \right. 
	    \end{aligned}
	\]
	Then,
	\[
	    \begin{aligned}
	    	II & = \int_0^{\infty} \pr \left( E(r, s) \, \cap \, \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& = \left[ \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} + \int_{\exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}}^{\infty} \right] \pr \left( E(r, s) \, \cap \, \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& = II_1 + II_2.
	    \end{aligned} 
	\]
	We first bound $II_2$. Write $II_2$ as
	\[
	    II_2 = \int_{\exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}}^{\infty} \pr \left( \frac{\lambda(1 - \mu_1)}{1 + 2 \lambda} < \overline{R}_{1,s} - \mu_1 <  \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} \right) \, \mathrm{d} r.
	\]
	By letting $s \longrightarrow \infty$,
	\[
	    \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} \, \uparrow \, \infty, \qquad \left\{ \frac{\lambda(1 - \mu_1)}{1 + 2 \lambda} < \overline{R}_{1,s} - \mu_1 <  \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} \right\}  \, \downarrow \, \varnothing,
	\]
	hence we have $II_2 \longrightarrow 0$. This implies  there exist $T_1 \in \mathbb{N}$ such that $II_2 \leq 1$ for any $s \geq T_1$. And for $II_1$, we take advantage of sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	II_1 & = \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( E(r, s) \ind \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& \leq \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \, \mathrm{d} r \\
	    	& \leq \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( \overline{R}_{1,s} - \mu_1 > \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \right) \, \mathrm{d} r \\
	    	\alignedoverset{\text{by sub-Gaussian inequality}}{\leq} \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}  \cdot \exp \left\{ - \frac{\lambda^2 (1 - 2 \mu_1)^2 s}{2 (1 + 2 \lambda)^2 \sigma_1^2}\right\} \\
	    	& = \exp \left\{ \left[ \frac{3}{2 \sigma_{\omega}^2} - \frac{\lambda^2 (1 - 2 \mu_1)^2}{2 (1 + 2 \lambda)^2 \sigma_1^2} \right] s \right\}.
	    \end{aligned}
	\]
	Therefore, for making $II_1$ have a upper a constant    free of $s$, a sufficient condition is
	\[
	    \frac{3}{2 \sigma_{\omega}^2} - \frac{\lambda^2 (1 - 2 \mu_1)^2}{2 (1 + 2 \lambda)^2 \sigma_1^2} \geq 0
	\]
	i.e.
	\begin{equation}\label{tuning_case_1}
		\lambda > \frac{\sqrt{3}\sigma_1}{(1 - 2\mu_1) \sigma_{\omega} - 2 \sqrt{3}\sigma_1} \qquad  \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{3} \sigma_1}{1 - 2\mu_1}.
	\end{equation}
	Combining these results, we conclude that if take \eqref{tuning_case_1}, we have $II \leq 2$ for any $s \geq T_1$. Now switching to case (ii). In case (ii), we will have:
	\begin{equation}\label{a_k_constant_II_fact1}
		\frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s} > 0 \qquad \text{ and } \qquad \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} < \overline{R}_{1, s} - \mu_1 < \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}.
	\end{equation}
	\[
	    \begin{aligned}
	    	E(r, s) & = \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r\right\} \\
	    	(\text{use \eqref{a_k_constant_II_fact1}}) & \subseteq \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^{2 - \epsilon}}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r \left[\frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}\right]^{-\epsilon}\right\} \\
	    	& =  \left\{  \overline{R}_{1, s} - \mu_1 : \left[ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r}\right]^{2 - \epsilon} > \left[ \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right]^2\right\} \\
	    	& =  \left\{  \overline{R}_{1, s} - \mu_1 : \left[ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r}\right]^{1 - \frac{\epsilon}{2}} > \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right\}
	    \end{aligned}
	\]
	For any $0 < \epsilon < 2$. Specially, we take $\epsilon = 1$, and 
	%We take $1 < \epsilon < \frac{4}{3}$, then $\frac{1}{3} < 1 - \frac{\epsilon}{2} < 1$ and $5 - 3\epsilon > 1$ . And denote the event
	\[
	    F(r, s) := \left\{ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^{3} r} \geq 1 \right\},
	\]
	then
	\[
	    \begin{aligned}
	    	II & = \int_0^{\infty} \pr \left\{ E (r, s)  \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right) \right\} \, \mathrm{d} r \\
	    	& \leq \int_0^{\infty} \left[\pr \left\{ \big[ E (r, s) \, \cap  \, F(r, s) \big] \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right) \right\} + \pr \left\{ \big[ F(r, s)^c \big] \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)\right\} \right]\, \mathrm{d} r \\
	    	& =: II_1 + II_2.
	    \end{aligned}
	\]
	For $II_2$, we write that
	\[
	    \begin{aligned}
	    	II_2 & \leq \int_0^{\infty} \pr \left\{ \big[ F(r, s)^c \big] \, \cap \, \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)\right\}\, \mathrm{d} r  \\
	    	& = \int_0^{\infty} \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \left[ \int_0^{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}} + \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \right] \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, \mathrm{d}r.
	    \end{aligned}
	\]
	For $II_2$, we write that
	\[
	    \begin{aligned}
	    	II_2 & = \int_0^{\infty} \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \left[ \int_0^{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}} + \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \right] \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, \mathrm{d}r.
	    	%\\
	    	%& \leq \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \log^{\frac{1}{2}} r  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{\frac{1}{2}} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, dr \\
	    	% & \leq \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \exp \left\{ - \frac{\log r}{2 (3s)^{\frac{2}{2 - \epsilon}} \sigma_1^2}\right\} \, dr \\
	    	% & = 1 + \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{- \frac{2(1 - \epsilon)}{2 - \epsilon}}\right\}}^{\infty} r^{- \frac{1}{2 (3s)^{\frac{2}{2 - \epsilon}} \sigma_1^2}} \, dr  
	    \end{aligned}
	\]
	By letting $s \longrightarrow \infty$, we have 
	\[
	    \exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\} \longrightarrow \infty, \qquad \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \longrightarrow 0.
	\]
	Thus, $II_2$ shows we must have $II_2 \leq 1$ bounded by a constant free of $s$ for enough big $s$, say $s \geq T_2$.
	And for $II_1$, we take advantage that $x \geq x^{1 - \frac{\epsilon}{2}}$ for $x > 1$ and $0 < 1 - \frac{\epsilon}{2}< 1$, 
	\[
	    \begin{aligned}
	    	& E(r, s) \, \cap \, F(r, s) \\
	    	\subseteq & \left\{  \overline{R}_{1, s} - \mu_1 :  \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r} > \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right\} \\
	    	= & \left\{  \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right\}.
	    \end{aligned}
	\]
	and in turn, we have
	\[
	    \begin{aligned}
	    	 & \big[ E(r, s) \, \cap \, F(r, s) \big] \ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \\
	    	 %\subseteq &  \left\{  \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  \vee\frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right\} \\
	    	 \subseteq & \left\{ \begin{array}{ll}
	    	 	\varnothing, & r \leq \overline{r}_1 (s) \\
	    	 	\left\{ \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right\}, & r > \overline{r}_1(s) 
	    	 \end{array}\right..
	    \end{aligned}
	\]
	where
	\[
	    \overline{r}_1 (s) := \exp \left\{ \left[ \frac{\sqrt{2 \pi}}{\left[ \sqrt{2} \lambda (1 - 2 \mu_1) - 2 \sqrt{\pi} / s\right] \sigma_{\omega}}\right]^{\frac{2}{1 + 3 \epsilon}} \left( \frac{\lambda (1 - 2\mu_1)}{1 + 2\lambda} \right)^{\frac{\epsilon}{1 + 3 \epsilon}} (3s)^{\frac{2(\epsilon - 1)}{(2 - \epsilon)(1 + 3 \epsilon)}}  \right\}.
	\]
	Therefore, 
	\[
	    \begin{aligned}
	    	II_1 & = \left[ \int_{0}^{\overline{r}_1(s)} + \int_{\overline{r}_1(s)}^{\infty} \right] \pr \left( \big[ E(r, s) \, \cap \, F(r, s) \big] \ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \right) \, \mathrm{d} r \\
	    	& \leq \int_{0}^{\overline{r}_1(s)} \pr \left(  \varnothing \right) \, \mathrm{d} r + \int_{\overline{r}_1(s)}^{\infty} \pr \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_1(s)}^{\infty} \pr \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right) \, \mathrm{d} r.
	    \end{aligned}
	\]
	Then, by sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	II_1 & \leq \int_{\overline{r}_1(s)}^{\infty} \exp \left( - \frac{s}{2 \sigma_1^2} \left[ \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right]^2\right) \, \mathrm{d} r \\
	    	\alignedoverset{\text{Cauchy inequality}}{\leq}\int_{\overline{r}_1(s)}^{\infty}  \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r\\ 
	    	& = \left[ \int_{\overline{r}_1(s)}^{\overline{r}_2(s)} + \int_{\overline{r}_2(s)}^{\infty} \right] \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& =: II_{11} + II_{12},
	    \end{aligned}
	\]
	where
	\[
	    \overline{r}_2(s) := \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}} s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}}\right\} 
	\]
	is a higher order of $\overline{r}_1(s)$ due to $0 < 2 (\epsilon - 1) < 2$. For $II_{12}$, 
	\[
	    \begin{aligned}
	    	II_{12} & \leq \int_{\overline{r}_2(s)}^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{2 \cdot 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_2(s)}^{\infty} \exp \left\{ - \frac{s}{8 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2} \right\} \, \mathrm{d} r \, \longrightarrow \, 0
	    \end{aligned}
	\]
	when $s \, \longrightarrow \, \infty$. Thus, there exists a $T_3$ such that, $II_{12} \leq 1$ whenever $s \geq T_3$. Finally, for $II_{11}$, 
	\[
	    \begin{aligned}
	    	II_{11} & \leq \int_{\overline{r}_1(s)}^{{\overline{r}_2(s)}} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{2 \cdot 3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r}\right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_1(s)}^{{\overline{r}_2(s)}} \exp \left\{  - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} r s^{\frac{- \epsilon}{2 - \epsilon}} \right\} \\
	    	& \leq \overline{r}_2(s) \exp \left\{  - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} s^{\frac{- \epsilon}{2 - \epsilon}} \big[ \log \overline{r}_2(s) \big]^{1 + 3\epsilon} \right\} \\
	    	& = \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}} s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}} - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} s^{\frac{- \epsilon}{2 - \epsilon}} \big[ \log \overline{r}_2(s) \big]^{1 + 3\epsilon}  \right\} \\
	    	& = \exp \left\{C_1 \cdot s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}} - C_2 \cdot s \right\} \, \longrightarrow \, 0
	    \end{aligned}
	\]
	when $s \, \longrightarrow \, \infty$, where $C_1$ and $C_2$ are some positive constants free of $s$. Again, when $s \, \longrightarrow \, \infty$. Thus, there exists a $T_4$ such that, $II_{11} \leq 1$ whenever $s \geq T_4$.
	\iffalse
	\red{
	Therefore, by sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	& \pr \left( E(r, s) \, \cap \, F(r, s)  \, \cap \,\left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \right)\\
	    	& = \pr \\
	    	& \leq 1 + \int_1^{\infty} \exp \left( - \frac{s}{2 \sigma_1^2} \left[ \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right]^2 \right) \, \mathrm{d}r \\
	    \alignedoverset{\text{Cauchy inequality}}{\leq} 1 + \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r\\
	    	& = 1 + \left[ \int_1^{\overline{r}(s)} +\int_{\overline{r}(s)}^{\infty}\right] \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& = : 1 + II_{21} + II_{22}:
	    \end{aligned}
	\]
	where $\overline{r}(s)$ is defined as 
	\[
	     \overline{r}(s) := \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3 s^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}}\right\}.
	\]
	For $r \leq \overline{r}(s)$, we have $3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r \geq 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}$, hence
	\[
	    \begin{aligned}
	    	II_{21} & \leq \int_1^{\overline{r}(s)} \exp \left(  - \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} rs^{\frac{2(1 - \epsilon)}{2 - \epsilon}}\right) \, d r \\
	    	& \leq \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} r s^{\frac{2(1 - \epsilon)}{2 - \epsilon}}\right) \, d r \\
	    	& \overset{\text{take } s = 1}{\leq}  \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{6 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 } r\right) \, d r \\
	    	& = \int_1^{\infty} r^{-  \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon}} \, d r
	    \end{aligned}
	\]
	Therefore, for making $II_{21}$ have a upper bound free of $s$, a sufficient condition is 
	\[
		\frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda} \right]^1 > 1
	\]
	i.e.
	\begin{equation}\label{tuning_sigma}
	    \lambda > \frac{12 \sigma_1^2}{(1 - 2\mu_1) \sigma_{\omega}^2 - 24 \sigma_1^2} \qquad \text{ and } \qquad \sigma_{\omega} > \frac{2 \sqrt{6} \sigma_1}{1 - 2\mu_1}
	\end{equation}	
	For $II_{22}$, we have
	\[
	    \begin{aligned}
	    	II_{22} \leq \int_{\overline{r}(s)}^{\infty} \exp \left\{ - \frac{1}{4 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2} s^2\right\} \, dr \longrightarrow 0
	    \end{aligned}
	\]
	when $s \longrightarrow \infty$, {there exist a $T_1$ such that $s \geq T_1$, $II_{22} < 1$.}}
	\fi
\end{itemize}
\fi
%Plug the above two bounds into \eqref{a_k_constant_2}, we obtain that
From the above expression, for proving $a_{k, s}$ is bounded by a constant free of $s$, it remains to show the expectation
\begin{equation}\label{a_k_constant_3}
	\E \exp \left\{ \frac{s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1 )^2}{\sigma_{\omega}^2\lambda^4}\right\} 
\end{equation}
%\begin{equation}\label{a_k_constant_3}
	%\begin{aligned}
		%a_{k, s} \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \ind \left(\mu_1 \neq \frac{1}{2}\right) + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
	%\end{aligned}
%\end{equation}
%with $\mu_1 \neq \frac{1}{2}$ is bounded by a constant free of $s$.
%For bounding the expectation in \eqref{a_k_constant_3}, 
We need the following lemma.
%It can be seen that this upper bound consists {of} three parts: the first part is the moment generation function (MGF) of the square of the sample mean $\overline{R}_{1, s} - \mu_1$, the second part is a function of $(\mu_1, \lambda, \sigma_{\omega}^2)$, and the third part is just a constant $\big[ 1 - \Phi(\sqrt{2 \pi}) \big]^{-1} $. Note that as long as $\frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)}$ is not an integer, the second part must be a finite number free of $s$. It remains to deal with the first part, we use the following lemma.

%Now for $\mu_1 \neq 1 / 2$, notice that ${R}_{1, i} - \mu_1$ for $i \in [s]$ is sub-Gaussian. 
%For dealing with the expectation, we need the following lemma.
%\red{Same comment as above. The sentence is just too long. Imagine you are presenting. We need rests between sentences. }
% by the fact with the following lemma.
\begin{lemma}\label{lem_subGtosubE}
    Suppose $\{X_i\}_{i = 1}^n$ are i.i.d. zero-mean sub-Gaussian with variance proxy $\sigma^2$, and $\overline{X} = \frac{1}{n} \sum_{i = 1}^n X_i$, then
    \[
        \E \exp\big( \lambda\overline{X}^2 \big) \leq e^{9 / 8}
        %\exp \left\{ \frac{64 \lambda^2 \sigma^4}{n^2} + \frac{\lambda \sigma^2}{n}\right\}, \qquad \forall \, |\lambda| \leq \frac{n}{8 \sqrt{2} \sigma^2}
    \]
    for any $|\lambda| \leq \frac{n}{8 \sigma^2}$.
\end{lemma}
\iffalse
Lemma \ref{lem_subGtosubE} ensures the expectation in \eqref{a_k_constant_3}
%\[
    %\begin{aligned}
    	%& \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2}\right\} \\
    	%= & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2} \cdot (\overline{R}_{1, s} - \mu_1)^2 \right\} \leq e^{9 / 8}.
    %\end{aligned}
%\]
\[
    \begin{aligned}
        & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \ind \left( \mu_1 > {1} / {2} \right) \\
        = & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2} \times(\overline{R}_{1, s} - \mu_1)^2 \right\} \ind \left( \mu_1 > {1} / {2} \right)  \leq e^{9/8} \times\ind \left( \mu_1 > {1} / {2} \right)
    \end{aligned}
\]
as long as we take
%\begin{equation}\label{cond.1}
    %\frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2} \leq \frac{s}{8 \sigma_1^2}.
%\end{equation}
\begin{equation}
\label{cond.1}
    \frac{3 s (1 + 2 \lambda)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2} \leq \frac{s}{8 \sigma_1^2}.
\end{equation}
%we will obtain $a_{k, s}$ is bounded by 
%\begin{equation}\label{a_k_constant}
    %a_{k, s} \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
%\end{equation}
%\red{If time permits, we should polish the proof for several more times to address issues as raised above.}
%\begin{remark}
   %Lemma \ref{lem_subGtosubE} actually is a special case for the fact that the mean of iid sub-Weibull sample with sample size $n$ will have the local sub-Gaussian property in the interval up to $\sqrt{n}$.
%\end{remark}
%{\color{blue}{More details about the tuning parameters. }}
The condition \eqref{cond.1} is equal to 
%\begin{equation}\label{tuning_condition}
    %\frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2}  \leq \frac{\sigma_{\omega}}{2 \sigma_1}.
%\end{equation}

%for bound $a_{k, s}$ with a constant, we write the inequality with regarding $\lambda$ as
%\begin{equation}\label{tuning_condition}
    %\big[ (2 \mu_1 - 1)^2 \sigma_{\omega}^2 - 48 \sigma_1^2 \big] \lambda^2 - 2 \big[ 24 \sigma_1^2 - \sqrt{2 \pi} / s (2 \mu_1 - 1) \sigma_{\omega}^2\big] \lambda - \big[ 12 \sigma_1^2 - (2 \pi / s^2) \sigma_{\omega}^2 \big] \geq 0. 
%\end{equation}
%\begin{equation}\label{tuning_condition}
    %\big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big] \lambda \geq 2 \sigma_1.
%\end{equation}
\begin{equation}\label{tuning_condition}
    \frac{\sqrt{3} (1 + 2 \lambda)}{\lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s } \leq \frac{\sigma_{\omega}}{2 \sigma_1}.
\end{equation}
Hence it is enough to ask $\lambda (2 \mu_1 - 1) > {2 \sqrt{3} \sigma_1} (1 + 2 \lambda) / \sigma_{\omega}$, i.e.
    \[
        \lambda \left[ 2 \mu_1 - 1 - \frac{4 \sqrt{3} \sigma_1}{\sigma_{\omega}}\right] >  \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}}.
	\]
Solving the above inequality for positive $\lambda$ and $\sigma_{\omega}$ and we get that 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}.
	\]
\iffalse
\begin{itemize}
	\item If $\mu_1 > 1 / 2$, the above inequality is equal to 
	\[
	    \lambda (2 \mu_1 - 1) + \frac{\sqrt{2\pi}}{s} > \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}} (1 + 2 \lambda).
	\]
	And hence it is enough to ask $\lambda (2 \mu_1 - 1) > {2 \sqrt{3} \sigma_1} (1 + 2 \lambda) / \sigma_{\omega}$, i.e.
    \[
        \lambda \left[ 2 \mu_1 - 1 - \frac{4 \sqrt{3} \sigma_1}{\sigma_{\omega}}\right] >  \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}}.
	\]
	Solving the above inequality for positive $\lambda$ and $\sigma_{\omega}$ and we get that 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}.
	\]
	\item If $\mu_1 < 1 / 2$, the above inequality is equal to 
	\[
	    \lambda (1 - 2\mu_1) + \frac{\sqrt{2\pi}}{s} > \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}} (1 + 2 \lambda).
	\]
	Similar to the case of $\mu_1 > 1 / 2$, the solution is 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(1 - 2 \mu_1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {1 - 2 \mu_1}.
	\]
\end{itemize}
\fi
%Use the case $\mu_1 > 1 / 2$. 
%Since in this case, we already have $(2 \mu_1  - 1) > 0$ in the indicator, we can get the solution of \eqref{cond.1} as follows

%And solve it, and we can get regularity condition for tuning parameter $(\lambda, \sigma_{\omega}^2)$ is  
%\[
    %\sigma_{\omega}^2 > \frac{48 \sigma_1^2}{(2 \mu_1 - 1)^2}, \qquad \lambda \geq \frac{- \sqrt{2 \pi } \left(2 \mu _1-1\right) \sigma
   %_{\omega }^2 + 2 \sqrt{3} s \sqrt{\frac{\sigma _1^2 \left(4 \mu _1^2 s^2+s^2-4 \mu _1
   %\left(s+2 \sqrt{2 \pi }\right) s+4 \sqrt{2 \pi } s+8 \pi \right) \sigma _{\omega
   %}^2}{s^2}} + 24 s \sigma _1^2}{s \left(\left(1-2 \mu _1\right)^2 \sigma
   %_{\omega }^2 - 48 \sigma _1^2 \right)}
%\]
%i.e.
%\begin{equation}\label{tuning_condition_exact}
    %\sigma_{\omega}^2 > \frac{48 \sigma_1^2}{(2 \mu_1 - 1)^2}, \quad \lambda \geq  \frac{ - \sqrt{2 \pi } \left(2 \mu _1-1\right) \sigma _{\omega }^2+2 \sqrt{3}
    %\sqrt{\left(\left(4 \mu _1^2-\left(4+8 \sqrt{2 \pi }\right) \mu _1+4 \sqrt{2 \pi }+8
   %\pi +1\right) \sigma _1^2 \sigma _{\omega }^2\right)} + 24 \sigma _1^2}{\left(1-2 \mu _1\right){}^2 \sigma _{\omega }^2 - 48 \sigma
   %_1^2}.
%\end{equation}
Hence, in the case $\mu_1 \neq \frac{1}{2}$, we can take the tuning condition as 
\begin{equation}\label{tuning_condition_exact}
    \begin{aligned}
    	& \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}, \qquad \text{ for } \qquad \mu_1 > \frac{1}{2} \\
    	& \lambda > \frac{\sqrt{3}\sigma_1}{(1 - 2\mu_1) \sigma_{\omega} - 2 \sqrt{3}\sigma_1} \qquad  \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{3} \sigma_1}{1 - 2\mu_1}, \qquad \text{ for } \qquad \mu_1 < \frac{1}{2}.
    \end{aligned}
\end{equation}	

\iffalse
\begin{equation}\label{tuning_condition_exact}
	\begin{aligned}
		 & \text{if the distribution of reward is symmetric:} \\
		 & ~~~~~~~~~~~~~~~~~~~~~ \lambda > \frac{2 \sqrt{3} \sigma_1}{|2 \mu_1 - 1| \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {|2 \mu_1 - 1|}  \\
	    & \text{if the distribution of reward is not symmetric} \\
	    & ~~~~~~~~~~~~~~~~~~~~~ \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1 - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1} \qquad \text{ for } \mu_1 > \frac{1}{2} \\
	    & ~~~~~~~~~~~~~~~~~~~~~ \lambda >  \frac{12 \sigma_1^2}{(1 - 2\mu_1) \sigma_{\omega}^2 - 24 \sigma_1^2} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{6} \sigma_1}{1 - 2\mu_1} \qquad \text{ for } \mu_1 < \frac{1}{2}
	\end{aligned}
\end{equation}
\fi
%and \eqref{a_k_constant_3} will give $a_{k, s} \leq \Big[ e^{9 / 8} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \Big] \ind \left(\mu_1 \neq \frac{1}{2}\right)$.
%\begin{equation}\label{tuning_condition_exact}
    %\lambda \geq \frac{2 \sigma_1}{\big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big]} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sigma_1}{2 \mu_1 - 1}.
%\end{equation}
%Directly, for the case $\mu_1 < 1 / 2$, we just need $\frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)} \in \mathbb{Z}$.
%This means under the case that $\mu_1 \neq 1 / 2$, if the tuning parameters $(\lambda, \sigma_{\omega}^2)$ satisfying \eqref{tuning_condition_exact}, the bound in \eqref{a_k_constant_2} will be further bounded by
%\begin{equation}\label{a_k_constant}
    %a_{k, s} \leq e^{9 / 8} 1 \{ \mu_1 > 1 / 2 \}  + \max_{s \in \mathbb{Z}} \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < {1} / {2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
%\end{equation}

For the case $\mu_1 = \frac{1}{2}$, we analyze it separately, $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)$ will become
\[
    \begin{aligned}
        Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) & = Q_{1, s} \left(\frac{1}{2}\right) \\
        & = \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \left( R_{1, i} - \frac{1}{2} \right) \omega_i > \frac{\lambda}{2} \sum_{i = 1}^s (\omega_i'' - \omega_i')  \right) \\
        & = \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \big( R_{1, i} - \mu_1 \big) \omega_i > \frac{\lambda}{2} \sum_{i = 1}^s (\omega_i'' - \omega_i')  \right) \\
        & = \pr_Z \left( Z > \frac{- s(\overline{R}_{1, s} - \mu_1)}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right) \\
        & \geq \ind \left( \overline{R}_{1, s} - \mu_1 \geq 0 \right) \times\frac{1}{2} + \ind \left( \overline{R}_{1, s} - \mu_1 < 0 \right) \times\pr_Z \left( Z > \frac{ s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right).
    \end{aligned}
\]
where $Z \sim \mathcal{N}(0, 1)$ is the standard Gaussian variable. 
And then by the inequality $\pr (Z \geq x) \geq e^{-x^2} / 4$ for any $x > 0$ in \cite{zhang2022sharper}, we will have
\[
     \begin{aligned}
        & \pr_Z \left( Z > \frac{s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right) \\
        (\text{by Cauchy inequality})\geq & \pr \left( Z \geq \frac{s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega} \sqrt{s (\mu_1 - \overline{R}_{1, s})^2 + \lambda^2 s  / 2}} \right)  \\
        \geq & \frac{1}{4} \exp\left\{ - \frac{s(\mu_1- \overline{R}_{1, s})^2}{4 (\mu_1- \overline{R}_{1, s})^2 + 2 \lambda^2} \right\}.
     \end{aligned}
\]
Therefore, by the fact \eqref{constant_bound} and Lemma \ref{lem_subGtosubE} again,
\[
    \begin{aligned}
        a_{k, s} & \leq Q_{1, s} \left(\frac{1}{2}\right) \\
        & \leq 2 \pr \left( \overline{R}_{1, s} - \mu_1 \geq 0 \right) + 4 \E \exp \left\{ \frac{s(\mu_1- \overline{R}_{1, s})^2}{4 (\mu_1- \overline{R}_{1, s})^2 + 2 \lambda^2} \right\} \\
        & \leq 2 + 4 \E \exp \left\{ \frac{s(\mu_1- \overline{R}_{1, s})^2}{ 2 \lambda^2} \right\} \\
        \alignedoverset{\text{apply Lemma \ref{lem_subGtosubE}}}{\leq} 2 \left( 1 + 2 e^{9 / 8} \right),
    \end{aligned}
\]
as long as we take
\[
    \frac{s}{2 \lambda^2} \leq \frac{s}{8 \sigma_1^2}
\]
which is equivalent to $\lambda \geq 2 \sigma_1$. 
%The result for $\mu_1 = \frac{1}{2}$ together with the results for the case $\mu_1 \neq \frac{1}{2}$, we get that for any $\mu_1 \in [0, 1]$, take 
%\begin{equation}\label{tuning_condition_exact_final}
    %\lambda \geq \frac{ 2 \sigma_1 1 (\mu_1 > 1 / 2) }{ \big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big]} + 2\sigma_1 1 (\mu_1 = 1 / 2) \quad \text{ and } \quad \frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)} \not\in \mathbb{Z}_+ \quad \text{ with } \quad \sigma_{\omega} > \frac{4 \sigma_1}{2 \mu_1 - 1},
%\end{equation}
\fi

By applying Lemma \ref{lem_subGtosubE}, we know that \eqref{a_k_constant_3} can be upper bounded by $e^{9 / 8}$, if we take
\[
    \frac{s(2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^4} \leq \frac{s}{8 \sigma_1^2}.
\]
A sufficient condition for this is
\[
    \frac{s(2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^4} \leq \frac{s}{16 \sigma_1^2}, \qquad \lambda^2 - \frac{8\sigma_1}{\sigma_{\omega}} \lambda - \frac{4 \sigma_1}{\sigma_{\omega}} \geq 0,
\]
i.e.
\begin{equation}\label{tuning_condition_exact}
	\lambda \geq \frac{4 \sigma_1}{\sigma_{\omega}} + \sqrt{\frac{4\sigma_1}{\sigma_{\omega}} \left( \frac{4 \sigma_1}{\sigma_{\omega}} + 1\right)}.
\end{equation}

%Combine the results for case of $\mu_1 \neq \frac{1}{2}$ and $\mu_1 = \frac{1}{2}$, $a_{k, s}$ has a constant upper bound as follows:
Therefore, if we take the tuning parameters $\lambda$ and $\sigma_{\omega}$ as in \eqref{tuning_condition_exact}, then $a_{k, s}$ will be bounded by a constant as 
\begin{equation}\label{a_k_constant_final}
	a_{k, s} \leq 2 + 4 e^{9 / 8}.
\end{equation}
%\begin{equation}\label{a_k_constant_final}
    %\begin{aligned}
        %a_{k, s} & \leq \big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ).
    %\end{aligned}
%\end{equation}
Note that this step derives the restriction conditions of the tuning parameters in Theorem \ref{thm.MAB}. 
%The exact same situation appears in other papers of MAB theory: the condition of tuning parameters is derived and only used in the step of bounding $a_{k, s}$ with a constant free of $T$. See \cite{kveton2019garbage} and \cite{wu2022residual} for instance.

%which is the reason why we need the restriction of tuning parameters in the Theorem.
%with some $C \geq 0$. Hence, a sufficient condition for any tuning parameter $\lambda > 0$ is that $12 \sigma_1^2 / \sigma_{\omega}^2 \leq 1$ for any round $T \geq 2$. Or some bounded interval for $\lambda$ will be required when $12 \sigma_1^2 / \sigma_{\omega}^2 \geq 1$. To be specific, if $\sigma_1^2 = \sigma_{\omega}^2 = 1$, a sufficient condition for \eqref{tuning_condition} is $12 (2 \lambda + 1)^2 \leq C \left[ (\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2\right]$ for some $C \geq 0$. For instance, if $\mu_1 = 1$, we can take $C = 12$, then our theory will be valid if take the tuning parameter $\lambda \in (0, 1]$ whenever the total round $T \geq 12$.

%{$\sigma_k^2 \in (0, 1]$ for $k \in [K]$ and $\sigma_{\omega}^2 = 1$}

%\textbf{$\leq sth. \log T$ holds for $T \geq C$. When $T < C$, take $sth.$ large enough we can still get the order $\log T$.
%}

%{$\lambda$ cannot depend on unknown variable}

%For instance, if we just take $\mu_1 = 1/2$, we will need $\sigma_{\omega}^2 \geq 24 \sigma_1^2$ with any $\lambda > 0$.

%\textit{sub-Gaussian parameter can be assumed to in $[0, 1]$, then we can solve the bound off $\lambda$. }

%\begin{remark}
   %Different from the bounded rewards setting, here $\lambda$ together with the bound of $\mu_1$ as well as $\sigma_{\omega}^2$ and $\sigma_k^2$ establish the restriction condition for the tuning parameters. But \eqref{tuning_condition_exact} can be served as a sufficient condition.
%\end{remark}

%\begin{remark}
   %It can be shown that for bounded rewards, we can use any positive $\lambda$ and $\sigma_{\omega}^2$ to ensure that $a_{k, s}$ can be bounded by a constant free of $T$. 
%\end{remark}


\subsubsection{Decomposition for bounding $a_k$}
\todorw{
The paragraphs below belong to the roadmap of this section and I would suggest moving them to the beginning of this section. 
I would suggest always provide the big picture first, and then zoom into detailed components, so readers will not be lost. 
Otherwise, e.g., readers will be curious about why we need to bound a by constant. Few people has the patience to finish what above without knowing the big picture. 
}


Next, we decompose $a_{k, s}$ as $a_{k, s} = a_{k, s, 1} + a_{k, s, 2} + a_{k, s, 3}$, and we can focus on these simpler components $a_{k, s, j}$ for $j = 1, 2, 3$. 

Following the idea in \cite{kveton2019garbage}, we are going to try to bound 
\[
    s_{a, j} = \max \{ s: a_{k, s, j} \geq T^{-1}\}, \qquad j = 1, 2, 3
\]
with a constant times $\log T$. Indeed, if we successfully do so, then 
\[
    \begin{aligned}
    	a_{k} & \leq \max_{s \in [T]} a_{k, s} \times s_{a, j} + T^{-1} \times (T - s_{a, j}) \\
    	& \asymp O(1) \times O(\log T) + O(1) = O  (\log T),
    \end{aligned}
\]
which does bound $a_{k} = \sum_{s = 0}^{T - 1} a_{k, s} \lesssim \log T$.


% \subsubsection{Bounding $s_{a, j}$}
% \blue{Recall that, after bounding XXX, the proof can be completed if we can decompose $a_{k, s}$ as $a_{k, s} = a_{k, s, 1} + a_{k, s, 2} + a_{k, s, 3}$ and bound each $s_{a, j} = \max \{ s: a_{k, s, j} \geq T^{-1}\}$ by $s_{a, j} = \max \{ s: a_{k, s, j} \geq T^{-1}\}$. 
% These would be the focus of this section. }
% \todorw{I added the above. Feel free to polish. It is OK and even recommended to remind the goal when necessary. Otherwise, the readers will take a lot of time to figure out your plan. }


%\todohw{I still need to go through the following part. I will get this done tonight and tomorrow.}
%giving an order $\log T$. 
%As we can see, decomposition will play an important role in this proof. 
For the decomposition, a common approach is using indicators on "\textit{good}" events to decompose. Denote the shifted version mean reward defined as 
\[
    \overline{R}_{k, s}^* := \frac{\sum_{i = 1}^s R_{k, i} + \lambda s}{s(1 + 2 \lambda)} = \frac{\lambda}{1 + 2 \lambda} + \frac{1}{1 + 2 \lambda} \overline{R}_{k, s}.
\]
Then we can define the following "good" events for $k$-th arm as
\[
    A_{k, s} := \left\{ - C_1 \Delta_k < \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  < C_1 \Delta_k \right\},
\]
and
\[
    G_{k', s} := \left\{ - C_2 \Delta_k \leq \overline{Y}_{k', s} - \overline{R}_{k', s}^* \leq C_2 \Delta_k \right\}.
\]
The definitions of $A_{k, s}$ and $G_{k, s}$ are intuitive: $A_{k, s} \, \cap \, A_{k, s}'$ represents the sample mean does not derivative from the true mean too far; and events on $G_{k', s}$ means $\overline{Y}_{k', s}$ is not too far away from the scaled-shifted sample mean $\overline{R}_{k, s}^*$. Here $0 < C_1, C_2 \leq 1$ are some constants.

%It is worthy to note that $k'$ in $G_{k', s}$ is different from the fixed index $k$ in $\Delta_k$. And it is also easy to see that under two good events $A_{k', s} \cap G_{k', s}$, our target function $\overline{Y}_{k', s}$ is close to the shifted mean $\frac{\mu_{k'} + \lambda}{1 + 2\lambda}$, which means $\overline{Y}_{k', s}$ does remain the order of expected mean of each arm. 
Therefore, by using these good events, we decompose $a_{k, s}$ as the following three parts:
\[
    a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}^c)\Big],
\]
\[
    a_{k, s, 2} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}) \ind (G_{1, s}^c)\Big], \qquad a_{k, s, 3} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}) \ind (G_{1, s})\Big].
\]
As we can see, $a_{k, s, 1}$ and $a_{k, s, 2}$ are defined on complement sets of the good events or say "bad" events,
and we will bound them by bounding the probability $\pr (A_{1, s}^c)$ and $\pr (G_{1, s}^c)$; while $a_{k, s, 3}$ defined on the "good" events, we will need extra steps to bound them, which we will specify later. 

\subsubsection{Bounding $a_{k, s, 1}$ by analyzing $s_{a, 1}$}

We will bound $a_{k, s, 1}$ by bounding the probability of $A_{k, s}^c$. Write
\begin{equation}\label{a_k_1_bound}
    a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}^c)\Big] \leq \E \Big[ T  \ind(A_{1, s}^c)\Big] = T \pr (A_{1, s}^c) 
\end{equation}
Since the summation of independent sub-Gaussian variables is still sub-Gaussian, \eqref{lem_subGtosubE_1} in Lemma \ref{lem_subGtosubE} gives $\overline{R}_{1, s} - \mu_1 \sim \subG (\sigma^2 /  s)$. And by the concentration inequality of the sub-Gaussian variable,
\[
    \begin{aligned}
        \pr (A_{1, s}^c) & = \pr \left( \big| \overline{R}_{1, s} - \mu_1 \big| \geq (1 + 2\lambda) C_1 \Delta_k \right) \\
        & \leq 2 \exp \left\{ - \frac{(1 + 2\lambda)^2 C_1^2 \Delta_k^2 s}{2 \sigma_1^2}\right\} \\
        \alignedoverset{\text{take } s \geq s_{a, 1} :=  \begin{matrix} \frac{\sigma_1^2}{C_1^2 (1 + 2 \lambda)^2 \Delta_k^2} \times\log (2 T) \end{matrix}}{\leq} \frac{1}{T^2}
    \end{aligned}
\]
Hence, we obtain that
\[
    a_{k, s, 1} \leq  T \pr(A_{1, s}^c) \leq T^{-1}, \qquad \text{ for any } s \geq s_{a, 1} \asymp \log T.
\]

%\begin{remark}
   %For bounded rewards, there we can just use Hoeffding inequality and still have $s_{a, 1} \asymp \log T$.
%\end{remark}

\subsubsection{Bounding $a_{k, s, 2}$ by tackling $s_{a, 2}$}
%\todorw{Tackling a number?}
For bounding the probability of $G_{1, s}^c$ conditioning on $\his_{1, s}$, we use the fact of the following lemma for Gaussian variable.
\begin{lemma}\label{lem_gau_frac}
	Suppose $X$ and $Y$ are Gaussian variables with means $\E X = 0$ and $\E Y > 0$, then
	\[
	    \pr \left(\frac{|X|}{|Y|} > c \right) \leq 2 \pr (X > c Y) + \pr \left( Y < 0 \right)
	\]
	for any $c > 0$.
\end{lemma} 
\todorw{This section is too long and readers will be lost. Please either provide a roadmap, or better organize, or move some details to later as a lemma. }
\todohw{I agree, I am thinking to add a extra lemma part including all technique details for bounding the inter-step terms in these section. }
% that $\omega_i, \omega_i', \omega_i''$ is symmetric about their means $1$: 
%we use the fact $G_{k', s}^c = \{ |\overline{Y}_{k', s} - \overline{R}^*_{k', s}| > C_3 \Delta_k\}$ 
%Since a symmetric event. Hence, 
By the above lemma, note that 
\[
    \begin{aligned}
    	& \E_{\omega, \omega', \omega''} \left[ \sum_{i = 1}^s \big[ (1 + 2\lambda) R_{1, i} - (\overline{R}_{1, s} + \lambda)\big] \omega_i + \sum_{i = 1}^s \lambda (1 + \lambda - \overline{R}_{1, s}) \omega_i' - \sum_{i = 1}^s \lambda (\overline{R}_{1, s} + \lambda) \omega_i'' \right] \\
    	 = & s \big( (1 + 2\lambda) \overline{R}_{1, s} - (\overline{R}_{1, s} + \lambda) + \lambda (1 + \lambda - \overline{R}_{1, s}) - \lambda (\overline{R}_{1, s} + \lambda) \big) = 0,
    \end{aligned}
\]
we can upper bound the tail probability $\pr (G_{1, s}^c \mid \his_{1, s})$ as, 
\[
    \begin{aligned}
        & \pr (G_{1, s}^c \mid \his_{1, s})\\
        = & \pr \big( |\overline{Y}_{k', s} - \overline{R}^*_{k', s}| > C_3 \Delta_k \mid \his_{1, s}\big)\\
        = & 2 \pr_{\omega, \omega', \omega''}  \left\{ \left| \frac{\sum_{i = 1}^s \big[ (1 + 2\lambda) R_{1, i} - (\overline{R}_{1, s} + \lambda)\big] \omega_i + \sum_{i = 1}^s \lambda (1 + \lambda - \overline{R}_{1, s}) \omega_i' - \sum_{i = 1}^s \lambda (\overline{R}_{1, s} + \lambda) \omega_i''}{(1 + 2 \lambda)(\sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i'')} \right| > C_2 \Delta_k \right\} \\
        \alignedoverset{\text{by Lemma \ref{lem_gau_frac}}}{\leq} 2 \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s \big[ (1 + 2\lambda) R_{1, i} - (\overline{R}_{1, s} + \lambda)\big] \omega_i + \sum_{i = 1}^s \lambda (1 + \lambda - \overline{R}_{1, s}) \omega_i'  \\
        & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ - \sum_{i = 1}^s \lambda (\overline{R}_{1, s} + \lambda) \omega_i'' - C_2 (1 + 2\lambda) \Delta_k \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] > 0\Bigg\} \\
        & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + \pr \left\{ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i'' < 0\right\}  =: I^{(1)} + II^{(1)}. 
    \end{aligned}
\]
To analyze the above probability, we first study $II^{(1)}$. We write it as
\[
    \begin{aligned}
    	II^{(1)} & = \pr \left( \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i'' < 0\right) \\
    	& = \pr \left( \frac{\sum_{i = 1}^s (\omega_i - 1) + \lambda \sum_{i = 1}^s (\omega_i' - 1) + \lambda \sum_{i = 1}^s (\omega_i'' - 1)}{\sqrt{s \sigma_{\omega}^2 (1 +2 \lambda^2)}} < - \frac{(1 + 2\lambda) s}{\sqrt{s \sigma_{\omega}^2 (1 +2 \lambda^2)}} \right) \\
    	& = \pr \left( Z < - \frac{(1 + 2\lambda) }{\sigma_{\omega} \sqrt{1 + 2 \lambda^2}} \times \sqrt{s} \right) \\
    	\alignedoverset{\text{by Lemma \ref{lemma:gaussian_weight}}}{\leq} \frac{1}{2} \exp \left\{ - \frac{s (1 + 2 \lambda)^2}{2 \sigma_{\omega}^2 (1 + 2 \lambda^2)}\right\}.
    \end{aligned}
\]
For studying $I^{(1)}$, we define the following functions of $\{ R_{1,i}\}_{i = 1}^s$:
\[
   f \big(\{ R_{1,i}\}_{i = 1}^s\big) := f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) + f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) - f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big)
\]
with 
\[
    \begin{aligned}
    	f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) & := \sum_{i = 1}^s \big[ (R_{1, i} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) - (1 + 2 \lambda ) C_2 \Delta_k  \big] \omega_i,\\
    	f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) & := \sum_{i = 1}^s \big[ \lambda (\lambda + 1  - \overline{R}_{1, s}) - (1 + 2 \lambda ) C_2 \Delta_k  \big] \omega_i', \\
    	f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big) & = \sum_{i = 1}^s \big[ \lambda (\overline{R}_{1, s} + \lambda) + (1 + 2 \lambda ) C_2 \Delta_k  \big] \omega_i''.
    \end{aligned}
\]
%\[
    %f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) = \sum_{i = 1}^s \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s} - C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i,
%\]
%\[
    %f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) = \sum_{i = 1}^s \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda - \lambda C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i',
%\] 
%\[
    %f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big) =  \sum_{i = 1}^s \big[ (\lambda^2 + \lambda \overline{R}_{1, s}) + \lambda C_3 (1 + 2\lambda) \Delta_k \big] \omega_i''.
%\]
Then we can write $I^{(1)} = 2 \pr_{\omega, \omega', \omega'} (f_1 + f_2 - f_3 > 0)$. Note that $f_1, f_2$, and $f_3$ are mutually independent. 
\todorw{Few decomposition are "by luck". You must have a reason to do so (e.g., is "independent" the motivation for such a decomposition? and they are independent for a reason.). Always share the motivation with readers. It also helps us to think more clearer about our proof strategy. }
The expectation is
\[
    \E \big[ f_1 + f_2 - f_3 \mid \his_{1, s}\big] = - 3 C_2 (1 + 2 \lambda) \Delta_k s,
\] 
and the variance is
\begin{equation}\label{bound_var_f}
    \begin{aligned}
        & \var \big(f_1 + f_2 - f_3 \mid \his_{1, s} \big) \\
        = & \sigma_{\omega}^2 \Bigg [ \sum_{i = 1}^s \big[ (R_{1, i} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) - (1 + 2 \lambda ) C_2 \Delta_k  \big]^2 \\
        & \qquad \qquad \qquad + \sum_{i = 1}^s \big[ \lambda (\lambda + 1  - \overline{R}_{1, s}) - (1 + 2 \lambda ) C_2 \Delta_k  \big]^2 + \sum_{i = 1}^s \big[ \lambda (\overline{R}_{1, s} + \lambda) + (1 + 2 \lambda ) C_2 \Delta_k  \big]^2 \Bigg] \\ 
        =: & \sigma_{\omega}^2 \Big[ I^{(2)} + II^{(2)} + III^{(2)} \Big].
    \end{aligned}
 \end{equation}
 %\todorw{Isn't I already used?}
 For bounding the conditional variance above. We calculate the components are:
 \begin{equation}\label{bound_I}
 	\begin{aligned}
 	    I^{(2)} & = \sum_{i = 1}^s  \big[ (R_{1, i} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) \big]^2  + s \lambda^2 (\lambda + 1  - \overline{R}_{1, s})^2 + s \lambda^2 (\overline{R}_{1, s} + \lambda)^2 \\
 	    & = \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 2 s \lambda^2 \big( 3 \overline{R}_{1, s}^2 - 3 \overline{R}_{1, s} + \lambda^2 + \lambda + 1 \big) \\
 	    & = \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + (6 \lambda^2 - 1)s (\overline{R}_{1, s} - \mu_1)^2 + 6  s \lambda^2 (2 \mu_1 - 3)  (\overline{R}_{1, s} - \mu_1) + 2 s \lambda^2 \big( \lambda^2 + \lambda + 1 + 3 \mu (\mu - 1) \big) \\
 	    \alignedoverset{\text{Cauchy inequality}}{\leq} 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2  + 6  s \lambda^2 (2 \mu_1 - 1)  (\overline{R}_{1, s} - \mu_1) + 2 s \lambda^2 \big( \lambda^2 + \lambda + 1 - \mu_1 (1 - \mu_1) \big) \\
 	    & = 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + 6  s \lambda^2 (2 \mu_1 - 1)  (\overline{R}_{1, s} - \mu_1)  + 2 s \lambda^2 \left( \lambda^2 + \lambda + 1 - \mu_1 (1 - \mu_1)\right),
 	\end{aligned}
 \end{equation}
 \[
     \begin{aligned}
         II^{(2)} & = - 2 (1 + 2\lambda) C_3 \Delta_k \bigg[ \sum_{i = 1}^s  \big( (R_{1, i} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) \big) + s \lambda (\lambda + 1  - \overline{R}_{1, s}) -  s \lambda (\overline{R}_{1, s} + \lambda) \bigg] \\
         & = - 2 s (1 + 2\lambda) C_3 \Delta_k \Big[ \big(\overline{R}_{1, s} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) + \lambda (\lambda + 1  - \overline{R}_{1, s}) \big) -  \lambda (\overline{R}_{1, s} + \lambda) \Big] = 0,
     \end{aligned}
 \]
 and $III^{(2)} = 3 s (1 + 2\lambda)^2 C_3^2 \Delta_k^2$. Therefore, the conditional variance in \eqref{bound_var_f} is bounded by
 \begin{equation}\label{bound_var_f_new}
 	\begin{aligned}
 		 \sigma_{\omega}^{-2}\var \big(f_1 + f_2 - f_3 \mid \his_{1, s} \big) & \leq I^{(2)} + II^{(2)} + III^{(2)} \\
 		 & \leq  \underbrace{6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + 6 s \lambda^2 (2\mu_1 - 1) \left( \overline{R}_{1, s} - \mu_1\right)}_{\text{the random part}} \\
 		 & ~~~~~~~~~~~~~~~~~~~ + \underbrace{2 s \lambda^2 \left( \lambda^2 + \lambda + 1 - 3 \mu_1 (1 - \mu_1)\right) + 3 s (1 + 2\lambda)^2 C_2^2 \Delta_k^2}_{\text{the determined part}} \\
 		 & =: \mathfrak{R}_1 + \mathfrak{R}_2 + \mathfrak{D},
 	\end{aligned}
 \end{equation}
 where
 \[
     \mathfrak{R}_1 := 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2, \qquad \mathfrak{D} = 3 s (1 + 2\lambda)^2 C_2^2 \Delta_k^2
 \]
 are strictly positive. For the random quantity,
 \[
     \mathfrak{R}_2 = 6 s \lambda^2 (2\mu_1 - 1) \left( \overline{R}_{1, s} - \mu_1\right) + 2 s \lambda^2 \left( \lambda^2 + \lambda + 1 - 3 \mu_1 (1 - \mu_1)\right),
 \]
 it is non-positive with a high probability. Indeed, note that $0 \leq 3 \mu_1 (1 - \mu_1) \leq \frac{3}{4}$
 \begin{equation}\label{R_2_pr}
     \begin{aligned}
     	\pr ( \mathfrak{R}_2 > 0) & = \pr \left( 3 (2 \mu_1 - 1)\left( \overline{R}_{1, s} - {\mu_1} / {2} \right) > \lambda^2 + \lambda + 1 - 3 \mu_1 (1 - \mu_1)\right) \\
     	& \leq \pr \left( \Big| 3 (2 \mu_1 - 1)\left( \overline{R}_{1, s} - {\mu_1} \right)\Big| > \Big| \lambda^2 + \lambda + 1 - 3 \mu_1 (1 - \mu_1) \Big| \right) \ind\left( \mu_1 \neq  \frac{1}{2}\right) + \pr (\varnothing) \times \ind\left( \mu_1 = \frac{1}{2}\right) \\
     	\alignedoverset{0 \leq 3 \mu_1 (1 - \mu_1) \leq \frac{3}{4}}{\leq} \pr \left( \Big| \overline{R}_{1, s} - {\mu_1} \Big| > \frac{\lambda^2 + \lambda + 1 / 4}{|3 (2 \mu_1 - 1)|} \right) \ind\left( \mu_1 \neq  \frac{1}{2}\right) + 0 \times \ind\left( \mu_1 = \frac{1}{2}\right) \\
     	\alignedoverset{\text{by sub-Gaussian inequality}}{\leq} \exp \left\{ - \frac{(\lambda^2 + \lambda + 1 / 4)^2 s}{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}\right\} \times \ind\left( \mu_1 \neq \frac{1}{2}\right) + 0 \times \ind\left( \mu_1 = \frac{1}{2}\right).
     \end{aligned}
 \end{equation}
 %\todohw{Need to continue}
 %\begin{equation}
     %\begin{aligned}
        %= & \sigma_{\omega}^2 \Bigg[ \overbrace{(1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 2 s \lambda (1 + 2 \lambda) (2 \overline{R}_{1, s} - 1 ) (\overline{R}_{1, i} - \overline{R}_{1, s}) + 2 s \lambda^2 \big(3 \overline{R}_{1, s}^2 - 3 \overline{R}_{1, s} + \lambda^2 + \lambda + 1 \big)}^{\text{the variance coming from the difference between $\overline{Y}_{k, s}$ and $\overline{R}_{k, s}$.}} \\
        %& \qquad \qquad \qquad + \underbrace{3 s (1 + 2\lambda)^2 C_3^2 \Delta_k^2}_{\text{the maximal variance expansion allowed on the event $G_{1, k}^c$ (the cross term cancelling out).}} \Bigg] \\
        %& = \sigma_{\omega}^2 \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 +  2 s \lambda^2 \big(3 \overline{R}_{1, s}^2 - 3 \overline{R}_{1, s} + \lambda^2 + \lambda + 1 \big) + 3 s (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \bigg] \\
        %& =: \sigma_{\omega}^2 \bigg[ \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \bigg]
    %\end{aligned}
%\end{equation}
%where we define
%\[
    %\mathbb{G}_1(s, \lambda) := (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2, \qquad \mathbb{G}_2 (s, \lambda) := 6 s \lambda^2 \overline{R}_{1, s} (\overline{R}_{1, s} - 1),
%\]
%and
%\[
    %g_3(s, \lambda) = s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2  \big].
%\]
%\iffalse
%\[
    %\begin{aligned}
        %& \var(f_1 + f_2 - f_3) = \var f_1 + \var f_2 + \var f_3 \\
        %= & \bigg\{ \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 4 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + 4 \lambda \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) (R_{1, i} - \mu_1) \\
        %& \qquad + 2 \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \sum_{i = 1}^s (R_{1,i} - \overline{R}_{1, s}) \\
        %& \qquad + 4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \sum_{ i =1}^s (R_{1, i} - \mu_1) + s \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big]^2 \bigg\} \\
        %& + \lambda^2 \bigg\{ s^2 (\overline{R}_{1, s} - \mu_1)^2 + 2 \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big] s (\overline{R}_{1, s} - \mu_1) +  s \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \bigg\} \\
        %& + \lambda^2 \bigg\{ s^2 (\overline{R}_{1, s} - \mu_1)^2 + 2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] s (\overline{R}_{1, s} - \mu_1) + s \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \bigg\} \\
        %= & (1 + 4 \lambda^2 + 4 \lambda) \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + (-s - 4 \lambda s + \lambda^2 s^2 + \lambda^2 s^2) (\overline{R}_{1, s} - \mu_1)^2 + \Big\{ 4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \\
        %& + 2 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] + 2 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big\} \sum_{i = 1}^s (R_{1, s} - \mu_1) \\
        %& + \Big\{ s \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big]^2 + s \lambda^2 \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \\
        %& + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \Big\} \\
        %=: & g_1(\lambda) \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + g_2(s, \lambda) (\overline{R}_{1, s} - \mu_1)^2 + g_3(\lambda) \sum_{i = 1}^s (R_{i, s} - \mu_1) + g_4(s, \lambda) \\
        %=: & \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda).
    %\end{aligned}
%\]
%\fi
%Here the hollow font $\mathbb{G}_{\cdot}$ represents random quantities whereas $g_{\cdot}$ is non-random.

%The $\mathbb{G}_j$ for $j = 1, 2$ and $g_3$ have relatively complex expressions, so we want to give some simpler upper bounds of them. We calculate it as
%First, we note that $\var (f_1 + f_2 - f_3)$ is strictly positive, and it has the following upper bound,
%\begin{equation}\label{G_function_bound}
    %\begin{aligned}
        %& \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \\
        %= & (1 + 2 \lambda)^2 \bigg[ \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 - s (\overline{R}_{1, s} - \mu_1)^2\bigg] \\
        %& \qquad + 6 s \lambda^2 \Big[ (\overline{R}_{1, s} - \mu_1)^2 + 2 (\mu_1 - 1) (\overline{R}_{1,  s} - \mu_1) + \mu_1 (\mu_1 - 1)\Big] + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) \\
        %& \qquad + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2  \big] \\
        %= & \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s (2 \lambda^2 - 4 \lambda - 1) (\overline{R}_{1, s} - \mu_1)^2 - 2s (1 - \mu_1) (\overline{R}_{1, s} - \mu_1) \bigg] \\
        %& \qquad \qquad + s \big[ - 6 \lambda^2 \mu_1 (1 - \mu_1) + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        %\overset{\text{dropping the negative terms}}{\leq} & \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s (2 \lambda^2 - 4 \lambda - 1) (\overline{R}_{1, s} - \mu_1)^2  \bigg]  \\
        %& + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        %\overset{\text{by Cauchy inequality}}{\leq} & \big[ (1 + 2 \lambda)^2 + (2 \lambda^2 - 4 \lambda - 1)  \big] \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 +  s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        %= & 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]. 
    %\end{aligned}
%\end{equation}
%As one can see, in this step, we bound $\mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda)$ by a sub-Exponential variable plus a strictly positive constant.
%\iffalse
%\begin{equation}\label{G_function_bound}
    %\begin{aligned}
        %& \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda) \\
        %= & s^2 g_1(\lambda) (\overline{R}_{1, s} - \mu_1)^2 + g_2(s, \lambda) (\overline{R}_{1, s} - \mu_1)^2  + s g_3(\lambda) (\overline{R}_{1, s} - \mu_1) + g_4(s, \lambda) \\
        %= & \big[ s^2 g_1(\lambda) + g_2(s, \lambda)\big](\overline{R}_{1, s} - \mu_1)^2 + s g_3(\lambda) (\overline{R}_{1, s} - \mu_1) + g_4(s, \lambda) \\
        %\leq & \Big\{ s^2(2 \lambda + 1)^2 + (2 \lambda^2 s^2 - 4 \lambda s - 1)\Big\} (\overline{R}_{1, s} - \mu_1)^2 \\
        %& \qquad + \Big\{ s \times4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + \lambda) + \lambda (\lambda + \mu_1) + C_3 \lambda (1 + 2 \lambda) \Delta_k \big] \Big\} (\overline{R}_{1, s} - \mu_1) \\
        %& \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \\
        %& \qquad + s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\} \\
        %\leq & 2 s^2 (6 \lambda^2 + 4 \lambda + 1) (\overline{R}_{1, s} - \mu_1)^2 + 4 s \lambda \big[ (2 C_3 \Delta_k + 1) \lambda^2 + (3 \mu_1 - 1 - C_3 + C_3 \Delta_k) \lambda - C_3 \big] (\overline{R}_{1, s} - \mu_1) \\
        %& \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \\
        %& \qquad + s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\} \\
        %\leq & 2s^2 (4 \lambda^2 + 4 \lambda + 1) (\overline{R}_{1, s} - \mu_1)^2  + 2 s \lambda (2 \lambda + 1) \times\lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \sqrt{s} (\overline{R}_{1, s} - \mu_1) \\
        %& \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + g_5(s, \lambda)\\
        %\leq & 2 s \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) +  \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2 + g_5(s, \lambda),
    %\end{aligned}
%\end{equation}
%where the last two $\leq$ use the fact that $s \geq 1$ and $\mu_1, C_3 \in (0, 1]$. And furthermore, $g_5(s, \lambda) = s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\}$ is a strict positive function for at least $\Delta_{k_1}, \ldots, \Delta_{k_{K - 3}}$, since
%\[
    %\frac{C_3 \Delta_k}{2(\mu_1 - C_3 \Delta_k) - 1} = \frac{1 - \mu_1 - C_3 \Delta_k}{2 C_3 \Delta_k - 1}.
%\]
%is a quadratic equation for $\Delta_k$ and cannot hold for all $k \in [K] / \{ 1\}$. And for $g_5(s, \lambda)$, it can be bounded by
%\[
    %\begin{aligned}
        %g_5(s, \lambda) & \leq s \lambda^2 \Big( \big[ 1 + C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ 1 + C_3 (1 + 2 \lambda) \Delta_k + (1 + \lambda) \big]^2 \Big) \\
        %& \leq 2 s \lambda^2 \left[ 1 + C_3^2 (\lambda^{-1} + 2)^2 \Delta_k^2 + (2 + \lambda)^2 + C_3^2 (1 + 2 \lambda)^2 \Delta_k^2\right] \\
        %& \leq 2 s \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big].
    %\end{aligned}
%\]

%\textit{{Why the restriction will appears. Adding something to make the above strictly positive.}}

%Therefore, 
%\[
    %\begin{aligned}
        %& \frac{\var (f_1 + f_2 - f_3)}{|\E (f_1 + f_2 - f_3)} 1(\overline{R}_{1, s} - \mu_1 \leq 0)\\ 
        %= & \frac{ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda)}{|\E (f_1 + f_2 - f_3)|} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & \frac{2 \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) + \sqrt{2} \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2}{C_3 (1 + 2 \lambda)^2 \Delta_k} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & \frac{2 \Big[\sqrt{2} \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2}{C_3 (1 + 2 \lambda)^2 \Delta_k} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & 8 C_3 \lambda^2 \Delta_k 1(\overline{R}_{1, s} - \mu_1 \leq 0).
    %\end{aligned}
%\]
%\fi
%For the standard Gaussian variable $Z$, we have $\pr (Z \geq x)\leq \exp \{ - {x^2} / {2}\}$ for $x > 0$.
Then by applying Lemma \ref{lemma:gaussian_weight} again,
\[
    \begin{aligned}
        \pr (G_{1, s}^c \mid \his_{1, s}) & = 2 \pr \left(\frac{f_1 + f_2 - f_3 - \E \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{\sqrt{\var \big(f_1 + f_2 - f_3 \mid \his_{1, s}\big)}} > - \frac{\E \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{\sqrt{\var \big(f_1 + f_2 - f_3 \mid \his_{1, s}\big)}} \right) \\
        & \leq \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \var \big(f_1 + f_2 - f_3 \mid \his_{1, s}\big)} \right\}.
        %(\text{by \eqref{bound_var_f}} )& \leq 2 \exp \left\{ - \frac{9 C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3(s, \lambda) \big]}\right\}.
    \end{aligned}
\]
Therefore, combining with \eqref{bound_var_f_new}, 
$a_{k, s, 2}$ will be bounded by 
\[
    \begin{aligned}
        a_{k, s, 2} & \leq \E \Big[ T  \ind(G_{1, s}^c)\Big] =  T \E \Big[ \pr(G_{1, s}^c \mid \his_{1, s}) \Big] \\
        & \leq T \E \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \var \big(f_1 + f_2 - f_3 \mid \his_{1, s}\big)} \right\} \\
        & \leq T \E \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \var \big(f_1 + f_2 - f_3 \mid \his_{1, s}\big)} \right\} \big( \ind (\mathfrak{R}_2 \leq 0) + \ind(\mathfrak{R}_2 > 0) \big) \\
        \alignedoverset{\text{by the decomposition \eqref{bound_var_f_new}}}{\leq} T \E \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \sigma_{\omega}^2 \big(\mathfrak{R}_1 + \mathfrak{R}_2 + \mathfrak{D} \big)}\right\} \ind (\mathfrak{R}_2 \leq 0) + T \pr (\mathfrak{R}_2 > 0) \\
        & \leq T \E \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \sigma_{\omega}^2 \big(\mathfrak{R}_1 + \mathfrak{D} \big)}\right\} + T \pr (\mathfrak{R}_2 > 0)
    \end{aligned}
\]
%On the other hand, 
Recall $R_{1, i} - \mu_1 \sim \subG(\sigma_1^2)$, and then $(R_{1, i} - \mu_1)^2 - \var (R_{1, i}) := \xi_i \sim \subE(8 \sqrt{2} \sigma_1^2)$.
%hence by Corollary 4.2 (a) in \cite{zhang2020concentration},
%\[
    %\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 - s \var (R_{1, i}) \, \sim \, \subE (8 \sqrt{2 s} \sigma_1^2).
%\]
Therefore, for furthermore bounding $\mathfrak{R}_1 + \mathfrak{D}$, we have
\begin{equation}\label{G_function_bound}
	\begin{aligned}
		\mathfrak{R}_1 + \mathfrak{D} & = 6 \lambda^2 \left[ \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 - s \var (R_{1, i}) \right] + \left[ s \var (R_{1, i}) + 3 s(1 + 2\lambda)^2 C_2^2 \Delta_k^2\right] \\
             & = 6 \lambda^2 \sum_{i = 1}^s \xi_i + s \left[ 6 \lambda^2\var (R_{1, i}) + 3 (1 + 2\lambda)^2 C_2^2 \Delta_k^2\right] \\
		%& =  6 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + s \left[ 6 \lambda^2\var (R_{1, i}) + 3 (1 + 2\lambda)^2 C_2 \Delta_k^2\right] \\
		\alignedoverset{\text{by $\var(R_{1, i}) \leq \sigma_1^2$}}{\leq}  6\lambda^2 \sum_{i = 1}^s \xi_i + 3 s \left[ 2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2\right]  \\
        & = 3 s \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \right],
	\end{aligned}
\end{equation}
%\begin{equation}\label{G_function_bound_2}
    %\begin{aligned}
        %2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3(s, \lambda) \big] & \overset{\text{by \eqref{G_function_bound}}}{\leq} 12 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        %& \sim 12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + 12 \lambda s \var (R_{1, 1}) +  s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) \\
        %& ~~~~~~~~~~~~~~ + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        %& \overset{\text{by } \var(R_{1, 1}) \leq \sigma_1^2}{\leq} 12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) \\
        %& ~~~~~~~~~~~~~ + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big].
    %\end{aligned}
%\end{equation}
%Here we use the $\subE(\lambda)$ to represent a random variable $Z \sim \subE(\lambda)$. And the distribution notation in the inequalities following will also have a similar meanings.
%\iffalse
%For tackling the expectation above, we first note that $\sqrt{s} (\overline{R}_{1, s} - \mu_1) \sim \subG (\sigma_1^2)$, then $\sqrt{s} (2\lambda + 1) (\overline{R}_{1, s} - \mu_1) \sim \subG \big((2\lambda + 1)^2\sigma_1^2 \big)$, and
%hence
%\[
    %\begin{aligned}
        %& \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) + \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2 \\
        %& \quad - \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 - (2 \lambda + 1 )^2 \var (R_{1,s}) \,  \sim \, \subE \big(8\sqrt{2}(2\lambda + 1)^2\sigma_1^2, 8(2\lambda + 1)^2\sigma_1^2 \big),
    %\end{aligned}
%\]
%\fi
where $\overline{\xi} = \frac{1}{s} \sum_{i = 1}^s \xi_i$ is the mean of $\{ \xi_i \}_{i = 1}^s$, Then applying Lemma \ref{lem_subE_ineq} in \eqref{G_function_bound} will furthermore give
\begin{equation}\label{a_2_bound}
	\begin{aligned}
		a_{k, s, 2} & \leq T \E \exp \left\{ - \frac{\E^2 \big( f_1 + f_2 - f_3 \mid \his_{1, s}\big)}{2 \sigma_{\omega}^2 \big(\mathfrak{R}_1 + \mathfrak{D} \big)}\right\} + T \pr (\mathfrak{R}_2 > 0) \\
		\alignedoverset{\text{by \eqref{G_function_bound} and \eqref{R_2_pr}}}{\leq} T \E\exp \left\{ - \frac{9 C_2^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{6  \sigma_{\omega}^2 s  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \right] }\right\} \\
		 & ~~~~~~~~~~~~~~~ + T \left[ \exp \left\{ - \frac{(\lambda^2 + \lambda + 1 / 4)^2 s}{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}\right\} \times \ind\left( \mu_1 \neq \frac{1}{2}\right) + 0 \times \ind\left( \mu_1 = \frac{1}{2}\right) \right] \\
		 & = T \E\exp \left\{ - \frac{3 C_2^2 (1 + 2\lambda)^2 \Delta_k^2 s }{ 2 \sigma_{\omega}^2  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \right] }\right\} \\
		 & ~~~~~~~~~~~~~~~ + T \left[ \exp \left\{ - \frac{(\lambda^2 + \lambda + 1 / 4)^2 s}{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}\right\} \times \ind\left( \mu_1 \neq \frac{1}{2}\right) + 0 \times \ind\left( \mu_1 = \frac{1}{2}\right) \right].
	\end{aligned}
\end{equation}
The next step is applying Lemma \ref{lem_subE_ineq}. We denote $h_{\ell} = h_{\ell} (\cdot, \cdot, \cdot, \cdot) > 0$ as the different functions with different $\ell \in \mathbb{N}$, then
\[
    \log \E\exp \left\{ - \frac{3 C_2^2 (1 + 2\lambda)^2 \Delta_k^2 s }{ 2 \sigma_{\omega}^2  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \right] }\right\} \leq - s \times h_1 (\sigma_1, \sigma_{\omega},\lambda, \Delta_k, C_2).
\]
For bounding \eqref{a_2_bound} with $T^{-1}$, we solve 
\[
    T \E\exp \left\{ - \frac{3 C_2^2 (1 + 2\lambda)^2 \Delta_k^2 s }{ 2 \sigma_{\omega}^2  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 + (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \right] }\right\} \leq \frac{1}{2T}, \qquad \text{i.e.} \qquad s \geq \frac{\log 2 + 2 \log T}{h_1(\sigma_1, \sigma_{\omega},\lambda, \Delta_k, C_2)},
\]
and
\[
    T \left[ \exp \left\{ - \frac{(\lambda^2 + \lambda + 1 / 4)^2 s}{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}\right\} \times \ind\left( \mu_1 \neq \frac{1}{2}\right) + 0 \times \ind\left( \mu_1 = \frac{1}{2}\right) \right] \leq \frac{1}{2T}, \quad \text{i.e.} \quad s \geq \frac{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}{(\lambda^2 + \lambda + 1 / 4)^2} \left[ \log 2 + 2 \log T \right].
\]
Therefore, if we take 
\[
    s_{a, 2} := \left[ \frac{1}{h_1(\sigma_1, \sigma_{\omega},\lambda, \Delta_k, C_2)} \vee \frac{18 \sigma_{\omega}^2 (2 \mu_1 - 1)^2}{(\lambda^2 + \lambda + 1 / 4)^2} \right] \times 3 \log T,
\]
we will have $a_{k, s, 2} \leq \frac{1}{T}$.
%\begin{equation}\label{a_2_bound}
    %\begin{aligned}
        %a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
        %& \overset{\text{by \eqref{G_function_bound_2}}}{\leq} 2 T \E\exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        %& \overset{\text{by } a \subE (\lambda) = \subE (a^2 \lambda)}{=} 2 T \E\exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{ \subE ( 1152 \sqrt{2} \lambda^4 \sigma_1^2) + \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        %& \overset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} 2 T \Big[ 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s ( h_1 + h_2) \Big] \exp \left\{  - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        %& \overset{\text{by } s \leq T}{\leq} 2 T^2 \Big[ 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 ( h_1 + h_2) \Big] \exp \left\{  - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\},
    %\end{aligned}
%\end{equation}
%\iffalse
%\begin{equation}\label{a_2_bound}
    %\begin{aligned}
        %a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s^2 }{2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
        %& \leq 2 T \times \\
        %& \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{4 \big[\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + (2 \lambda + 1 )^2 \var (R_{1,s})\big] + 2 s^{-1}g_5(s, \lambda)}\right\} \\
        %& \leq 2 T \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 4 (2 \lambda + 1 )^2 \var (R_{1,s}) + 2 s^{-1} g_5(s, \lambda)}\right\} \\
        %& \qquad \times \Big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s (h_1 + h_2) \Big]\\
        %& \leq 2 T^2 \Big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1 + h_2) \Big] \\
        %& \exp \left\{ - \frac{C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 4 (2 \lambda + 1 )^2 \sigma_1^2 + 4 \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big]}\right\}.
    %\end{aligned}
%\end{equation}
%\fi
%where $h_1$ and $h_2$ are finite and free of $s$ by following Lemma \ref{lem_subE_ineq}. 
%And we use the fact that for $s$ big enough one must have $b \leq \sqrt{2 c a \cdot 8 \sigma_1^2}$ with $a := 4$, $b := 8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 2 (2 \lambda + 1 )^2 \var (R_{1,s})\big] + 4 s^{-1}g_5(s, \lambda)$, and $c := C_3^2 (1 + 2 \lambda)^4 \Delta_k s$. 

%\iffalse
%\begin{lemma}[Need to be corrected!]\label{lem_subE_ineq}
    %Suppose zero-mean random variable $X \sim \subE(\lambda, \alpha)$, and positive constants $a, b, c$ satisfying $a X + b > 0$,
    %then
    %\[
        %\E \exp \left\{ - \fracC_1{a X + b}\right\}  \leq e^{- c / b} \big[1 + c h_1(a, b, \alpha) + c h_2(a, b, \lambda) \big]
    %\]
    %where $h_1$ and $h_2$ are finite positive functions.
%\end{lemma}

%\begin{proof}
    %Note that differentiable $f$ is positive, we have $0 \leq \E f(X) \leq f(0) + \int_0^{\infty} \big[ f'(u) - f'(-u) \big]\pr (|X| > u) \, du$, then 
    %\[ 
        %\begin{aligned}
            %& \E \exp \left\{ - \fracC_1{a X + b}\right\} \\
            %\leq & e^{-c / b} + \int_0^{\infty} \bigg[ \exp \left\{ - \fracC_1{a u + b}\right\}  \frac{ca }{ (a u + b)^2} - \exp \left\{ - \fracC_1{ - a u + b}\right\}  \frac{ca }{ (- a u + b)^2} \bigg] \, \pr (|X| > u) \, du \\
            %\leq & \int_0^{\infty} \bigg[ \exp \left\{ - \fracC_1{a u + b}\right\}  \frac{ca }{ (a u + b)^2} - \exp \left\{\fracC_1{ a u - b}\right\}  \frac{ca }{ (a u - b)^2} \bigg] \, \exp \left\{ - \frac{1}{2} \left( \frac{u^2}{\lambda^2} \wedge\frac{u}{\alpha} \right) \right\} \, du \\
            %= & \int_0^{\infty} \exp \left\{ - \fracC_1{a u + b}\right\} \bigg[   \frac{ca }{ (a u + b)^2} - \exp \left\{\frac{b + au}{ b - au}\right\}  \frac{ca }{ (a u - b)^2} \bigg] \, \exp \left\{ - \frac{1}{2} \left( \frac{u^2}{\lambda^2} \wedge\frac{u}{\alpha} \right) \right\} \, du \\
            %\leq & \exp (-c / b) \int_0^{\infty} \Bigg[ \frac{ca}{(a u + b)^2} \exp \left\{ - \frac{u}{2 \alpha}\right\} + \frac{ca}{(a u - b)^2} \exp \left\{ - \frac{1}{2}\frac{u^2}{ \lambda^2}  \wedge \frac{u}{ \alpha} + \frac{b + au}{b - au}\right\} \Bigg] \, du \\
            %=: &  \exp (-c / b) \big[ I_1 + I_2 \big].
        %\end{aligned}
    %\]
    %Denote $\Gamma(\cdot, \cdot)$ as incomplete gamma function, then one can calculate that
    %\[
        %I_1 = \fracC_1{b} - \frac{c e^{\frac{b}{2 a \alpha}}\Gamma(0, \frac{b}{2 a \alpha})}{2 a \alpha} =: c h_1 (a, b, \alpha),
    %\]
    %which is finite as long as $a, \alpha$ is positive.
    %For calculating $I_2$, we write $I_2$ as
    %\[
        %\begin{aligned}
            %I_2 = & c a \int_{0}^{\lambda^2 / \alpha} \frac{1}{(a u - b)^2} \exp \left\{ - \frac{u^2}{2 \lambda^2}  + \frac{b + a u}{b - au}\right\} \, du  + \int_{\lambda^2 / \alpha}^{\infty}  \frac{1}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + a u}{b - au}\right\} \, du \\
            %=: & ca ( I_{21} + I_{22}).
        %\end{aligned}
    %\]
    %As $I_{21}$ and $I_{22}$ are both free of $c$, we only need to care its irregular point $\frac{b}{a}$ and $\infty$. We separate it as the following two cases:
    %\begin{itemize}
        %\item[(i)] If $\frac{b}{a} \leq \frac{\lambda^2}{\alpha}$, then 
        %\[
            %\lim_{u \rightarrow \frac{b}{a}} (a u - b)^{1 / 2}\frac{1}{(a u - b)^2} \exp \left\{ - \frac{u^2}{2 \lambda^2} + \frac{b + au}{b - au}\right\} = 0,
        %\]
        %and 
        %\[
            %\lim_{u \rightarrow \infty} u^{3 / 2}\exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} = 0.
        %\]
        %\item[(ii)] If $\frac{b}{a} \geq \frac{\lambda^2}{\alpha}$, then $I_{21}$ will be strictly finite. And for $I_{22}$, it will be
        %\[
            %lim_{u \rightarrow \frac{b}{a}} (a u - b)^{1 / 2}\frac{1}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} = \lim_{u \rightarrow \infty},
        %\]
        
    %\end{itemize}
    %Hence, $\exists \, I_2 \in \mathbb{R}$, and then
    %\[
        %\exists \, I_2 = c \int_0^{\infty} \frac{a}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} =: c h_2(a, b, \lambda) \in c \times (0, \infty)
    %\]
    %with $h_1$ and $h_2$ are finite positive functions.
%\end{proof}
%\fi

\begin{lemma}[sub-Exponential concentration]\label{lem_subE_ineq}
    Suppose zero-mean independent random $ X_i \sim \subE(\lambda_i)$, and positive constants $a$ and $b$ satisfy $a \overline{X} + b > 0$ with the mean $\overline{X} := \frac{1}{s} \sum_{i = 1}^s X_i$. Then,
    \[
        \log \E \exp \left\{ - \frac{s}{a \overline{X} + b}\right\} \, \lesssim \, - s,
    \]
    for $s \in \mathbb{N}$.
    %where $h_1$ and $h_2$ are finite positive functions free of $c$.
    %\todohw{Need to revised. I find $h_1$ and $h_2$ have simple expression.}
\end{lemma}

%\red{
%Let us take
%\[
    %\begin{aligned}
        %s \geq s_{a, 2} := \frac{ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2}{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log \Big[ 2 T^3 \big( 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 ( h_1 + h_2) \big) \Big]
    %\end{aligned}
%\]
%\[
    %\begin{aligned}
        %s \geq s_{a, 2} := & \frac{12 \big(2\lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 6 (2 \lambda + 1 )^2 \sigma_1^2 + \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big] \big)}{C_3^2 (1 + 2\lambda)^4 \Delta_k^2}\\
        %& \qquad \times \log \Big[  2 C_3^2 \lambda^2 (1 + 2\lambda)^4 \Delta_k^2 \big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1 + h_2) \big] \Big] \log T
    %\end{aligned}
%\]
%in the last step of \eqref{a_2_bound}, we will obtain $a_{k, s, 2} \leq T^{-1}$.}

\subsubsection{Bounding $a_{k, s, 3}$ by analyzing $s_{a, 3}$}

In the previous section, we control the probability of "bad" events to bound $a_{k, s, 1}$ and $a_{k, s, 2}$. But since $a_{k, s, 3}$ is defined on good events, we need a different technique to deal with $a_{k, s, 3}$.

Different from dealing with $a_{k, s, 1}$ and $a_{k, s, 2}$, in which we control the probability of the bad events with $O(T^{-2})$,
$a_{k, s, 3}$ is defined on "good" events. Hence, 
We need a special technique to deal with $a_{k, s, 3}$. Note that 
%\todorw{The "(reason) = " is very confusing to read in this layout. }
\begin{equation}\label{a_k_3_sw}
    \begin{aligned}
        \{N_{1, s}(\tau_{k})<T^{-1}\} & \supseteq \{N_{1, s}(\tau_{k}) < (T^{2}-1)^{-1}\} \\
        \alignedoverset{\text{by } (T^2 - 1)^{-1} \leq T^{-1}}{=} \big\{Q_{1, s}\left(\tau_{k}\right)^{-1}<1+\left(T^{2}-1\right)^{-1}\big\} \\
        & = \big\{Q_{1, s}(\tau_{k})^{-1} < (1-T^{-2})^{-1}\big\} = \big\{\left[1-Q_{1, s}(\tau_{k})\right]<T^{-2}\big\},
    \end{aligned}
\end{equation}
and $a_{k, s, 3} \leq \E \big[ N_{1, s} (\tau_k) \ind (A_{1, s} \cap G_{1, s}) \big]$. 
Thus, similar to 
\cite{wang2020residual}, it is sufficient to find $s \geq s_{a,3}$ satisfying $\big\{[1-Q_{1,s}(\tau_{k})]<T^{-2}\big\}$ on the event $\{A_{1, s} \cap G_{1, s}\}$.

We write 
\[
    \big[1-Q_{1, s}(\tau_{k})\big]  \ind (A_{1, s})\ind  (G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, s} \big)  \ind (A_{1, s} \, \cap \, G_{1, s})
\]
with $\Gamma_1 := \Gamma_1(\tau_1) = \tau_1 - \overline{R}_{1, s}^*$ measuring the difference between $\overline{Y}_{1, s}$ and $\overline{R}_{1,s}^*$. And on the event $A_{1, s} \, \cap \, G_{1, s}$, $\Gamma_1$ can be bounded in an interval.
%It is not hard to see $\Gamma_1$ should be negative with a moderate value. And $\Gamma_1$ does have an appropriate on the event $A_{1, s} \, \cap \, G_{1, s}$, this can be true. 
To see this, we write 
\[
    \begin{aligned}
    	A_{1, s} & = \bigg\{ \overline{R}_{1, s}^* - \frac{\mu_1 + \lambda}{1 + 2\lambda} > - C_1 \Delta_k \bigg\} \, \cap \, \bigg\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  < C_1 \Delta_k \bigg\} \\
    	& = \bigg\{ \Gamma_1 < C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} + \tau_1 \bigg\} \, \cap \, \bigg\{ \Gamma_1 > - C_2 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} + \tau_1 \bigg\} \\
    	& = \bigg\{ \tau_1 - C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda}  < \Gamma_1 < \tau_1 + C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda}  \bigg\}
    \end{aligned}
\]
and
\[
    \begin{aligned}
        G_{1, s} = \big\{ - C_2 \Delta_k \leq \overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq C_2 \Delta_k \big\} & = \big\{ \tau_1 -C_2 \Delta_k \leq \overline{Y}_{1, s} + \Gamma_1 \leq \tau_1 + C_2 \Delta_k \big\} \\
        & = \big\{ \tau_1 - C_2 \Delta_k - \overline{Y}_{1, s} \leq \Gamma_1 \leq \tau_1 + C_2 \Delta_k - \overline{Y}_{1, s}\big\} \\
        \alignedoverset{\text{by } - C_2 \Delta_k + \overline{R}_{1, s}^* \leq \overline{Y}_{1, s}  \leq C_2 \Delta_k + \overline{R}_{1, s}^*}{\subseteq} \big\{ \tau_1 - 2 C_2 \Delta_k - \overline{R}_{1, s}^* \leq \Gamma_1 \leq \tau_1 + 2 C_2 \Delta_k - \overline{R}_{1, s}^* \big\}.
        %(\text{by plugging in the inequality for } \overline{Y}_{1, s})& \subseteq 
        % & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2 \lambda}\bigg\},
    \end{aligned}
\]
Then combine the above two result, if we take $C_1 = 2 C_2$, we will have
%\todohw{Need to revise for the first step.}
%\[
    %\begin{aligned}
        %A_{1, s} \, \cap \, G_{1, s} \\
        % & = \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 < \tau_1 + C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} \bigg\} \\
        %(\text{by plugging the inequality for $\overline{R}_{1, s}^*$ in } A_{1, s})\subseteq & \bigg\{ \tau_1 -  2 C_3 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\} \\
        %(\text{take } C_1 \geq 2 C_3 ) \subseteq & \bigg\{ \tau_1 -  C_1 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\}.
    %\end{aligned}
%\]
\[
    \begin{aligned}
    	& A_{1, s} \, \cap \, G_{1, s} \subseteq \bigg\{ \tau_1 - C_1 \Delta_k - \overline{R}_{1, s}^* \wedge \frac{\mu_1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + C_1 \Delta_k - \overline{R}_{1, s}^* \vee \frac{\mu_1 + \lambda}{1 + 2 \lambda}  \bigg\} \\
    	\alignedoverset{\text{by} \frac{\mu_1 +  \lambda}{1 + 2 \lambda} - C_1 \Delta_k  < \overline{R}_{1, s}^* < \frac{\mu_1 +  \lambda}{1 + 2 \lambda} + C_1 \Delta_k }{\subseteq} \bigg\{\tau_1 - 2 C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + 2 C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \bigg\} \\
    	\alignedoverset{\text{by } \mu_1 < 1 + \lambda \text{ and } \mu_1 < \frac{2 \lambda}{2 \lambda - 1}}{\subseteq} \bigg\{ \tau_1 -  2 C_1 \Delta_k - 1 \leq \Gamma_1 \leq \tau_1 + 2 C_1 \Delta_k - \frac{\mu_1}{2}\bigg\}.
    	% & (\text{by plugging the inequality for $\overline{R}_{1, s}^*$ in } A_{1, s})\subseteq \left\{ \tau_1 - (2 C_2 - C_1) \Delta_k - \frac{\mu_1 + \lambda{}}{1 + 2 \lambda} < \Gamma_1 < \tau_1 + (2 C_2 - C_1) \Delta_k - \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\}\\
    	%(\text{by } \begin{matrix} \frac{\mu_1}{2} < \frac{\mu_1 + \lambda}{1 + 2 \lambda} < 1 \end{matrix})\subseteq & \bigg\{ \tau_1 - (2 C_2 -  C_1) \Delta_k - 1 \leq \Gamma_1 < \tau_1 + (2 C_2 - C_1) \Delta_k  - \frac{\mu_1}{2}\bigg\}.
    \end{aligned}
\]
%It is easy to see that in the above derivation, we add the requirement that
%\red{
%Since $\tau_1 - C_1 \Delta_k - 1 < 0$, to control $\Gamma_1$ within a small interval, we add conditions: 
%\begin{equation}\label{requirement_1}
     %\Delta_k + \tau_1 - \frac{\mu_1}{2} \leq 0 \qquad \text{ together with }  \qquad C_1 \geq 2C_2.
%\end{equation}
%Hence, we obtain the range of the positive quantity $-\Gamma_1$ lies in
%\[
    %C_1 \Delta_k = \frac{\mu_1 }{2} - \tau_1 - C_1 \Delta_k <  - \Gamma_1 \leq 1 + C_1 \Delta_k  - \tau_k = 1 - \frac{\mu_1}{2} + 3 C_1 \Delta_k < 4.
%\]
%}
%Now fix
%\begin{equation}\label{requirement_2}
    %\tau_1 = \frac{\mu_1}{2} - \Delta_k,
%\end{equation}
Now take 
\[
    \tau_1 := \frac{\mu_1}{2} - 3 C_1 \Delta_k
\]
satisfying \eqref{requirement_0} as $ \tau_1  < \frac{\mu_1}{2} < \frac{\mu_1 + \lambda}{1 + 2 \lambda}$. We furthermore get on $A_{1, s} \, \cap \, G_{1, s}$, 
\[
    \Gamma_1 \leq \tau_1 + 2 C_1 \Delta_k - \frac{\mu_1}{2} \leq - C_1 \Delta_k < 0
\]
and
\[
    0 > \Gamma_1 \geq \tau_1 - 2 C_1 \Delta_k - 1 \geq \frac{\mu_1}{2} - 1 - 3 C_1 \Delta_k \geq 0 - 1 - 3 = - 4.
\]
Thus, we get $ (- \Gamma_1) \in (C_1 \Delta_k, 4) \subseteq (0, + \infty)$. Returning to the quantity we care about, $ \big[ 1 - Q_{1,s} (\tau_k)\big] \ind (A_{1, s}) \ind (G_{1, s})$, we write it as 
\[
    \begin{aligned}
        & \big[ 1 - Q_{1,s} (\tau_k)\big] \ind (A_{1, s}) \ind (G_{1, s}) \\
        = & \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, s} \big)  \ind (A_{1, s} \, \cap \, G_{1, s})\\
        = & \E \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) \omega_i + \lambda \sum_{i = 1}^s (2 R_{1, i} \omega_i - \overline{R}_{1, s} \omega_i' - \overline{R}_{1, s} \omega_i'') 
        \\
        & \qquad \qquad + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega''_i) - \Gamma_1 (1 + 2\lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] < 0\Bigg\} \ind (A_{1, s} \, \cap \, G_{1, s}).
    \end{aligned}
\]
Similar to the technique we use to bound conditional probability $\pr (G_{1, s}^c \mid \his_{1, s})$, we just need to replace $C_2 \Delta_k$ by $(-\Gamma_1)$ in \eqref{a_2_bound}. We get that 
\begin{equation}\label{Gamma_1_bound_next}
    \begin{aligned}
         & \big[ 1 - Q_{1,s} (\tau_k)\big] \ind (A_{1, s}) \ind(G_{1, s}) \\
         \alignedoverset{\text{apply steps in  \eqref{bound_I}}}{\leq} T \E\exp \left\{ - \frac{9 (- \Gamma_1)^2 \Delta_k^2 s^2 }{6  \sigma_{\omega}^2 s  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 +(- \Gamma_1)^2   \right] }\right\} \\
         \alignedoverset{\text{by the bound of } \Gamma_1}{\leq} T \E\exp \left\{ - \frac{256 \Delta_k^2 s^2 }{6  \sigma_{\omega}^2 s  \left[ 2 \lambda^2 \overline{\xi} +  2 \lambda^2 \sigma_1^2 +C_1^2 \Delta_k^2  \right] }\right\}  \\
         \alignedoverset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} T \exp \left\{ - s \times h_2 (\sigma_1, \sigma_{\omega},\lambda, \Delta_k, C_1)\right\}.
    \end{aligned}
\end{equation}
%
%in the above section. By using the same technique, one can get that
%\iffalse
%\begin{footnotesize}
%\[
    %\begin{aligned}
        %& \big[ 1 - Q_{1,s} (\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \\
        %\leq & \E \exp \left\{ - \frac{\Gamma_1^2 (1 + 2\lambda)^4 s}{4 (\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) + (1 + 2 \lambda) \Gamma_1 \big]^2 + (2 \lambda + 1 )^2 \sigma_1^2 + 2 \lambda^2(\sqrt{5} + \lambda)^2 + 2 (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 ) }\right\} \\
        %\leq & \E \exp \left\{ - \frac{C_1^2 \Delta_k^2 (1 + 2\lambda)^4 s}{4 (\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) -  (1 + 2 \lambda) 4 \big]^2 + (2 \lambda + 1 )^2 \sigma_1^2 + \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2) }\right\} \\
        %\leq &  T  \exp \left\{ - \frac{C_1^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 (7 \lambda + 4 - \mu_1)^2 + 4 (2 \lambda + 1 )^2 \sigma_1^2 + 4 [ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2]}\right\} \\
        %& \times \big[1 + C_1^2 \Delta_k^2 (1 + 2\lambda)^4  (h_1^* + h_2^*)\big] 
    %\end{aligned}
%\]
%\end{footnotesize}
%\fi
Therefore, to find $s$ such that $[1 - Q_{1, s} (\tau_k)] < T^{-2}$ on $\{ A_{1, s} \, \cap \, G_{1, s}\}$, let
\[
   \begin{aligned}
       s \geq s_{a, 3} := \frac{2 \log T}{h_2(\sigma_1, \sigma_{\omega},\lambda, \Delta_k, C_1)}.
   \end{aligned}
\]
%where $h_1^*$ and $h_2^*$ free of $s$ are $h_1(\cdot, \cdot, \cdot)$ and $h_2(\cdot, \cdot, \cdot)$ in Lemma \ref{lem_subE_ineq} by replacing the corresponding parameters. By the argument in \eqref{a_k_3_sw}, we have $a_{k, s, 3} \leq T^{-1}$ whenever $s \geq s_{a,3}$ defined above.

\todorw{People will think the below is part of C.2.5, which makes the structure confusing. If the decomposition has already been given at the begining and readers are clear that you just want to deal with components in each subsection, then we can omit the below. Otherwise, maybe make it a separate section.}
Now, combining all the results in Section C.2, we get that 
\[
    a_{k} \leq \underbrace{\max_{s = 0, \ldots, T -  1} a_{k, s}}_{\text{bound by a constant in \eqref{a_k_constant_3}}} \times\overbrace{\max _{j = 1, 2, 3} s_{a, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{a, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Here we do not give the explicit expression of the bound as it involves several complicated integrals, but its order is exactly $\log T$. However, for some explicit distributions, the expectation in Lemma \ref{lem_subE_ineq} can be bounded by some simpler displays, and hence we can get explicit expressions for the bounds in these cases. See Corollary \ref{cor_ber} and Corollary \ref{cor_gau}.
\end{remark}

\subsection{Bounding $b_k$}

Similar to the previous sections, for bounding $b_k = \sum_{s = 0}^{T - 1} b_{k, s}$, we decompose $b_{k, s} = \pr \big( Q_{k, s} (\tau_k) > T^{-1}\big) + 1$ as $b_k = b_{k, s, 1} + b_{k, s, 2} + b_{k, s, 3} + 1$ with
\[
    b_{k, s, 1} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A_{k, s}^{c} )\big],
\]
\[
    b_{k, s, 2} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A_{k, s}) \ind (G_{k, s}^c)\big],
\]
and
\[
    b_{k, s, 3} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A_{k, s}) \ind (G_{k, s})\big].
\]
Since $b_{k, s}$ is naturally bounded {the} constant $2$, it only needs to bound $s_{b, j}: = \max \{ s: b_{k, s, j} \geq T^{-1}\}$ with the $C \log T$ for $j = 1, 2, 3$ with some positive constant $C$.
%\hl{I would say "show xx is of order O(), or bound xx by c LogT where c is a constant. I am not familiar with "bound xx by order xx" - an order itself is not an upper bound.}

% \hl{the next sentence is not correct. Please carefully check every sentence to make sure they are readable, and then we can move to the proof logic. }


%For any $\star \in \{ (a, j), (b, j): j \in 1, 2, 3\}$, we denote $s_{\star}'$ as the quantity where we {replaces} $C_2$ in $s_{\star}$  by $C_1$. 

It is easy to see that $\pr (A^{c}_{k, s}) \leq T^{-2} \leq T^{-1}$ when $s \geq s_{a, 1}$. Next, similar as bounding $a_{k, s, 2}$, we take
\[
    s_{b, 2} := \frac{3 \log T}{h_1(\sigma_{k}, \sigma_{\omega}, \lambda, \Delta_k, C_2)}
\]
we have $b_{k, s, 2} \leq \E \big[ \ind(G_{k, s}^c) \big] \leq T^{-2} \leq T^{-1}$ (by just replacing $\sigma_1$ with $\sigma_k$ in $s_{a, 2}$).
%Then by the results on bounding $a_{k, s, 2}$, we have $\max\{ b_{k,s, 1}, \, b_{k, s, 2}\} \leq T^{-2} < T^{-1}$ as long as $s \geq \max \{ s_{a, 1}, \, s_{a, 2} \} \asymp \log T$. 
It remains to deal with $b_{k, s, 3}$. The basic idea is the same as bounding $a_{k, s, 3}$. We will first bound $\Gamma_k = \overline{Y}_{k, s}  - \overline{R}_{k, s}^*$ on the event $A_{k, s} \, \cap \, G_{k, s}$. %Write
%\[
    %A'_{k, s} = \bigg\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} < C_2 \Delta_k \bigg\} = \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \bigg\},
%\]
%and
%\[
    %\begin{aligned}
        %G_{k, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{k, s} - \overline{R}_{k, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_k -C_3 \Delta_k \leq \overline{Y}_{k, s} + \Gamma_k \leq \tau_k + C_3 \Delta_k \big\} \\
        %& = \big\{ \tau_k - 2 C_3 \Delta_k - \overline{R}_{k, s}^* \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \overline{R}_{k, s}^* \big\}.
        %& \subseteq \bigg\{ \tau_k - 2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2\lambda} \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2\lambda}\bigg\}.
    %\end{aligned}
%\]
%\hl{2 sentences (a common observation)}
%Hence, we conclude that 
%\[
    %\begin{aligned}
        %A_{k, s} \, \cap \, G_{k, s}\\
        %(\text{by plugging the inequality for $\overline{R}_{k, s}^*$ in } A'_{k, s}) \subseteq & \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \leq\tau_k + C_2 \Delta_k - \frac{\lambda}{1 + 2\lambda} \bigg\} \\
        %(\text{let } 2 C_3 \geq C_2) \subseteq & \bigg\{ \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2}  < \Gamma_k < \tau_k + C_2 \Delta_k \bigg\}
    %\end{aligned}
%\]
% It is worthwhile to recall that the construction of $s_{a, 1, 2}$ is free of any $\tau_k$, hence this argument is valid. 
Exactly the same as before, if we take
\[
    \tau_k := \frac{\mu_k}{2} - 3 C_1 \Delta_k,
\]
%we require $\tau_k - C_2 \Delta_k - \frac{\mu_k }{2} \leq 0$ to ensure $\Gamma_k$ falls in a relatively small interval. 
%To achieve this, we can just take
%\begin{equation}\label{requirement_4}
    %\tau_k = 2 C_2 \Delta_k + \mu_k / 2
%\end{equation}
%together with
%\begin{equation}\label{requirement_3}
    %2 C_3 \geq C_2.
%\end{equation}
then we will obtain that a bound for $\Gamma_k$ is $- \Gamma_k \in (C_1\Delta_k, 4) \subseteq (0, \infty)$, then 
%\[
    %C_1 \Delta_k = \tau_k  - C_1 \Delta_k - \frac{\mu_k}{2} < \Gamma_k < \tau_k + C_1 \Delta_k = 3 C_1 \Delta_k + \frac{\mu_k}{2} \leq \frac{7}{2} < 4,
%\]
%\hl{avoid notations like below.. $1 > 2 < 3$.}
%i.e. $\Gamma_k \in (C_2 \Delta_k, 4) \subset (0, + \infty)$. Similar to the technique in \eqref{a_2_bound}, we have
% \hl{I understand that equations are part of the text, but I would still recommend at least putting one or two words in between (such as "we have" }
\[
    \begin{aligned}
         &  Q_{k,s} (\tau_k)\big] \ind (A_{k, s}) \ind(G_{k, s}) \\
         \alignedoverset{\text{apply steps in  \eqref{bound_I}}}{\leq} T \E\exp \left\{ - \frac{9 (- \Gamma_k)^2 \Delta_k^2 s^2 }{6  \sigma_{\omega}^2 s  \left[ 2 \lambda^2 \overline{\zeta^{(k)}} +  2 \lambda^2 \sigma_1^2 +(- \Gamma_k)^2   \right] }\right\} \\
         \alignedoverset{\text{by the bound of } \Gamma_1}{\leq} T \E\exp \left\{ - \frac{256 \Delta_k^2 s^2 }{6  \sigma_{\omega}^2 s  \left[ 2 \lambda^2 \overline{\zeta^{(k)}} +  2 \lambda^2 \sigma_1^2 +C_1^2 \Delta_k^2  \right] }\right\}  \\
         \alignedoverset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} T \exp \left\{ - s \times  h_3 (\sigma_k, \sigma_{\omega},\lambda, \Delta_k )\right\}.
    \end{aligned}
\]
%\[
    %\begin{aligned}
        %& Q_{k, s}\left(\tau_{k}\right) \ind\left(A_{k, s}^{\prime}\right) \ind\left(G_{k, s}\right) = \E \pr \left(\overline{Y}_{k, s}-\overline{R}_{k, s}^{*}>\Gamma_{k} \mid \mathcal{H}_{k, T}\right) \ind\left(A_{k, s}^{\prime}\right) \ind\left(G_{k, s}\right) \\
        %= & \E \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s (R_{k, i} - \overline{R}_{k, s}) \omega_i + \lambda \sum_{i = 1}^s (2 R_{k, i} \omega_i - \overline{R}_{k, s} \omega_i' - \overline{R}_{k, s} \omega_i'')
        %\\
        %& \qquad \qquad \qquad + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega''_i) - \Gamma_k (1 + 2\lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] < 0\Bigg\}\\
        %\overset{\text{apply steps in  \eqref{G_function_bound_2}}}{\leq} & \E \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 \Gamma_k^2 s^2 }{12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_k^2) + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 \Gamma_k^2  \big]}\right\} \\
        %\overset{\text{by the bound of } \Gamma_k}{\leq} & \E \exp \left\{ - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 s }{12 \lambda^2 \subE (8 \sqrt{2} \sigma_k^2) + \big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \big]}\right\}\\
        %\overset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} & \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s ( h_1^{**} + h_2^{**}) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2 \big]}\right\} \\
        %\overset{\text{by }s \leq T}{\leq} & T \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 ( h_1^{**} + h_2^{**}) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2 \big]}\right\}.
    %\end{aligned}
%\]
%\hl{Not understandable.}
where $h_3$ is defined in Lemma \ref{lem_subE_ineq} by replacing the corresponding parameters again and $\overline{\zeta^{(k)}} = \frac{1}{s} \sum_{i = 1}^s \zeta^{(k)}_i$ with $\zeta^{(k)}_i$ are independent sub-Exponential variable such that $\zeta^{(k)}_i \sim \subE(8 \sqrt{2} \sigma_k^2)$. Therefore, one can just take 
\[
    \begin{aligned}
         s \geq s_{b, 3} := \frac{2 \log T}{h_3(\sigma_k, \sigma_{\omega},\lambda, \Delta_k, C_1)}
    \end{aligned}
\]
to ensure $b_{k, s, 3} \leq T^{-1}$.
%\hl{The sentence break is weird, if not wrong..}
And then, by using a similar argument, we have 
\[
    b_{k} \leq 2 \times\overbrace{\max _{j = 1, 2, 3} s_{b, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{b, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Similarly, for specific reward distributions, we can bound $b_k$ in $\log T$ with some simple and specific coefficients. See Corollary \ref{cor_ber} and Corollary \ref{cor_gau}.
\end{remark}

%Finally, {what} remains is to show {that} the restrictions (\ref{requirement_0}), (\ref{requirement_1}), (\ref{requirement_2}), (\ref{requirement_3}), and (\ref{requirement_4}) are compatible. Indeed, they will build the following system of constraints,
%\[
    %\left\{ \begin{array}{l}
         %\frac{\mu_1}{2} - 2 C_1 \Delta_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
         %2 C_` \Delta_k + \frac{\mu_k}{2} \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
        %\tau_k - \frac{\mu_1}{2} - C_1 \Delta_k  \leq \tau_k + C_1\Delta_k - \frac{\mu_k }{2} \\
        %C_1 \geq 2C_2 \\
        %2 C_2 \geq C_1 \\
        %\frac{\mu_1}{2} - 2 C_1 \Delta_k = 2 C_1 \Delta_k + \frac{\mu_k}{2}
    %\end{array}\right..
%\]
%We can see that 
%\[
    %C_1 = \frac{1}{8}, \qquad C_2 = \frac{1}{16},
%\]
%is the unique solution of the above system. 
Up to now, we have finished the first part in Theorem \ref{thm.MAB}. For the second part, 
\begin{equation*}
    \begin{aligned}
        \operatorname{Reg}_T & = \sum_{\Delta_k : \Delta_k < \Delta} \Delta_k \E J_{k, T} + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k \E J_{k, T} \\
        & \lesssim T \Delta + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k  +  \sum_{\Delta_k : \Delta_k \geq \Delta} \frac{\log T}{\Delta_k} \\
        & \lesssim T \Delta + \frac{ K \log T}{\Delta} \lesssim \sqrt{K T \log T}.
    \end{aligned}
\end{equation*}
for any previously specified $\Delta \in (0, 1)$ by Cauchy inequality. Therefore, we finish the proof of Theorem \ref{thm.MAB}.



%\textit{{Bounded case need to separate to prove?}}

%As all the restrict conditions for $C_1, C_2, C_3$ are exactly the same as previous, we still take $C_1 = C_2 = \frac{1}{8}$ and $C_3 = \frac{1}{16}$. And the final bounds need to be doubled.

\section{Proof of Corollary \ref{cor_ber}}

TBA.

\iffalse
The similar as stated in Section \ref{proof_thm}. Take advantage of Bernoulli rewards are bounded in $[0, 1]$, one can get that 
\[
    \begin{aligned}
        a_{k, s} & \leq \big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ).
    \end{aligned}
\]
\todohw{Need to revise later}
as long as the parameters satisfying the restrictions in Theorem \ref{thm.MAB}. Then we need to control $a_{k, s, j}$ with $\log T$ for $j \in \{ 1, 2, 3\}$. These steps will be completed in the following.
\begin{itemize}
    \item For $a_{k, s, 1}$, recall the inequality \eqref{a_k_1_bound}. We use the fact that the rewards are bounded in $[0,1]$, Hoeffding inequality will give
    \[
        \pr (A_{1, s}^c) = \pr (\mu_1 - \overline{R}_{1, s} \geq (1 +2  \lambda) C_1 \Delta_k) \leq \exp \left\{ - 2 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2 s\right\}.
    \]
    Hence, take
    \[
        s \geq s_{a, 1} := \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} \log T,
    \]
    we have $\pr (A_{1, s}^c) \leq T^{-2}$ , and $a_{k, s, 1} \leq T^{-1}$ then.
    
    \item For $a_{k, s, 2}$, one can {follow} the same steps as in the proof of Theorem \ref{thm.MAB}, while constants in the upper bound can be simpler and sharper due to the distribution of rewards being Bernoulli.
    To be specific, the variance $\sigma_{\omega}^{-2} \var(f_1 + f_2 - f_3)$ in \eqref{bound_var_f} can be bound by a deterministic quantity:
    
    % \hl{Can not find this one by one. We should make sure the writing is readable, and then discuss the proof.}
    \[
        \begin{aligned}
            & \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \\
            \overset{\text{by the same steps in} \eqref{G_function_bound_2}}{\leq} & 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
            \overset{\text{use the fact } R_{1, i} \in [0, 1]}{\leq} & 6 \lambda^2 s + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big].
        \end{aligned}
    \]
    Then use \eqref{a_2_bound} again, 
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^{2} \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
            & \leq 2 T \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s}{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }\right\}.
        \end{aligned}
    \]
    Hence, if we take 
    \[
        \begin{aligned}
            s \geq s_{a, 2} & := \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log T \\
            (
            \text{require } T \geq 2) & \geq \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{9\sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log (2 T^2)
        \end{aligned}
    \]
    and then $a_{k, s, 2} \leq T^{-1}$.
    \iffalse
    Then if we denote 
    \[
        f(x) := \exp \left\{ - \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k^2 s}{4 \Big[ s^{- 1 / 2} (2 \lambda + 1) (x - s \mu_1) + \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] \Big]^2 + 2 s^{-1} g_5(s, \lambda) \big]^2} \right\},
    \]
    then $f(x)$ is a decreasing function on $0 \leq x \leq s \mu_1$ and an increasing function on $x \geq s \mu_1$. By symmetric technique of Binomial distribution and Lemma 2 in \cite{kveton2019garbage}, we have
    \[
        a_{k, s, 2} \leq {\red{4}} T \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x ; s, \mu_1) f(x) \leq 4 T \left[ \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s})+\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \right].
    \]
    Similarly to \cite{kveton2019garbage}, we can show that 
    \[
        \begin{aligned}
            & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s}) +\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            \leq & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] \exp \left\{- \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k^2 s}{4 \left[ \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] - (2 \lambda + 1) (i + 1)\right]^2 + 2 s^{-1} g_5(s, \lambda)} \right\} \\
            & \qquad +\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            \leq & \int_1^{s \mu_1 + 1} \exp \{ - 2 (u - 1)^2 \} \exp \left\{ - \frac{c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3}\right\}  \, du \\
            = & \int_1^{s \mu_1 + 1} \exp \left\{ - \left[ 2 (u - 1)^2 + \frac{c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3} \right] \right\}  \, du \\
            \leq & \int_1^{s \mu_1 + 1} \exp \left\{- \left[ 2 s^2 \mu_1^2 + \frac{c_1 s}{4(c_2 - (2 \lambda + 1) (s \mu_1 + 1))^2}\right] \right\} \, du \\
            \leq & \int_1^{s \mu_1 + 1} \exp \left\{ - 2 s \mu_1^2 \right\} \, du \leq T \mu_1 \exp \left\{ - 2 s \mu_1^2 \right\}
            %\leq & s \mu_1 \exp \left\{ - s \mu_1 \right\} \leq T \mu_1 \exp \{ - s \mu_1 \}
            % \leq & \left[ \int_1^{s \mu_1 + 1} \exp \{- 4 (u - 1)^2 \} \, du \right]^{1 / 2} \left[\int_1^{s \mu_1 + 1} \exp \left\{ - \frac{2c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3}\right\} \, du \right]^{1 / 2} \\
            %= & \left[ \right] \exp 
        \end{aligned}
    \]
    with $c_1 = 64^{-1} (1 + 2 \lambda)^4 \Delta_k^2$, $c_2 = \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big]$, and $c_3 = \lambda^2 \big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \big\}$. Therefore, if $T \geq 2$, by taking 
    \[
        \red{s_{a, 2} \geq \frac{5 \log T}{\mu_1^2}\geq \frac{\log 4 T^3 \mu_1}{\mu_1^2}}
    \]
    one will have 
    \[
        a_{k, s, 2} \leq T^{-1}
    \]
    \fi
    \item To deal with $a_{k, s, 3}$,
    %recall we have bound $s^{-1} \var(f_1 + f_2 - f_3)$ with a constant times $s$. Then, 
    by taking the same technique as $a_{k, s, 2}$, we have
    \[
        \begin{aligned}
             \big[ 1 - Q_{1,s} (\tau_k)\big] \ind(A_{1, s}) \ind(G_{1, s}) & \leq \E \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 (- \Gamma_1)^2 s^2 }{ s \big[ 4 \lambda^2 (\lambda^2 + \lambda + 4)  + 6  (1 + 2\lambda)^2 (- \Gamma_1)^2  \big]}\right\} \\
             & \leq \exp \left\{ - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 s }{ 4 \lambda^2 (\lambda^2 + \lambda + 4)  + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2 }\right\} \leq T^{-2}
        \end{aligned}
    \]
    as long as 
    \[
        s \geq s_{a, 3} := \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \log T.
    \]
    \iffalse
    \[
        g(x) = \exp \left\{ - \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k s}{4 \Big[ s^{- / 2} (2 \lambda + 1) (x - s \mu_1) + \lambda \big[ (\lambda + \mu_1) + 4 (1 + 2 \lambda)\big] \Big]^2 + 2 s^{-1} g_5(s, \lambda)}\right\}
    \]
    one can show that
    \[
        \begin{aligned}
            \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq 2 \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x; s, \mu_1) g(x) \leq 2 s \mu_1 \exp \{ - s \mu_1\} \leq T^{-1}
        \end{aligned}
    \]
    as long as $s \geq s_{a, 3} := s_{a, 2}$. And hence, in this case, one will have $a_{k, s, 3} \leq T^{-1}$.
    \fi
\end{itemize}

Combining these results above with 
\[
    \begin{aligned}
        &\max \left\{ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2}, \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3\sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \right\} \\
        \leq & \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2}\\
        = & \frac{36 (1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} + \frac{32^2 \lambda^2 \sigma_{\omega}^{2}  (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2},
    \end{aligned}
\]
we obtain that 
\[
    \begin{aligned}
        a_k & \leq \max_{s = 0, \ldots, T -  1} a_{k, s} \times\max _{j = 1, 2, 3} s_{a, j} + 3 T^{-1} \cdot\big(T - \max_{j = 1, 2, 3} s_{a, j}\big) \\
        & \leq \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big] \\
        & \qquad \qquad \times \left[  \frac{36 (1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{- 2}  (1 + 2 \lambda)^2} + \frac{32^2 \lambda^2 \sigma_{\omega}^{2}  (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2} \right] 
        \log T + 3.
    \end{aligned}
\]
%Specially, if $\sigma_{\omega}^2 \geq 1$ and $\lambda \geq 1$, by using the fact that $\lambda^2\big[ (\lambda - 1)^2 + \lambda^2\big] \geq \lambda (\lambda + 1)$, one will have 
%\[
    %a_k \leq  \left[ e^{ 3 (2\lambda + 1)^2 / 2} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right] \left[ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \red{\frac{5}{\mu_1^2}}\right] \log T + 3.
%\]
By using the same technique, one can show that 
\[
    \begin{aligned}
        b_k & \leq 2 \times\max _{j = 1, 2, 3} s_{b, j} + 3 T^{-1} \cdot\big(T - \max_{j = 1, 2, 3} s_{b, j}\big) \\
        & \leq 2 \times \left\{ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_2^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \right\} \log T + 3 \\
        & \leq  2 \left[  \frac{18(1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{- 2}  (1 + 2 \lambda)^2} + \frac{2 \times16^2  \sigma_{\omega}^{2}  \lambda^2 (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2} \right] 
        \log T + 3
    \end{aligned}
\]
These results together with Lemma \ref{lem.a.b} give Corollary \ref{cor_ber}.
\fi

\section{Proof of Corollary \ref{cor_gau}}

TBA.

\iffalse
The basic proof idea is the same as the proof of Corollary \ref{cor_ber}. Since the Gaussian variable is still sub-Gaussian, the constant bound in \eqref{a_k_constant_3} is still available for this case. And next we will bound $s_{a,  j} :=  \min \{ s: a_{k, s, j} \leq T^{-1}\}$ with $\log T$ under the Gaussian case.
%except the constant bound of $a_{k, s}$ is simpler due to the nice property of Gaussian distribution. And we follow the steps below:
\iffalse
\begin{itemize}
    \item[1.] By using the fact that $s^2 (\overline{R}_{1, s} - \mu_1) \sim \chi^2(s)$,
    \[
        \begin{aligned}
            a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
            & \leq 
        \end{aligned}
    \]
    \[
        \begin{aligned}
            a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \\
            (\text{by using the MGF of } \chi^2(s))& = \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]s^2}\right]^{- \frac{s}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
            (\text{take } s = 1) & \leq \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        \end{aligned}
    \]
    since $s = 0$ naturally satisfies the above inequality. This further implies we will need
    \[
        \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]} < 1
    \]
    with its sufficient condition as 
    \[
        \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \leq 1
    \]
    i.e. $\lambda \geq 1 + \sqrt{2}$. In a word, under the assumptions in Corollary \ref{cor_gau}, one will have
    \[
        \begin{aligned}
            a_{k, s} & \leq \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
            & \leq \left[ 1 - \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}. 
        \end{aligned}
    \]
    with $\sigma_{\omega}^2 \geq 1$ for $s \in \{ 0, \ldots, T - 1\}$.
    
    \item[2.] For controlling $a_{k}$, one can easily show that 
    \[
        a_k \leq \left\{ \left[ 1 - \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right\} \left[ \frac{65}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{6}{\log 2} \right] \log T + 3.
    \]
    by the following statements.
    \begin{itemize}
        \item[2.1] Still use sub-Gaussian inequality to get that we have $a_{k, s, 1} \leq T^{-1}$ when
        \[
            s \geq s_{a, 1} = \frac{64 }{(1 + 2 \lambda)^2 \Delta_k^2} \log T.
        \]
        
        \item[2.2] For dealing with $a_{k, s, 2}$, we again use the fact that 
        \[
            \Big[ \sqrt{s} (\overline{R}_{1, s} - \mu_1) + \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] \Big]^2 \, \sim \, \chi^2(s; s^{-1}\lambda^2 \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big]^2 )
        \]
        is a noncentral chi-squared distribution, then it will lead to the result that 
        \[
            \begin{aligned}
                a_{k, s, 2} & \leq 2 T \E \exp \left\{ - \frac{64^{-1}(1 + 2 \lambda)^4 \Delta_k^2 s}{4\big[ \chi^2(s; s^{-1}\lambda^2 \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k) + 2 s^{-1}g_5(s, \lambda)\big]}\right\} \\
                & \leq 2 T \E \exp \left\{ - \frac{64^{-1} (1 + 2\lambda)^4 \Delta_k^2 s}{4  \big[ \chi^2(s) + s^{-1}g_5(s, \lambda)\big]}\right\} \\
                & \leq 2 T \int_0^{\infty} \frac{2^{- s / 2}}{\Gamma(s / 2)} u^{-s / 2-1} e^{-1 /(2 u)} e^ { - 256^{-1} (1 + 2\lambda)^4 \Delta_k^2 s u} \, du \\
                (\text{by Cauchy inequality})& \leq  2 T \frac{2^{- s / 2}}{\Gamma(s / 2)}  \int_0^{\infty} u^{- s / 2 - 1} e^{- 1 / u} e^{- 16 (1 + 2 \lambda)^4 \Delta_k \sqrt{s}} \, du  \\
                & =  2 T \frac{2^{- s / 2}}{\Gamma(s / 2)}  \Gamma(s /2 ) e^{- 16 (1 + \lambda)^2 \Delta_k \sqrt{s}} \\
                & \leq 2 T \exp \left\{ - \left[ \frac{\log 2}{2} s + 16 (1 + 2 \lambda)^2 \Delta_k \sqrt{s}\right]\right\} \leq T^{-1}
            \end{aligned} 
        \]
        if 
        \[
            s \geq s_{a, 2} :=  \left[ \frac{1}{8(1 + 2 \lambda)^2 \Delta_k} + \frac{4}{\log 2}\right] \log T
        \]
        \item[2.3] Just by replacing $C_3 \Delta_k$ by $(- \Gamma_1)$ which is bounded in $(C_1 \Delta_k, 4)$, and we will get that
        \[
            \begin{aligned}
                \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq  \exp \left\{ - \left[ \frac{\log 2}{2} s + 16 (1 + 2 \lambda)^2 \Delta_k \sqrt{s}\right]\right\} \leq T^{-1}
            \end{aligned}
        \]
        i.e. $a_{k, s, 3} \leq T^{-1}$ whenever 
        \[
            s \geq s_{a, 3} := \left[ \frac{1}{16(1 + 2 \lambda)^2 \Delta_k} + \frac{2}{\log 2}\right] \log T.
        \]
    \end{itemize}
    
    \item[3.] Exactly the same as 2., we can get that 
    \[
        b_{k} \leq 2 \left[ \frac{33}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{6}{\log 2}\right] \log T + 3.
    \]
\end{itemize}
These results give Corollary \ref{cor_gau}.
\fi

\begin{itemize}
    \item For $a_{k, s, 1}$, we still use the same steps of proof in Theorem \ref{thm.MAB} directly: take
    \[
        s \geq s_{a, 1} = \frac{\sigma_1^2}{C_1^2 (1 + 2 \lambda)^2 \Delta_k^2} \log T,
    \]
    we have $a_{k, s, 1} \leq T^{-1}$.
    
    \item For $a_{k, s, 2}$, we note that
    \begin{equation}\label{chi_square}
    	\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 = \sigma_1^2 \sum_{i = 1}^s \left( \frac{R_{1, i} - \mu_1}{\sigma_1} \right)^2 \, \sim \, \sigma_1^2 \chi^2(s).
    \end{equation}
    is a chi-square distribution.
    By using the density of chi-square distribution, we have a bound of \eqref{a_2_bound} as
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T \E \exp \left\{ - \frac{9 C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2}{2 \sigma_{\omega}^{2} \big[ \mathbb{G}_{1} (s, \lambda) + \mathbb{G}_{2} (s, \lambda) + g_3(s, \lambda)\big]}\right\} \\
            & \overset{\text{use the bound in \eqref{G_function_bound_2} and \eqref{chi_square}}}{\leq} 2 T \E \exp \left\{ - \frac{9 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2}{12 \lambda^2 \sigma_1^2 \chi^2(s) + 2 s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big] }\right\} \\
            & =  2 T \int_0^{\infty} \exp \left\{ - \frac{D_1 s^2}{D_2 u + D_3}\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u / 2} \, du \\
            & = 2 T \int_0^{\infty} \exp \left\{ - \left[ \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \right]\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u / 4} \, du
        \end{aligned}
    \]
    %{\color{blue}{
    with
    \[
        D_1 = 9 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2, \qquad D_2 = 12 \lambda^2 \sigma_1^2, \qquad D_3 = 2 \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big].
    \]
    Write 
    \[
        \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} = D_4 s^2 + \frac{D_2 u^2 + (D_3 - 4 D_2 D_4 s^2) u + 4 (D_1 - D_3 D_4) s^2}{4 (D_2 u + D_3) }
    \]
    with $D_4 > 0$ is a constant making
    \begin{equation}\label{gau_D_4}
        D_2 u^2 + (D_3 - 4 D_2 D_4 s^2) u + 4 (D_1 - D_3 D_4) s^2 \geq 0
    \end{equation}
    strictly holds on $u \in (0, \infty)$. A sufficient condition for \eqref{gau_D_4} is
    \[
         \begin{aligned}
             \boldsymbol\Delta & = (D_3 - 4 D_2 D_4 s^2)^2 - 4 D_2 \big[ 4 (D_1 - D_3 D_4) s^2 \big] \\
             & = 16 D_2^2 D_4^2 s^4 + 8 D_2 (D_3 D_4 - 2) s^2 + D_3^2 > 0, \qquad s \in [T].
         \end{aligned}
    \]
    For ensuring the above holds, one only needs to ask
    \[
        D_3 D_4 -  2 \geq 0.
    \]
    Therefore, we choose 
    \[
        D_4 := \frac{2}{D_3} = \frac{1}{\big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big]}.
    \]
    and hence 
    \[
        \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \geq \frac{2}{D_3} s^2, \qquad \forall \, u > 0.
    \]
    It will furthermore give
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T \int_0^{\infty} \exp \left\{ - \left[ \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \right]\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u  / 4}\, du \\
            & \leq 2 T \int_0^{\infty} \exp \left\{ - \frac{2 s^2 }{D_3} \right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u /4} \, du \\
            (\text{use the density of Gamma distribution})& = 2 T \exp \left\{ - \frac{2 s^2}{D_3} \right\} 2^{s / 2} \\
            & = 2 T \exp \left\{ -  \frac{2 s^2}{D_3} + \frac{s \log 2} {2} \right\} \leq 2 T \exp \left\{ -  \frac{2 s^2}{D_3} \right\} .
        \end{aligned}
    \]
    Hence, we can take
    \[
        s \geq s_{a, 2} := \frac{3 D_3 \log T}{2} = 3 \sigma_{\omega}^{2} \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big] \log T.
    \]
    to guarantee $a_{k, s, 2} \leq T^{-1}$ for any $T \geq 2$.
    \item The approach to deal with $a_{k, s, 3}$ is the same as above, and we can get we have $a_{k, s, 3} \leq T^{-1}$ whenever
    \[
        s \geq s_{a, 3} = 3  \sigma_{\omega}^{2}  \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2\big] \log T.
    \]

    %}}
\end{itemize}

Combining the expressions of $a_{k, s, j}$, $j \in 1, 2, 3$, we obtain 
    \[
        \begin{aligned}
            a_{k} & \leq \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big] \\
            & \qquad \qquad \times \left[  \frac{16 \sigma_1^2}{(1 + 2 \lambda)^2 \Delta_k^2} + 12 \lambda^2  \sigma_{\omega}^{2} (\lambda^2 + \lambda + 4)  + \frac{153}{256} (1 + 2 \lambda)^2  \sigma_{\omega}^{2}  \Delta_k^2 \right] 
        \log T + 3.
        \end{aligned}
    \]
And similarly the bound of $b_k$ can be also proven as follows:
\[
     b_k \leq 2 \left[  \frac{16 \sigma_k^2}{(1 + 2 \lambda)^2 \Delta_k^2} + 9 \lambda^2  \sigma_{\omega}^2 (\lambda^2 + \lambda + 4)  + \frac{297}{512} (1 + 2 \lambda)^2 \sigma_{\omega}^{2} \Delta_k^2 \right] \log T + 3.
\]
\fi

==> 9_Proof_Lemmas.tex <==
\section{Proof of Lemmas}\label{sec:proof_lemma}

\subsection{Proof of Lemma \ref{lem.a.b}}
\begin{proof}
    % Here we prove this lemma briefly for understanding what $a_k$ and $b_k$ actually is and how we bound $a_k$ and $b_k$ in a proper sense. 
    First, we note that
    $\operatorname{Reg}_T = \sum_{k = 2}^K \Delta_k \E \sum_{s = 1}^T \ind(I_t = k)$. If we denote $E_{k, t} := \{ \overline{Y}_{k, t} \leq \tau_k \}$, then we have the following decomposition,
    \[
        \E J_{k, T} := \E \sum_{t = 1}^T \ind(I_t = k) = \E \sum_{t = 1}^T \ind(I_t = k, E_{k, t} \text{ occurs}) + \E \sum_{t = 1}^T \ind(I_t = k, E_{k, t}^c \text{ occurs}).
    \]
    Then, we can have $a_k$ and $b_k$ bound the two quantities above respectively. Indeed, we have
    \[
        \sum_{t = 1}^T \ind(I_t = k, E_{k, t} \text{ occurs}) \leq \sum_{s = 0}^{T - 1} \sum_{t = 1}^T \ind \left\{ \max_{j} \overline{Y}_{j, t} \leq \tau_k, J_{1, t - 1} =  s \right\} ,
    \]
    then apply the Doob extension theory (see Theorem 5.2 in Chapter II of \cite{doob1953stochastic}), we have got the above can be bounded by $N_{1, s}(\tau) \wedge T$, i.e. $\E \sum_{t = 1}^T \ind(I_t = k, E_{k, t} \text{ occurs})  \leq a_k$. Here $a_k$ can be understood as the anti-concentration property on pre-specific level $\tau$ of the rewards from the optimal arm. 
    
    %Fortunately, under our case, if we choose proper $\tau_k$, we can only focus on the anti-concentration of the optimal arm, while the that of other arms can be transformed to their major probability (one minus the tail probability). 
    
    For obtaining $b_k$, we let $\mathcal{T} = \{ t \in [T] : Q_{k, J_{k, t - 1}} (\tau_k )\geq 1 / T \}$,
    %which actually represents the time points such that the action in the last step does have some possibility to choose itself. 
    then, we have
    \[
        \begin{aligned}
            \E \sum_{t = 1}^T \ind(I_t = k, E_{k, t}^c \text{ occurs}) & \leq \E \sum_{t \in \mathcal{T}} \ind(I_t = k) + \E \sum_{t \notin \mathcal{T}} \ind (E_{k, t}^c) \\
            & \leq \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) \geq 1 / T \big) + 1 =: b_k. 
        \end{aligned}
    \]
    It is obvious that $b_k$ is the summation of the probability of tail probability larger than $T^{-1}$. 
    
    
    %And $a_k$ and $b_k$ here should be explained as expectation.
\end{proof}

\subsection{Proof of Lemma \ref{lemma:gaussian_weight}}

%This lemma gives a relative lower but easy upper and lower bound for Gaussian tail, the proof can be also seen in the proof part of \cite{zhang2022sharper}.

\begin{proof}
	Denote $Q(x) := \pr (Z > x)$ for $x > 0$ as the tail probability for standard Gaussian variable $Z$. Let $Z_1$ and $Z_2$ are two independent standard Gaussian random variables, then
	\[
	    \begin{aligned} 
	        \pr (Z_1 \leq x, \, Z_2 \leq x) &=\int_{-x}^x \int_{-x}^x \frac{1}{2 \pi} \exp \left[\left(-z_1^2-z_2^2\right) / 2\right] \, \mathrm{d} z_1 \mathrm{d} z_2 \\ 
	        & \leq \int_0^{\sqrt{2} x} \int_0^{2 \pi} \frac{1}{2 \pi} \exp \left(-r^2 / 2\right) r \, \mathrm{d} \theta \, \mathrm{d} r \\ 
	        &=1-\exp (-x^2)
	    \end{aligned}
	\]
	giving $[1-2 Q(x)]^2 \leq 1-\exp (-x^2)$ for $x \geq 0$, or, equivalently, $\exp (-x^2) \leq 4 Q(x)-4 Q^2(x)$. But, since $4 Q^2(x)>0$ for all $x$, we get that
	\[
	    Q(x) > \frac{1}{4} \exp (-x^2)
	\]
    which is a lower bound of the form desired. For the upper bound, we note that
    \[
        \begin{aligned}
            \exp \left(x^2 / 2\right) Q(x) &=\exp \left(x^2 / 2\right) \int_x^{\infty}(2 \pi)^{-1 / 2} \exp \left(-t^2 / 2\right) \mathrm{d} t \\
            &=\int_x^{\infty}(2 \pi)^{-1 / 2} \exp \left(-\left(t^2-x^2\right) / 2\right) \mathrm{d} t \\
            &<\int_x^{\infty}(2 \pi)^{-1 / 2} \exp \left(-(t-x)^2 / 2\right) \mathrm{d} t =\frac{1}{2},
         \end{aligned}
    \]
    which gives the upper bound.
\end{proof}

%\iffalse
%\subsection{Proof of Lemma \ref{lem:gau_low}}
%\begin{proof}
    %Denote $Z : = \sum_{i = 1}^n x_i \omega_i - y \sim N(\sum_{i = 1}^n x_i - y, \sigma_{\omega}^2 \sum_{i = 1}^n x_i^2)$, then
    %\[
        %\begin{aligned}
            %& \pr \left( \sum_{i = 1}^n x_i \omega_i > y \right)\\
            %= & \pr (Z > 0) \\
            %= & \Bigg[ 1 \left(\sum_{i = 1}^n x_i - y > 0 \right) + 1 \left(\sum_{i = 1}^n x_i - y \leq 0 \right) \Bigg] \pr \left( \frac{Z - \left( \sum_{i = 1}^n x_i - y \right)}{\sigma_{\omega} \sqrt{\sum_{i = 1}^n x_i^2}} > - \frac{\left( \sum_{i = 1}^n x_i - y \right)}{\sigma_{\omega} \sqrt{\sum_{i = 1}^n x_i^2}}\right) \\
            %\geq & \Bigg[ 1 \left(\sum_{i = 1}^n x_i - y > \sqrt{2 \pi} \right) + 1 \left(0 < \sum_{i = 1}^n x_i - y \leq \sqrt{2 \pi} \right) \Bigg] \pr \left( \frac{Z - \left( \sum_{i = 1}^n x_i - y \right)}{\sigma_{\omega} \sqrt{\sum_{i = 1}^n x_i^2}} > - \frac{\left( \sum_{i = 1}^n x_i - y \right)}{\sigma_{\omega} \sqrt{\sum_{i = 1}^n x_i^2}}\right) \\
            %\geq & \exp \left\{ -\frac{3 \left(\sum_{i = 1}^n x_i - y \right)^2}{2 \sigma_{\omega}^2 \sum_{i = 1}^n x_i^2} \right\} 1 \left(\sum_{i = 1}^n x_i - y > \sqrt{2 \pi} \right) + \big[ 1 - \Phi(\sqrt{2 \pi})\big]  1 \left(0 < \sum_{i = 1}^n x_i - y \leq \sqrt{2 \pi} \right) 
        %\end{aligned}
    %\]
    %where we use the following inequality 
    %\begin{equation*}
        %\pr (Z \geq t) \geq \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot 1 (0 \leq t \leq \sqrt{2\pi}) + \exp (- 3 t^2  / 2) \cdot 1(t \geq \sqrt{2 \pi})
    %\end{equation*}
    %for any $Z \sim N(0, 1)$. 
%\end{proof}
%\fi

%\subsection{Proof of Lemma \ref{lemma:gaussian_weight}}
%\begin{proof}
    %Define $Z: = \sum_{i = 1}^n x_i \omega_i - \left(\sum_{i = 1}^n y_i \omega'_i + \sum_{i = 1}^n z_i \omega''_i)\right)$, then $Z \sim N \big(S_x - S_y - S_z, (T_x + T_y + T_z) \sigma_{\omega}^2 \big)$, and 
    %\begin{equation*}
    %    \begin{aligned}
          %  & \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{i = 1}^n y_i \omega'_i + \sum_{i = 1}^n z_i \omega''_i \right) = \pr (Z > 0)  \\
         %   = & \ind(S_x - S_y - S_z \geq 0) \cdot \pr \bigg( \frac{Z - (S_x - S_y - S_z )}{\sigma_{\omega} \sqrt{T_x + T_y + T_z} } > \frac{S_x - S_y - S_z}{\sigma_{\omega} \sqrt{T_x + T_y + T_z} }\bigg) \\
        %    & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + \ind(S_x - S_y - S_z < 0) \cdot \pr \bigg( \frac{Z - (S_x - S_y - S_z )}{\sigma_{\omega} \sqrt{T_x + T_y + T_z} } > \frac{S_x - S_y - S_z}{\sigma_{\omega} \sqrt{T_x + T_y + T_z} }\bigg) \\
       %     \geq & \exp \bigg\{ - \frac{3(S_x - S_y - S_z)^2}{2 \sigma_{\omega}^2(T_x + T_y + T_z)}\bigg\} \cdot \ind \big(S_x \geq S_y + S_z + \sqrt{2\pi} \big) + \big( 1 - \Phi(\sqrt{2\pi} )\big) \cdot \ind \big(S_y + S_z  < S_x \leq S_y + S_z + \sqrt{2\pi}\big) \\
      %      & \qquad \qquad \qquad \qquad + \frac{1}{2} \cdot \ind (S_x \leq S_y + S_z) \\
     %       \geq & \exp \bigg\{ - \frac{3(S_x - S_y - S_z)^2}{2 \sigma_{\omega}^2(T_x + T_y + T_z)}\bigg\} \cdot \ind \big(S_x \geq S_y + S_z + \sqrt{2\pi} \big) + \big( 1 - \Phi(\sqrt{2\pi} )\big) \cdot \ind\big(S_x \leq S_y + S_z + \sqrt{2\pi}\big). 
    %    \end{aligned}
    %\end{equation*}
    %where we use the following inequality 
    %\begin{equation*}
    %    \pr (Z \geq t) \geq \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot \ind (0 \leq t \leq \sqrt{2\pi}) + \exp (- 3 t^2  / 2) \cdot \ind(t \geq \sqrt{2 \pi})
    %\end{equation*}
    %for any $Z \sim N(0, 1)$. Combining this result with the Cauchy inequality concludes our proof for $n \geq 2$. 
    % which gives the first result. And the second result is by the Cauchy inequality. 
%\end{proof}

\subsection{Proof of Lemma \ref{lem_subGtosubE}}

\begin{proof}
    Note that $X - \mu \sim \subG (\sigma^2)$ implies
    \begin{equation}\label{lem_subGtosubE_1}
        \overline{X} - \mu \sim \subG (\sigma^2 / n)
    \end{equation}
    by the fact that
    \[
        \begin{aligned}
        	\E \exp \left\{ s (\overline{X} - \mu) \right\} & = \prod_{i = 1}^n \exp \left\{ \frac{s}{n} ({X}_i - \mu) \right\} \\
        	(\text{by } X_i - \mu \text{ is sub-Gaussian}) & \leq \prod_{i = 1}^n \exp \left\{ \frac{s^2}{n^2} \frac{\sigma^2}{2}\right\} = \exp \left\{ \frac{s^2 (\sigma^2 / n)}{2}\right\}.
        \end{aligned}
    \]
    And then by Proposition 4.3 in \cite{zhang2020concentration}, $(\overline{X} - \mu)^2 - n^{-1} \var (X) \sim \subE (8\sqrt{2}\sigma^2 / n, 8\sigma^2 / n)$. Therefore,
    \[
        \begin{aligned}
            \E \exp\left\{ \lambda(\overline{X} - \mu)^2 \right\} & = \E \exp\left\{ \lambda \big( (\overline{X} - \mu)^2 - n^{-1}\var(X) \big) \right\} \E \exp \{ \lambda n^{-1}  \var(X)\} \\
            & \leq \exp \left\{ \frac{(8 \sqrt{2} \sigma^2 / n)^2 \lambda^2}{2}\right\} \cdot \exp \left\{ \lambda n^{-1} \sigma^2 \right\} = \exp \left\{ \frac{64 \lambda^2 \sigma^4}{n^2} + \frac{\lambda \sigma^2}{n}\right\} \leq e^{9 / 8}.
        \end{aligned}
    \]
    for any $\lambda \leq \frac{n}{8 \sigma^2}$.
\end{proof}

\subsection{Proof of Lemma \ref{lem_gau_frac}}

\begin{proof}
	Write the probability as
	\[
	    \begin{aligned}
	    	\pr \left(\frac{|X|}{|Y|} > c \right) & = \pr \left(|X| > c |Y| \right) \\
	    	& = \pr \left( \{ X > c Y \} \, \cap \, \{ X > 0\} \, \cap \, \{ Y > 0 \} \right) + \pr \left( \{ - X > c Y \} \, \cap \, \{ X \leq 0\} \, \cap \, \{ Y > 0 \} \right) \\
	    	& ~~~~~~~~~~ + \pr \left( \{ X >-  c Y \} \, \cap \, \{ X > 0\} \, \cap \, \{ Y \leq 0 \} \right) + \pr \left( \{ - X > - c Y \} \, \cap \, \{ X \leq 0\} \, \cap \, \{ Y \leq 0 \}\right) \\
	    	& = \pr \left( \{ X > c Y \} \, \cap \, \{ X > 0\} \, \cap \, \{ Y > 0 \} \right)  + \pr \left( \{ - X > c Y \} \, \cap \, \{ - X \geq 0\} \, \cap \, \{ Y > 0 \} \right) + \pr (Y \leq 0) \\
	    	\alignedoverset{\text{by using $X$ is symmetric about $0$.}}{\leq} 2 \pr (  X > c Y ) + \pr (Y \leq 0) 
	    \end{aligned}
	\]
	for any $c > 0$.
\end{proof}

\subsection{Proof of Lemma \ref{lem_subE_ineq}}
%We need the following lemma.
%\begin{lemma}
    %Suppose $X$ be any zero-mean random variable, and $f$ be a differentiable function, then
    %\[
        %\begin{aligned}
            %\E f(X) & = f(0) \big[ \pr (X  > 0) - \pr (X < 0) \big] + \int_0^{\infty} f'(u) \pr (X > u) \, du - \int_{-\infty}^0 f'(u) \pr (X < u) \, du \\
            %& =  f(0) \big[ \pr (X  > 0) - \pr (X < 0) \big] + \int_0^{\infty} \big[ f'(u) - f'(-u) \big] \pr (|X| > u) \, du.
        %\end{aligned}
    %\]
    %Furthermore, if $f(0) \geq 0$ and $X$ is positive, then
    %\[
        %\E f(X) \leq f(0) + \int_0^{\infty} f'(u) \pr (X > u) \, du.
    %\]
%\end{lemma}
\begin{proof}
    %Denote $Y := a X + b$ is a strictly positive random variable, then by the above lemma,
    Denote $Y := a \overline{X} + b$ is a strictly positive random variable, recall for any non-negative strictly increasing function $f$, we have
    \[
        \E f(Y) = \int_0^{\infty} \pr \left( f(Y) > r\right) \, \mathrm{d} r = \int_0^{\infty} \pr \left( Y > f^{-1} (r)\right) \, \mathrm{d} r.
    \]
    Then for any fixed $s \in \mathbb{N}$,
    \[
        \begin{aligned}
        	\E \exp \left\{ - \frac{s}{a\overline{X} + b}\right\} & = \E \exp \left\{ - \frac{s}{Y} \right\} = \int_0^{\infty} \pr \left( \exp \left\{ - \frac{s}{Y}\right\} > r \right) \, \mathrm{d} r \\
        	& = \int_0^1 \pr \left( Y > \frac{s}{\log r^{-1}} \right) \, \mathrm{d} r \\
        	& = \int_0^1 \pr \left( \overline{X} > \frac{1}{a} \left[ \frac{s}{\log r^{-1}} - b \right]\right) \, \mathrm{d} r \\
        	& = \int_0^{\exp \left\{ -\frac{s}{b}\right\}} \pr \left( \overline{X} > \underbrace{\frac{1}{a} \left[ \frac{s}{\log r^{-1}} - b \right]}_{\leq 0}\right) \, \mathrm{d} r + \int_{\exp \left\{ -\frac{s}{b}\right\}}^{1} \pr \left( \overline{X} > \underbrace{\frac{1}{a} \left[ \frac{s}{\log r^{-1}} - b \right]}_{> 0}\right) \, \mathrm{d} r \\
        	& \leq \exp \left\{ -\frac{s}{b}\right\} \times 1 + \int_{\exp \left\{ -\frac{s}{b}\right\}}^{1} \pr \left( \overline{X} > \underbrace{\frac{1}{a} \left[ \frac{s}{\log r^{-1}} - b \right]}_{> 0}\right) \, \mathrm{d} r \\
        	\alignedoverset{\text{by letting $u = \frac{s}{\log r^{-1}}$}}{=} \exp \left\{ -\frac{s}{b}\right\} + \int_b^{\infty} \pr \left( \overline{X} > \underbrace{\frac{u - b}{a}}_{>0} \right) \exp\left\{ - \frac{s}{u}\right\} \frac{s}{u^2} \, \mathrm{d} r.
        \end{aligned} 
    \]
    Recall $\overline{X}$ is the mean of some independent zero mean sub-exponential distribution, denote $\lambda := \left(\frac{1}{s} \sum_{i=1}^s \lambda_i^2\right)^{1 / 2}$, then 
    \[
        \pr \left( \overline{X} > t \right) \leq \exp \left\{ -\frac{1}{2}\left(\frac{s t^2}{{\lambda}^2} \wedge \frac{s t}{\lambda}\right) \right\}
    \]
    for any $t > 0$ by Corollary 4.2.(c) in \cite{zhang2020concentration}. Therefore, we can furthermore bound the expectation as
    \[
        \begin{aligned}
            \E \exp \left\{ - \frac{s}{a\overline{X} + b}\right\} \alignedoverset{\text{by sub-Exponential inequality}}{\leq} \exp \left\{ -\frac{s}{b}\right\} +\int_b^{\infty} \frac{s}{u^2} \exp \left\{ - \frac{s}{u}\right\} \exp \left\{- \frac{1}{2} \frac{s (u - b)^2}{\lambda^2 a^2} \wedge \frac{s (u - b)}{\lambda a} \right\} \, \mathrm{d} u \\
        	& \leq \exp \left\{ -\frac{s}{b}\right\} +\frac{s}{b^2} \int_b^{\infty} \exp \left\{- \left[ \frac{s}{u} + \frac{1}{2} \frac{s(u - b)^2}{\lambda^2 a^2} \wedge \frac{s(u - b)}{\lambda a} \right] \right\} \, \mathrm{d} u \\
        	& = \exp \left\{ -\frac{s}{b}\right\} + \left[ \int_b^{b + \lambda  a} + \int_{b + \lambda a }^{\infty} \right] \frac{s}{u^2} \exp \left\{- \left[ \frac{s}{u} + \frac{1}{2} \frac{s(u - b)^2}{\lambda^2 a^2} \wedge \frac{s(u - b)}{\lambda a} \right] \right\} \, \mathrm{d} u \\
        	& =: \exp \left\{ -\frac{s}{b}\right\} + \big[ I + II\big].
        \end{aligned}
    \]
    The next step is bounding both $I$ and $II$. For $I$, we obtain
    \[
        \begin{aligned}
        	I & = \int_b^{b + \lambda  a} \frac{s}{u^2}  \exp \left\{ - \left[ \frac{s}{u} + \frac{s(u - b)^2}{2 \lambda^2 a^2}\right]\right\} \, \mathrm{d} u \\
        	& \leq \int_b^{b + \lambda  a} \frac{s}{b^2} \exp \left\{ - \left[ \frac{s}{b + \lambda  a} + \frac{s(u - b)^2}{2 \lambda^2 a^2}\right]\right\} \, \mathrm{d} u \\
        	& = \frac{s}{b^2} \exp \left\{ - \frac{s}{b + \lambda a}\right\} \int_b^{b + \lambda  a} \exp \left\{ - \frac{ s (u - b)^2}{2 \lambda^2 a^2}\right\} \, \mathrm{d} u \\
        	& \leq \frac{s}{b^2} \exp \left\{ - \frac{s}{b + \lambda a}\right\} \int_b^{\infty} \exp \left\{ - \frac{(u - b)^2}{2 \lambda^2 a^2 / s}\right\} \, \mathrm{d} u = \frac{\sqrt{2 \pi} \lambda a }{2 b^2} \exp \left\{ -\frac{s}{b + \lambda a}\right\}
        \end{aligned}
    \]
    For $II$, we need to be more careful to decompose it as
    \[
        \begin{aligned}
            II &= \int_{b + \lambda  a}^{\infty} \frac{s}{u^2}  \exp \left\{ - \left[ \frac{s}{u} + \frac{s(u - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u \\
            & = \left[ \int_{b + \lambda a}^{\frac{2 \lambda a s}{b}} + \int_{\frac{2 \lambda a c}{b}}^{\infty} \right] \frac{s}{u^2}  \exp \left\{ - \left[ \frac{s}{u} + \frac{s(u - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u \\
            & = \int_{b + \lambda a }^{\frac{2 \lambda a s}{b}} \frac{s}{u^2}  \exp \left\{ - \left[ \frac{s}{u} + \frac{s(u - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u + \exp \left\{ -\frac{s}{b}\right\} \int_{\frac{2 \lambda a s}{b}}^{\infty} \frac{s}{u^2} \exp \left\{ - \frac{s(u - b) ( u - \frac{2 \lambda a s}{b})}{2 \lambda a u}\right\} \, \mathrm{d} u \\
            & =: II_1 + II_2 .
        \end{aligned}
    \] 
    And for $II_1$, 
    \[
        \begin{aligned}
            II_1 & = \int_{b + \lambda a}^{\frac{2 \lambda a s}{b}} \frac{s}{u^2}  \exp \left\{ - \left[ \frac{s}{u} + \frac{s(u - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u \\
            & = \int_{b + \lambda a}^{\frac{2 \lambda a s}{b}} \frac{s}{u^2}  \exp \left\{ - s \times \left[ \frac{1}{u} + \frac{(u - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u \\
            \alignedoverset{g(u) = \frac{1}{u} + \frac{(u - b)}{2 \lambda a } \text{ is increasing on } u \geq \sqrt{2 \lambda a}}{\leq} \int_{b + \lambda a}^{\frac{2 \lambda a s}{b}} \frac{s}{u^2}  \exp \left\{ - s \times \left[ \frac{1}{\sqrt{2 \lambda a} \vee (b + \lambda a )} + \frac{(\sqrt{2 \lambda a} \vee (b + \lambda a ) - b)}{2 \lambda a }\right]\right\} \, \mathrm{d} u  \\
            & \leq \frac{s}{(b + \lambda a) } \left[ \frac{2 \lambda a s}{b} - \big( b + \lambda a \big) \right] \exp \left\{ - \frac{s}{\sqrt{2 \lambda a} \vee (b + \lambda a )}\right\}.
        \end{aligned}
    \]
    %\todohw{still dealing with}
    %\[
        %\begin{aligned}
        	%II_1 & = \int_{b + \lambda^2  a/ \alpha}^{\frac{2 \alpha a s}{b}} \frac{s}{u^2} \exp \left\{ - \frac{(u - b) (u - \frac{2 \alpha a s}{b})}{2 \alpha a u}\right\} \, \mathrm{d} u \\
        	%& \leq  \frac{s}{\left( b + \lambda^2  a/ \alpha \right)^2} \int_{b + \lambda^2  a/ \alpha}^{\frac{2 \alpha a s}{b}} \exp \left\{ - \frac{(u - b) (u - \frac{2 \alpha a s}{b})}{2 \alpha a u}\right\} \, \mathrm{d} u \\
        	%& \leq \ind \left( b + \lambda^2  a/ \alpha \leq \frac{2 \alpha a s}{b} \right) \left[ \frac{2 \alpha a s}{b} - \left(  b + \lambda^2  a/ \alpha \right) \right] \max_{ b + \lambda^2  a/ \alpha \leq u \leq {2 \alpha a s} / {b}}  \exp \left\{\frac{(u - b) ({2 \alpha a s} / {b} - u)}{2 \alpha a u}\right\}.
        %\end{aligned}
    %\]
    %Note that
    %\[
        %\begin{aligned}
        	%\exp \left\{\frac{(u - b) ({2 \alpha a s} / {b} - u)}{2 \alpha a u}\right\} & = \exp \left\{ \frac{1}{2 \alpha a} \left[ \frac{2 \alpha a s}{b} + b - \left( u + \frac{2 \alpha a s}{u}\right) \right] \right\} \\
        	%& \leq \exp \left\{ \frac{1}{2 \alpha a} \left[ \frac{2 \alpha a s}{b} + b - 2 \sqrt{u \frac{2 \alpha a s}{u}}\right] \right\} \\
        	%& = \exp \left\{ \frac{s}{b} + \frac{b}{2 \alpha a} - \sqrt{\frac{2 s}{\alpha a}}\right\},
        %\end{aligned}
%\]
    %\red{
    %we have the bounded $II_1$ as
    %\[
        %\begin{aligned}
        	%II_1 & \leq \ind \left( b + \lambda^2  a/ \alpha \leq \frac{2 \alpha a s}{b} \right) \left[ \frac{2 \alpha a s}{b} - \left(  b + \lambda^2  a/ \alpha \right) \right] \exp \left\{ \frac{s}{b} + \frac{b}{2 \alpha a} - \sqrt{\frac{2 s}{\alpha a}}\right\} \\
        	%\alignedoverset{\frac{2s}{\alpha a} \geq \frac{b^2}{\alpha^2 a^2} + \frac{b \lambda^2}{\alpha^3 a}}{\leq} \ind \left( b + \lambda^2  a/ \alpha \leq \frac{2 \alpha a s}{b} \right) \left[ \frac{2 \alpha a s}{b} - \left(  b + \lambda^2  a/ \alpha \right) \right] \exp \left\{ \frac{b}{2 \alpha a}\right\}.
        %\end{aligned}
    %\]
    %}
    For $II_2$, we obtain that
    \[
        \begin{aligned}
        	II_2 & = \exp \left\{ -\frac{s}{b}\right\}  \int_{\frac{2 \lambda a s}{b}}^{\infty} \frac{s}{u^2} \exp \left\{ - \frac{s(u - b) ( u - \frac{2 \lambda a s}{b})}{2 \lambda a u}\right\} \, \mathrm{d} u \\
        	& \leq \exp \left\{ -\frac{s}{b}\right\}  \int_{\frac{2 \lambda a s}{b}}^{\infty} \frac{s}{u^2} \exp \left\{ - \frac{s(u - \frac{2 \lambda a s}{b})^2}{2 \lambda a u}\right\} \, \mathrm{d} u \\
                & \leq \exp \left\{ -\frac{s}{b}\right\}  \int_{\frac{2 \lambda a s}{b}}^{\infty} \frac{s}{u^2} \exp \left\{ - \frac{(u - \frac{2 \lambda a s}{b})^2}{2 \lambda a u}\right\} \, \mathrm{d} u \\
        	& \leq c \sqrt{\frac{b}{2 \lambda a s}} \exp \left\{ -\frac{s}{b}\right\} \int_{\frac{2 \lambda a s}{b}}^{\infty} \frac{1}{u^{3 / 2}} \exp \left\{ - \frac{(u - \frac{2 \lambda a s}{b})^2}{2 \lambda a u}\right\} \, \mathrm{d} u \\
        	& = \sqrt{\frac{b s}{2 \lambda a}} \cdot \frac{b}{2s}\sqrt{\frac{\pi}{2 \lambda a}} \exp \left\{ -\frac{s}{b}\right\}  \left[ 1 - e^{4 s / b} \frac{2}{\sqrt{\pi}} \int_{2 \sqrt{s / b}}^{\infty} e^{-t^2} \,  \mathrm{d} t \right] \\
        	\alignedoverset{\text{by Lemma \ref{lem_erfc}}}{\leq}\sqrt{\frac{b s}{2 \lambda a}} \cdot \frac{b}{2s}\sqrt{\frac{\pi}{2 \lambda a}} \exp \left\{ -\frac{s}{b}\right\}  \cdot (1 - 0) \\
            & = \sqrt{\frac{\pi b}{s}} \frac{b}{4 \lambda a} \exp \left\{ -\frac{s}{b}\right\} .
        \end{aligned}
    \]
    Combining these results, we obtain that
    \[
        \begin{aligned}
        	\E \exp \left\{ - \frac{s}{aX + b}\right\} & \leq \exp \left\{ -\frac{s}{b}\right\} + I +  II_1 + II_2 \\
        	& \leq \exp \left\{ -\frac{s}{b}\right\} + \frac{\sqrt{2 \pi} \lambda a s}{2 b^2} \exp \left\{ -\frac{s}{b + \lambda^2 a / \alpha}\right\} \\
        	& \qquad + \frac{s}{(b + \lambda a) } \left[ \frac{2 \lambda a s}{b} - \big( b + \lambda a \big) \right] \exp \left\{ - \frac{s}{\sqrt{2 \lambda a} \vee (b + \lambda a )}\right\} + \sqrt{\frac{\pi b}{s}} \frac{b}{4 \alpha a} \exp \left\{ -\frac{s}{b}\right\} .
        \end{aligned}
    \]
    By taking $\log$ transform, and we get the result.
\end{proof}

\begin{lemma}\label{lem_erfc}
	For any $x \geq 0$,
	\[
	    \frac{2 e^{x^2}}{\sqrt{\pi}} \int_x^{\infty} e^{-t^2} \, \mathrm{d} t \leq 1.
	\]
\end{lemma}

\begin{proof}
	\[
	    \begin{aligned}
	    	\frac{2 e^{x^2}}{\sqrt{\pi}} \int_x^{\infty} e^{-t^2} \, \mathrm{d} t & = \frac{2}{\sqrt{\pi}} \int_x^{\infty} e^{- (t^2 - x^2)} \, \mathrm{d} t \\
	    	& = \frac{2}{\sqrt{\pi}} \int_x^{\infty} e^{- (t^2 - x^2)} \, \mathrm{d} t\\
	    	& \leq \frac{2}{\sqrt{\pi}} \int_x^{\infty} e^{- (t - x)^2} \, \mathrm{d} t \\
	    	& = \frac{2}{\sqrt{\pi}} \int_0^{\infty} \frac{e^{- t^2}}{2 \times \frac{1}{2}} \, \mathrm{d} t = \frac{2}{\sqrt{\pi}} \frac{\sqrt{2 \pi \times \frac{1}{2}}}{2} = 1.
	    \end{aligned}
	\]
\end{proof}



==> 9_Special_Case.tex <==

%\section{Justification of Optimistic and Special Cases of Rewards under MAB}\label{sec_spe_case}

\section{Special Cases of Rewards under MAB}\label{sec_spe_case}


%Regarding the claim $\overline{Y}_{k, s}$ is optimistic. We will argue in two statements.

%denote $\overline{R}_{k, s}^*$ as the mean of the shifted version and consider the event that the scaled-shifted sample mean of the optimal arm is less than the expectation some specific level, i.e.
%\[
    %E(\varepsilon) : = \left\{ \frac{\mu_1 + \lambda}{1 + 2 \lambda} - 2 \varepsilon \leq \overline{R}_{1, s}^* \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \varepsilon \right\}, \qquad \text{ for some } \qquad \varepsilon > 0
%\]
%$E(\varepsilon)$ is the event, we do not hope it happens, and its probability can be bounded by
%\[
    %\begin{aligned}
        %\pr \big( E(\varepsilon) \big) &  = \pr \big( - 2 \varepsilon (1 + 2 \lambda) \leq (\overline{R}_{1, s} - \mu_1) \leq - \varepsilon (1 + 2 \lambda)\big) \\
        %& \leq \left[ \Phi \left(\frac{2 \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) - \Phi \left(\frac{ \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) \right] + \frac{0.3328\left(\E |R_{1, 1} - \mu_1|^3+ 0.429 \var(R_{1,1})^{3 / 2} \right)}{\var(R_{1,1})^{3 / 2} \sqrt{s}}
    %\end{aligned}
%\]
%where we use the improved Berry–Esseen bounds \cite{shevtsova2011absolute}.
%On the other hand, we calculate the probability that the target has chance to escape this dilemma under this bad event. Denote 
%\[
    %F := \left\{ \sum_{i = 1}^s \big[ (R_{1, i} - \mu_1) + \lambda (2 R_{1, i} - 1) \big] \omega_i + \lambda \sum_{i = 1}^s (\lambda + 1  - \mu_1) \omega_i' - \lambda (\mu_1 + \lambda) \sum_{i = 1}^s \omega_i'' > 0 \right\},
%\]
%then
%\[
    %\begin{aligned}
        %\pr \left( \overline{Y}_{1, s} \geq  \frac{\mu_1 + \lambda}{1 + 2 \lambda} \mid E(\varepsilon) \right) & = \E \left[ \pr \left( \overline{Y}_{1, s} \geq  \frac{\mu_1 + \lambda}{1 + 2 \lambda} \mid \his_{1, s} \right) \mid E(\varepsilon) \right] = \frac{\pr \big(F \, \cap \, E(\varepsilon) \big)}{\pr \big( E (\varepsilon)\big)}.
    %\end{aligned}
%\]
%And for the probability $\pr \big(F \, \cap \, E (\varepsilon) \big)$, we write that
%\[
   % \begin{aligned}
        %& W \mid \his_{1, s} :=  \sum_{i = 1}^s \big[ (R_{1, i} - \mu_1) + \lambda (2 R_{1, i} - 1) \big] \omega_i + \lambda \sum_{i = 1}^s (\lambda + 1  - \mu_1) \omega_i' - \lambda (\mu_1 + \lambda) \sum_{i = 1}^s \omega_i'' \\
        %\sim & N \left( s (1 + 2 \lambda) (\overline{R}_{1, s} - \mu_1), \sigma_{\omega}^2 \left[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + 2 s \lambda (1 + 2 \lambda) (2 \mu_1 - 1 ) (\overline{R}_{1, i} - \mu_1) + 2 s \lambda^2 \big(3 \mu^2 - 3 \mu + \lambda^2 + \lambda + 1 \big) \right] \right).
    %\end{aligned}
%\]
%Hence, denote $Z$ as the standard normal distribution, we can bound it as 
%\[
    %\begin{aligned}
        %\pr \big( F \, \cap \, E (\varepsilon) \big) & = \pr \left( \left\{ \frac{W - s (1 + 2 \lambda)(\overline{R}_{1, s} - \mu_1)}{\var^{1 / 2}(W \mid \his_{1, s})} \geq \frac{- s (1 + 2 \lambda)(\overline{R}_{1, s} - \mu_1)}{\var^{1 / 2}(W \mid \his_{1, s})}  \right\} \, \cap \, E(\varepsilon) \right)  \\
        %& = \pr \left( \left\{ Z \geq \frac{- s (1 + 2 \lambda)(\overline{R}_{1, s} - \mu_1)}{\var^{1 / 2}(W \mid \his_{1, s})} \right\} \, \cap \, E(\varepsilon) \right) \\
        %(\text{use the event } E (\varepsilon)) & \geq \pr \left( \left\{ Z \geq \frac{2 s (1 + 2 \lambda)^2 \varepsilon}{\var^{1 / 2}(W \mid \his_{1, s})}\right\} \, \cap \, E (\varepsilon) \right)  \\
        %(E (\varepsilon) \text{ plus Cauchy})& \geq  \pr \left( \left\{ Z \geq \frac{2 s (1 + 2 \lambda)^2 \varepsilon}{ \sigma_{\omega}(1 + 2 \lambda) \sqrt{s}}\right\} \, \cap \, E (\varepsilon) \right) \\
        %(\text{choose } \sigma_{\omega}^2 \geq 4 \var(R_{1, 1}) ) & \geq \left[ \Phi \left(\frac{2 \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) - \Phi \left(\frac{ \varepsilon (1 + 2 \lambda)\sqrt{s}}{\sigma_{\omega}} \right) \right].
    %\end{aligned}
%\]
%which implies
%\[
    %\frac{\pr \left( \overline{Y}_{1, s} \geq  \frac{\mu_1 + \lambda}{1 + 2 \lambda} \mid E(\varepsilon) \right)}{\pr \big( E (\varepsilon)\big)} \geq  \frac{\left[ \Phi \left(\frac{2 \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) - \Phi \left(\frac{ \varepsilon (1 + 2 \lambda)\sqrt{s}}{\sigma_{\omega}} \right) \right]}{\left( \left[ \Phi \left(\frac{2 \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) - \Phi \left(\frac{ \varepsilon (1 + 2 \lambda)\sqrt{s}}{\var^{1 / 2}(R_{1, 1})} \right) \right] + \frac{0.3328\left(\E |R_{1, 1} - \mu_1|^3+ 0.429 \var(R_{1,1})^{3 / 2} \right)}{\var(R_{1,1})^{3 / 2} \sqrt{s}}\right)^2}
%\]
%Now by choose the parameter $\lambda$ and $\sigma_{\omega}$ carefully, one can always achieve the left side of the above inequality no less than one, i.e.
%\[
    %\pr \left( \overline{Y}_{1, s} \geq  \frac{\mu_1 + \lambda}{1 + 2 \lambda} \mid E(\varepsilon) \right) \geq \pr \big( E (\varepsilon) \big).
%\]
%This means any unfavorable history is less likely than being optimistic under that history. Thus, $\overline{Y}_{k, s}$ is optimistic.
%\fi

As said previously, due to undetermined structure of a general sub-Gaussian distribution, Theorem \ref{thm.MAB} can only give the rate of $\log T$ without the specific coefficients. However, for specific distributions, the coefficients can be derived with relatively simple expressions. See the following two corollaries. 

\todohw{All need to revise the coefficients.}

{\color{red}{
\begin{corollary}[Bernoulli]
\label{cor_ber}
    Consider a $K$-armed bandit with Bernoulli rewards. 
    With the tuning parameter $(\lambda, \sigma_{\omega}^2)$ satisfying the restriction in Theorem \ref{thm.MAB}, then 
    the expected $T$-round regret of Algorithm \ref{alg:MBTS-MAB-2} is bounded from above as
    \[
        \begin{aligned}
            \operatorname{Reg}_T & \leq \sum_{k = 2}^K \Delta_k \left\{ B_1 (\lambda, \sigma_{\omega}) \left[ 2 B_2 (\lambda, \sigma_{\omega}) + \frac{\sigma_{\omega}^2 \Delta_k^2}{3 \times 16^2}\right] 
            \log T + 3 \right\} \\
            & \qquad \qquad \qquad  \qquad \qquad  + \sum_{k = 2}^K \Delta_k \left\{ 2 \left[  B_2 (\lambda, \sigma_{\omega}) + \frac{\sigma_{\omega}^2 \Delta_k^2}{3 \times 16^2}\right] \log T + 3 \right\}
        \end{aligned}
    \]
    where 
    \[
       \begin{aligned}
           B_1  (\lambda, \sigma_{\omega}) :=  \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big]
       \end{aligned}
    \]
    \[
        B_2 (\lambda, \sigma_{\omega}) := \frac{36 (1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{- 2} (1 + 2 \lambda)^2} + \frac{32^2 \sigma_{\omega}^{ 2} \lambda^2 (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2},
    \]
    for $T \geq 2$.
\end{corollary}


% The coefficients in Corollary \ref{cor_ber} is quite similar tod the result in Theorem 2 of \cite{kveton2019garbage}. Indeed, compare coefficients of two parts in the bound in Corollary \ref{cor_ber} with Theorem 2 in \cite{kveton2019garbage} and denote $\lambda > 1 / \sqrt{2}$ as the tuning parameter in their algorithm, the coefficients in \cite{kveton2019garbage} are 
% \[
%     \frac{16(2 \lambda +1)}{\Delta_{k}^{2}} \frac{2 e^{2} \sqrt{2 \lambda +1}}{\sqrt{2 \pi}} \exp \left[\frac{8 (2 \lambda +1) /[\lambda(\lambda+1)]}{2-(2 \lambda +1) /[\lambda(\lambda+1)]}\right]\left(1+\sqrt{\frac{2 \pi}{4-2 (2 \lambda +1) /[\lambda(\lambda + 1)]}}\right) \log T + 2
% \]
% and 
% \[
%     \frac{8(2 \lambda  + 1)}{\Delta_k^{2}} \log T + 2.
% \]

% For general chosen tuning parameter $\lambda$,  the first part of ours is slightly smaller than theirs, while for the second part, theirs will be smaller than ours. 

\begin{corollary}[Gaussian]
\label{cor_gau}
    Consider a $K$-armed bandit with the rewards sampled from $\mathcal{N}(\mu_k, \sigma_k^2)$. With the tuning parameter $(\lambda, \sigma_{\omega}^2)$ satisfying the restriction in Theorem \ref{thm.MAB},  the expected $T$-round regret of Algorithm \ref{alg:MBTS-MAB-2} is bounded from above as

    % If $K$-armed bandit is 1-Gaussian rewards with its mean bounded in $(0, 1)$, then the regret has the following explicit bound
    \[
      \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \left[ 6 + \left\{  C_1(\lambda, \sigma_{\omega}) +C_2(\lambda, \sigma_k) \Delta_k^{-2} \right\} \log T\right],
    \]
    where the constants $C_{1}(\lambda, \sigma_{\omega})$ and $C_{2}(\lambda, \sigma_k)$ are defined as 
    \[
        C_1 (\lambda, \sigma_{\omega}) = \big[ C_3 (\lambda, \sigma_{\omega}) + 2 \big] \sigma_{\omega}^2 \big[ 12 \lambda^2 (\lambda^2 + \lambda + 4) + (1 + 2 \lambda)^2\big], \quad  C_2 (\lambda, \sigma_{k}) = 16 \big[ C_3 (\lambda, \sigma_{\omega}) + 2 \big] (1 + 2 \lambda)^{-2} (\sigma_1^2 + \sigma_k^2)
    \]
    \[
       \begin{aligned}
           C_3 (\lambda, \sigma_{\omega}) & = \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big]
       \end{aligned}
    \]
     for any $T \geq 2$.
    %{\color{red}{$C_1(\lambda, \sigma_{\omega}) = \left\{ C_3(\lambda) + 2 \right\}  (1 + \sqrt{2})\sqrt[4]{3 \times 2^{13}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda)}$}} and  $C_2(\lambda, \sigma_k) = \left\{  C_3(\lambda) +  2 \sigma_1^2 + \sigma_k^2 \right\} \frac{32}{(1 + 2 \lambda)^2}$. Here, $C_3(\lambda) = \left[ 1 - \frac{3 (2\mu_1 - 1)^2 (2 \lambda + 1)^2}{ 4 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} \big]^2}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}$. 
\end{corollary}
}}

==> ARCHIVE/00_main.tex <==
% \input{FRONT}
\input{Style}
\title{Multiplier Bootstrap-based Thompson Sampling}
\date{\today}
\author{}


\begin{document}
\maketitle
\linenumbers

In this paper, we study Multiplier Bootstrap-based Thompson Sampling.
We first introduce the formulation of the bandit problem, 
then introduce the Thompson sampling algorithm and the limitation of its vanilla form, 
and finally provide a general form of Multiplier Bootstrap-based Thompson Sampling (MBTS). 

The main objective is to understand the theoretical performance (regret bound) of MBTS, and what kind of second-order adjustment/variance inflation (if needed) might be required for MBTS to yield a desired performance. 


\section{Bandit Problem and Thompson Sampling}

We consider a general (context-free) form, where at each round $t$, the agent needs to choose an action $A_t \in \mathcal{A}_t$ and then receive the corresponding reward $R_t = f(A_t;\theta) + \epsilon_t$, where $\epsilon_t$ is a mean-zero noise term. 
The goal is to minimize the cumulative regret $\sum_t \Mean \big[ max_{a \in \mathcal{A}_t} f(a;\theta)  - f(A_t;\theta) \big]$. 
When $\mathcal{A}_t$ is a fixed finite set and $f(A_t;\theta)$ equals to some $r_{A_t}$, we are considering MAB. 
When $A_t$ is a vector and $f(A_t;\theta) = A_t^T \theta$, we are considering linear bandits. 
We can use these two as our main examples, with more complicated ones in mind. 


A greedy approach is to train a supervised learning model $f(;\hat{\theta}_t)$ with all available data and then choose $A_t = \argmax_{a \in \mathcal{A}_t} f(a;\hat{\theta}_t)$. 
This is a common practice in the company and upon which we would like to add exploration via quantifying uncertainty so that one can escape from the local optimum. 

There are two popular algorithmic frameworks, Upper Confidence Bound (UCB) and Thompson Sampling (TS). 
UCB adopts a frequentist viewpoint and construct an upper confidence bound for $f(a;\hat{\theta}$ as $\hat{U}_t(a)$, for every $a$. 
UCB then chooses $A_t = \argmax_a \hat{U}_t(a)$. 
 
TS adopts a Bayesian viewpoint, maintain a posterior over the model, and sample action from it. 
Specifically, we can maintain a posterior over $\theta$ as $Q_t(\theta)$, sample $\Tilde{\theta}_t \sim Q_t(\theta)$, and then 
choose $A_t = \argmax_a f(a; \Tilde{\theta}_t)$. 
This is equivalent to directly maintaining a posterior over $A^*_t = \argmax_{a \in \mathcal{A}_t} f(a;\theta)$ and then sample $A_t$. 

However, UCB and TS are typically only analytically/computationally feasible when $f$ is simple. 
For a complex or even black-box (pipeline-like) $f$, some perturbation/bootstrapping-based UCB/TS-type exploration would be a natural option. 
Besides, such an approach is more data-driven (as Bootstrapping directly utilizes the uncertainty in data) and requires less assumptions on the DGP. 

However, the theoretical understanding is still largely missing. 
Moreover, a naive adaption of Bootstrapping is probably not sufficient, as the type of guarantees we have is typically asymptotic or non-asymptotic but for i.i.d. data, while bandits typically require non-asymptotic results for dependent data. 
Certain additional perturbation or variance inflation might be needed to ensure enough exploration. 



\section{Multiplier Bootstrap-based Thompson Sampling}

There are many types of bootstrapping. 
Non-parametric bootstrapping is resampling of training examples with replacement. 
Yet in bandits, the data size grows and it could be computationally challenging to implement in an online fashion. 
This can be approximated computationally efficiently by i.i.d. Poisson weights. 
We outline our mental algorithm first. 
Modifications (such as appropriate variance inflation) might be needed to yield desired regret. 

\textbf{Mental Algorithm.}
We assume the existence of an efficient cost-sensitive least-squares oracle $\mathcal{O}_f$, i.e., give a parameterized model $f(;\theta)$ and the history $\{(R_t, A_t, W_t)\}$ where $W_t$ is some weight associated with the $t$-th data point, 
we can obtain the weighted least square solution for $\theta$ as $\mathcal{O}_f \big( \{(R_t, A_t, W_t)\} \big)$. 
We maintain $M$ models. 
In round $t$, one model is chosen uniformly at random and the best action under that model is taken. 
After we get the observation $(R_t, A_t)$, 
for each model $m$, 
we sample a weight $W_t$ from certain distribution with mean $1$ (e.g., $Poisson(1)$), and then update the model with the weighted least square. 
We note that maintaining $M$ models with fixed multiplier weights is only a computationally tractable way to approximate the full version, which re-assigns the weights for all data points every time. 
In our theory, we can focus on the latter one. 
% all models are updated with it. 
% In each model, the observation is perturbed by additive Gaussian noise or weighted by a Poisson weight. 

\section{Method}
Our MAB with mean reward between $[0,1]$, based on my (toy) simulation study, 
I suspect that two pseudo rewards (perturbed also necessary) might be enough? 
Guassian multiplier seems also enough and much faster (due to the ease of sampling). 

{\color{blue}{
Q: would be symmetric be a concern?
}}

\textbf{DGP:}
\begin{itemize}
    \item MAB: Gaussian, Bernoulli, Beta
    \item Contextual: linear, logisitc
    \item Structured Bandits
\end{itemize}

\textbf{Baseline:}
\begin{itemize}
\item Brano: GIRO (computationally slow; non-parametric + pseudo reward), PHE-MAB, PHE-linear. 
% How to beat PHE-linear? (empirical better, as they have not fully utilize the data-dependent uncertainty)
\item Guang Cheng: residual Bootstrap-based UCB for MAB (-> linear bandits), residual Bootstrap-based TS with pseudo rewards (only MAB)
\item TS, UCB
\end{itemize}



Note that MAB can be regarded as a special case of linear bandits where we have a fixed set of $K$ arms, each one is parameterized as an indicator vector. 
We conjecture that, 

become perturbed again? what is the main difference?

\input{main_alg_MAB}

% \input{main_alg_LB}

% \input{main_alg_GP}

Intuitively, the above two procedures add some randomness to each dimension of $\vthe$, which works similarly with the prior. 
For more complicated models with a potentially infinite dimension, 
we can consider sample some features and attach some random rewards to boost our exploration.

\clearpage
\newpage

\section{Theory}

\subsection{Proof Scheme for MAB}

Several things we should note during our derivations, which possibly will affect our algorithm design as well: 
\begin{itemize}
    
    {\color{blue}{
    \item Maintaining $B$ models is just a way to approximate the true bootstrapping sample. In analysis, we may want to analyze the full version (i.e., re-sample a totally new sample at every time point)
    }}
    \item It may/should not be a good idea to add a fixed amount of additional noise at the beginning. All existing literature adds a noise with variable $ta$, where $t$ is the current time point. Though one conjecture is that $ta$ might be too much (not adaptive to $t$ at least), a fixed amount of randomness may not be sufficient (though enough in  small-scale experiments)
\end{itemize}

We can see that Algorithm 1 and 2 use different injecting artificial randomness to deal with MAB, Algorithm 3 deals with linear bandits, and Algorithm 4 tackles kernel bandits. The three types algorithms require different proof techniques. We can start with MAB where can use the similar techniques in \cite{wang2020residual}.

\subsection{Theory for Algorithm 1 (details will add later)}

\subsubsection{Schedule of Proof}

The aim is to show the cumulative regret $\operatorname{Reg}_T$ is no more than the order $\log T$. So our main task is to show that $\operatorname{Reg}_T \lesssim \log T$.

\noindent The proof of $\operatorname{Reg}_T \lesssim \log T$ can be divided into three parts:

\begin{itemize}
    \item[1.] The first step is to conclude (or state) the result in \cite{kveton2019garbage}, that is
    \begin{equation*}
        \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
    \end{equation*}
    with
    \begin{equation*}
        a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] = \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1
    \end{equation*} 
    where $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_s  \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$ for some $\tau > 0$. So our target switch from $\operatorname{Reg}_T$ to $a_k$ and $b_k$. And the next two main steps will be bounding $a_k$ and $b_k$ separately.
    
    \item[2.] The second step is bounding $a_k = \sum_{s = 0}^{T - 1} a_{k, s}$. Note that
    \begin{equation*}
        a_{k, s} \leq \E Q_{1, s}(\tau_k)^{-1} \leq \E \big[ \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})^{-1} ) \big],
    \end{equation*}
    we need to first find the lower bound of the tail probability $\pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})$ and then find the upper bound of the expectation.
    \begin{itemize}
        \item[2.1.] The lower bound of tail probability $\pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})$.
        Note that 
        \begin{equation*}
            \overline{Y}_{1, s} = \left(0 + {\color{red}{\omega_0 \cdot \lambda_1}} + \sum_{\ell = 1}^{|\his_{1, s}|} \omega_{\ell} R_{1, \ell} \right) / \left( {\color{red}{\lambda_2}} + \sum_{\ell = 1}^{|\his_{1, s}|} \omega_{\ell} \right)
        \end{equation*}
    \end{itemize}
    will be only random on the bootstrap weights $\omega_{\ell}$ when conditions on $\his_{1, s}$ and the lower bound of the tail probability must require the exact distribution of $\omega_{\ell}$ or the harsh restriction for $\omega_{\ell}$ will be involved (see the discussion of \cite{zhang2020non} for details), where $\lambda_1$ and $\lambda_2$ is the tuning parameter.
    
    For simplicity, we assume $\omega_{\ell} \sim \operatorname{Exp}(1)$ and define $R_{1, 0} := \lambda_1 + \mu_1$ then
    \begin{equation*}
    \begin{aligned}
        \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s}) & = \pr_{\omega} \left(  \sum_{\ell = 0}^{|\his_{1, s}|} (R_{1, \ell} - \mu_1) \cdot \omega_{\ell} \geq \lambda_2 \cdot \mu_1 \right) \\
        & \geq \pr_{\omega} \left( \bigcap_{\ell = 0}^{|\his_{1, s}|} \big\{ (R_{1, \ell} - \mu_1) \omega_{\ell} \geq |\his_{1, s}|^{-1} \lambda_2 \mu_1 \big\} \right) \\
        {\color{red}{& = 2 \prod_{\ell = 0}^{|\his_{1, s}|} \pr_{\omega} \left( (R_{1, \ell} - \mu_1) \omega_{\ell} \geq |\his_{1, s}|^{-1} \lambda_2 \mu_1 \right) \\
        & = \prod_{\ell = 0}^{|\his_{1, s}|} \exp \left\{ - \frac{\lambda_2 \mu_1}{|\his_{1, s}| (R_{1, \ell} - \mu_1)} \right\}}} \\
        & = \exp \left\{ - \frac{\lambda_2 \mu_1}{|\his_{1, s}| \lambda_1}\right\} \prod_{\ell = 1}^{|\his_{1, s}|} \exp \left\{ - \frac{\lambda_2 \mu_1}{|\his_{1, s}| (R_{1, \ell} - \mu_1)} \right\}.
    \end{aligned}
\end{equation*}

    {\color{red}{
        For simplify this question, we first assume
        some specific distributions. 
        
        \begin{itemize}
            \item the Gaussian distribution $R_{1, \ell } \sim N(\mu_1, \sigma^2)$ (used in \cite{wang2020residual}) requires $R_{1, \ell } - \mu_1 > 0$ guaranteeing an upper bound $\lesssim \frac{1}{\sigma \sqrt{\pi}} G^{3, 0}_{0, 0}\left( \left. - \frac{1}{2} \ 0 \ 0\right| \frac{1}{8 \sigma^2}\right)$ with Meijer G-function. However, if we do not require $R_{1, \ell } - \mu_1  > 0$, then $\E \exp \left\{ 1 / (R_{1, \ell } - \mu_1) \right\} = \infty$;
            
            \item  another common assumption is $R_{1, \ell} \sim \operatorname{ber} (\mu_1, 1)$. In this case,
            \begin{equation*}
                \E \exp \left\{ \frac{\lambda_2 \mu_1}{|\his_{1, s}| (R_{1, \ell} - \mu_1)} \right\} = \exp \left\{ - \frac{\lambda_2}{|\his_{1, s}|}\right\} (1 - \mu_1) + \exp \left\{ \frac{\lambda_2 \mu_1}{|\his_{1, s}|(1 - \mu_1)}\right\} \mu_1.
            \end{equation*}
            Note that For any positive number $\mu, \lambda > 0$ and $n \in \mathbb{N}$, we have
                \begin{equation*}
                    \begin{aligned}
                        & \Bigg[ \exp \bigg\{ - \frac{\lambda}{n}\bigg\} (1 - \mu) + \exp \bigg\{ \frac{\lambda \mu}{n (1 - \mu)}\bigg\} \mu \Bigg]^n \\
                        = & e^{-\lambda} (1 - \mu)^n \Bigg[ 1 + \frac{1}{n} \frac{n \mu}{1 - \mu} \exp \bigg\{ \frac{n}{\lambda} + \frac{\lambda \mu}{n(1 - \mu)}\bigg\} \Bigg]^n \\
                        \leq & e^{- \lambda} (1 - \mu)^n \exp \Bigg\{ \frac{n \mu}{1 - \mu} \exp \bigg\{ \frac{n}{\lambda} + \frac{\lambda \mu}{n(1 - \mu)}\bigg\}\Bigg\} \\
                        = & \exp \Bigg\{ n 
                         \log (1 - \mu) + \frac{n \mu}{1 - \mu} \exp \bigg\{ \frac{n}{\lambda} + \frac{\lambda \mu}{n(1 - \mu)}\bigg\} - \lambda \Bigg\}
                    \end{aligned}
                \end{equation*}
                by using the fact $(1 + x / n)^n \leq e^x$. Let the above inequality less than $1$, it sufficiently has $\mu > 1 / 2$, i.e. the optimal arm's mean reward large than $1/2$, this requirement also can be seen in \cite{wang2020residual}.
        \end{itemize}
        
        Up to now, we can conclude that for any $s \in [T]$, the $a_{k, s}$ has the upper bound
        \begin{equation*}
            \begin{aligned}
                a_{k, s} & \leq \exp \left\{ \frac{\lambda_2 \mu_1}{|\his_{1, s}| \lambda_1}\right\} \prod_{\ell = 1}^{|\his_{1, s}|} \E \exp \left\{ \frac{\lambda_2 \mu_1}{|\his_{1, s}| (R_{1, \ell} - \mu_1)} \right\} \\
                & = \exp \Bigg\{ \frac{\lambda_2 \mu_1}{|\his_{1, s}| \lambda_1} + |\his_{1, s}| \log (1 - \mu_1) + \frac{|\his_{1, s}| \mu_1}{1 - \mu_1} \exp \bigg\{ \frac{|\his_{1, s}|}{\lambda_1} + \frac{\lambda_1 \mu_1}{|\his_{1, s}|(1 - \mu_1)}\bigg\} - \lambda_1 \Bigg\}.
            \end{aligned}
        \end{equation*}
        with $\lambda_1$ and $\lambda_2$ still need to verify later. So we have partly finished section 2.1.
        
        \begin{itemize}
            \item[2.2] We denote $\overline{Y}_{1, s}^* := \frac{1}{|\his_{1, s}|} \sum_{\ell = 1}^{|\his_{1, s}|} \omega_{\ell} R_{1, \ell}$ is the true weighted target function, and then
            \begin{equation*}
                \overline{Y}_{1, s} = \frac{\omega_0 \cdot \lambda_1 + |\his_{1, s}| \overline{Y}_{1, s}^*}{\lambda_2 + \sum_{\ell = 1}^{|\his_{1, s}|} \omega_{\ell}}.
            \end{equation*}
            
            Specify some good events such that $A_{k, s} := \{ \overline{Y}_{k, s} - \mu_k > C_1 \Delta_k\}$ and $A_{k, s}^* := \{ \overline{Y}_{k, s}^* - \mu_k > C_1 \Delta_k\}$ and define
            \begin{equation*}
                a_{k, s, 1} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) \Big], \qquad a_{k, s, 2} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}^c) \Big],
            \end{equation*}
            with $s_{a, j} (T) := \min \{ s : a_{k, s, j} \leq T^{-1}\}$ (it is well-defined by the fact $\mu_1 > 0.5$). In this step, we will show that $\max_{j = 1, 2} s_{a, j} (T) \lesssim \log T$.
        \end{itemize}
        
        \begin{itemize}
            \item[] \begin{itemize}
                \item[2.2.0] On the event $A_{1, s}^*$ and  $A_{1, s}$ 
            \end{itemize}
        \end{itemize}
        \begin{equation*}
            \begin{aligned}
                \pr \big(A_{1, s}^* \, | \, \his_{1, s} \big) & = \pr \bigg\{ \sum_{\ell = 1}^{|\his_{1, s}|} \frac{R_{1, \ell}}{|\his_{1, s}|} (\omega_{\ell} - 1) \geq C_1 \Delta_k + \mu_1 - \overline{R}_{1, s}\bigg\} \\
                & \leq \exp \bigg\{ - \frac{1}{2} \frac{|\his_{1, s}|(C_1 \Delta_k + \mu_1 - \overline{R}_{1, s})^2}{\sqrt{\sum_{\ell = 1}^{|\his_{1,s}|} R_{1, \ell}^2}} \wedge \frac{|\his_{1, s} | (C_1 \Delta_k + \mu_1 - \overline{R}_{1, s})}{\max_{\ell\in [|\his_{1, s}|]} R_{1, \ell}}\bigg\} \\
                & \lesssim \exp \Big\{  - \frac{1}{2}(C_1 \Delta_k + \mu_1 - \overline{R}_{1, s})^2 \Big\},
            \end{aligned}
        \end{equation*}
        and
        \begin{equation*}
            \begin{aligned}
                & \pr \big(A_{1, s} \, | \, \his_{1, s} \big) \\
                = & \, \pr \bigg\{ \lambda_1 \cdot (\omega_0 - 1) + \sum_{\ell = 1}^{|\his_{1, s}|} (R_{1, \ell} - \mu_1 - C_1 \Delta_k) \cdot (\omega_{\ell} - 1) \\
                & \qquad \qquad \qquad \qquad \qquad \qquad \geq \lambda_2 \cdot (\mu_1 + C_1 \Delta_k) - \lambda_1 + |\his_{1, s}| (\mu_1 + C_1 \Delta_k - \overline{R}_{1, s})\bigg\} \\
                \leq & \exp \Bigg\{ - \frac{1}{2} \frac{\big[ (\lambda_2 + |\his_{1, s}|) \mu_1 + C_1 (\lambda_2 + |\his_{1, s}|) \Delta_k - \lambda_1 - |\his_{1, s}| \overline{R}_{1, s}\big]^2}{\lambda_1^2 + \sum_{\ell = 1}^{|\his_{1, s}|} R_{1, \ell}^2} \\
                & \qquad \qquad \qquad \qquad \qquad \qquad \wedge \frac{(\lambda_2 + |\his_{1, s}|) \mu_1 + C_1 (\lambda_2 + |\his_{1, s}|) \Delta_k - \lambda_1 - |\his_{1, s}| \overline{R}_{1, s}}{\lambda_1 \,  \vee \, 1} \Bigg\} \\
                \overset{\lambda_1 = O(|\his_{1, s}|)}{\leq} &  \exp \Bigg\{ - \frac{1}{2}\frac{\big[ (\lambda_2 + |\his_{1, s}|) \mu_1 + C_1 (\lambda_2 + |\his_{1, s}|) \Delta_k - \lambda_1 - |\his_{1, s}| \overline{R}_{1, s}\big]^2}{\lambda_1^2 + s} \\
                &  \qquad \qquad \qquad \qquad \qquad \qquad \wedge \frac{(\lambda_2 + |\his_{1, s}|) \mu_1 + C_1 (\lambda_2 + |\his_{1, s}|) \Delta_k - \lambda_1 - |\his_{1, s}| \overline{R}_{1, s}}{\lambda_1}\Bigg\}
            \end{aligned}
        \end{equation*}
        by concentration inequality and the fact that $\lambda_1 \geq 1$ (or it will be meaningless). From this, a possible choose is {\color{blue}{$\lambda_1 = C_1 |\his_{1, s}|\Delta_k$ (?????)}} and $\lambda_2 = 0$, then
        \begin{equation*}
            \begin{aligned}
                \pr (A_{1, s}) & = \E \big[ \pr \big(A_{1, s} \, | \, \his_{1, s} \big) \big] \\
                & \leq \E \exp \left\{ - \frac{(\overline{R}_{1, s} - \mu_1)^2}{C_1 \Delta_k^2 + s}\right\} = 
            \end{aligned}
        \end{equation*}
        
        \begin{itemize}
            \item[] \begin{itemize}
                \item[2.2.1] Bound $s_{a, 1}(T)$: only need to note that
            \end{itemize}
        \end{itemize}
        
        \begin{equation*}
            \{ N_{1, s} (\tau_k) < T^{-1} \} \supseteq \left\{\left[1-Q_{1, s}(\tau_{k})\right]<T^{-2}\right\}
        \end{equation*}
        with
        \begin{equation*}
            \begin{aligned}
                \big[ 1-Q_{1, s}(\tau_{k}) \big] 1(G_{1, s}) & = \pr_{\omega} \left(  \left\{ \sum_{\ell = 0}^{|\his_{1, s}|} (R_{1, \ell} - \mu_1) \cdot \omega_{\ell} \geq \lambda_2 \cdot \mu_1 \right\} \cap G_{1, s} \right) \\
                & = 
            \end{aligned}
        \end{equation*}
        the construction of $G_{1, s}$ is intuitive from the above event.
    }}
\end{itemize}
~~~~\\


\iffalse

{\color{blue}{
{\color{red}{First, we assume $R_{k, \ell}$ is bernoulli such that $R_{k, \ell} \, \overset{\text{i.i.d.}}{\sim} \, \ber(\mu_k, 1)$.}} in Algorithm 1, we have $\overline{Y}_{k, s} =  \sum_{\ell = 1}^{|\his_s|} w_{\ell} \cdot R_{k, \ell}$ for $k \in [K]$ and $s \in [T]$ with $\omega_{\ell} \overset{\text{i.i.d}}{\sim } \rho(\omega)$, it is enough to deal with the algorithm 1 with $\overline{Y}_{k}$ replaced by $\overline{Y}_{k, s} $. 

Denote $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_s  \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$. Then from Theorem 1 in \cite{kveton2019garbage}, we have 
\begin{equation*}
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\end{equation*}
with
\begin{equation*}
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] = \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1
\end{equation*} 
for any $\tau_k \in \mathbb{R}$. So it is enough to bound $a_k$ and $b_k$.

\noindent $\circ$ \textbf{Bound $a_k$:}

\noindent Define the good events:
\begin{equation*}
    A_{1, s} := \big\{ \overline{Y}_{1, s} - \mu_1 > - \Delta_k / 4 \big\}, \qquad G_{1, s} := \{ \}.
\end{equation*}
For $\tau_k \leq \mu_1$, we have $a_{k, s} \leq \E Q_{1, s}(\tau_k)^{-1} \leq \E \big[ \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})^{-1} \big]$. We need to deal with tail probability of $\rho(\omega)$, which first be assumed as $\operatorname{Exp}(1)$,
\begin{equation*}
    \begin{aligned}
        \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s}) & = \pr_{\omega} \left( |\his_s|^{-1} \sum_{\ell = 1}^{|\his_{1, s}|} \omega_{\ell} R_{1, \ell} > \mu_1 \right) \\
        & = \pr_{\omega} \left( \sum_{\ell = 1}^{|\his_{1, s}|}  R_{1, \ell} \cdot ( \omega_{\ell} - 1) > - \sum_{\ell = 1}^{|\his_{1, s}|}  (R_{1, \ell} - \mu_1)\right) \\
        & \geq \pr_{\omega} \left( \bigcap_{\ell = 1}^{|\his_{1, s}|} \Big\{ R_{1, \ell} \cdot ( \omega_{\ell} - 1) > -   (R_{1, \ell} - \mu_1) \Big\} \right)\\
        & = \prod_{\ell = 1}^{|\his_{1, s}|} \exp \left\{ - \left( \frac{\mu_1 - R_{1, \ell}}{R_{1, \ell}} + 1\right) \right\} = \exp \left\{ - \mu_1 \sum_{\ell = 1}^{|\his_{1, s}|} \frac{1}{R_{1, \ell}}\right\},
    \end{aligned}
\end{equation*}

\textbf{(first method:)}

which implies
\begin{equation*}
    \begin{aligned}
        a_{k, s} & \leq \E \exp \left\{  \mu_1 \sum_{\ell = 1}^{|\his_{1, s}|} \frac{1}{R_{1, \ell}}\right\} = \left( \E \exp \{ \mu_1 R_{1, 1}^{-1} \}\right)^{|\his_{1, s}|}  \\
        (R_{1, 1} \neq 0) & \leq \Big[ e \pr (R_{1, 1} > \mu_1) + ( 1 - \epsilon \mu_1 )^{|\his_{1, s}| + 1 / 2} \Big] ^{|\his_{1, s}|}
    \end{aligned}
\end{equation*}
where $\epsilon$ is some lower bound for the reward of the optimal arm by the fact that for there exists some $\epsilon > 0$,
\begin{equation*}
    \begin{aligned}
        \E \exp \{ \mu_1 R_{1, 1}^{-1} \} & \leq e \pr (R_{1, 1} > \mu_1 ) + \int_{x \leq \mu_1} \exp (x^{-1} \mu_1) \, f_1(x) \, d x \\
        & \leq  e \pr (R_{1, 1} > \mu_1 ) + \int_{\frac{1}{\epsilon |\his_{1, s}|} < x \leq \mu_1} \left( 1 - \frac{\mu_1}{|\his_{1, s}| x}\right)^{|\his_{1, s}| + \frac{x}{2 \mu_1}} f_1(x) \, d x \\
        & \leq e \pr (R_{1, 1} > \mu_1) + \int_{\frac{1}{\epsilon |\his_{1, s}|} < x \leq \mu_1} \left( 1 - \epsilon \mu_1 \right)^{|\his_{1, s}| + 1 / 2} \, f_1(x) \, dx \\
        & \leq e \pr (R_{1, 1} > \mu_1) + ( 1 - \epsilon \mu_1 )^{|\his_{1, s}| + 1 / 2}.
    \end{aligned}
\end{equation*}
This implies we have bounded $a_{k, s}$ given $\pr \big(R_{1, 1} - \E R_{1, 1} > 0\big) < 1 / e$. 

\textbf{(second method:)} 

This first method requires $\pr \big(R_{1, 1} - \E R_{1, 1} > 0\big) < 1 / e$, which is anti-intuitive for many symmetric distributions such that $\pr \big(R_{1, 1} - \E R_{1, 1} > 0\big) =  \pr \big(R_{1, 1} - \E R_{1, 1} \leq 0\big) = 1 / 2$. Here, we can give another method to bound $a_{k, s}$ by using the Theorem in \cite{mond2000inequalities}, which gives
\begin{equation*}
    1 \leq \frac{e^{-x} - x e^{-1 / x}}{1 - x} \leq \frac{3}{e}, \qquad x \in (0, 1),
\end{equation*}
By applying this inequality, 
\begin{equation*}
    \begin{aligned}
        & \E \exp \{ \mu^{-1} R_{1, 1}\} \\
        \leq & \E \frac{\mu_1^{-1}R_{1, 1}}{e^{- \mu_1^{-1} R_{1, 1}} - \frac{3}{e} (1 - \mu_1^{-1} R_{1, 1})} \mathbb{I} (R_{1, 1} \leq \mu_1) + \E \frac{\mu_1^{-1}R_{1, 1}}{(\mu_1^{-1}R_{1, 1} - 1) + e^{-\mu_1^{-1}R_{1, 1}}} \mathbb{I} (R_{1, 1} > \mu_1) \\
        =:& I + II
    \end{aligned}
\end{equation*}
with
\begin{equation*}
    \begin{aligned}
        I & \leq \E \frac{\mu_1^{-1}R_{1, 1}}{\frac{3}{e} (1 - \mu_1^{-1} R_{1, 1})} \mathbb{I} (R_{1, 1} \leq \mu_1)  - \E \frac{\mu_1^{-1}R_{1, 1}}{e^{- \mu_1^{-1} R_{1, 1}}} \mathbb{I} (R_{1, 1} \leq \mu_1)  \\
        & \leq \frac{e}{3} \E \frac{R_{1, 1} \mathbb{I} (R_{1, 1} \leq \mu_1)}{\mu_1 - R_{1, 1}} - \frac{1}{\mu_1} \E R_{1, 1} e^{\mu_1^{-1}R_{1, 1}}\mathbb{I} (R_{1, 1} \leq \mu_1) := I_1 - I_2
    \end{aligned}
\end{equation*}
satisfying
\begin{equation*}
    \begin{aligned}
        I_1 \leq \frac{e}{3} \sum_{k = 1}^{\infty} \E (\mu_1^{-1}R_{1, 1})^k \mathbb{I} (R_{1, 1} \leq \mu_1)  \leq \frac{e}{3} \E \exp (\mu_1^{-1} R_{1, 1})\mathbb{I} (R_{1, 1} \leq \mu_1) \leq \frac{e^2}{6} \cdot \exp \left\{ \frac{1}{2 \mu_1^2 \sigma_1^2}\right\}
    \end{aligned}
\end{equation*}
and
\begin{equation*}
    \begin{aligned}
        I_2 \geq \frac{1}{\mu_1} \E R_{1, 1} = 1
    \end{aligned}
\end{equation*}
impling $I \leq e^{2 + 1/(2 \mu_1^2 \sigma_1^2)} / 6 - 1$. And similarly, we have $II \leq e^{1 + 1/(2 \mu_1^2 \sigma_1^2)} / 2 - 1$, which gives the bound 
\begin{equation*}
    a_{k, s} \leq \big( e^{2 + 1/(2 \mu_1^2 \sigma_1^2)} / 6 + e^{1 + 1/(2 \mu_1^2 \sigma_1^2)} / 2 - 3 \big)^{|\his_{1, s}|}, \qquad k \in [K], \qquad s = 0, \ldots, T - 1
\end{equation*}
as long as $R_{1, 1}$ is psuedo-symmetric sub-Gaussian variable with 
\begin{equation*}
    \E e^{(R_{1, 1} - \mu)t} \mathbb{I}(R_{1, 1} \leq \mu_1) \vee \E e^{(R_{1, 1} - \mu)t} \mathbb{I}(R_{1, 1} > \mu_1) \leq \frac{1}{2} e^{\frac{t^2\sigma_1^2}{2}},
\end{equation*}
and $y := 1 / (2 \mu_1^2 \sigma_1^2)$ gives $e^{2 + y}/ 6 + e^{1 + y} / 2 - 3 \in (0, 1)$, i.e. $\mu_1 \sigma_1 > \sqrt{\frac{e (e + 3)}{48}} \approx 0.5690618$, which implies the mean reward of the optimal arm cannot be too small.

\noindent Then we decompose $a_{k,s}$ as $a_{k, s} = a_{k, s, 1} + a_{k, s, 1} + a_{k, s, 1}$
\begin{gather*}
    a_{k, s, 1} := \E \big[ (N_{1, s} (\tau_k) \wedge T) \mathbb{I} (A_{1, s}) \mathbb{I} (G_{1, s})\big] \\
    a_{k, s, 2} := \E \big[ (N_{1, s} (\tau_k) \wedge T) \mathbb{I} (A_{1, s}^c) \mathbb{I} (G_{1, s})\big] \\
    a_{k, s, 3} := \E \big[ (N_{1, s} (\tau_k) \wedge T) \mathbb{I} (G_{1, s}^c)\big],
\end{gather*}
the next step we need to do is bounding $s_{a, j} := \{s : a_{k, s, j} \leq T^{-1} \}$ for $j = 1, 2, 3$.
\vspace{2ex}

\noindent $\circ$ $\circ$ \textbf{Bound $s_{a, 1}$:} 

\noindent First note that $\{ N_{1, s}(\tau_k) < T^{-1} \} \supseteq \{ N_{1, s}(\tau_k) < (T^2 - 1)^{-1} \} = \{ [1 - Q_{1, s}(\tau_k)] < T^{-2}\}$ with
\begin{equation*}
    \begin{aligned}
        1 - Q_{1, s}(\tau_k) = \pr (\overline{Y}_{1, s} \leq \mu_1 \, | \, \his_{1, s}) \leq \pr ()
    \end{aligned}
\end{equation*}
}}


\fi


\iffalse
{\color{red}{
As we can see, Algorithm 2 and 3 as a practical supplementary for Algorithm 1. Hence, it is enough to deal with Algorithm 1.
Note that in Algorithm 1, we have $\overline{Y}_{k, s} =  \sum_{\ell = 1}^{|\his_s|} w_{\ell} \cdot R_{k, \ell}$ for $k \in [K]$ and $s \in [T]$ with $\omega_{\ell} \overset{\text{i.i.d}}{\sim } \rho(\omega)$, it is enough to deal with the algorithm 1 with $\overline{Y}_{k}$ replaced by $\overline{Y}_{k, s} $. 

Denote $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_s  \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$. Then from Theorem 1 in \cite{kveton2019garbage}, we have 
\begin{equation*}
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\end{equation*}
with
\begin{equation*}
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] = \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1
\end{equation*} 
for any $\tau_k \in \mathbb{R}$. So it is enough to bound $a_k$ and $b_k$.

\noindent $\circ$ \textbf{Bound $a_k$:}

\noindent Define the good events:
\begin{equation*}
    A_{1, s} := \big\{ \overline{Y}_{1, s} - \mu_1 > - \Delta_k / 4 \big\}, \qquad G_{1, s} := \{ \}.
\end{equation*}
For $\tau_k \leq \mu_1$, we have $a_{k, s} \leq \E Q_{1, s}(\tau_k)^{-1} \leq \E \big[ \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})^{-1} \big]$. To deal with tail probability, we need to use lower bound of tail probability of Gaussian variables, such that
\begin{equation*}
    \begin{aligned}
        \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s}) & = \pr_{\omega} \left( \sum_{\ell = 1}^{|\his_s|} \omega_{\ell} R_{1, \ell} > \mu_1 \right) \\
        (\text{assume } \omega_s \sim N(0, \sigma_{\omega}^2)) & \geq \left\{ \begin{array}{ll}
            \exp \left\{ - \frac{\mu_1^2}{\sigma_{\omega}^2 \sum_{\ell = 1}^{|\his_s|} R_{1, \ell}^2} \right\},  &  \mu_1 \geq  \sigma_{\omega} \| R_{1, s}\|_2\\
            1 - \Phi(\sqrt{2 \pi}), & \mu_1 < \sigma_{\omega} \| R_{1, s}\|_2
        \end{array}\right.
    \end{aligned}
\end{equation*}
where $\| R_{1, s}\|_2^2 = {\sum_{\ell = 1}^{\his_s} R_{1, \ell}}^2 $. Hence
\begin{equation*}
    \begin{aligned}
        a_{k, s} & \leq \E \big[ \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, s})^{-1} \big] \\
        & \leq \E \exp \left\{ \frac{\mu_1^2}{\sigma_{\omega}^2 \| R_{1, s}\|_2^2} \right\} \I \big(\| R_{1, s}\|_2 \leq \sigma_{\omega}^{-1} \mu_1 \big) + \big[ 1 - \Phi(\sqrt{2 \pi}) \big]^{-1} \pr \big( \| R_{1, s}\|_2 >  \sigma_{\omega}^{-1} \mu_1  \big)
    \end{aligned}
\end{equation*}

\begin{equation*}
    \begin{aligned}
        \pr (\overline{Y}_{1, s}^{b_s} > \mu_1 \, | \, \his_{1, s}) & = \pr \big(\overline{Y}_{1, s}^{B} > \mu_1 \, | \, \his_{1, s} \big ) \\
        & \leq \pr \left( \overline{Y}_{1, s}^{B - 1} > \frac{(c_{1, s} + 1)\mu_1 - R_s \cdot \omega_B}{c_{1, s}} \, \Big| \, \his_{1, s }\right) \\
        & \leq \pr \left( \overline{Y}_{1, s}^{0} > \Big( \frac{c_{1, s} + 1}{c_{1, s}}\Big)^B \cdot \mu_1 - \frac{R_s}{c_{1, s}} \sum_{b = 1}^B \omega_b \, \Big| \, \his_{1, s} \right) \\
        & \leq  \pr \left( \sum_{b = 1}^B w_b > \Big\{ \Big( \frac{c_{1, s} + 1}{c_{1, s}}\Big)^B \mu_1 - \overline{Y}_{1, s}^{0} \Big\} \cdot \frac{c_{1, s}}{R_s} \, \Big| \, \his_{1, s} \right) \\
        & \leq \exp \left\{ - \frac{2}{n} \left(\Big\{ \Big( \frac{c_{1, s} + 1}{c_{1, s}}\Big)^B \mu_1 - \overline{Y}_{1, s}^{0} \Big\} \cdot \frac{c_{1, s}}{R_s} - \frac{B}{2} \right)^2 \right\} 
    \end{aligned}
\end{equation*}
Note the fact that $\overline{Y}_{1, s}^0 = \frac{1}{c_{1, s} - 2} \sum_{\ell = 1}^{c_{1, s} - 2} Y_{1,\ell}$, hence
\begin{equation*}
    \begin{aligned}
        a_{k, s} & \leq \E \exp \left\{ \frac{2}{n} \left(\Big\{ \Big( \frac{c_{1, s} + 1}{c_{1, s}}\Big)^B \mu_1 - \overline{Y}_{1, s}^{0} \Big\} \cdot \frac{c_{1, s}}{R_s} - \frac{B}{2} \right)^2 \right\} \\
        & \leq e^ {\frac{B^2}{2 n}} \cdot \E \Bigg\{ \E \exp \bigg[\frac{2 c_{1, s}^2}{n R_s^2 } \big( \overline{Y}_{1, s} - \mu_1\big)^2 \, \Big| \, R_s  \bigg] \cdot \exp \bigg[ \frac{2 c_{1, s}^2 \mu_1^2}{n R_s^2 } \Big( 1 - \frac{(1 + c_{1, s})^B}{c_{1, s}^B}\Big)^2 \bigg] \Bigg\} \\
        & \leq e^ {\frac{B^2}{2 n}} \E \exp \bigg[ \frac{2 c_{1, s}^4}{n^2 R_s^4 } \frac{16\sigma_1^4}{(c_{1, s} - 2)^2} + \frac{2 c_{1, s}^2 \mu_1^2}{n R_s^2 } \Big( 1 - \frac{(1 + c_{1, s})^B}{c_{1, s}^B}\Big)^2 \bigg] \\
        & = 
    \end{aligned}
\end{equation*}
by the fact
\begin{equation*}
    \overline{Y}_{1, s}^0 - \mu_1 \, \sim \, \operatorname{subG} \left( \frac{\sigma_1^2}{c_{1, s} - 2}\right) \quad \text{ and } \quad \big(\overline{Y}_{1, s}^0 - \mu_1 \big)^2 \, \sim \, \operatorname{subE} \left( \frac{16\sigma_1^2}{c_{1, s} - 2}\right).
\end{equation*}
}}
\fi


1. nonrandom or random weights in each step?


% \subsection{Proof Scheme for Linear bandits}


% The novelty in analyzing the above algorithm would be that it is the first analysis of the multiplier bootstrap in the setting where observations are collected adaptively. We can decide whether to do a frequentist or Bayesian analysis. I suggest that we go Bayesian for the following reasons. First, Bayesian should be easier and cleaner if done right. Second, most analyses of the perturbation-based methods are frequentist. So this is yet another place where we can differentiate from others.


% There are two places where we can start:

% 1. Linear model.
% 2. An arbitrary hypothesis space with an efficient least-squares oracle.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width = \linewidth]{Fig/derivation_1.png}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}


\input{Related_Work}

\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{aaai2021.bst}
\bibliography{0bib}

\end{document}

==> ARCHIVE/0_Main_backup.tex <==
\input{0_ICLR_front}
\usepackage{lineno}
\usepackage{soul}
\linenumbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{document}
\maketitle


\input{1_abstract}

\input{1_Intro}

\input{1_Related_Work}

\input{2_Setup}

\input{2_Algorithm}



\input{3_Theory}

\input{4_Experiments}

\input{6_Discussion}

% \input{Alg/main_alg_MAB}

\newpage


\bibliography{0_bib.bib}
\bibliographystyle{iclr2022_conference}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\appendix
\renewcommand{\appendixname}{Appendix~\Alph{section}}

\input{9_More_MBTS}

\input{9_exp_details}

\input{9_Main_Proof_new}

\input{9_Supporting_Lemmas}

\input{9_Technique_Lemmas}

%\input{9_Main_proof}

%\input{9_Proof_Lemmas}

%\input{9_Special_Case}

\end{document}


==> ARCHIVE/9_Main_proof_backup.tex <==
\todorw{It is not appropriate to divide one proof into multiple subsections. The typical flow is to present the main proof in one subsection, with intermediate results stated as lemmas in this subsection and proved in latter subsections.}

\todorw{Another suggestion is to be aware of the punctuation before/after equations. Equations are part of the sentences, so any rules will still apply. }

\todorw{I suggest to replace $1()$ with $\I()$}
\todorw{In the final version, we need to use less $:=$ to define notations/shorthands. This is not a rigorous and clear way to define variables. 
For example, in `$b_k = \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1 =: \sum_{s = 0}^{T - 1} b_{k, s} + 1$`, what is the definition of $b_{k,s}$? We can guess, but this should not be left to the readers. 
}

% \todorw{One tool that might be helpful is `grammarly.com`. I may need to read again to begin to follow the mathematical derivations, after the presentation is improved.}

\todorw{I suggest to always first present the intention/goal in plain English, before mathematical derivations. }

\section{Proof of Theorem \ref{thm.MAB}}



The proof Theorem \ref{thm.MAB} can be divided into three main parts. The first part is recapping a decomposition of the cumulative regret as our proof relies on the following decomposition from \cite{kveton2019garbage}. 
We recap its proof in Appendix \ref{sec:proof_lemma} for completeness. 


\begin{lemma}\label{lem.a.b}
% When we select arms according to the
Recall that we select arms according to the rule 
$A_t = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 
% in the MAB problem, then 
For any $\{ \tau_k \}_{k = 2}^K \subseteq \mathbb{R}^{K - 1}$, 
we have the bound
\begin{equation*}
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\end{equation*}
with
\begin{equation*}
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] =: \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1 =: \sum_{s = 0}^{T - 1} b_{k, s} + 1
\end{equation*} 
where $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_{k, T} \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$.
\end{lemma}

From the definition of $a_{k, s}$ and $b_{k, s}$, $a_k$ controls that the tail probability of the optimal arm is not too small, while $b_k$ controls that the tail probabilities of rewards of all arms are not too large in general. 
%\todorw{What is the tail probability of an arm?}
It is worthy to note that for here we only need to consider the lower bound of the tail of the optimal arm. The intuition is that we only need to the probability of taking a relatively large value in the optimal arm is not too small. And we do not care about how small the probability of a large value occurred in the other arms. And this Lemma is valid for any algorithm in MAB problem as long as the action step is $A_{t} = \arg \max_{k \in [K]} \overline{Y}_{k, t}$.

% \todorw{I had a hard time understanding the explanations above in English. We can probably just check how the other papers describe these variables.}

Based on Lemma \ref{lem.a.b}, it is enough to bound $a_k$ and $b_k$ separately. We will do this as the following framework.

% \todorw{We should avoid overloading notations. For example, $s^*$ in the diagram below.}

\todorw{$\cdot$ is also typically not recommended. Suggest to either remove, or replace with $\times$ when necessary.}

\begin{tikzpicture}[node distance=2cm]
    \node (step1) [startstop] {Decomposition with Lemma \ref{lem.a.b}}; 
    
    \node (step2) [process, below of=step1, xshift=-5cm] {Step I : Bound $a_k = \sum_{s = 0}^{T - 1} a_{k, s}$ as order $\log T$}; 
    
    \node (step2.0) [process, below of=step2, xshift=0cm] {Consider $s_a := \max \{{s : a_{k, s}} \geq T^{-1} \}$, then $$a_k \leq \max_{s} a_{k, s} \cdot s_a + T^{-1} \cdot (T - s_a).$$};
    
    \node (step2.1) [startstop, below of=step2.0, xshift=-2.5cm] {Bound $a_{k, s}$ with a constant};
    
    \node (step2.1.1) [startstop, below of=step2.0, xshift=-2.5cm] {Bound $a_{k, s}$ with a constant};
    
    \node (step2.1.2) [startstop, below of=step2.1.1, xshift=-1cm] {Use anti-concentraction};
    
    \node (step2.2.1) [startstop, below of=step2.0, xshift=2.5cm] {Bound $s_a$ as $\log T$};
     
    \node (step2.1.2) [startstop, below of=step2.2.1, xshift=-0.5cm] {May need to decompose $a_{k, s} = \sum_{j = 1}^3 a_{k, s, j}$};
     
    \node (step3) [process, below of=step1, xshift=4cm] {Step II : Bound $b_k = \sum_{s = 0}^{T - 1} b_{k, s} + 1$ as order $\log T$}; 
    
    \node (step3.0) [process, below of=step3, xshift=0cm] {Consider $s_b := \max \{{s : b_{k, s}} \geq T^{-1} \}$, then $$b_k \leq s_b + T^{-1} \cdot (T - s_b).$$};
    
    \node (step3.1) [startstop, below of=step3.0, xshift=0cm] {Bound $s_b$ as $\log T$};
    
    \node (step3.2) [startstop, below of=step3.1, xshift=0cm] {Also need to decompose $b_{k, s} = \sum_{j = 1}^3 b_{k, s, j}$};
    
    \draw [arrow] (step1) -- (step2);

    \draw [arrow] (step1) -- (step3);
    
\end{tikzpicture}

%\red{Definitions of these terms can be more u nclear.}
%with any $\{ \tau_k \}_{k = 2}^K \subseteq \mathbb{R}^{K - 1}$ where $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_{k, T} \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$ for some $\tau > 0$. So our target switch from $\operatorname{Reg}_T$ to $a_k$ and $b_k$. And the next two main steps will be bounding $a_k$ and $b_k$ separately. 

%\red{To be added: Intuitively, what is the meaning of $a_k$ and $b_k$? Intuitively, why the regret can be bounded by them?}


\subsection{First Step: Bounding $a_k$}
% \todorw{The relationship between subsections is still not clear. 
% I recommend writing in this way (an example) (always stating clearly what we try to do in this section. Do not assume the reviewer will patiently read the whole section and finally understand the whole idea after reading   the last sentence): 
% }
% \red{\begin{itemize}
%     \item Section A: we aim to bound B by decomposing B = B1 + B2. Below, we bound them separately. 
%     \item Section A1: in this section, we aim to bound B1 by xxx (main idea).
%     \item Section A2: in this section, we aim to bound B2 by xxx (main idea).
% \end{itemize}
% }

As the diagram above, for bounding $a_k$ as order $\log T$, what we need to do first is up-bounding $a_{k, s}$ with a constant (free of $T$), and then bound $s_a$ as order $\log T$

%\todorw{Introduce the plan in words clearly. Such as bounded xx by constant (in Section xxx).}
\subsubsection{Bound $a_{k,s}$ as a constant}

For doing this, note that if
\begin{equation}\label{condition.1}
    \tau_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda}
\end{equation}
we will have
\begin{equation*}
    a_{k, s} \leq \E Q_{1, s}(\tau_k)^{-1} \leq  \E \left[ Q_{1, s}^{-1}\left(  \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \right] = \E \Bigg[ \pr \bigg(\overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \, \Big| \, \his_{1, T} \bigg)^{-1} \Bigg],
\end{equation*}
we need to first find the lower bound of the tail probability $\pr (\overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \, | \, \his_{1, T})$ and then bound its expectation over the optimal arm's history $\his_{1, T}$, where $\his_{k, t}$ represents the rewards of $k$-th arm up to $t$-th round.

%\todorw{The paragraph above is not easy to understand. For example, the probability of taking a relatively large value in the optimal arm is not too small`}


% \subsubsection{Lower bound of the tail probability $\pr (\overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}  \, | \, \his_{1, T})$}

% \subsubsection{A possible construction of $\overline{Y}_{1, s}$.}
%\todorw{This section is confusing. The notation s is not well-defined. Do we only need to study arm 1?}
Recall in our algorithm, the target function is for some fixed arm $k$. 
For a fixed arm $k$, we can denote that $s := |\his_{k, T}|$ as the total number of pulling the $k$-th arm. 
Under this simplicity, we have 
\begin{equation*}
    \overline{Y}_{k, s} = \frac{\sum_{i = 1}^s (\omega_{i} R_{k, i} + \lambda  \omega_{i}') }{\sum_{i = 1}^s (\omega_{i} + \lambda\omega_{i}' + \lambda \omega_{i}'')}. 
\end{equation*}
% will be only random on the bootstrap weights $\omega_{\ell}$, conditioned on $\his_{1, s}$. 
We use $\pr_{\omega} (A)$ to emphasize that the probability is only taken over the random variable $\omega$ alone. We have 
% as the random elements in $A$, then
% as calculating the probability of the event $A$ with only regarding
%\red{In the modified algorithm, this task would be similar to Thm 4 in GIRO. However, their proof heavily depends on the Bernoulli distribution (if necessary, we can use probably use some other distribution for the weight as well, e.g., two bernoulli? We may need some technical tools from multiplier bootstrap literature, finite-sample bound.)}
%and the lower bound of the tail probability require the exact distribution of $\omega_{\ell}$ or the harsh restriction for $\omega_{\ell}$ will be involved (see the discussion of \cite{zhang2020non} for details), this is the reason why we specify the distribution of $\omega_{\ell}$ as normal distribution.
\todorw{The reason that I added $| H$ in line 3 before, is because the current notation ($\pr_{\omega} (A)$ ) is not rigorously defined.}
\begin{equation*}
        \begin{aligned}
            & \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \, \Big| \, \his_{1, s} \right) \\
            = \, & \pr \bigg( \sum_{i = 1}^s \omega_i (R_{1, i} - \mu_1) + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s  (\omega_i' - \omega_i'') + \lambda \sum_{i = 1}^s (2 \omega_i R_{1, i} - \omega_i' \mu_1 - \omega_i'' \mu_1) > 0 \mid \ \his_{1, s} \bigg) \\
            = \, &  \pr_{\omega, \omega', \omega''} \bigg\{ \sum_{i = 1}^s \big( (2 \lambda + 1) R_{1, i} - (\mu_1 + \lambda)\big) \omega_i > \lambda (\mu_1 - 1 - \lambda) \sum_{i = 1}^s \omega_i' + \lambda (\lambda + \mu_1) \sum_{i = 1}^s \omega_i''  \bigg\} \\
            \geq \, & \exp \bigg\{ - \frac{3s(2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left[s \lambda^2 (\lambda + 1 - \mu_1)^2 + s\lambda^2 (\lambda + \mu_1)^2\right]}\bigg\} \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \\
            & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ ~~~~~~~~~~~~~~~~~~~~~~~~~~ + \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
            \geq \, & \exp \bigg\{ - \frac{3(2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2\lambda^2  \left[ (\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2\right]}\bigg\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        \end{aligned}
\end{equation*} 
where the last inequality is based on the property of Gaussian random variables, which we summarize in the following lemma. 

% where we generally suppose the Bootstrap weight are $N(1, \sigma_{\omega}^2)$ distributed with using the following lemma. 
\begin{lemma}\label{lemma:gaussian_weight}
    Suppose $x_i, y_i, z_i \in \mathbb{R}$ and 
    % and $\omega, \omega', \omega''$ are 
    % iid $N(1, \sigma_{\omega}^2)$ random variables
    % , then $\pr (x \omega > y \omega' + z \omega'')$ is bounded by some tail probability and indicator. Furthermore, if 
    $\{\omega_i, \omega_i', \omega_i''\}$ are independent $N(1, \sigma_{\omega}^2)$ random variables, then
    \begin{equation*}
        \begin{aligned}
            & \pr \bigg( \sum_{i = 1}^n x_i \omega_i > \sum_{i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \bigg) \\
            \geq & \exp \bigg\{ - \frac{3(S_x - S_y - S_z)^2}{2 \sigma_{\omega}^2(T_x + T_y + T_z)}\bigg\} \cdot 1 \big(S_x \geq S_y + S_z + \sqrt{2\pi} \big) + \big( 1 - \Phi(\sqrt{2\pi} )\big) \cdot 1 \big(S_x \leq S_y + S_z + \sqrt{2\pi}\big), 
        \end{aligned}
    \end{equation*}
    for any $n \in \mathbb{N}$ where we denote $S_x = \sum_{i = 1}^n x_i$ and $T_x = \sum_{i = 1}^n x_i^2$, and similar notation for $S_y, S_z, T_y, T_z$.
\end{lemma}


\iffalse
\begin{remark}
    If we choose to use same weight version, Algorithm 3, to analyze, we need to compute 
    \begin{equation*}
    \begin{aligned}
        \pr \left( \overline{Y}_{1, s} > \frac{\mu + \lambda}{1 + 2 \lambda}\right) = \pr \bigg( (2\lambda + 1) \sum_{i = 1}^s \omega_i (R_{1, i} - \mu_1) > 0 \bigg) = \pr \bigg( \sum_{i = 1}^s \omega_i (R_{1, i} - \mu_1) > 0 \bigg).
    \end{aligned}
    \end{equation*}
    It can be seen that this degenerate to the analysis in Algorithm 1.
\end{remark}
\fi



Hence, we immediately have that $a_{k, s}$ is bounded by
\begin{equation*}
    \begin{aligned}
        a_{k, s} & \leq \E \exp \bigg\{\frac{3(2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \lambda^2 ((\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2 )}\bigg\} + \big[ 1 - \Phi(\sqrt{2\pi} )\big]^{-1}  \\
        & \leq \exp \bigg\{\frac{3(2 \lambda + 1)^2 \cdot 1}{2 \sigma_{\omega}^2 \lambda^2 ((\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2 )}\bigg\} + \big[ 1 - \Phi(\sqrt{2\pi} )\big]^{-1} \\
        & \leq \exp \bigg\{\frac{3(2 \lambda + 1)^2}{2 \sigma_{\omega}^2 \lambda^2 \big[(\lambda + 1 )^2 + \lambda^2 \big]}\bigg\} + \big[ 1 - \Phi(\sqrt{2\pi} )\big]^{-1} 
    \end{aligned}
\end{equation*}
where we utilize the \red{boundedness} of the rewards. Hence, we get an upper bound for $a_{k, s}$.

\red{
    In this step, we can see that to bound $a_{k, s}$, one only need to have the MGF of $(\overline{R}_{1, s} - \mu_1)^2$ is bounded, hence the bounded assumption is not essential here. 
    % On the other hand, in the algorithm, our construction needs $R_{1, i}$ are bounded in some interval intuitively. The mathematical reason why we need $R_{k, i}$ is bounded, need to clarify later.
}


\todorw{$(\overline{R}_{1, s} - \mu_1)^2$ is sub-exponential, the MGF of which is only bounded in an interval around $0$. We can hence derive the required condition on $\lambda$ and $\sigma_{\omega}$.}
\todohw{Yes, $(\overline{R}_{1, s} - \mu_1)^2$ is sub-exponential when $R_{k, i}$ is sub-Gaussian. Indeed, the restriction of tuning parameter $\lambda$ in other literature is always derived from this step.}
\todorw{So, if we have time, I suggest to derive it (after finishing the other parts)}

% \begin{framed}
% \begin{equation*}
%     \begin{aligned}
%         \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, T}) & = \pr_{\omega} \left(  \sum_{\ell = 0}^{s} (R_{1, \ell} - \mu_1) \cdot \omega_{\ell} \geq 0 \right) \geq \pr_{\omega} \left( \bigcap_{\ell = 0}^{s} \big\{ (R_{1, \ell} - \mu_1) \omega_{\ell} \geq 0 \big\} \right) \\
%         & = {\color{red}{1(\lambda_1 s \geq \mu_1)}} \prod_{\ell = 1}^{s} \pr_{\omega} \left( (R_{1, \ell} - \mu_1) \omega_{\ell} \geq 0 \right),
%     \end{aligned}
% \end{equation*}
% with $R_{0, \ell} = \lambda_1 s$, and then under the condition $\lambda_1 s \geq \mu_1$ holds, 
% \begin{equation*}
%     \begin{aligned}
%         a_{k, s} & \leq  \E \big[ \pr (\overline{Y}_{1, s} > \mu_1 \, | \, \his_{1, T})^{-1} \big] = \prod_{\ell = 1}^{s} \pr (R_{1, \ell} - \mu_1 \geq 0) = p_{1}^s .
%     \end{aligned}
% \end{equation*}
% where $p_k := \pr (R_k > \mu_k)$. Hence, $a_{k, s}$ is a least bound by 1, as long as $p_1 \in (0, 1]$.
% \end{framed}


\subsubsection{Bound $s_a$ with a order $\log T$}
% \subsubsection{Using the good events to restrict the outliers of $a_{k, s}$}

Let $a_T \lesssim b_T$ represent $a_T \leq c  b_T$ for some constant $c$.
After bounding $a_{k, s}$, then next step is to find $s_a := \max \{s: a_{k, s} \geq  T^{-1}\}$ and prove that $s_a \lesssim \log T$. However, this may be difficult by the instinct construction of $a_{k, s}$. Fortunately, we can decompose $a_{k, s}$ as $a_{k, s} = \sum_{j = 1}^m a_{k, s, j}$ with some simple $a_{k, s, j}$, and then construct $s_{a, j} := \max \{ s: a_{k, s, j} \geq T^{-1} \}$ and show $s_{a, j} \lesssim \log T$. Recall in the proof sketch diagram we have the decomposition that
\begin{equation*}
    a_k \leq \max_{s} a_{k, s} \cdot \max_j s_{a, j} + m T^{-1} \cdot (T - \max_j s_{a, j}).
\end{equation*}
and we have bounded $a_{k, s}$ as a constant, what remains is bounding $s_{a, j}$ for $j \in [m]$ as $\log T$.

For establish simpler $a_{k, s, j}$, a common method is decomposing $a_{k, s}$ on some good events with their complement sets. Recall the essential ingredient in the algorithm is based on the mean rewards of each arm. We denote the shifted version of average reward as
\begin{equation*}
    \overline{R}_{k, s}^* := \frac{\sum_{i = 1}^s R_{k, i} + \lambda s}{s (1 + 2 \lambda)} = \frac{\lambda}{1 + 2 \lambda} + \frac{1}{1 + 2\lambda } \overline{R}_{k, s} + \frac{\lambda}{1 + 2 \lambda} \cdot 0,
\end{equation*}

% \begin{framed}
% Denote the shifted version of average reward as
% \begin{equation*}
%     \overline{R}_{k, s}^* := \frac{\lambda_k s + \sum_{\ell = 1}^s R_{k, \ell}}{s} = \lambda_k + \overline{R}_{k, s}
% \end{equation*}
% \end{framed}


where $\overline{R}_{k, s} = \frac{1}{s} \sum_{i = 1}^s R_{k, i}$ and then define good events\footnote{In the original version: we set that $A_{k, s} := \{ \overline{R}_{k, s}^* - \mu_k > - C_1 \Delta_k\}$ and $A_{k, s}^{\prime} := \{ \overline{R}_{k, s}^* - \mu_k < C_2 \Delta_k\}$} with some $C_1, C_2 \in (0, 1)$,
\begin{equation*}
    A_{k, s} := \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} > - C_1 \Delta_k\right\}, \qquad A'_{k, s} := \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} < C_2 \Delta_k\right\}
\end{equation*}
\iffalse
\todohw{The major difference between now and previous verison is that the original verison $C_1, C_2$ do not relate to tuning parameter $\lambda$. Indeed, I do not know whether is correct that $C_1$ and $C_2$ are functions of $\lambda$ (which will furthermore ask that $\tau_k$ depends on $\lambda$)...}
\todohw{There is no way to avoid this problem as $\lambda$ appears on the denominator. The only possible solution is to drop the denominator...}
\todohw{Although we can take any $\{ \tau_k\}$, but I am not sure whether they can depend on $\lambda$.}
\todohw{However, I find there is no way to use $A_{k, s}$ in the previous verison, as it will lead to 
\begin{equation*}
    - C_1 \Delta_k (1 + 2\lambda) + 2 \lambda (2 \mu_1 - 1) \leq 0,
\end{equation*}
i.e. $C_1 \Delta_k (1 + 2 \lambda) > \lambda (2 \mu_1 - 1)$, which asks $\mu_1 \leq \frac{1}{2}$. And then the iternation by the algorithm will make $\mu_1 \equiv 0$.
}
\todohw{I find that if we change the $\overline{Y}_{k, s}$ to 
\begin{equation*}
    \overline{Y}_{k, s} = \frac{\omega R + \lambda \omega'}{\omega + \omega'}
\end{equation*}
all proof can be give with the original $A_{k, s}$. But the problem is how to explain.
}
\fi
Define:
\begin{equation*}
    a_{k, s, 1} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) \Big], \qquad a_{k, s, 2} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}^c) \Big],
\end{equation*}
with $s_{a, j} := \max \{ s: a_{k, s, j} \geq T^{-1} \}$. What we need to do is bounding $s_{a, j}$ as order $\log T$.
% \todorw{Where does the '0.5' come from? An assumption?}


%\todohw{I do not notice any issue from the fact that these constants will depend on our tuning parameter (which is part of our algorithm). }

\iffalse
In this step, our target is to show that 
\begin{align*}
\max_{j = 1, 2} s_{a, j} \lesssim \log T, 
\end{align*}
which implies
\begin{equation*}
    \begin{aligned}
        a_k & = \sum_{s = 0}^{T - 1} a_{k, s} \leq \max_{s} a_{k, s} \cdot \max_{j = 1, 2} s_{a, j}  + (T -  \max_{j = 1, 2} s_{a, j}) \cdot (T^{-1} + T^{-1})\\
        & \leq \left[ \exp \bigg\{\frac{3(2 \lambda + 1)^2 ((1 - \mu_1)^2 + \mu_1^2 )}{4 \sigma_{\omega}^2 \lambda^2 ((\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2 )}\bigg\} + \big[ 1 - \Phi(\sqrt{2\pi} )\big]^{-1} \right] \cdot & \max_{j = 1, 2} s_{a, j} (T)  + (T - \max_{j = 1, 2} s_{a, j} (T)) \cdot 2 T^{-1} \\
        & \lesssim 2 + \log T.
    \end{aligned}
\end{equation*}
\fi
% As a result, it is sufficient to show that $\max_{j = 1, 2} s_{a, j} (T) \lesssim \log T$. 

%\todorw{Where did we state the first inequality?}

\paragraph{Tackling $s_{a, 2}$}
% \todorw{$a_{k, s, 2}$ does not even appear in this section, which will make readers confusing.}
The construction of $\overline{R}_{k, s}^*$ indicates that the behaviour of $\overline{R}_{k, s}^*$ should be close to the true quantity $\overline{Y}_{k, s}$. 
Therefore, we first focus on studying the probability of the bad event $A_{1, s}^c$ defined previously. 
By the Hoeffding's inequality, we have\footnote{In the original verison we have :$\pr (A_{1, s}^c) = \pr \bigg( \mu_1 - \overline{R}_{1, s} \geq C_1 \Delta_k + \frac{\lambda}{1 + 2 \lambda}\bigg) \leq \exp \bigg\{ - 2s \Big(  C_1 \Delta_k + \frac{ \lambda}{1 + 2 \lambda} \Big) \bigg\} \leq T^{-2}, $}
\begin{equation*}
    \begin{aligned}
        \pr (A_{1, s}^c) & = \pr \bigg( \frac{\overline{R}_{1, s} - \mu_1}{1 + 2 \lambda} \leq - C_1 \Delta_k \bigg) = \pr \big( \mu_1 - \overline{R}_{1, s} \geq (1 + 2 \lambda) C_1 \Delta_k \big) \\
        & \leq \exp  \bigg\{ - \frac{2(1 + 2 \lambda)^2 C_1^2 \Delta_k^2 s^2 }{s \cdot (1 - 0)^2}\bigg\} = \exp \big\{ - 2 s C_1^2 (1 + 2\lambda)^2 \Delta_k^2  \big\}
    \end{aligned}
\end{equation*}
as $\{ R_{k, i} \}_{i = 1}^s$ are all bounded in $[0, 1]$.
If we take 
\begin{equation*}
    s \geq s_{a, 2} : = \frac{\log T}{C_1^2 (1 + 2\lambda)^2 \Delta_k^2}
\end{equation*}
and then we will have
\begin{equation*}
    a_{k, s, 2} \leq T \E 1\big( A_{1, s}^c \big) \leq T^{-1}.
\end{equation*}
i.e the above $s_{a, 2}$ is what we need.

%\todorw{The section is still incomplete. If the goal is to bound $s_{a,2}$, then conclude with a statement on the bound, instead of `if we take`.}

\begin{remark}
    In this step, we use the \red{boundedness} of the rewards $R_{k, s}$ so that we can apply the Hoeffding's inequality. However, the boundedness assumption is not essential to derive the final bound above. 
    In fact, as long as we have 
    \begin{equation*}
        \log \pr \big( \mu_1 - \overline{R}_{1, s} \geq (1 + 2 \lambda) C_1 \Delta_k \big) \lesssim -s, 
    \end{equation*}
    we can still find a proper $s_{a,2}$. It can be easy to hold when the rewards are sub-Gaussian variables.
\end{remark}


% \begin{framed}

% \begin{equation*}
%     \begin{aligned}
%         \pr (A_{1, s}^c) & = \pr \bigg\{ \sum_{i = 1}^s R_{1, i} \leq (\mu_1 - C_1 \Delta_k - \lambda_1) s  \bigg\}  = \pr \Big( \mu_1 - \overline{R}_{1, s} \geq  \lambda_1 + C_1 \Delta_k \Big) \\
%         & = \exp \bigg\{ - \frac{2 s (\lambda_1 + C_1 \Delta_k)^2}{(b - a)^2}\bigg\} \leq T^{-\eta}
%     \end{aligned}
% \end{equation*}
% for any $\eta > 1$ if we take $s \geq s_{a, 2} := \frac{\eta (b - a)^2 }{2 (\lambda_1 + C_1 \Delta_k)^2} \log T$, and hence we will get
% \begin{equation*}
%     a_{k, s, 2} \leq T \cdot T^{-\eta} = T^{-\eta + 1}.
% \end{equation*}

% \end{framed}


\paragraph{Dealing with $s_{a, 1}$}

To study $a_{k, s, 1}$, recall we have $a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) \Big] \approx \E N_{1, s} (\tau_k)$ as we have large possibility on the good event $A_{1, s}$: we have $\pr (A_{1, s}) \geq 1 - T^{-2}$ when we have $s \geq s_{a, 2}$.
% \green{(as the good event XX is true with high probability.)}. 
%\todorw{Which good event? When we write, it is clear to ourselves. But this is not the case for reviewers and readers. }
However, as $N_{k, s}(\tau_k)$ depends on $Y_{k, s}$ rather than $R_{k, s}$. It is worthy to study the gap between them, and define another good event based on the gap. 

The gap between $\overline{Y}_{1, s}$ and $\overline{R}_{1, s}^*$ is
\begin{equation*}
    \begin{aligned}
        \overline{Y}_{1, s} - \overline{R}_{1, s}^* \, | \, \his_{1, T} = \frac{D_1 + D_2 + D_3 }{(1 + 2 \lambda)\sum_{i = 1}^s  (\omega_i + \lambda \omega_i' + \lambda \omega_i'')}
    \end{aligned}
\end{equation*}
with
%\begin{gather*}
    %D_1 :=  \sum_{i = 1}^s \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big] \omega_i, \\
    %D_2 := \sum_{i = 1}^s \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big] \omega_i', \\
    %D_3 = \sum_{i = 1}^s - (\lambda^2 + \lambda \overline{R}_{1, s}) \omega_i''.
%\end{gather*}
%\todorw{the logic above and below is unclear to me. Is this a re-organization of variables?}
%Equivalently, we can re-organize variables and define 
% it is better to write as
\begin{gather*}
    D_1 : = \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) \omega_i, \\
    D_2 := \lambda \sum_{i = 1}^s (2 R_{1, i} \omega_i - \overline{R}_{1, s} \omega_i' - \overline{R}_{1, s} \omega_i''), \\
    D_3 := \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega_i''). 
\end{gather*}
Notice that we have $D_j$ concentrate around zero. Conditioning on the history, $D_1 + D_2 + D_3$ follows a Gaussian distribution as
%\todorw{Below is just one event. If is is a series, introduce the range of subscripts.}
\begin{equation*}
    D_1 + D_2 + D_3 \, | \, \his_{1, T} \, \sim \, N \left( 0, \, \sigma_{\omega}^2 \sum_{i = 1}^s \bigg[ \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big]^2 + \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big]^2 \Big] + s (\lambda^2 + \lambda \overline{R}_{1, s})^2  \right).
\end{equation*}
That is the numerator of the difference between $\overline{Y}_{1, s}$ and $\overline{R}_{1, s}^*$ is a zero mean normal distribution and its variance is $O(s)$. Note that the denominator is also order $s$, $\overline{Y}_{1, s} - \overline{R}_{1, s}^*$ will behave like a zero mean distribution with $O(s^{-1})$ variance, which will converge to zero in probability. 
% \begin{framed}
% \begin{equation*}
%     \begin{aligned}
%         \overline{Y}_{1, s} - \overline{R}_{1, s}^* \, | \, \his_{1, T} & = \frac{\lambda_1 s (s - \sum_{i = 1}^s \omega_i) + s \sum_{i = 1}^s R_{1, i} \omega_i - \sum_{j = 1}^s R_{1, j} \sum_{i = 1}^s \omega_i }{s \sum_{i = 1}^s \omega_{i}},
%     \end{aligned}
% \end{equation*}

% hence, $\overline{Y}_{1, s} - \overline{R}_{1, s}^* \, | \, \his_{1, T}$ may not be always positive. We need to define a series of good events such that 
% \begin{gather*}
%     G_{k, s} := \{\overline{Y}_{k, s} - \overline{R}_{k, s}^* \geq 0 \}, 
% \end{gather*}
% \end{framed}
Therefore, in non-asymptotic sense, there is also a high probability that $\overline{Y}_{1, s} - \overline{R}_{1, s}^* \, | \, \his_{1, T}$ is close to zero. We define a series of good events 
\begin{equation*}
    G_{k', s} := \bigg\{- C_3 \Delta_k \leq \overline{Y}_{k', s} - \overline{R}_{k', s}^* \leq C_3 \Delta_k \bigg\},
\end{equation*}
for some $C_3 > 0$. 
% \todorw{"The conditional probability outside" seems not a valid phrase.}
\todorw{Same suggestion that we should have shorter sentence with clearer logic. For example, the sentence below spans at least 13 lines. }
The probability of $G^c_{1, s}$ conditioned on the history $\his_{1, T}$ is 
\begin{equation*}
    \begin{aligned}
        \pr \big(G_{1, s}^{c}\, | \, \his_{1, T}\big) & = 2 \pr_{\omega, \omega', \omega''} \Bigg\{ (D_1 + D_2 + D_3) - C_3 (1 + 2 \lambda) \Delta_k \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] > 0 \Bigg\} \\
        & \leq 2 \exp \bigg\{ -\frac{C_3^2 (1 + 2 \lambda)^4 s^{2}}{2 \sigma_{\omega}^2 \left[2 s (\lambda^2 + 1) + s \lambda^2 + s \lambda^2 (\lambda + 1)^2 + s ( C_3^2 \Delta_k^2 + 2 C_3 \Delta_k ) (1 + 2 \lambda)^2 (1 + 2 \lambda^2) \right]} \bigg\} \\
        & \leq 2 \exp \bigg\{ - s \cdot \frac{C_3^2(1 + 2 \lambda)^4}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + ( C_3^2 \Delta_k^2 + 2 C_3 \Delta_k ) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\right]}\bigg\}.
    \end{aligned}
\end{equation*}
Here the first inequality we use the fact that 
%\todorw{
%1. Conditioned on the history. Otherwise, incorrect
%2. The two parts are correlated?
%3. Do not skip. How do we achieve line 2? Writing down the reasons will help avoid mistakes.
%}
\begin{equation*}
    \begin{aligned}
        & (D_1 + D_2 + D_3) - C_3 (1 + 2 \lambda) \Delta_k \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] \, \big| \, \his_{1, T}\\
        & =  \sum_{i = 1}^s \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s} - C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i + \sum_{i = 1}^s \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda - \lambda C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i'  \\
        & ~~~~~~~~~~~~~~~~~~ + \sum_{i = 1}^s \big[ - (\lambda^2 + \lambda \overline{R}_{1, s}) - \lambda C_3 (1 + 2\lambda) \Delta_k \big] \omega_i'' \\
        & \sim N \Bigg( - C_3 (1 + 2 \lambda)^2 s,  \, \sigma_{\omega}^2 \sum_{i = 1}^s \bigg[ \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big]^2 + \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big]^2 \Big] \\
        & \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad + s \sigma_{\omega}^2 (\lambda^2 + \lambda \overline{R}_{1, s})^2 + s  \sigma_{\omega}^2 C_3^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\\
        & \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad + 2 s \lambda (\lambda - 1) (1 + 2 \lambda) C_3 \Delta_k \big[ 2 \overline{R}_{1, s} - 1\big]  \Bigg) \\
        & =: N \big( - C_3 (1 + 2 \lambda)^2 s, \, \sigma_{\omega}^2 \Sigma_{G_{1, s}} \big)
    \end{aligned}
\end{equation*}
\todorw{I do not recommend using $:=$ to define stuffs.}
where we use the fact that the cross term is
\begin{equation*}
    \begin{aligned}
        & - \sum_{i = 1}^s \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big] C_3 (1 + 2 \lambda) \Delta_k - \sum_{i = 1}^s\big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big] \lambda C_3 (1 + 2 \lambda) \Delta_k \\
        & ~~~~~~~~~~~~ + \sum_{i = 1}^s (\lambda^2 + \lambda \overline{R}_{1, s}) \lambda C_3 (1 + 2\lambda) \Delta_k \\
        & = \lambda C_3 (1 + 2 \lambda) \Delta_k \sum_{i = 1}^s \Big( \big[ \lambda^2 + \lambda \overline{R}_{1, s}\big] - \big[ \lambda (1 + \lambda) - \lambda \overline{R}_{1, s}\big] - \big[ 2 R_{1, i} - 1 \big]\Big) \\
        & = s \lambda (\lambda - 1) (1 + 2 \lambda) C_3 \Delta_k \big[ 2 \overline{R}_{1, s} - 1\big].
    \end{aligned}
\end{equation*}
Indeed, $\Sigma_{G_{1, s}} := \Sigma_{G_{1, s}, 1} + \Sigma_{G_{1, s}, 2} + \Sigma_{G_{1, s}, 3} + \Sigma_{G_{1, s}, 4} + \Sigma_{G_{1, s}, 5}$ can be furthermore bounded by four positive terms
\begin{equation*}
    \Sigma_{G_{1, s}, 1} := \sum_{i = 1}^s  \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big]^2 \leq 2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 2 \lambda^2 \sum_{i = 1}^s (2 R_{1, i} - 1)^2 \leq 2 s (\lambda^2 + 1),
\end{equation*}
\begin{equation*}
    \Sigma_{G_{1, s}, 2} := \sum_{i = 1}^s  \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big]^2 = \sum_{i = 1}^s \lambda^2 (1 - \overline{R}_{1, s})^2 = s\lambda^2 (1 - \overline{R}_{1, s})^2 \leq s \lambda^2,
\end{equation*}
\begin{equation*}
    \Sigma_{G_{1, s}, 3} := s (\lambda^2 + \lambda \overline{R}_{1, s})^2 \leq s \lambda^2 (\lambda + 1)^2, \qquad \Sigma_{G_{1, s}, 4} := s C_3^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)
\end{equation*}
and a potential negative term
\begin{equation*}
    \Sigma_{G_{1, s}, 5} := 2 s \lambda (\lambda - 1) (1 + 2 \lambda) C_3 \Delta_k \big[ 2 \overline{R}_{1, s} - 1\big] \in \big[ - 2 s |\lambda^2 - \lambda| (1 + 2 \lambda) C_3 \Delta_k, \, 2s |\lambda^2 - \lambda| (1 + 2 \lambda) C_3 \Delta_k \big].
\end{equation*}
\todohw{Adding the cross-term will case the extra term $\Delta_k$ to the denominator.}

by the fact $R_{k, i} \in [0, 1]$, which implies
\begin{equation*}
    \begin{aligned}
        0 < \Sigma_{G_{1, s}} & \leq 2 s (\lambda^2 + 1) + s \lambda^2 + s \lambda^2 (\lambda + 1)^2 + s C_3^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) +  2s |\lambda^2 - \lambda| (1 + 2 \lambda) C_3 \Delta_k \\
        & \leq 2 s (\lambda^2 + 1) + s \lambda^2 + s \lambda^2 (\lambda + 1)^2 + s  (1 + 2 \lambda)^2 (1 + 2 \lambda^2) +  s (1 + 2 \lambda)^2 (1 + 2 \lambda^2) \big( C_3^2 \Delta_k^2 + 2 C_3 \Delta_k \big).
    \end{aligned}
\end{equation*}
as $|\lambda^2 - \lambda|  \leq 1 + 2 \lambda^2$.

\todorw{Another general comment. I find a lot of `that` are missing. We can omit it in limited cases. Even in those cases, as your sentences are typically long, omitting  the conjunctions will make the sentence hard to read. 
I suggest to keep all of them. }
Thus, if we take 
\begin{equation*}
    \begin{aligned}
        s = s_{a, 1, 2} & := \bigg[ \frac{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + ( C_3^2 \Delta_k^2 + 2 C_3 \Delta_k ) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\right]}{C_3^2(1 + 2 \lambda)^4} \bigg] \cdot \big[ \log 2 + 2 \log T\big] \\
        & \leq \frac{6 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + ( C_3^2 \Delta_k^2 + 2 C_3 \Delta_k ) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\right]}{C_3^2(1 + 2 \lambda)^4} \log T \\
        & =: H_1 (\lambda, \sigma_{\omega}^2, C_3, \Delta_k) \log T
    \end{aligned}
\end{equation*}
for any $T \geq 2$, then 
\begin{equation*}
    a_{k, 1, 2} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) 1(G_{1, s}^c)\Big] \leq T \pr (G_{1, s}^c) \leq T^{-1}.
\end{equation*}

%{\color{red}
%\begin{remark}
    %In this step, we can generally take that $\alpha \equiv 0$, then $s_{a, 1, 2}$ has general rate $\log T$. However, take $\alpha \equiv 0$ will give that $G_{k', s}$ only implies $\overline{Y}_{1, s} $ and $\overline{R}_{1, s}^*$ will close enough but will not imply the gap will more and more close when the round increase. But whether we can directly take $\alpha$ as zero may need to study later.
%\end{remark}
%}

\todorw{Same comment as for the last section. Always make sure the logic is complete. The goal is to bound $s_{a,1,2}$, the conclude with it by stating the result clearly. Do not leave the step to readers. }



\todorw{We need to understand why we only need the difference to be bounded. }

\begin{remark}
    The \red{boundedness} assumption is again not essential here, since we only require
    \todorw{State, explicitly, where above we need this inequality. (It is very difficult to find why we `only require` since it is hard to find the corresponding part from derivations above.)}
    \begin{equation*}
        \begin{aligned}
            & \log \E \exp \left\{ - \frac{C_3 (1 + 2\lambda)^2 s}{\sigma_{\omega}^2 \Sigma_{G_{1, s}}}\right\} \\
            = & \log \E \exp \left\{ - \frac{\operatorname{const} \cdot s}{\operatorname{const} + \sum_{i = 1}^s (R_{k, i} - \overline{R}_{k, s})^2 + \sum_{i = 1}^s (\text{upper bound of } \mu_k - R_{k, i})^2 + \sum_{i = 1}^s (R_{k, i} - \text{lower bound of } \mu_k )^2}\right\} \lesssim - s
        \end{aligned}
    \end{equation*}
    to ensure that take $s_{a, 1, 2}$ as order $\log T$ to achieve $a_{k, 1, 2} \leq T^{-1}$. A normal distribution $R_{k, s}$ will lead $\sum_{i = 1}^s (R_{k, i} - \overline{R}_{k, s})^2$ and $\sum_{i = 1}^s R_{k, i}^2$ are (non-centerized) chi-square distributed. They can achieve $\pr (G_{1, s}) \leq T^{-1}$ with $s$ at most $\log T$.
\end{remark}


% \begin{framed}
% for some fixed $N$ free of $s$, then
% \begin{equation*}
%     \begin{aligned}
%         \pr \big(G_{1, s}^{c}\, | \, \his_{1, T}\big) & = \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \bigg[ \lambda_1 s + \sum_{j = 1}^s R_{1, j} - s R_{1,i} \bigg] \omega_i  > \lambda_1 s^2 \Bigg\}\\
%         & \leq \exp \bigg\{ -\frac{1}{2} \frac{\lambda_1^2 s^4}{\|\lambda_1 s + \sum_{j = 1}^s R_{1, j} - s R_{1,i} \|_2^2 } \wedge \frac{\lambda_1 s^2}{\max_{i \in [s]}[\lambda_1 s + \sum_{j = 1}^s R_{1, j} - s R_{1,i} ]}\bigg\} \\
%         & \leq \exp \bigg\{ -\frac{1}{2} \frac{\lambda_1^2 s^4}{s(\lambda_1 s + m_{1, s})^2} \wedge \frac{\lambda_1 s^2}{\lambda_1 s + m_{1, s}}\bigg\} \leq \exp \bigg\{ - \frac{s}{2} \frac{\lambda_1^2}{(\lambda_1 + b)^2} \wedge \frac{\lambda_1}{\lambda_1 + b} \bigg\}
%     \end{aligned}
% \end{equation*}
% where $m_{1, s} = \sum_{i = 1}^s R_{1, i} \in [as, bs]$. For any $\eta > 1$, by taking 
% \begin{equation*}
%      s_{a, 1, 2} = 2 \eta \left( \frac{\lambda_1 + b}{\lambda_1}\right)^2 \log T 
% \end{equation*}
% then for any $s \geq s_{a, 1, 2}$
% \begin{equation*}
%     a_{k, 1, 2} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) 1(G_{1, s}^c)\Big] \leq T^{- \eta + 1}.
% \end{equation*}
% \end{framed}


\paragraph{Dealing with $s_{a, 1, 1}$}

Now, what remains to do is to bound $s_{a, 1, 1} = \max \{ s: a_{k, 1, 1} \geq T^{-1}\}$ with order $
\log T$ where
\begin{equation*}
    a_{k, 1, 1} = a_{k, 1} - a_{k, 1, 2} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) 1(G_{1, s})\Big].
\end{equation*}
% Note that $\{N_{1, s}\left(\tau_{k}\right)<T^{-1}\} \supseteq \{\left[1-Q_{1, s}\left(\tau_{k}\right)\right]<T^{-2}\}$, what we need to deal with is finding $s \geq s_{a,1,1}$ such that $\big\{[1-Q_{1,s}(\tau_{k})]<T^{-2}\big\}$ on the event $A_{1, s} \cap G_{1, s}$. 

It maybe a little bit involved to tackle with $a_{k, 1, 1}$ directly as we said previously, $a_{k, 1, 1}$ defined on the good events, it will behave largely like $\E \big[ N_{1, s} (\tau_k) \wedge T \big]$. 
\todorw{The above is not a correct sentence. Same for the above. Again, if it is complex, one suggestion is to always make the sentence shorter, and then make sure the logic between sentences is clear. }
Hence, we cannot use something like $a_{k, 1, 1} \leq T \pr (\text{Event}_s) \leq T \cdot T^{-2} = T^{-2} $, other technique need to introduced: transform the expectation to probability that connected with the good events $A_{1, s}$ and $G_{1, s}$.

Note that, we have
\begin{equation*}
    \begin{aligned}
        \{N_{1, s}(\tau_{k})<T^{-1}\} & \supseteq \{N_{1, s}(\tau_{k}) < (T^{2}-1)^{-1}\} = \big\{Q_{1, s}\left(\tau_{k}\right)^{-1}<1+\left(T^{2}-1\right)^{-1}\big\} \\
        &=\big\{Q_{1, s}(\tau_{k})^{-1} < (1-T^{-2})^{-1}\big\} = \big\{\left[1-Q_{1, s}(\tau_{k})\right]<T^{-2}\big\},
    \end{aligned}
\end{equation*}
and $a_{k, s} \leq \E \big[ N_{1, s} (\tau_k) 1(A_{1, s} \cap G_{1, s}) \big]$. As a result, it is sufficient to  find $s \geq s_{a,1,1}$ such that $\big\{[1-Q_{1,s}(\tau_{k})]<T^{-2}\big\}$ on the event $\{A_{1, s} \cap G_{1, s}\}$. 


\todorw{Everything below belongs to ONE paragraph. It makes the paper very hard to read and affect the logic. }

Note that
\begin{equation*}
    \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, T} \big)  1(A_{1, s}) 1(G_{1, s})
\end{equation*}
with $\Gamma_1 := \Gamma_1(\tau_1) = \tau_1 - \overline{R}_{1, s}^*$ serving as a measurement to balance the difference between $\overline{Y}_{1, s}$ and $\overline{R}_{1,s}^*$. It is not hard to see $\Gamma$ should be negative with a moderate value. Fortunately, on $G_{1, s}$, we have the gap between $\overline{Y}_{1, s}$ and $\overline{R}_{1, s}^*$ not to large. For any fixed $\Gamma_1$ has been chosen,
\begin{equation*}
    \begin{aligned}
        & D_1 + D_2 + D_3 - \Gamma_1 (1 + 2 \lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg]  \\
        & \qquad \sim \, N \Bigg( - \Gamma_1 (1 + 2 \lambda)^2 s, \, \sigma_{\omega}^2 \sum_{i = 1}^s \bigg[ \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s}\big]^2 + \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda \big]^2 \Big] \\
        &  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + s \sigma_{\omega}^2 (\lambda^2 + \lambda \overline{R}_{1, s})^2 + s \sigma_{\omega}^2 \Gamma_1^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\Bigg),
    \end{aligned}
\end{equation*}
will give the inequality
\begin{equation*}
    \begin{aligned}
        & \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) \\
        = & \, \pr_{\omega, \omega', \omega''} \bigg( D_1 + D_2 + D_3 - \Gamma_1 (1 + 2 \lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg]  \leq 0\bigg) 1 (A_{1, s} \cap G_{1, s}) \\
        \leq & \exp \left\{ - \frac{(- \Gamma_1)^2 (1 + 2 \lambda)^4 s^2}{2 \Big[ \sigma_{\omega}^2 \big( 2 s (\lambda^2 + 1)  + s \lambda^2 \big) + s \lambda^2 (\lambda + 1)^2 + s \sigma_{\omega}^2 ( \Gamma_1^2 + 2 \Gamma_1) (1 + 2 \lambda)^2 (1 + 2 \lambda^2) \Big]}\right\} 1 (A_{1, s} \cap G_{1, s}) \\
        = & \exp \left\{ -\frac{(- \Gamma_1)^2 (1 + 2 \lambda)^4 s}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + ( \Gamma_1^2 + 2 \Gamma_1) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)  \right]}\right\} 1 (A_{1, s} \cap G_{1, s}).
    \end{aligned}
\end{equation*}
where we use the same technique as in handling $s_{a, 2, 2}$ to deal with the variance of $D_1 + D_2 + D_3 - \Gamma_1 (1 + 2 \lambda) \left[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\right]$.
%\todorw{The below is too long, and not a grammarly correct sentence.}
\todorw{Another general suggestion. When you have a system of equations, please let the readers know how you jump from one to the next, unless it is trivial. Equations should ALWAYS be part of a readable paragraph. }

Recast that, on $A_{1, s} \, \cap \, G_{1, s}$, we have
\begin{equation*}
    A_{1, s} = \bigg\{ \overline{R}_{1, s}^* - \frac{\mu_1 + \lambda}{1 + 2\lambda} > - C_1 \Delta_k \bigg\} = \bigg\{ \Gamma_1 < C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} + \tau_1 \bigg\} 
\end{equation*}
and
\begin{equation*}
    \begin{aligned}
        G_{1, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_1 -C_3 \Delta_k \leq \overline{Y}_{1, s} + \Gamma_1 \leq \tau_1 + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_1 - C_3 \Delta_k - \overline{Y}_{1, s} \leq \Gamma_1 \leq \tau_1 + C_3 \Delta_k - \overline{Y}_{1, s}\big\} \\
        & \subseteq \big\{ \tau_1 - 2 C_3 \Delta_k - \overline{R}_{1, s}^* \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \overline{R}_{1, s}^* \big\} \\
        & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2 \lambda}\bigg\}
    \end{aligned}
\end{equation*}
then
\begin{equation*}
    \begin{aligned}
        A_{1, s} \, \cap \, G_{1, s} & = \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 < \tau_1 + C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} \bigg\} \\
        & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\} \\
        (\text{if } C_1 \geq 2 C_3 )& \subseteq \bigg\{ \tau_1 -  C_1 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\}
    \end{aligned}
\end{equation*}
and hence we derive the requirement that $C_1 \Delta_k - \mu_1 / 2 + \tau_1 < 0$, i.e. $\tau_1 < \mu_1  / 2 - C_1 \Delta_k$, which will give
\begin{equation*}
    \begin{aligned}
        & \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) \\
        \leq & \exp \left\{ -\frac{(- \Gamma_1)^2 (1 + 2 \lambda)^4 s}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + (- \Gamma_1)^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)  \right]}\right\} 1 (A_{1, s} \cap G_{1, s}) \\
        (\text{by taking } \tau_k = \mu_1 / 2 - 2 C_1 \Delta_k)\leq & \exp \left\{ - \frac{C_1^2 \Delta_k^2 (1 + 2 \lambda)^4 s}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + C_1^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)  \right]}\right\} 1 (A_{1, s} \cap G_{1, s})
    \end{aligned}
\end{equation*}
by 
\begin{equation*}
    C_1 \Delta_k = \frac{\mu_1 }{2} - \tau_1 - C_1 \Delta_k <  (- \Gamma_1) \leq 1 + C_1 \Delta_k  - \tau_k = 1 - \frac{\mu_1}{2} + 3 C_1 \Delta_k < 4
\end{equation*}
and the fact that the function
\begin{equation*}
    \begin{aligned}
        f_1(x) & := \frac{ x^2 (1 + 2 \lambda)^4}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + (x^2 + 2x) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)  \right]} \\
        & \geq  \frac{ x^2 (1 + 2 \lambda)^4}{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + 3 x^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) / 2 \right]} =: f_2(x), \qquad 0 \leq x \leq 4,
    \end{aligned}
\end{equation*}
with $f_2(x)$ increasing on $[0, + \infty)$. By letting 
\begin{equation*}
    \begin{aligned}
        s = s_{a, 1, 1} :=  \frac{4 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + 3 C_1^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) / 2  \right]}{C_1^2 \Delta_k^2 (1 + 2 \lambda)^4} \log T =: H_2 (\lambda, \sigma_{\omega}^2, C_1, \Delta_k) \cdot \log T
    \end{aligned}
\end{equation*}
then
\begin{equation*}
    a_{k, 1, 1} := \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1 (A_{1, s}) 1(G_{1, s})\Big] \leq T^{-1}.
\end{equation*}
Combining these results, we know if we take
\begin{equation*}
    \begin{aligned}
        s \geq \max \{ s_{a, 2}, s_{a, 1, 1}, s_{a, 1, 2}\} & = \max \left\{ \frac{1}{C_1^2 (1 + 2\lambda)^2 \Delta_k^2},\,  H_1 (\lambda, \sigma_{\omega}^2, C_3, \Delta_k), \, H_2 (\lambda, \sigma_{\omega}^2, C_1, \Delta_k)  \right\} \log T \\
        & =: H' (\lambda, \sigma_{\omega}^2, C_1, C_3, \Delta_k) \cdot \log T
    \end{aligned}
\end{equation*}
then we have orcale that
\begin{equation*}
    \begin{aligned}
        a_k & \leq 3 + \left[\exp \bigg\{\frac{6(2 \lambda + 1)^2}{2\sigma_{\omega}^2 \lambda^2 ((\lambda + 1 )^2 + \lambda^2 )}\bigg\} + \big[ 1 - \Phi(\sqrt{2\pi} )\big]^{-1} \right]  H'(\lambda, \sigma_{\omega}^2, C_1, C_3, \Delta_k)  \log T \\
        & =: 3 + H(\lambda, \sigma_{\omega}^2, C_1, C_3, \Delta_k)  \log T.
    \end{aligned}
\end{equation*}
It is worthy to recall that the above inequality is obtained by taking
\begin{equation}\label{condition.2}
    \tau_k = \mu_1 / 2 - 2 C_1 \Delta_k
\end{equation}
with 
\begin{equation}\label{condition.3}
    C_1 \geq 2 C_3.
\end{equation}

%{\color{red}{
%\begin{remark}
    %From these steps, we know that, to bound $a_k$ with rate $\log T$, one only require the tuning parameter $\lambda > 0$. This situation may be due to that the denominator contains $1 + 2 \lambda$.
%\end{remark}
%}}

%with the derivative as
%\begin{equation*}
    %f'(x) := \frac{(1 + 2\lambda)^2}{2 \sigma_{\omega}^2} \cdot \frac{2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) - (1 + 2 \lambda)^2 (1 + 2 \lambda^2) x^2}{\left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + x^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2)  \right]^2}, \qquad x > 0
%\end{equation*}
%which is decreasing in the interval
%\begin{equation*}
    %\left[0, \, \frac{2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2)}{(1 + 2 \lambda)^2 (1 + 2 \lambda^2) } \right].
%\end{equation*}
\iffalse
{\color{blue}
If we note that $(- \Gamma_1) = \overline{R}_{1, s}^* - \tau_1$ lies in the interval $\left[ - \tau_1, \frac{1 + \lambda}{1 + 2\lambda} - \tau_1 \right]$, which will be bounded by $\frac{1 + \lambda}{1 + 2\lambda}$ if $\tau_1 \geq 0$, and in this case, put 
\begin{equation*}
     \frac{2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2)}{(1 + 2 \lambda)^2 (1 + 2 \lambda^2) } \leq \frac{1 + \lambda}{1 + 2\lambda}
\end{equation*}
we get that $\lambda^4 - 8 \lambda^2 + 3 \lambda - 1 \geq 0$. We get a possible range for $\lambda$ is $\lambda \geq 2 \sqrt{2}$. Compared with the existent results:
\begin{itemize}
    \item In \cite{kveton2019garbage}, the pseudo rewards $a \in (0, 1)$ should larger than $1 / \sqrt{2}$ due to they need to control the anti concentration of Bernoulli distribution, i.e. control $ \E \big[ \pr^{-1} (U_{1, s} \geq (\mu_1 + s) \, | \, V_{1, s})\big]$;
    
    \item Similarly in \cite{kveton2019perturbed}, the condition $a > 2$ for tuning parameter is same as that in \cite{kveton2019garbage} to ensure the anti concentration having a valid upper bound;
    
    \item The tuning parameter of the pseudo residual $\sigma_a > 3 / 2$ in \cite{wang2020residual} is also essential by again controlling  the anti concentration;
\end{itemize}
Hence, the condition for the tuning parameter is not equivalent with the existent work (we use the condition to bound $a_{k, 1, 1}$ instead of $a_{k, s}$.). 
}
\fi


% \begin{framed}
% Denote
% \begin{equation*}
%     \Delta_1^* := \tau_1 - \overline{R}_{1, s}^*,
% \end{equation*}
% if $\Delta_1^* \leq 0$, i.e. $\lambda_1 \geq \tau_1$ (recall $\tau_k \leq \mu_1$), then
% \begin{equation*}
%     \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Delta_1^* \, | \, \his_{1, T} \big)  1(A_{1, s}) 1(G_{1, s}) = 0 < T^{-2};
% \end{equation*}
% if $\Delta_1^* \geq 0$, in this case, $\lambda_1 \leq \tau_1 \leq \mu_1$, then
% \begin{equation*}
%     \begin{aligned}
%         & \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Delta_1^* \, | \, \his_{1, T} \big)  1(A_{1, s}) 1(G_{1, s}) \\
%         = \, & \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \bigg[ (\lambda_1 + \Delta_1^* - R_{1,i}) s + \sum_{j = 1}^s R_{1, j}\bigg] w_i \geq \lambda_1 s^2 \Bigg\} 1 (A_{1, s}) 1(G_{1, s}) \\
%         \leq \, & \exp \bigg\{ -\frac{1}{2} \frac{\lambda_1^2 s^4}{\|(\lambda_1 + \Delta_1^* - R_{1,i}) s + \sum_{j = 1}^s R_{1, j}\|_2^2 } \wedge \frac{\lambda_1 s^2}{\max_{i \in [s]}[(\lambda_1 + \Delta_1^* - R_{1,i}) s + \sum_{j = 1}^s R_{1, j}]}\bigg\} 1 (A_{1, s} \cap G_{1, s}) \\
%         \leq \, & \exp \bigg\{ -\frac{s}{2} \frac{\lambda_1^2}{(\lambda_1 + b + \Delta_1^*)^2} \wedge \frac{\lambda_1}{\lambda_1 + b + \Delta_1^*}\bigg\} 1 (A_{1, s} \cap G_{1, s}).
%     \end{aligned}
% \end{equation*}
% Recast that, on $A_{1, s}$, we have
% \begin{equation*}
%     A_{1, s} = \big\{ \overline{R}_{1, s}^* - \mu_1 > - C_1 \Delta_k \big\} = \big\{ \Delta_1^* < C_1 \Delta_k - \mu_1 + \tau_1 \big\}
% \end{equation*}
% and hence
% \begin{equation*}
%     \begin{aligned}
%         \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) & = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Delta_1^* \, | \, \his_{1, T} \big)  1(A_{1, s}) 1(G_{1, s}) \\
%         & \leq \exp \bigg\{ -\frac{s}{2} \frac{\lambda_1^2}{(C_1 \Delta_k - \mu_1 + \tau_1)^2} \wedge \frac{\lambda_1}{C_1 \Delta_k - \mu_1 + \tau_1}\bigg\} 1 (A_{1, s} \cap G_{1, s}) \\
%         (\text{letting } \tau_1 = \mu_1) & \leq  \exp \bigg\{ -\frac{s}{2} \frac{\lambda_1^2}{(C_1 \Delta_k )^2} \wedge \frac{\lambda_1}{C_1 \Delta_k}\bigg\} \leq T^{-\eta}
%     \end{aligned}
% \end{equation*}
% with letting $s \geq s_{a, 1, 1} := 2 \eta \log T \left[ ( \lambda_1^{-1} C_1 \Delta_k)^2 \vee ( \lambda_1^{-1} C_1 \Delta_k) \right]$.
% \vspace{2ex}

% Now let $\eta = 2$, conclude from the Section 2.2.1 and 2.2.2, we know that as long as 
% \begin{equation*}
%     \begin{aligned}
%         s \geq \max \{ s_{a, 2}, s_{a, 1, 2}, s_{a, 1, 1} \} & =  \max \left\{ \frac{(b - a)^2}{(\lambda_1 + C_1 \Delta_k)^2}, \, 4 \left( \frac{\lambda_1 + b}{\lambda_1}\right)^2, \, 4 ( \lambda_1^{-1} C_1 \Delta_k)^2 \vee ( \lambda_1^{-1} C_1 \Delta_k) \right\} \cdot \log T \\
%         & =: H_1(\lambda_1, C_1, \Delta_k) \cdot \log T
%     \end{aligned} 
% \end{equation*}
% we must have 
% \begin{equation*}
%     \begin{aligned}
%         a_{k} & \leq H_1(\lambda_1, C_1, \Delta_k) \log T + 3 \big[ T - H_1(\lambda_1, C_1, \Delta_k) \log T \big] T^{-1} \\
%         & \leq 3 + H_1(\lambda_1, C_1, \Delta_k) \log T = 3 + H_1(\lambda_1, C_1, \Delta_k) \log T.
%     \end{aligned}
% \end{equation*}
% \end{framed}

\subsection{Second Step: Bounding $b_k$}

The second step is bounding $b_k = \pr \big( Q_{k, s} (\tau_k) > T^{-1}\big) + 1$. Recall in the diagram, what we only to do is bounding $s_b = \max \{ s: b_{k, s} \geq T^{-1}\}$ as order $\log T$ (this is by $b_{k, s}$ is naturally bounded by one).


We also need to decompose $b_k$ as $b_k = b_{k, 1, 1} + b_{k, 1, 2} + b_{k, 2} + 1$ with
\begin{gather*}
    b_{k, 1, 1} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A'_{k, s}) 1(G_{k, s})\big], \\
    b_{k, 1, 2} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A'_{k, s}) 1(G_{k, s}^c)\big], \\
    b_{k, 2} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A_{k, s}^{\prime c} )\big].
\end{gather*}
with $A'_{k, s} = A_{k, s}$ using the second definition, then $\pr (A^{\prime c}_{k, s}) $ when $s \geq \frac{1}{2}s_{a, 2}'$ with $C_1$ replaced by $C_2$. Then we must have $b_{k, 1, 2} \vee b_{k, 2} \leq T^{-2} < T^{-1}$ as long as $s \geq s'_{a, 2}  / 2 \vee s_{a,1, 2}$.
%\begin{framed}
%\begin{equation*}
    %\begin{aligned}
        %\pr (A_{k, s}^c) & = \pr \bigg\{ \sum_{\ell = 1}^s (R_{k, \ell} - \mu_k) \geq s C_2 \Delta_k - \lambda_k s \mu_k\bigg\} \leq \exp \bigg\{ -2 \frac{(C_2 \Delta_k - b \lambda_k )^2 s }{(b - a)^2}\bigg\}.
    %\end{aligned}
%\end{equation*}
%\begin{remark}
    %The above inequality confirms why $\lambda_1$ cannot be too large since we need that $\lambda_k < C_2 \Delta_1$.
%\end{remark}
%Hence, define a new $s_{a, 2}' = \frac{(b - a)^2 \log T}{2 (C_2 \Delta_k - \lambda_k)^2}$, we must have $b_{k, 1, 2} \vee b_{k, 2} \leq T^{-2} < T^{-1}$ as long as $s \geq s'_{a, 2} \vee s_{a,1, 2}$.
%\end{framed}
It remains to bound $b_{k, 1, 1}$. Indeed, we note that on $A’_{k, s}$, we have
\begin{equation*}
    A'_{k, s} = \bigg\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} < C_2 \Delta_k \bigg\} = \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \bigg\}.
\end{equation*}
Again, on the event 
\begin{equation*}
    \begin{aligned}
        G_{k, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{k, s} - \overline{R}_{k, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_k -C_3 \Delta_k \leq \overline{Y}_{k, s} + \Gamma_k \leq \tau_k + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_k - 2 C_3 \Delta_k - \overline{R}_{k, s}^* \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \overline{R}_{k, s}^* \big\} \\
        & \subseteq \bigg\{ \tau_k - 2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2\lambda} \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2\lambda}\bigg\}
    \end{aligned}
\end{equation*}
we can conclude that 
\begin{equation*}
    \begin{aligned}
        A'_{k, s} \, \cap \, G_{k, s} & \subseteq  \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \leq\tau_k + C_2 \Delta_k - \frac{\lambda}{1 + 2\lambda} \bigg\} \\
        & \subseteq \bigg\{ \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2}  < \Gamma_k < \tau_k + C_2 \Delta_k \bigg\}
    \end{aligned}
\end{equation*}
% It is worthy to recall that the construction of $s_{a, 1, 2}$ is free of any $\tau_k$, hence this argument is valid. 
if
\begin{equation}\label{condition.4}
    2 C_3 \geq C_2
\end{equation}
Under this establishment, we need $\tau_k - C_2 \Delta_k - \frac{\mu_k }{2} \leq 0$, then we can take
\begin{equation}\label{condition.5}
    \tau_k = 2 C_2 \Delta_k + \mu_k / 2
\end{equation}
and we will obtain that
\begin{equation*}
    C_2 \Delta_k = \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2} < \Gamma_k < \tau_k + C_2 \Delta_k = 3 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{7}{2} < 4,
\end{equation*}
then we will have
\begin{equation*}
    \begin{aligned}
         Q_{k, s} (\tau_k) 1(A'_{k, s}) 1(G_{k, s}) & = \pr \big(\overline{Y}_{k, s} - \overline{R}_{k, s}^* > \Gamma_k \, | \, \his_{k, T} \big) 1(A'_{k, s}) 1(G_{k, s}) \\
         & = \pr_{\omega, \omega^{\prime}, \omega^{\prime \prime}} \Bigg\{ (D_1 + D_2 + D_3) - \Gamma_k (1 + 2 \lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i^{\prime} + \lambda  \sum_{i = 1}^s \omega_i^{\prime \prime} \bigg] > 0 \Bigg\} 1(A'_{k, s}\cap G_{k, s}) \\
         & \leq 2 \exp \bigg\{ - \frac{\Gamma_k^{2} (1 + 2 \lambda)^4s }{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + (\Gamma_k^2 + 2 \Gamma_k) (1 + 2 \lambda)^2 (1 + 2 \lambda^2)\right]}\bigg\} 1(A'_{k, s}\cap G_{k, s}) \\
         & \leq 2 \exp \bigg\{ - \frac{\Gamma_k^{2} (1 + 2 \lambda)^4s }{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + 3\Gamma_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) / 2\right]}\bigg\} 1(A'_{k, s}\cap G_{k, s}) \\
         & \leq 2 \exp \bigg\{ - \frac{C_2^2 \Delta_k^2 (1 + 2 \lambda)^4s }{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + 3 C_2^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) /  2\right]}\bigg\} \leq T^{-1}
    \end{aligned}
\end{equation*}
by letting 
\begin{equation*}
    s = s_{a, 1, 1}^{\prime} = \frac{2 \sigma_{\omega}^2 \left[ 2 + 3 \lambda^2 (4 + 2 \lambda + \lambda^2) + 3 C_2^2 \Delta_k^2 (1 + 2 \lambda)^2 (1 + 2 \lambda^2) / 2 \right]}{C_2^2 \Delta_k^2 (1 + 2 \lambda)^4} \log T =: G_1 (\lambda, \sigma_{\omega}^2, C_2, \Delta_k) \cdot \log T.
\end{equation*}

As a consequence, as long as we have
\begin{equation*}
    \begin{aligned}
        s \geq \max\{ s_{a, 2}^{\prime} / 2, s_{a, 1, 2},  s_{a, 1, 1}^{\prime}\} & = \max \left\{ \frac{1}{2 C_2^2 (1 + 2\lambda)^2 \Delta_k^2},\,  H_1 (\lambda, \sigma_{\omega}^2, C_3, \Delta_k), \, G_1 (\lambda, \sigma_{\omega}^2, C_2, \Delta_k)  \right\} \log T \\
        & =: G(\lambda, \sigma_{\omega}^2, C_2, C_3, \Delta_k) \cdot \log T,
    \end{aligned}
\end{equation*}
%\todorw{What does oracle means here?}
then the inequality holds for 
\begin{equation*}
    b_k \leq 4 + G(\lambda, \sigma_{\omega}^2, C_2, C_3, \Delta_k) \cdot \log T.
\end{equation*}
%\todorw{Below is another example. Is it one, two, or three sentence(s)? Conjunctions and punctuations are missing. }

Finally, we combine the restrictions (\ref{condition.1}), (\ref{condition.2}), (\ref{condition.3}), (\ref{condition.4}), and (\ref{condition.5}), then we get that $C_1, C_2, C_3 > 0$ should satisfy the following system of equations
\begin{equation*}
    \left\{ \begin{array}{l}
         \frac{\mu_1}{2} - 2 C_1 \Delta_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
         2 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
        \tau_k - \frac{\mu_1}{2} - C_1 \Delta_k  \leq \tau_k + C_2\Delta_k - \frac{\mu_k }{2} \\
        C_1 \geq 2C_3 \\
        2 C_3 \geq C_2 \\
        \frac{\mu_1}{2} - 2 C_1 \Delta_k = 2 C_2 \Delta_k + \frac{\mu_k}{2}
    \end{array}\right.
\end{equation*}
thus, we only have
\begin{equation*}
    C_1 = C_2 = \frac{1}{8}, \qquad C_3 = \frac{1}{16},
\end{equation*}
is the unique solution for the above equations.
\todorw{The following is incomplete. Only the one who writes the proof knows why it is done. Either remind the readers of the decomposition, or, combining all result so far until we really reach the final conclusion. Do not skip. }
\todohw{I have added some details, maybe more details can be added if others still cannot understand.}
up to now, we get Theorem \ref{thm.MAB}.

% \todorw{Taken $\sigma_{\omega}^2 = 1$ ? Isn't it a tuning parameter?}



% \begin{framed}
% Under this establishment,
% \begin{equation*}
%     \begin{aligned}
%         Q_{k, s} (\tau_k) 1(A_{k, s}) 1(G_{k, s}) & = \pr \big(\overline{Y}_{k, s} - \overline{R}_{k, s}^* > \Delta_k^{*} \, | \, \his_{k, T} \big) 1(A_{k, s}) 1(G_{k, s}) \\
%         & = \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \bigg[ (\lambda_k + \Delta_k^{*} - R_{k,i}) s + \sum_{j = 1}^s R_{k, j}\bigg] w_i < \lambda_k s^2 \Bigg\} 1 (A_{k, s}) 1(G_{k, s}) \\
%         & \leq \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \bigg[ (\lambda_k + \tau_k - C_2 \Delta_k - \mu_k - R_{k,i}) s + \sum_{j = 1}^s R_{k, j}\bigg] w_i < \lambda_k s^2 \Bigg\} \\
%         & \leq \exp \bigg\{ - \frac{(\lambda_k s^2 + bs^2)^2}{2 s \cdot (2 \lambda_k s^2 + bs^2) + 2 (2 \lambda_k s^2 + bs^2)}\bigg\} \leq \exp \bigg\{ - \frac{(\lambda_k + b)s^2}{8s}\bigg\} = \exp \bigg\{ - \frac{(\lambda_k + b)s}{8}\bigg\}
%     \end{aligned}
% \end{equation*}
% is less than $T^{-1}$ when $s_{a, 1, 1}^{\prime} \geq \frac{8 \log T}{(\lambda_k + b)}$ by the fact that $\E w_i = 1$ with 
% \begin{equation*}
%     \begin{aligned}
%         \sum_{i = 1}^s \bigg[ (\lambda_k + \tau_k - C_2 \Delta_k - \mu_k - R_{k,i}) s + \sum_{j = 1}^s R_{k, j}\bigg] \leq 2 \lambda_k s^2 + bs^2
%     \end{aligned}
% \end{equation*}
% by letting $\tau_k = \lambda_k + C_2 \Delta_k + \mu_k + b$ and the standard expansional $\omega_i \, \sim \, \operatorname{sub \Gamma}(1, 1)$.

% As a result, as long as we have
% \begin{equation*}
%     \begin{aligned}
%         s \geq \max \{ s'_{a, 2}, s'_{a, 1, 2}, s'_{a, 1, 1} \} & =  \max \left\{ \frac{(b - a)^2 }{2 (C_2 \Delta_k - \lambda_k)^2}, \, 4 \left( \frac{\lambda_k + b}{\lambda_k}\right)^2, \, \frac{8}{(\lambda_k + b)}\right\} \cdot \log T \\
%         & =: H_2(\lambda_k, C_1, \Delta_k) \cdot \log T
%     \end{aligned} 
% \end{equation*}
% we must have 
% \begin{equation*}
%     \begin{aligned}
%         b_{k} & \leq H_2(\lambda_k, C_2, \Delta_k) \log T + 3 \big[ T - H_2(\lambda_k, C_2, \Delta_k) \log T \big] T^{-1} + 1 \\
%         & \leq 4 + H_2(\lambda_k, C_1, \Delta_k) \log T = 3 + H_2(\lambda_k, C_2, \Delta_k) \log T.
%     \end{aligned}
% \end{equation*}
% Finally, we let $C_1 = C_*$, $C_2 = C^*$, and $0 < \lambda_k < \Delta_k$. And we prove Theorem \ref{thm}.
% \end{framed}

\newpage

\section{Discussions}

\subsection{Some discussions on the proof}

\subsubsection{Discussion on Hyper-parameters:}
\begin{itemize}
    \item In \cite{kveton2019garbage}, the pseudo rewards $a \in (0, 1)$ should larger than $1 / \sqrt{2}$ due to they need to control the anti concentration of Bernoulli distribution, i.e. control $ \E \big[ \pr^{-1} (U_{1, s} \geq (\mu_1 + s) \, | \, V_{1, s})\big]$;
    
    \item Similarly in \cite{kveton2019perturbed}, the condition $a > 2$ for tuning parameter is same as that in \cite{kveton2019garbage} to ensure the anti concentration having a valid upper bound;
    
    \item The tuning parameter of the pseudo residual $\sigma_a > 3 / 2$ in \cite{wang2020residual} is also essential by again controlling  the anti concentration;
\end{itemize}

which is the exact the place we ask our parameter $\lambda > 0$.

\subsubsection{Why we still use $G_{k, s}$}

As we can see in the proof, only combine $G_{k, s}$ with $A_{k, s}$ could we give $\Gamma_k$ bounded in some closed finite interval. It is not enough to only use $A_{k, s}$. The only reason we can drop $G_{k, s}$ is that when $R_{k, s}$ is bounded, $f(x)$ we mentioned before is increasing.

\section{Proof of Corollary \ref{cor.MAB.main}}

The proof of transforming problem-dependent to problem-independent problem is just based on Cauchy inequality. Indeed, we note that
\begin{equation*}
    H(\lambda, \sigma_{\omega}^2, \Delta_k) \lesssim \frac{1}{\Delta_k^2} + \Delta_k^2 + \Delta_k 
\end{equation*}
and similarly,
\begin{equation*}
    G(\lambda, \sigma_{\omega}^2, \Delta_k) \lesssim \frac{1}{\Delta_k^2} + \Delta_k^2 + \Delta_k 
\end{equation*}
for any $\lambda$ and $\sigma_{\omega}^2$. Hence, consider any $\Delta>0$,
\begin{equation*}
    \begin{aligned}
        \operatorname{Reg}_T & \leq \sum_{\Delta_k : \Delta_k < \Delta} \Delta_k \E J_{k, T} + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k \E J_{k, T} \\
        & \lesssim T \Delta + \sum_{k = 2}^K \Delta_k + \sum_{k = 2}^K \Delta_k \bigg[ \frac{1}{\Delta_k^2} + \Delta_k^2 + \Delta_k \bigg] \cdot \log T \\
        & \lesssim T \Delta + \sum_{k = 2}^K \Delta_k +  \sum_{k = 2}^K \frac{\log T}{\Delta_k} + K \log T \\
        & \lesssim  T \Delta  +  K \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k  +  \sum_{\Delta_k : \Delta_k \geq \Delta} \frac{\log T}{\Delta_k} + K \log T \\
        & \lesssim T \Delta + \frac{ K \log T}{\Delta} +  K \mu_1 + K \log T \lesssim \sqrt{K T \log T} + K \mu_1 + K \log T 
    \end{aligned}
\end{equation*}
by Cauchy inequality.


\section{Proof of Corollary \ref{cor.MAB}}

For the first result only need to note that
\begin{equation*}
    \operatorname{Reg}_T \leq 7 \sum_{k = 2}^K \Delta_k + \Big( 164.084 \times 774 + 1152 \Big) \sum_{k = 2}^K \frac{\log T}{\Delta_k} =  7 \sum_{k = 2}^K \Delta_k + 128153 \sum_{k = 2}^K \frac{\log T}{\Delta_k}
\end{equation*}
as $\lambda \rightarrow \infty$. For the second result, similarly as proof in the previously section, consider any $\Delta > 0$
\begin{equation*}
    \begin{aligned}
        \operatorname{Reg}_T & = \sum_{\Delta_k : \Delta_k < \Delta} \Delta_k \E J_{k, T} + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k \E J_{k, T} \\
        & \leq T \Delta + 7 \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k  +  128153 \sum_{\Delta_k : \Delta_k \geq \Delta} \frac{\log T}{\Delta_k} \\
        & \leq T \Delta + \frac{ 128153 K \log T}{\Delta} + 7 K \mu_1 \leq 948 \sqrt{K T \log T} + 7 K \mu_1.
    \end{aligned}
\end{equation*}
by Cauchy inequality.



==> ARCHIVE/9_Main_proof_backup_220904.tex <==
\section{Proof of Theorem \ref{thm.MAB}}\label{proof_thm}


Before starting our proof, we define the sub-exponential variable that mimics the tail of the exponential random variable. To {be} specific, we call a \textit{zero-mean} variable $X$ sub-exponential with parameter $\lambda$ and $\alpha$ if
\[
    \E \exp \{ t X \} \leq \exp \{ t^2 \lambda^2 / 2\}, \qquad |t| \leq \frac{1}{\alpha} \red{,}
\]
and we denote $X \sim \subE(\lambda, \alpha)$. 
Similar to the sub-Gaussian variables, we have the following concentration {property}
\[
    \pr (X \geq t) \leq \exp \left\{ - \frac{1}{2} \left( \frac{t^2}{\lambda^2} \wedge \frac{t}{\alpha}\right) \right\}, \qquad  {\forall} \, t \geq 0.
\]

%\red{(Move to the main text?)} 
%Now suppose each arms' rewards' setting is as follows
%\begin{itemize}
    %\item $\{ R_{k, \ell}\}$ are sub-Gaussian independent sample such that $\mu_k = \E R_{k, \ell} \in [0, 1]$ with finite sub-Gaussian parameter $\sigma_k^2 $.
%\end{itemize}

Recall the quantity of what we care about is the cumulative regret 
\[
    \operatorname{Reg}_{T} := \E \operatorname{Reg}_{T}(Y,\mathcal{A}) = \E \sum_{t=1}^{T} [R_1 - R_{A_{t}}]=\sum_{k=2}^{K} \Delta_{k} \E \Big[\sum_{t=1}^{T} 1 \left\{A_{t}=k\right\}\Big],
\]
where we assume $\mu_1 = \max_{k \in [K]} \mu_k$. In other words, the first arm
is the best arm with the {highest} expected reward. We want to show $\operatorname{Reg}_T$ can be bounded by $C \cdot \log T$ for any $T \in \mathbb{N}$ under our algorithm, {specially} under Algorithm 3. Here $C$ is free of the round $T$. 
%\red{(Bounded by order is not correct. Either "has the same order with xxx", or bounded by xxx. Any if you talk about order, there is no need to say $\forall T$, by definition.)} 



\subsection{Basic Idea}

% Here we want to use is the following lemma, which is a  decomposition of the cumulative regret as 
Our proof relies on the following decomposition of the cumulative regret from \cite{kveton2019garbage}. 
We recap its proof in Appendix \ref{sec:proof_lemma} for completeness.


\begin{lemma}\label{lem.a.b}
% When we select arms according to the
Recall that we select arms according to the rule 
$A_t = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 
% in the MAB problem, then 
For any $\{ \tau_k \}_{k = 2}^K \subseteq \mathbb{R}^{K - 1}$, 
we have the bound
\[
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\]
with
\[
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] =: \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1 =: \sum_{s = 0}^{T - 1} b_{k, s} + 1
\]
where $Q_{k, s} (\tau) = \pr \big( \overline{Y}_{k, s} > \tau \, | \his_{k, s} \big)$ and $N_{k, s} (\tau) = 1 / Q_{k, s} (\tau) - 1$ with $\his_{k, s}$ is the history $s$ rewards of $k$-th arm.
\end{lemma}
Here the summation index $s$ is the time we pull the $k$-th arm in the total $T$ round{s}. 
%\red{[(a and b) are just numbers, and they can not control anything. They represent something, and bounding them means something is controlled.]}
From the definition of $a_{k, s}$ and $b_{k, s}$, $a_k$ represents that the tail probability of pulling the optimal arm is not too small, while $b_k$ expresses that the tail probabilities of rewards of all arms are not too large in general. 
%\red{[A general comment: I suggest to add more "," and prepositions such as "that" to provide a better flow. Omitting them is convennient for ourselves, but not the readers. 
%E.g., ", for here, "}
It is worthy to note that for here we only need to consider the lower bound of the tail of the distribution of the rewards from optimal arm. 
%\red{(Like commented last time, an arm does not have tail, but its reward distribution has. As commented above, clarifying the logic will help our proof as well.)}
The intuition is that: (i) we only need the probability of the rewards of the optimal arm taking a relatively large value is not too small; (ii) we do not care about how small the probability of a large value occurred in the other arms. 
%\red{(this is part of the intuition; should not put a "." here. Maybe something like "the intuition is that (i) xxx and (ii) xxx.)}
% And this Lemma is valid for any algorithm in MAB problem as long as the action step is $A_{t} = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 


Hence, in the following steps, we will bound $a_k$ and $b_k$ separately up to order $\log T$. Recall that we denote two functions $a(s, T) \lesssim b(s, T)$ if $a(s, T) \leq c \times b(s, T)$ for $c$ free of $s$ and $T$. 
And we write $a(s, T) \asymp b(s, T)$ if $a(s, T) \lesssim b(s, T)$ and $a(s, T) \gtrsim b(s, T)$. 
The proof of all lemmas can be found in Appendix \ref{sec:proof_lemma}. 



\todorw{Can we have one paragraph (for each) to summarize how we plan to bound a and b below? 
If we can summarize it concisely using plain English, it means we really understand the logic. 
}

\subsection{Bounding $a_k$}
%\red{Grammar: Should be split into two sentence. "(we) recall" is one and "it is" is another.}
Recall that our target is bounding $a_k$ and $b_k$ up to order $
\log T$, it is enough to show that {this can hold}
for 
{any large enough} $T$. For doing this, we first prove a weaker statement: $a_{k, s}$ as a function of $T$ can be bounded by some constants free of $T$, 
%\red{$a_{k,s}$ is ONE constant, and bounded by constants? I know what you want to say. Just be more careful with these wordings. }
which will give the weaker bound $a_{k} \lesssim T$. 
Note that if we take
%\red{If one equation will not be cited, we should not give it an index}
\begin{equation}\label{requirement_0}
    \tau_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda},
\end{equation}
then we will have
\begin{equation}\label{constant_bound}
    a_{k, s} = \E \left[ \left( \frac{1}{Q_{1, s}(\tau_k)}  - 1\right) \wedge T \right] \leq \E \frac{1}{Q_{1, s}(\tau_k)} \leq \E Q_{1, s}^{-1} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right),
\end{equation}
where in the second inequality we use the fact that $Q_{1, s}(\cdot)$ is a decreasing function. Hence, we need to find a lower bound %\red{(Maybe I am wrong): lower bound is not a verb. Bound from below or sth else.} 
the tail probability $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right) = \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right)$. The tail probability can be written as the weighted summation of Gaussian bootstrap weights and hence can use the Gaussian inequality as follows
\[
    \begin{aligned}
        & \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right) \\
        = & \pr \left( {\red{\frac{\sum_{i = 1}^s \omega_i R_{1, i} + s \lambda}{\sum_{i = 1}^s \omega_i + 2 s \lambda}}} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s} \right) \\
        = & \pr_{\omega} \left( \sum_{i = 1}^s \big[  (1 + 2 \lambda) R_i - (\mu_1 + \lambda) \big] \omega_i > s \lambda (2 \mu_1 - 1) \right) \\
        \geq & \exp \left\{ - \frac{3 s^2 (1 + 2 \lambda)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \frac{1}{s} s^2 \left[  (1 + 2 \lambda) \overline{R}_{1, s} - (\mu_1 + \lambda) \right]^2 }\right\} \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        \geq & \exp \left\{ - \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left[  \overline{R}_{1, s} - (\mu_1 + \lambda) / (1 + 2 \lambda) \right]^2 }\right\} \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        \geq & \exp \left\{ - \frac{3 s (1 + 2 \lambda)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big] \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} 
    \end{aligned}
\]
where the $\geq$ is by the following lemma, which states the lower bound of the tail probability of Gaussian variables.

\begin{lemma}\label{lem:gau_low}
    Suppose $\{x_i\}_{i = 1}^n \cup y \in \mathbb{R}$ and $\{ \omega_i\}_{i = 1}^n$ are independent $N(1, \sigma_{\omega}^2)$ random variables, then $\pr \left( \sum_{i = 1}^n x_i \omega_i > y \right) \geq \exp \left\{ -\frac{3 \left(\sum_{i = 1}^n x_i - y \right)^2}{2 \sigma_{\omega}^2 \frac{1}{n} \left(\sum_{i = 1}^n x_i \right)^2 } \right\} 1 \left(\sum_{i = 1}^n x_i - y > \sqrt{2 \pi} \right) + \big[ 1 - \Phi(\sqrt{2 \pi})\big]  1 \left(0 < \sum_{i = 1}^n x_i - y \leq \sqrt{2 \pi} \right)$.
\end{lemma}
%\red{1. ", by"; 2. equations are also part of the sentence. Avoid a long sentence. Try something like ". the equality/inequality is due to the following lemma."}
%\begin{lemma}\label{lemma:gaussian_weight}
    %Suppose $x_i, y_i, z_i \in \mathbb{R}$ and $\{ \omega_i, \omega_i', \omega_i''\}$ are independent $N(1, \sigma_{\omega}^2)$ random variables, then
    %\[
        %\begin{aligned}
            %& \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{ i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \right)\\
            %\geq & \exp \left\{-\frac{3\left(S_{x}-S_{y}-S_{z}\right)^{2}}{2 \sigma_{\omega}^{2}\left(T_{x}+T_{y}+T_{z}\right)}\right\} \cdot 1\left(S_{x} \geq S_{y}+S_{z}+\sqrt{2 \pi}\right)+(1-\Phi(\sqrt{2 \pi})) \cdot 1\left(S_{x} \leq S_{y}+S_{z}+\sqrt{2 \pi}\right).
       % \end{aligned}
    %\]
%\end{lemma}
And as $a_{k,s}$ is bounded by the reciprocal of the lower bound of the tail probability in \eqref{constant_bound}, we obtain that 
\[
    \begin{aligned}
        a_{k, s} & \leq \E \exp \left\{ \frac{3 s (1 + 2 \lambda)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \cdot 1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}   + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} 
        %& \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}
    \end{aligned}
\]
Notice that ${R}_{1, i} - \mu_1$ for $i \in [s]$ is sub-Gaussian. 
For dealing with the expectation, we need the following lemma.
%\red{Same comment as above. The sentence is just too long. Imagine you are presenting. We need rests between sentences. }
% by the fact with the following lemma.
\begin{lemma}\label{lem_subGtosubE}
    Suppose $\{X_i\}_{i = 1}^n$ are i.i.d.  sub-Gaussian with mean $\mu$, then 
    \[
        \E \exp\left\{ \lambda(\overline{X} - \mu)^2 \right\} \leq \exp \left\{ \frac{64 \lambda^2 \sigma^4}{n^2} + \frac{\lambda \sigma^2}{n}\right\} \leq e^{9 / 8}
    \]
    for any $|\lambda| \leq \frac{n}{8 \sigma^2}$.
\end{lemma}
Hence, if we take
\begin{equation}
\label{cond.1}
    \frac{3 s (1 + 2 \lambda)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2} \leq \frac{s}{8 \sigma_1^2},
\end{equation}
we will obtain $a_{k, s}$ is bounded by 
\begin{equation}\label{a_k_constant}
    a_{k, s} \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
\end{equation}
%\red{If time permits, we should polish the proof for several more times to address issues as raised above.}
\begin{remark}
   Lemma \ref{lem_subGtosubE} actually is a special case for the fact that the mean of iid sub-Weibull sample with sample size $n$ will have the local sub-Gaussian property in the interval up to $\sqrt{n}$.
\end{remark}
%{\color{blue}{More details about the tuning parameters. }}
Take consideration of \eqref{cond.1}, for bound $a_{k, s}$ with a constant, we write the inequality with regarding of 
\begin{equation}\label{tuning_condition}
    \big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big] \lambda \geq 2 \sigma_1
\end{equation}
One can easily see that a immediately necessary condition for \eqref{tuning_condition} hold is $\mu_1 \geq \frac{1}{2}$. And solve it, and we can get regularity condition for tuning parameter $(\lambda, \sigma_{\omega}^2)$ is  
\begin{equation}\label{tuning_condition_exact}
    \lambda \geq \frac{2 \sigma_1}{\big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big]} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sigma_1}{2 \mu_1 - 1}.
\end{equation}
This step derives the whole restriction of tuning parameter in the Theorem. The exactly same situation appears in other literature: the condition of tuning parameter is derived in the step of bounding $a_{k, s}$ with a constant free of $T$, see \cite{kveton2019garbage} and \cite{wu2022residual} for instance.
%which is the reason why we need the restriction of tuning parameter in the Theorem.
%with some $C \geq 0$. Hence, a sufficient condition for any tuning parameter $\lambda > 0$ is that $12 \sigma_1^2 / \sigma_{\omega}^2 \leq 1$ for any round $T \geq 2$. Or some bounded interval for $\lambda$ will be required when $12 \sigma_1^2 / \sigma_{\omega}^2 \geq 1$. To be specific, if $\sigma_1^2 = \sigma_{\omega}^2 = 1$, a sufficient condition for \eqref{tuning_condition} is $12 (2 \lambda + 1)^2 \leq C \left[ (\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2\right]$ for some $C \geq 0$. For instance, if $\mu_1 = 1$, we can take $C = 12$, then our theory will be valid if take the tuning parameter $\lambda \in (0, 1]$ whenever the total round $T \geq 12$.

%{$\sigma_k^2 \in (0, 1]$ for $k \in [K]$ and $\sigma_{\omega}^2 = 1$}

%\textbf{$\leq sth. \log T$ holds for $T \geq C$. When $T < C$, take $sth.$ large enough we can still get the order $\log T$.
%}

%{$\lambda$ cannot depend on unknown variable}

%For instance, if we just take $\mu_1 = 1/2$, we will need $\sigma_{\omega}^2 \geq 24 \sigma_1^2$ with any $\lambda > 0$.

%\textit{sub-Gaussian parameter can be assumed to in $[0, 1]$, then we can solve the bound off $\lambda$. }

%\begin{remark}
   %Different from the bounded rewards setting, here $\lambda$ together with the bound of $\mu_1$ as well as $\sigma_{\omega}^2$ and $\sigma_k^2$ establish the restriction condition for the tuning parameters. But \eqref{tuning_condition_exact} can be served as a sufficient condition.
%\end{remark}

\begin{remark}
   It can be shown that for bounded rewards, we can use any positive $\lambda$ and $\sigma_{\omega}^2$ to ensure that $a_{k, s}$ can be bounded by a constant free of $T$. 
\end{remark}

Next, we decompose $a_{k, s}$ as positive several simple expressions $a_{k, s, 1}$, $a_{k, s, 2}$, and $a_{k, s, 3}$ i.e. $a_{k, s} = a_{k, s, 1} + a_{k, s, 2} + a_{k, s, 3}$, and we can focus on these simpler components. Following the idea in \cite{kveton2019garbage}, we will try to bound 
\[
    s_{a, j} = \max \{ s: a_{k, s, j} \geq T^{-1}\}, \qquad j = 1, 2, 3
\]
with an upper bound having order $\log T$. Indeed, if we successfully do so, then 
\[
    a_{k, s, j} \leq a_{k, s} \times s_{a, j} + T^{-1} \times (T - s_{a, j}) \lesssim \log T
\]
giving an order $\log T$. 

As we can see, decomposition will play an important role in this proof. For decomposition, a common approach is using indicators on good events. We define the following good events for $k$-th arm
\[
    A_{k, s} = \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  > - C_1 \Delta_k \right\}, \qquad A_{k, s}^{\prime} = \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  < C_2 \Delta_k \right\}, 
\]
and
\[
    G_{k', s} := \left\{ - C_3 \Delta_k \leq \overline{Y}_{k', s} - \overline{R}_{k', s}^* \leq C_3 \Delta_k \right\}
\]
with the shifted version mean defined as 
\[
    \overline{R}_{k, s}^* = \frac{\sum_{i = 1}^s R_{k, i} + \lambda s}{s(1 + 2 \lambda)} = \frac{\lambda}{1 + 2 \lambda} + \frac{1}{1 + 2 \lambda} \overline{R}_{k, s}
\]
It is worthy to note that $k'$ in $G_{k', s}$ is different from the fixed index $k$ in $\Delta_k$. And it is also easy to see that under two good events $A_{k', s} \cap G_{k', s}$, our target function $\overline{Y}_{k', s}$ is close to the shifted mean $\frac{\mu_{k'} + \lambda}{1 + 2\lambda}$, which means $\overline{Y}_{k', s}$ does remain the order of expected mean of each arm. 
Therefore, we decompose $a_{k, s}$ as the following three parts
\[
    a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1(A_{1, s}^c)\Big],
\]
\[
    a_{k, s, 2} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1(A_{1, s}) 1 (G_{1, s}^c)\Big], \qquad a_{k, s, 3} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) 1(A_{1, s}) 1 (G_{1, s})\Big].
\]
As we can see, $a_{k, s, 1}$ and $a_{k, s, 2}$ defined on "bad" events and hence we will bound the tail probability $\pr (A_{1, s}^c)$ and $\pr (G_{1, s}^c)$, while $a_{k, s, 3}$ defined on good events will need extra steps to bound (we will specify it later). 

\subsubsection{Tackling $a_{k, s, 1}$ with $s_{a, 1}$}

Since the summation of independent sub-Gaussian variable is still sub-Gaussian (see Lemma \ref{lem_subGtosubE}), we can find that $\overline{R}_{1, s} - \mu_1 \sim \subG (\sigma^2 /  s)$. And by the inequality of sub-Gaussian variable,
\[
    \begin{aligned}
        \pr (A_{1, s}^c) & = \pr \left( \mu_1 - \overline{R}_{1, s} \geq (1 + 2\lambda) C_1 \Delta_k \right) \leq \exp \left\{ - \frac{(1 + 2\lambda)^2 C_1^2 \Delta_k^2 s}{2 \sigma_1^2}\right\} \leq \frac{1}{T^2}
    \end{aligned}
\]
when we take
\[
    s \geq s_{a, 1} := \frac{\sigma_1^2}{C_1^2 (1 + 2 \lambda)^2 \Delta_k^2} \cdot \log T.
\]
Hence, under this setting, we obtain that
\[
    a_{k, s, 1} \leq \E \Big[ T  1(A_{1, s}^c)\Big] =  T \pr(A_{1, s}^c) \leq T^{-1}
\]
when $s \geq s_{a, 1} \asymp \log T$.

\begin{remark}
   For bounded rewards, there we can just use Hoeffding inequality and still have $s_{a, 1} \asymp \log T$.
\end{remark}

\subsubsection{Tackling $a_{k, s, 2}$ with $s_{a, 2}$}

As $G_{k', s} = \{ |\overline{Y}_{k', s} - \overline{R}^*_{k', s}| \leq C_3 \Delta_k\}$ is a symmetric event, we have 
\[
    \begin{aligned}
        & \pr (G_{1, s}^c \mid \his_{1, s}) \\
        = & 2 \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - C_3 \Delta_k (1 + 2 \lambda)\big] \omega_i \geq s \lambda \big[ 2 C_3 \Delta_k (1 + 2 \lambda) + 2 \overline{R}_{1, s} - 1 \big] \Bigg\} \\
        = &  2 \pr_{\omega} \Bigg\{  \frac{\sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - C_3 \Delta_k (1 + 2 \lambda)\big] \omega_i - s \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big] }{\sigma_{\omega}^2 \sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - C_3 \Delta_k (1 + 2 \lambda)\big]^2} \\
        & \qquad \qquad \geq \frac{s \lambda \big[ 2 C_3 \Delta_k (1 + 2 \lambda) + 2 \overline{R}_{1, s} - 1 \big] - s \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big] }{\sigma_{\omega}^2 \sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - C_3 \Delta_k (1 + 2 \lambda)\big]^2}\Bigg\} \\
        \leq &  2 \pr \left( Z \geq \frac{ C_3 \Delta_k (1 + 2 \lambda)^2 s}{\sigma_{\omega}^2 \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big]^2} \right)
    \end{aligned}
\]
where $Z$ is the standard Gaussian variable. By applying the concentration inequality for standard Gaussian variable such that $\pr (Z \geq x) \leq \exp \left\{ - x^2 / 2\right\}$, we get that 
\begin{equation}\label{a_k_s_2}
    \begin{aligned}
        a_{k, s, 2} & \leq \E \Big[ T  1(G_{1, s}^c)\Big] =  T \E \Big[ \pr(G_{1, s}^c \mid \his_{1, s}) \Big] \\
        & \leq 2 T \E \exp \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^2 }{2 \sigma_{\omega}^2 \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big]^4} \right\} \\
        & =  2 T \E \exp \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^4}{2 \sigma_{\omega}^2 \Big[ 2 \lambda \sqrt{s}(\overline{R}_{1, s} - \mu_1) - \sqrt{s} \big(\lambda (1 - 2 \mu_1) + C_3 \Delta_k (1 + 2 \lambda) \big) \Big]^4} \right\}.
    \end{aligned}
\end{equation}
%On the other hand, 
For tackling the expectation above, we first note that $\sqrt{s} (\overline{R}_{1, s} - \mu_1) \sim \subG (\sigma_1^2)$, then $ 2\lambda \sqrt{s} (\overline{R}_{1, s} - \mu_1) \sim \subG \big(4\lambda^2 \sigma_1^2 \big)$. Therefore, by applying Corollary 4 in \cite{zhang2020concentration}, $2 \sigma_{\omega}^2 \Big[ 2 \lambda \sqrt{s}(\overline{R}_{1, s} - \mu_1) - \sqrt{s} \big(\lambda (1 - 2 \mu_1) + C_3 \Delta_k (1 + 2 \lambda) \big) \Big]^4$ can be written as $A(s) X + B(s)$ with some zero-mean random variable $X \sim \subW(1/2)$ and polynomial $A(\sqrt{s})$ and $B(\sqrt{s})$ with the degree at most $4$. Denote $a = A(\sqrt{s}) / s^2$ and $b = B(\sqrt{s}) / s^2$ are free of $s$, then we can apply the following lemma.
\begin{lemma}[sub-Weibull concentration]\label{lem_subE_ineq}
    Suppose zero-mean random variable $X \sim \subW(\theta)$, and positive constant $a, b, c$ satisfying $a X + b > 0$, then
    \[
        \E \exp \left\{ - \frac{c}{a X + b}\right\}  \leq e^{- c / b} \big[1 + c h_1(a, b, \| X\|_{\psi_{\theta}}) + c h_2(a, b, \| X\|_{\psi_{\theta}}) \big],
    \]
    where $h_1$ and $h_2$ are finite positive functions free of $c$.
\end{lemma}
Hence, the right side of \eqref{a_k_s_2} can be furthermore bounded by 
\[
    a_{k, s, 2} \leq 2 T \E \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^2}{a X + b} \right\}.
\]
Now let us take
\[
    \begin{aligned}
        s \geq s_{a, 2} := & \frac{12 b}{C_3^2 (1 + 2\lambda)^4 \Delta_k^2} \times \log \Big[  2 C_3^2 \lambda^2 (1 + 2\lambda)^4 \Delta_k^2 \big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1 + h_2) \big] \Big] \log T
    \end{aligned}
\]
we will have $a_{k, s, 2} \leq T^{-1}$.

\subsubsection{Tackling $a_{k, s, 3}$ with $s_{a, 3}$}

As state previously, $a_{k, s, 3}$ defined on good events, we need a special technique to deal with. Write 
\[
    \begin{aligned}
        \{N_{1, s}(\tau_{k})<T^{-1}\} & \supseteq \{N_{1, s}(\tau_{k}) < (T^{2}-1)^{-1}\} = \big\{Q_{1, s}\left(\tau_{k}\right)^{-1}<1+\left(T^{2}-1\right)^{-1}\big\} \\
        &=\big\{Q_{1, s}(\tau_{k})^{-1} < (1-T^{-2})^{-1}\big\} = \big\{\left[1-Q_{1, s}(\tau_{k})\right]<T^{-2}\big\},
    \end{aligned}
\]
and $a_{k, s, 3} \leq \E \big[ N_{1, s} (\tau_k) 1(A_{1, s} \cap G_{1, s}) \big]$. Thus, it is sufficient to find $s \geq s_{a,3}$ such that $\big\{[1-Q_{1,s}(\tau_{k})]<T^{-2}\big\}$ on the event $\{A_{1, s} \cap G_{1, s}\}$. 
Note that
\[
    \big[1-Q_{1, s}(\tau_{k})\big]  1(A_{1, s}) 1(G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, s} \big)  1(A_{1, s}) 1(G_{1, s})
\]
with $\Gamma_1 := \Gamma_1(\tau_1) = \tau_1 - \overline{R}_{1, s}^*$ measuring the difference between $\overline{Y}_{1, s}$ and $\overline{R}_{1,s}^*$. It is not hard to see $\Gamma_1$ should be negative with a moderate value. And $\Gamma_1$ does have an appropriate on the event $A_{1, s} \, \cap \, G_{1, s}$, this can be true. To see this, we write 
\[
    A_{1, s} = \bigg\{ \overline{R}_{1, s}^* - \frac{\mu_1 + \lambda}{1 + 2\lambda} > - C_1 \Delta_k \bigg\} = \bigg\{ \Gamma_1 < C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} + \tau_1 \bigg\} 
\]
and
\[
    \begin{aligned}
        G_{1, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_1 -C_3 \Delta_k \leq \overline{Y}_{1, s} + \Gamma_1 \leq \tau_1 + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_1 - C_3 \Delta_k - \overline{Y}_{1, s} \leq \Gamma_1 \leq \tau_1 + C_3 \Delta_k - \overline{Y}_{1, s}\big\} \\
        & \subseteq \big\{ \tau_1 - 2 C_3 \Delta_k - \overline{R}_{1, s}^* \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \overline{R}_{1, s}^* \big\} \\
        & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2 \lambda}\bigg\},
    \end{aligned}
\]
then
\[
    \begin{aligned}
        A_{1, s} \, \cap \, G_{1, s} & = \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 < \tau_1 + C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} \bigg\} \\
        & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\} \\
        (\text{if } C_1 \geq 2 C_3 )& \subseteq \bigg\{ \tau_1 -  C_1 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\}.
    \end{aligned}
\]
It is easy to see that in the above derivation, we add the requirement that
\begin{equation}\label{requirement_1}
     \Delta_k + \tau_1 - \frac{\mu_1}{2} = 0 \leq 0 \qquad \text{ and }  \qquad C_1 \geq 2C_3.
\end{equation}
Therefore, we obtain the range of the positive quantity $-\Gamma_1$ is
\[
    C_1 \Delta_k = \frac{\mu_1 }{2} - \tau_1 - C_1 \Delta_k <  (- \Gamma_1) \leq 1 + C_1 \Delta_k  - \tau_k = 1 - \frac{\mu_1}{2} + 3 C_1 \Delta_k < 4
\]
i.e. $ (- \Gamma_1) \in (C_1 \Delta_k, 4)$ when we take
\begin{equation}\label{requirement_2}
    \tau_1 = \frac{\mu_1}{2} - \Delta_k.
\end{equation}
Besides, as the tail probability we care is 
\[
    \begin{aligned}
        & \big[ 1 - Q_{1,s} (\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \\
        = & 2 \pr_{\omega} \Bigg\{ \sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - \Gamma_1 (1 + 2 \lambda)\big] \omega_i \geq s \lambda \big[ 2 \Gamma_1 (1 + 2 \lambda) + 2 \overline{R}_{1, s} - 1 \big] \Bigg\},
    \end{aligned}
\]
what we need to deal with is by replacing  $C_3 \Delta_k$ by $(-\Gamma_1)$ in the above section. By using the same technique, one can get that
\[
    \begin{aligned}
        \big[ 1 - Q_{1,s} (\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq T^{-2}
    \end{aligned}
\]
when
\[
   \begin{aligned}
       s \geq s_{a, 3} := & \frac{6 b^* }{C_1^2 (1 + 2\lambda)^4 \Delta_k^2 } \times \log \Big[ 1 + C_1^2 \Delta_k^2 (1 + 2\lambda)^4  (h_1^* + h_2^*)\Big] \log T,
   \end{aligned}
\]
where $b^*$, $h_1^*$, and $h_2^*$ free of $s$ are the parameters in Lemma \ref{lem_subE_ineq}.

Now combine all results in Section C.2, we get that 
\[
    a_{k} \leq \underbrace{\max_{s = 0, \ldots, T -  1} a_{k, s}}_{\text{bound by a constant in \eqref{a_k_constant}}} \cdot \overbrace{\max _{j = 1, 2, 3} s_{a, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{a, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Here, we do not give the explicit expression of the bound as it involves several numeric integral terms, while its order is exactly $\log T$. However, for some explicit reward distributions, the expectation in Lemma \ref{lem_subE_ineq} can be bounded by some simpler expression, and hence we have the explicit expression for the bounds in these cases, see Corollary \ref{cor_ber} and Corollary \ref{cor_gau}.
\end{remark}

\subsection{Bounding $b_k$}

For bounding $b_k = \sum_{s = 0}^{T - 1} b_{k, s}$, we decompose $b_{k, s} = \pr \big( Q_{k, s} (\tau_k) > T^{-1}\big) + 1$ as $b_k = b_{k, s, 1} + b_{k, s, 2} + b_{k, s, 3} + 1$ with
\[
    b_{k, s, 1} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A_{k, s}^{\prime c} )\big],
\]
\[
    b_{k, s, 2} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A'_{k, s}) 1(G_{k, s}^c)\big],
\]
\[
    b_{k, s, 3} := \E \big[ 1( Q_{k, s} (\tau_k) > T^{-1}) 1(A'_{k, s}) 1(G_{k, s})\big].
\]
Since $b_{k, s}$ is naturally bounded $2$, it only needs to bound $s_{b, j}: = \max \{ s: b_{k, s, j} \geq T^{-1}\}$ up to $\log T$ for $j = 1, 2, 3$.

It is easy to see that $\pr (A^{\prime c}_{k, s}) \leq T^{-2} $ when $s \geq \frac{1}{2}s_{a, 2}'$. Here $s_{\cdot}'$ is the value of $s_{\cdot}$ but in it $C_1$ is replaced by $C_2$. Then we have $b_{k,s, 1} \vee b_{k, s, 2} \leq T^{-2} < T^{-1}$ as long as $s \geq (s'_{a, 1}  / 2 \vee s'_{a, 2}) \asymp \log T$. It remains to tackle $b_{k, s, 1}$. We will first bound $\Gamma_k = \overline{Y}_{k, s}  - \overline{R}_{k, s}^*$ on $A_{k, s}' \, \cap \, G_{k, s}$. Decompose
\[
    A'_{k, s} = \bigg\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} < C_2 \Delta_k \bigg\} = \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \bigg\},
\]
and
\[
    \begin{aligned}
        G_{k, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{k, s} - \overline{R}_{k, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_k -C_3 \Delta_k \leq \overline{Y}_{k, s} + \Gamma_k \leq \tau_k + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_k - 2 C_3 \Delta_k - \overline{R}_{k, s}^* \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \overline{R}_{k, s}^* \big\} \\
        & \subseteq \bigg\{ \tau_k - 2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2\lambda} \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2\lambda}\bigg\},
    \end{aligned}
\]
hence, we conclude that 
\[
    \begin{aligned}
        A'_{k, s} \, \cap \, G_{k, s} & \subseteq  \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \leq\tau_k + C_2 \Delta_k - \frac{\lambda}{1 + 2\lambda} \bigg\} \\
        & \subseteq \bigg\{ \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2}  < \Gamma_k < \tau_k + C_2 \Delta_k \bigg\}
    \end{aligned}
\]
% It is worthy to recall that the construction of $s_{a, 1, 2}$ is free of any $\tau_k$, hence this argument is valid. 
if
\begin{equation}\label{requirement_3}
    2 C_3 \geq C_2.
\end{equation}
Under this establishment, we need $\tau_k - C_2 \Delta_k - \frac{\mu_k }{2} \leq 0$, then we can take
\begin{equation}\label{requirement_4}
    \tau_k = 2 C_2 \Delta_k + \mu_k / 2
\end{equation}
and we will obtain that the bound for $\Gamma_k$ is
\[
    C_2 \Delta_k = \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2} < \Gamma_k < \tau_k + C_2 \Delta_k = 3 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{7}{2} < 4,
\]
i.e. $\mathbb{R}_+ \ni \Gamma_k \in (C_2 \Delta_k, 4)$. Similar to previous, 
\[
    \begin{aligned}
        & Q_{k, s}\left(\tau_{k}\right) 1\left(A_{k, s}^{\prime}\right) 1\left(G_{k, s}\right) = \E \pr \left(\overline{Y}_{k, s}-\overline{R}_{k, s}^{*}>\Gamma_{k} \mid \mathcal{H}_{k, T}\right) 1\left(A_{k, s}^{\prime}\right) 1\left(G_{k, s}\right) \\
        = & \E \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s \big[ (1 + 2\lambda) R_i - (\overline{R}_{1, s} + \lambda) - \Gamma_k (1 + 2 \lambda)\big] \omega_i \geq s \lambda \big[ 2 \Gamma_k (1 + 2 \lambda) + 2 \overline{R}_{1, s} - 1 \big]\Bigg\}\\
        \leq &  T \exp \left\{ - \frac{C_2^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 b^{**}}\right\} \times \Big[ 1 + C_2^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1^{**} + h_2^{**} )\Big].
    \end{aligned}
\]
where $b^{**}$, $h_1^{**}$, and $h_2^{**}$ are the parameters in Lemma \ref{lem_subE_ineq} similarly defined as previous. Therefore, one can just take 
\[
    \begin{aligned}
        s \geq s_{b, 3} & :=  \frac{8 b^{**}}{C_2^2 (1 + 2\lambda)^4 \Delta_k^2 s} \times \log \Big[ 1 + C_2^2 \Delta_k^2 (1 + 2\lambda)^4  (h_1^{**} + h_2^{**})\Big] \log T
    \end{aligned}
\]
and then by using the similar argument, we have 
\[
    b_{k} \leq 2 \cdot \overbrace{\max _{j = 1, 2, 3} s_{b, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{b, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Similarly, for specific reward distributions, we can bound $b_k$ in $\log T$ with some simple and specific coefficients, see Corollary \ref{cor_ber} and Corollary \ref{cor_gau}.
\end{remark}
Finally, what remains is to show the restrictions (\ref{requirement_0}), (\ref{requirement_1}), (\ref{requirement_2}), (\ref{requirement_3}), and (\ref{requirement_4}) are compatible. Indeed, they will build the following system of equations,
\[
    \left\{ \begin{array}{l}
         \frac{\mu_1}{2} - 2 C_1 \Delta_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
         2 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
        \tau_k - \frac{\mu_1}{2} - C_1 \Delta_k  \leq \tau_k + C_2\Delta_k - \frac{\mu_k }{2} \\
        C_1 \geq 2C_3 \\
        2 C_3 \geq C_2 \\
        \frac{\mu_1}{2} - 2 C_1 \Delta_k = 2 C_2 \Delta_k + \frac{\mu_k}{2}
    \end{array}\right..
\]
We can see that 
\[
    C_1 = C_2 = \frac{1}{8}, \qquad C_3 = \frac{1}{16},
\]
is the unique solution for the above system. Up to now, we have finished the first part of our proof. For the second part, 
\begin{equation*}
    \begin{aligned}
        \operatorname{Reg}_T & = \sum_{\Delta_k : \Delta_k < \Delta} \Delta_k \E J_{k, T} + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k \E J_{k, T} \\
        & \lesssim T \Delta + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k  +  \sum_{\Delta_k : \Delta_k \geq \Delta} \frac{\log T}{\Delta_k} \\
        & \lesssim T \Delta + \frac{ K \log T}{\Delta} \lesssim \sqrt{K T \log T}.
    \end{aligned}
\end{equation*}
for any previously specified $\Delta \in (0, 1)$ by Cauchy inequality. Therefore, we finish the proof of Theorem \ref{thm.MAB}.



%\textit{{Bounded case need to separate to prove?}}

%As all the restrict conditions for $C_1, C_2, C_3$ are exactly the same as previous, we still take $C_1 = C_2 = \frac{1}{8}$ and $C_3 = \frac{1}{16}$. And the final bounds need to be doubled.

\section{Proof of Corollary \ref{cor_ber}}

As stated in Section \ref{proof_thm}, for bounded Bernoulli rewards, we still have $a_{k, s} \leq e^{9 /8} + \big[ 1 - \Phi (\sqrt{2 \pi}) \big]^{-1}$ as long as the tuning parameter $(\lambda, \sigma_{\omega}^2)$ satisfying \eqref{tuning_condition_exact}.
And similar, one can prove that for bounding $a_{k, s, j}$, one can easily show that
\begin{itemize}
    \item For $a_{k, s, 1}$, we have $a_{k, s, 1} \leq T^{-1}$ as long as
    \[
        s \geq s_{a, 2} := \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} \log T.
    \]
    \item For $a_{k, s, 2}$, one can following the same steps to get that 
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq \E \Big[ T  1(G_{1, s}^c)\Big] =  T \E \Big[ \pr(G_{1, s}^c \mid \his_{1, s}) \Big] \\
            & \leq 2 T \E \exp \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^2 }{2 \sigma_{\omega}^2 \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big]^4} \right\} \\
            & = 2 T \E \exp \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^6 }{2 \sigma_{\omega}^2 \big[ s \lambda (2 \overline{R}_{1, s} - 1) - s C_3 \Delta_k (1 + 2 \lambda)\big]^4} \right\}  =: 2 T \E f(s \overline{R}_{1, s})
        \end{aligned}
    \]
    where the function $f(x)$ is
    \[
        f(x) := \exp \left\{ - \frac{ C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^6 }{2 \sigma_{\omega}^2 \big[  \lambda (2 x - s) - s C_3 \Delta_k (1 + 2 \lambda)\big]^4} \right\}.
    \]
    Then $f(x)$ is a decreasing function on $0 \leq x \leq s / 2$ and an increasing function on $x \geq s / 2$. By symmetric technique of Binomial distribution and Lemma 2 in \cite{kveton2019garbage}, we have
    \[
        a_{k, s, 2} \leq 4 T \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x ; s, \mu_1) f(x) \leq 4 T \left[ \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s})+\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \right].
    \]
    Similarly to \cite{kveton2019garbage}, we can show that 
    \[
        \begin{aligned}
            & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s}) +\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            = & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] \exp \left\{-  \frac{C_3^2 \Delta_k^2 (1 + 2 \lambda)^4 s^4}{2 \sigma_{\omega}^2 \left\{ \sqrt{s}\left[ \lambda (2 \mu_1 - 1) -C_3 (1 + 2\lambda)\right] - 2 \lambda (i + 1) \right\}^4}\right\} + \exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            \leq & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[- \left(2 i^{2} + \frac{  \Delta_k^2 (1 + 2\lambda)^4 s^4}{ 2 \sigma_{\omega}^2 c_1^{* 4} s^2} \right) \right] + \exp \left[-2 s^{2} \mu_1^2 \right]  \\
            \leq & \exp \left\{ - (2 \mu_1^2 \wedge \sigma_{\omega}^{-2} c_1^{* - 4}  \Delta_k^2 (1 + 2 \lambda)^4) s^2 \right\} \left( 1 + \sum_{i=0}^{\lfloor s \mu_1 \rfloor}  \exp \left[-2 i^{2}\right] \right) \\
            = & \left( 1 + \sqrt{\pi / 8}\right) \exp \left\{ - (2 \mu_1^2 \wedge  \sigma_{\omega}^{-2} c_1^{* - 4} \Delta_k^2 (1 + 2 \lambda)^4) s^2 \right\}
            %\leq & s \mu_1 \exp \left\{ - s \mu_1 \right\} \leq T \mu_1 \exp \{ - s \mu_1 \}
            % \leq & \left[ \int_1^{s \mu_1 + 1} \exp \{- 4 (u - 1)^2 \} \, du \right]^{1 / 2} \left[\int_1^{s \mu_1 + 1} \exp \left\{ - \frac{2c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3}\right\} \, du \right]^{1 / 2} \\
            %= & \left[ \right] \exp 
        \end{aligned}
    \]
    with $c_1^*$ is defined as
    \begin{equation}\label{c_1_star}
        c_1^{*} = c_1 (\lambda, \Delta_k) :=  \min_{0 \leq i \leq \lfloor s\mu_1 \rfloor, \, i \in \mathbb{N}} \frac{1}{\sqrt{s}} \big| \sqrt{s}\left[ \lambda (2 \mu_1 - 1) - (1 + 2\lambda) / 16 \right] - 2 \lambda (i + 1) \big|  > 0
    \end{equation}
    \red{In general, we have
    \[
        c_1^{*4} \geq \max_{k \in [K] / 1} \frac{2 \sigma_{\omega}^2 \mu_1^2}{\Delta_k^2 (1 + 2 \lambda)^4},
    \]
    and thus, $a_{k, s, 2} \leq 4 T (1 + \sqrt{\pi / 8}) \exp \left\{ - \sigma_{\omega}^{-2} c_1^{*-4} \Delta_k^2 (1 + 2 \lambda)^4 s^2 \right\}$.
    }
    Therefore, by taking 
    \[
        s_{a, 2} \geq \frac{5 \sigma_{\omega} \log T}{2 c_1^{* 2} \Delta_k (1 + 2 \lambda)^2} \geq \frac{\sigma_{\omega}}{c_1^{* 2} \Delta_k (1 + 2 \lambda)^2} \cdot \sqrt{\log \big( 4 (1 + \sqrt{\pi / 8}) T^2 \big)}
    \]
    one will have $ a_{k, s, 2} \leq T^{-1}$.\\
    
    \item By taking the same technique as $a_{k, s, 2}$, 
    one can show that
    \[
        \begin{aligned}
            \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq 2 \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x; s, \mu_1) g(x) \leq 2 s \mu_1 \exp \{ - s \mu_1\} \leq T^{-1}
        \end{aligned}
    \]
    as long as $s \geq s_{a, 3} := s_{a, 2}$. And hence in this case, one will have $a_{k, s, 3} \leq T^{-1}$.
\end{itemize}

Combining these results, we obtain that 
\[
    \begin{aligned}
        a_k & \leq \max_{s = 0, \ldots, T -  1} a_{k, s} \cdot \max _{j = 1, 2, 3} s_{a, j} + 3 T^{-1} \cdot\big(T - \max_{j = 1, 2, 3} s_{a, j}\big) \\
        & \leq \left[ e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right] \left[ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{5}{2  (1 + 2 \lambda)^2 c_1^{* 2} \Delta_k }\right] 
        \log T + 3.
    \end{aligned}
\]
Specially, if $\sigma_{\omega}^2 \geq 1$ and $\lambda \geq 1$, by using the fact that $\lambda^2\big[ (\lambda - 1)^2 + \lambda^2\big] \geq \lambda (\lambda + 1)$, one will have 
\[
    a_k \leq  \left[ e^{ 9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right] \left[ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{5}{2  (1 + 2 \lambda)^2 c_1^{* 2} \Delta_k } \right] \log T + 3.
\]
By using the same technique, one can show that 
\[
    b_k \leq 2 \cdot \left[ \frac{2}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{5}{2  (1 + 2 \lambda)^2 c_k^{* 2} \Delta_k } \right] \log T + 3
\]
for any $\lambda > 0$ with
\begin{equation}\label{c_k_star}
    c_k^{*}  :=  \min_{0 \leq i \leq \lfloor s\mu_k \rfloor, \, i \in \mathbb{N}} \frac{1}{\sqrt{s}} \big| \sqrt{s}\left[ \lambda (2 \mu_k - 1) - (1 + 2\lambda) / 16 \right] - 2 \lambda (i + 1) \big|  > \max_{k \in [K] / 1} \frac{2 \sqrt{\sigma_{\omega} \mu_k}}{\sqrt{\Delta_k} (1 + 2 \lambda)}.
\end{equation}
Therefore, we complete the proof.

\section{Proof of Corollary \ref{cor_gau}}

Follow the steps in Proof of Corollary \ref{cor_ber}. We claim the following statements:
\begin{itemize}
    \item[1.] Note the fact that $\sigma_{1}^{-2} s^2 (\overline{R}_{1, s} - \mu_1)^2 \sim \chi^2(s)$, here one give more precise condition for the tuning parameter. Indeed, one can show that
    \[
        \begin{aligned}
            a_{k, s} & \leq \E \exp \left\{ \frac{3 s (1 + 2 \lambda)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}  \\
            (\text{by using the MGF of } \chi^2(s))& = \left[ 1 - \frac{3 \sigma_1^2 (2 \lambda + 1)^2}{ s \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right]^{- \frac{s}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
            (\text{take } s = 1) & \leq \left[ 1 - \frac{3 \sigma_1^2 (2 \lambda + 1)^2}{ \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} \big]^2}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        \end{aligned}
    \]
    %stop here 220831.
    since $s = 0$ naturally satisfies the above inequality. This further implies we will need
    \[
       \frac{3 \sigma_1^2 (2 \lambda + 1)^2}{ \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} \big]^2} < 1
    \]
    with its sufficient condition as 
    \[
        3 (2 \lambda + 1)^2 < \frac{12}{(2 \mu_1 - 1)^2}  \big[ (2 \mu_1 - 1) \lambda + \sqrt{2 \pi} \big]^2
    \]
    i.e. 
    \begin{equation}\label{cor_2_tuning_suf}
        4 \left[ \frac{2 \sqrt{2 \pi}}{2 \mu_1 - 1} - 1\right] \lambda > 1 - \frac{8 \pi}{(2 \mu_1 - 1)^2}
    \end{equation}
    if we take $\sigma_{\omega}^2 \geq \frac{12 \sigma_1^2}{(2 \mu_1 - 1)^2}$. Note that $2 \mu_1 - 1 \in (0, 1]$, we have $\left[ \frac{2 \sqrt{2 \pi}}{2 \mu_1 - 1} - 1\right] > 0$ and $1 - \frac{8 \pi}{(2 \mu_1 - 1)^2} < 0$, \eqref{cor_2_tuning_suf} always hold for any $\lambda > 0$. 
    In a word, under the assumptions in Corollary \ref{cor_gau}, one will have
    \[
        \begin{aligned}
            a_{k, s} \leq \left[ 1 - \frac{3 (2\mu_1 - 1)^2 (2 \lambda + 1)^2}{ 4 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} \big]^2}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        \end{aligned}
    \]
    with $\sigma_{\omega}^2 \geq \frac{12 \sigma_1^2}{(2 \mu_1 - 1)^2}$ for $s \in \{ 0, \ldots, T - 1\}$.
    
    \item[2.] For controlling $a_{k}$, one can easily show that 
    \[
        \begin{aligned}
            a_k & \leq \left\{ \left[ 1 - \frac{3 (2\mu_1 - 1)^2 (2 \lambda + 1)^2}{ 4 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} \big]^2}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right\} \\
            & \qquad \qquad \left[ \frac{64 \sigma_1^2}{(1 + 2 \lambda)^2 \Delta_k^2} + (1 + \sqrt{2})\sqrt[4]{3 \times 2^{13}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda) \sqrt{\Delta_k}}  \right] \log T + 3.
        \end{aligned}
    \]
    by the following statements.
    \begin{itemize}
        \item[2.1] Still use sub-Gaussian inequality to get that we have $a_{k, s, 1} \leq T^{-1}$ when
        \[
            s \geq s_{a, 1} = \frac{64 \sigma_1^2}{(1 + 2 \lambda)^2 \Delta_k^2} \log T.
        \]
        
        \item[2.2] For dealing with $a_{k, s, 2}$, we again use the fact that
        \[
            \begin{aligned}
                \big[ \lambda(2 \overline{R}_{1, s} - 1) - C_3 \Delta_k (1 + 2 \lambda)\big]^4 & = \big[  2 \lambda (\overline{R}_{1, s} - \mu_1) + \lambda (2 \mu_1 - 1) - C_3 \Delta_k (1 + 2 \lambda) \big]^4 \\
                & =: \big[ \xi + \lambda (2 \mu_1 - 1) - C_3 \Delta_k (1 + 2 \lambda) \big]^4
            \end{aligned}
        \]
        with $\xi \sim N (0, 4 s^{-1} \lambda^2)$. Denote
        \[
            A: = C_3^2 (1 + 2 \lambda)^4 \Delta_k^2, \qquad B:= \lambda(2 \mu_1 - 1) - C_3 \Delta_k (1 + 2 \lambda),
        \]
        then it will lead to the result that 
        \[
            \begin{aligned}
                a_{k, s, 2} & \leq 2 T \E \exp \left\{ - \frac{C_3^2 (1 + 2 \lambda)^4 \Delta_k^2 s^2}{ 2 \sigma_{\omega}^2 \big[ \xi + \lambda (2 \mu_1 - 1) - C_3 \Delta_k (1 + 2 \lambda) \big]^4}\right\} = 2 T \E \exp \left\{ - \frac{A s^2}{  2 \sigma_{\omega}^2 \big[ \xi + B \big]^4}\right\} \\
                & = \frac{T}{\lambda} \sqrt{\frac{s}{2 \pi}} \int_{- \infty}^{\infty} \exp \left\{ - \left[ \frac{A s^2}{ 2 \sigma_{\omega}^2(u + B)^4} + \frac{s u^2}{32 \sigma_{\omega}^2 \lambda^2}\right] \right\} \exp \left\{ - \frac{s u^2}{ 32 \sigma_{\omega}^2 \lambda^2} \right\} \, du \\
                & \leq \frac{3 T}{\lambda}  \sqrt{\frac{s}{2 \pi}} \exp\left\{ - 3 \left[ \frac{A s^4}{2^7 \sigma_{\omega}^6 \lambda^4}\right]^{1 / 3} \right\} \int_{- \infty}^{\infty} \exp \left\{ - \frac{s u^2}{32 \sigma_{\omega}^2 \lambda^2} \right\} \, du = 12 \sigma_{\omega} T \exp\left\{ - 3 \left[ \frac{A s^4}{2^7 \sigma_{\omega}^2 \lambda^4}\right]^{1 / 3} \right\}.
            \end{aligned} 
        \]
        Therefore, for any $T \geq \lceil 2 \sigma_{\omega} \rceil $, take
        \[
            s \geq s_{a, 2} := \sqrt[4]{3 \times 2^{15}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda) \sqrt{\Delta_k}} \log T \geq \sqrt[4]{\frac{2^{15}}{3^3}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda) \sqrt{\Delta_k}} \log^{3 / 4} \big( 2 \sigma_{\omega} T^2 \big)
        \]
        we will get that $a_{k, s, 2} \leq T^{-1}$.\\
        
        \item[2.3] Just by replacing $C_3 \Delta_k$ by $(- \Gamma_1)$ which is bounded in $(C_1 \Delta_k, 4)$, and we will get that
        \[
            \begin{aligned}
                \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq T^{-1}
            \end{aligned}
        \]
        i.e. $a_{k, s, 3} \leq T^{-1}$ whenever 
        \[
            s \geq s_{a, 3} := \sqrt[4]{3 \times 2^{13}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda) \sqrt{\Delta_k}} \log T .
        \]
    \end{itemize}
    
    \item[3.] Exactly the same as 2., we can get that 
    \[
        b_{k} \leq 2 \left[ \frac{32 \sigma_k^2}{(1 + 2 \lambda)^2 \Delta_k^2} + (1 + \sqrt{2})\sqrt[4]{3 \times 2^{13}} \frac{\lambda \sigma_{\omega}^{3/2}}{(1 + 2\lambda) \sqrt{\Delta_k}}  \right] \log T + 3.
    \]
\end{itemize}
These results give Corollary \ref{cor_gau}.

==> ARCHIVE/9_Main_proof_backup_221124.tex <==


\section{Proof of Theorem \ref{thm.MAB}}\label{proof_thm}


Before starting our proof, we first give the definition of sub-exponential variables. To be specific, we call a \textit{zero-mean} variable $X$ sub-exponential with parameters $\lambda$ and $\alpha$ if
\[
    \E \exp \{ t X \} \leq \exp \left\{ \frac{t^2 \lambda^2}{2}\right\}, \qquad |t| \leq \frac{1}{\alpha} ,
\]
denoted as $X \sim \subE(\lambda, \alpha)$. Specially, we denote $\subE(\lambda) := \subE(\lambda, \lambda)$. 
Similar to the sub-Gaussian variables, we have the following concentration {property}
\[
    \pr (X \geq t) \leq \exp \left\{ - \frac{1}{2} \left( \frac{t^2}{\lambda^2} \wedge \frac{t}{\alpha}\right) \right\}, \qquad  {\forall} \, t \geq 0.
\]

%\red{(Move to the main text?)} 
%Now suppose each arms' rewards' setting is as follows:
%\begin{itemize}
    %\item $\{ R_{k, \ell}\}$ are sub-Gaussian independent sample such that $\mu_k = \E R_{k, \ell} \in [0, 1]$ with finite sub-Gaussian parameter $\sigma_k^2 $.
%\end{itemize}

%Recall that the quantity of what we care about is the sum of our cumulative regret:
%\[
    %\operatorname{Reg}_{T} := \E \operatorname{Reg}_{T}(Y,\mathcal{A}) = \E \sum_{t=1}^{T} [R_1 - R_{A_{t}}]=\sum_{k=2}^{K} \Delta_{k} \E \Big[\sum_{t=1}^{T} 1 \left\{A_{t}=k\right\}\Big],
%\]
%where we assume $\mu_1 = \max_{k \in [K]} \mu_k$. In other words, the first arm
%is the best arm with the {highest} expected reward. We want to show $\operatorname{Reg}_T$ can be bounded by a log regret, i.e. $C \times\log T$ for any $T \in \mathbb{N}$ under Algorithm 3. 
%Here $C$ is free of the round $T$. 
%\red{(Bounded by the order is not correct. Either "has the same order with xxx", or bounded by xxx. Any if you talk about order, there is no need to say $\forall T$, by definition.)} 



\subsection{Basic Idea}

% Here we want to use is the following lemma, which is a  decomposition of the cumulative regret as 
Our proof relies on the following decomposition of the cumulative regret from \cite{kveton2019garbage}. 
We will recap its proof in Appendix \ref{sec:proof_lemma} for completeness. Let the history of arm $k$ after $s$ pulls be a set $\his_{k, s}$ of cardinality $s$, $Q_{k, s} (\tau) := \pr \big( \overline{Y}_{k, s} > \tau \, | \his_{k, s} \big)$ be the tail probability that $\overline{Y}_{k, s}$ conditioned on history $\his_{k, s}$ is a least $\tau$ for some tunable parameter $\tau$, and $N_{k, s} (\tau) := 1 / Q_{k, s} (\tau) - 1$.
\begin{lemma}\label{lem.a.b}
% When we select arms according to the
Suppose in MAB we select arms according to the rule 
$A_t = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 
% in the MAB problem, then 
Then for any $\{ \tau_k \}_{k = 2}^K \subseteq \mathbb{R}^{K - 1}$, 
the expected $T$-round regret can be bounded above as
\[
    \operatorname{Reg}_T \leq \sum_{k = 2}^K \Delta_k \big( a_k + b_k \big)
\]
where
\[
    a_k = \sum_{s = 0}^{T - 1} \E \big[N_{1, s}(\tau_k) \wedge T\big] =: \sum_{s = 0}^{T - 1} a_{k, s}, \qquad b_k = \sum_{s = 0}^{T - 1} \pr \big( Q_{k, s} (\tau_k) > T^{-1} \big) + 1 =: \sum_{s = 0}^{T - 1} b_{k, s} + 1.
\]
\end{lemma}
Recall the summation index $s$ is the time we pull the $k$-th arm in the total $T$ round{s}. 
%\red{[(a and b) are just numbers, and they can not control anything. They represent something, and bounding them means something is controlled.]}
The definition of $a_{k}$ and $b_{k}$ have important meaning, $a_{k}$ represents the expected number of rounds that optimal arm $1$ has been being underestimted, while $b_{k}$ is the probability that the suboptimal arm $k$ is being overestimated.
%$a_k$ represents that the  probability of pulling the optimal arm is not too small in its tails, while $b_k$ is the tail probabilities of rewards of all arms are not too large. 
%\red{[A general comment: I suggest adding more "," and prepositions such as "that" to provide a better flow. Omitting them is convenient for ourselves, but not the readers. 
Here we only need to consider the lower bound of the tail of the distribution of the rewards from the optimal arm. 
%\red{(Like commented last time, an arm does not have a tail, but its reward distribution has. As commented above, clarifying the logic will help our proof as well.)}
The intuition is: (i) we only need the rewards from the optimal arm taking a relatively large value with a probability that is not too small; (ii) we do not care about the tiny probability of a large reward from suboptimal arms. 
%\red{(this is part of the intuition; should not put a "." here. Maybe something like "the intuition is that (i) xxx and (ii) xxx.)}
% And this Lemma is valid for any algorithm in MAB problem as long as the action step is $A_{t} = \arg \max_{k \in [K]} \overline{Y}_{k, t}$. 


In the following steps, we will bound $a_k$ and $b_k$ separately up to order $\log T$. Denote $\pr_{\xi}(A)$ is the probability of event $A$ concerning the law of $\xi$ and taking other quantities as deterministic. Recall that we denote two functions $a(s, T) \lesssim b(s, T)$ if $a(s, T) \leq c \times b(s, T)$ for some constant $c$ free of $s$ and $T$. 
And we write $a(s, T) \asymp b(s, T)$ if both $a(s, T) \lesssim b(s, T)$ and $a(s, T) \gtrsim b(s, T)$. 
The proof of all lemmas can be found in Appendix \ref{sec:proof_lemma}. 

\subsection{Bounding $a_k$}
%\red{Grammar: Should be split into two sentence. "(we) recall" is one and "it is" is another.}
%Recall that our target is bounding $a_k$ and $b_k$ up to order $\log T$, it is enough to show that {this can hold}
%for 
%{any large enough} $T$. 
For bounding $a_{k}$ with $C\times\log T$ for some constant $C > 0$, we will need first prove a weaker statement: $a_{k, s}$ as a function of $T$ can be upper bounded by some constants free of $T$. As we can see later, this is a critical intermediate step for proving $a_{k, s}$ has an order $\log T$.
%This is a   
%\red{$a_{k,s}$ is ONE constant, and bounded by constants? I know what you want to say. Just be more careful with these wordings. }
%weaker condition for $a_{k} \lesssim \log T$. 
%\blue{And we will see later control $a_{k, s}$ with a constant is a critical intermediate step to bound 
%\[
    %\log T \gtrsim a_k = \sum_{s = 0}^{T - 1} a_{k, s} \underbrace{\lesssim T}_{\text{by bounding $a_{k, s}$ with a constant.}}.
%\]}
%\red{Why we want to do this first? Tell readers the motivation/plan.}


Note that if we take
%\red{If one equation will not be cited, we should not give it an index}
\begin{equation}\label{requirement_0}
    \tau_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda},
\end{equation}
then we will have
\begin{equation}\label{constant_bound}
    \begin{aligned}
    	a_{k, s} & = \E \left[ \left( \frac{1}{Q_{1, s}(\tau_k)}  - 1\right) \wedge T \right] \\
    	(\text{by } Q_{1, s}(\cdot) \text{ is decreasing})&\leq \E \frac{1}{Q_{1, s}(\tau_k)} \leq \E Q_{1, s}^{-1} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right),
    \end{aligned}
\end{equation}
Hence, we need to find a lower bound of %\red{(Maybe I am wrong): lower bound is not a verb. Bound from below or sth else.} 
the tail probability $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2\lambda}\right) = \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right)$. And throughout the proof, we will use the choice of \eqref{requirement_0} for $\tau_k$, and we can take advantage of the bound \eqref{constant_bound}. 

For further analyzing \eqref{constant_bound}, we write it as the probability with respect to the weighted random summation of Gaussian random variable $\{ \omega_i, \omega_i', \omega_i''\}$.

\begin{lemma}\label{lemma:gaussian_weight}
    Suppose $\{x_i, y_i, z_i\}_{i = 1}^n \subseteq \mathbb{R}$ and $\{ \omega_i, \omega_i', \omega_i''\}_{i = 1}^n$ i.i.d. $\mathcal{N} (1, \sigma_{\omega}^2)$ random variables, then 
    \[
        \begin{aligned}
            & \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{ i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \right)\\
            \geq & \exp \left\{-\frac{3\left(S_{x}-S_{y}-S_{z}\right)^{2}}{2 \sigma_{\omega}^{2}\left(T_{x}+T_{y}+T_{z}\right)}\right\}\times\ind \left(S_{x} \geq S_{y}+S_{z}+\sqrt{2 \pi}\right)+(1-\Phi(\sqrt{2 \pi})) \times\ind \left(S_{x} \leq S_{y}+S_{z}+\sqrt{2 \pi}\right),
    \end{aligned}
    \] 
    if $T_x + T_y + T_z \neq 0$. Furthermore, if $S_x + S_y + S_z \neq 0$, we will have 
    \[
        \begin{aligned}
            & \pr \left( \sum_{i = 1}^n x_i \omega_i > \sum_{ i = 1}^n y_i \omega_i' + \sum_{i = 1}^n z_i \omega_i'' \right)\\
            \geq & \exp \left\{-\frac{3\left(S_{x}-S_{y}-S_{z}\right)^{2}}{2 \sigma_{\omega}^{2} / n \left(S_x + S_y + S_z\right)^2}\right\} \times\ind \left(S_{x} \geq S_{y}+S_{z}+\sqrt{2 \pi}\right)+(1-\Phi(\sqrt{2 \pi})) \times\ind \left(S_{x} \leq S_{y}+S_{z}+\sqrt{2 \pi}\right),
        \end{aligned}
    \] 
    where $S_x = \sum_{i = 1}^n x_i$ and $T_x = \sum_{i = 1}^n x_i^2$. And $S_y, S_z, T_y, T_z$ are similarly defined. 
\end{lemma}

And we first consider the case that $\mu_1 \neq {1} / {2}$. By applying Lemma \ref{lemma:gaussian_weight}
\[
    \begin{aligned}
        & Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) \\
        = & \pr \left( \overline{Y}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} \mid \his_{1, s}\right) \\
        = & \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \big( (2 \lambda + 1) R_{1, i} - (\mu_1 + \lambda) \big)\omega_i > \lambda (\mu_1 - 1 - \lambda) \sum_{i = 1}^s \omega_i' + \lambda (\lambda + \mu_1) \sum_{i = 1}^s \omega_i'' \right).
    \end{aligned}
\]
Let $x_i := (2 \lambda + 1) R_{1, i} - (\mu_1 + \lambda)$, $y_i := \lambda (\mu_1 - 1 - \lambda) $, $z_i :=  \lambda (\lambda + \mu_1) $ for $i \in [s]$, then
\[
    S_x = \sum_{i = 1}^s x_i = s \big( (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big), \quad S_y = \sum_{i = 1}^s y_i = s \lambda (\mu_1 - 1 - \lambda), \quad S_z = \sum_{i = 1}^s z_i = s \lambda (\lambda + \mu_1),
\]
with $S_x - S_y - S_z = s (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1)$ and
\[
    T_x = \sum_{i = 1}^s x_i^2 = \sum_{i = 1}^s \big[  (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big]^2, \quad T_y = \sum_{i = 1}^s y_i^2 = s \lambda^2 (\mu_1 - 1 - \lambda)^2, \quad T_z = \sum_{i = 1}^s z_i^2 = s \lambda^2 (\lambda + \mu_1)^2,
\]
with $T_x + T_y + T_z = \sum_{i = 1}^s \big[  (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big]^2  + s \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]$. Hence, by applying the first inequality in Lemma \ref{lemma:gaussian_weight} and use the fact that $T_x + T_y + T_z \geq T_x \geq S_x^2 / s$\footnote{If one use $T_x + T_y + T_z \geq T_x$, one cannot give a valid tuning condition.}.
\[
    \begin{aligned}
        & Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) \\
        = & \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s x_i \omega_i > \sum_{i = 1}^s y_i \omega_i' + \sum_{i = 1}^s z_i \omega_i'' \right) \\
        \geq & \exp \left\{-\frac{3s^2 (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2}\left(T_{x}+T_{y}+T_{z}\right)}\right\}\times\ind \left(s (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) \geq \sqrt{2 \pi}\right) \\
        & ~~~~~~~~~~~~~~~~~~~~~~~~~ + (1-\Phi(\sqrt{2 \pi})) \times\ind \left(s (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) \leq \sqrt{2 \pi} \right) \\
        \alignedoverset{T_x + T_y + T_z \geq S_x / s}{\geq} \exp \left\{-\frac{3(2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2} s \big( (2 \lambda + 1) \overline{R}_{1, s} - (\mu_1 + \lambda) \big)^2 }\right\}\times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}   \\
        & ~~~~~~~~~~~~~~~~~~~~~~~~~ + (1-\Phi(\sqrt{2 \pi})) \times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} 
    \end{aligned}
\]
%which gives the lower bound of $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)$ in the last step.
%where the $\geq$ is by the following lemma.
%\red{1. ", by"; 2. equations are also part of the sentence. Avoid a long sentence. Try something like ". the equality/inequality is due to the following lemma."}
Then this result combined with the fact \eqref{constant_bound} gives the upper bound for $a_{k, s}$ as
%\[
    %\begin{aligned}
        %a_{k, s} & \leq \E \exp \left\{\frac{3s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2} \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]}\right\}\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        % ~~~~~~~~~~~~~~~~~~~~~~~~ + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times \pr \left( \overline{R}_{1, s} - \mu_1 \leq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \\
        %\leq \E \exp \left\{\frac{3s (2 \lambda + 1)^2 (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^{2} \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]}\right\}\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}
    %\end{aligned}
%\]
\begin{equation}\label{a_k_constant_2}
    \begin{aligned}
        a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        & ~~~~~~~~~~~~~~ + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times \pr \left( \overline{R}_{1, s} - \mu_1 \leq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \\ 
        & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times\ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \ind \left( \mu_1 > \frac{1}{2} \right) \\
        & ~~~~ + \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right)  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        & = : I + II + III, 
        %& \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \\
        %& \qquad + \E \exp \left\{ \frac{3 \pi }{\sigma_{\omega}^2 \big[ (1 + 2 \lambda) \overline{R}_{1, s} - (\mu_1 + \lambda)\big]^2}\right\} 1 \left\{ \mu_1 \leq \frac{1}{2} - \frac{\sqrt{2 \pi}}{2 s \lambda}\right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        %& \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        %& \qquad \qquad \qquad \qquad \qquad \qquad + \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < \frac{1}{2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
        %& \leq  \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} 1\left\{ \mu_1 > \frac{1}{2} \right\} 1 \left\{ \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
        %& \qquad \qquad \qquad \qquad \qquad \qquad  + \max_{s \in \mathbb{Z}} \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < \frac{1}{2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        %& \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}
    \end{aligned}
\end{equation}
where $III = \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}$ is a constant. We will bound $I$ and $II$ as follows. 
\begin{itemize}
	\item Bounding $I$: 
	\[
	    \begin{aligned}
	    	I & = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \times\ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	   \alignedoverset{\overline{R}_{1, s} > \mu_1 > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \text{ when } \mu_1 > \frac{1}{2}}{\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \mu_1 +\frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 \ind \left( \overline{R}_{1, s}  \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) }\right\} \\
	    	   %\alignedoverset{\lambda(2 \mu_1 - 1) + \sqrt{2 \pi} / s > 0 \text{ when } \mu_1 > 1 / 2}{\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \\
	    	   %& ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 + \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	  %& \overset{\text{by using both event in the first two indicators}}{=} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2 \ind \left( \overline{R}_{1, s}  > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)}{2 \sigma_{\omega}^2  \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2  }\right\} \\
	    	  %& ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 + \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \ind \left(  \mu_1 > \frac{1}{2} \right) \\
	    	  %& {\leq} \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2  \left(  \mu_1 +\frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 \ind \left( \overline{R}_{1, s}  \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) }\right\} \\
	    	  & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \times\ind \left( \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)  \ind \left(  \mu_1 > \frac{1}{2} \right)\\
	    	  \alignedoverset{\text{by using } \mu_1 > \frac{1}{2}}{\leq} \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\}  \ind \left( \overline{R}_{1, s }- \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \ind \left(  \mu_1 > \frac{1}{2} \right).
	    \end{aligned}
	\]
	
	\item Bounding $II$: 
	
	%Consider two cases: 
	
	%(i) \textit{If $R_{1, s} - \mu_1$ is symmetric about $0$}, then
	%\[
	    %\begin{aligned}
	    	%II & = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%& = \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \mu_1 + \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%\alignedoverset{\text{by symmetry}} = \E \exp \left\{ \frac{3 s (\mu_1 - \overline{R}_{1, s})^2}{2 \sigma_{\omega}^2 \left((\mu_1 - \overline{R}_{1, s})  +  \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)^2 }\right\} \times \ind \left( \mu_1 - \overline{R}_{1, s} > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right)  \\
	    	%\alignedoverset{\text{by } \frac{\mu_1 + \lambda}{1 + 2 \lambda} > \mu_1}{\geq} \E \exp \left\{ \frac{3 s (\mu_1 - \overline{R}_{1, s})^2}{2 \sigma_{\omega}^2 \left( \mu_1 - \frac{\mu_1 + \lambda}{1 + 2 \lambda} + \frac{\sqrt{2\pi}}{s (2\lambda + 1)}\right)^2 }\right\} \times \ind \left( \mu_1 - \overline{R}_{1, s} > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)  \ind \left( \mu_1 < \frac{1}{2} \right) \\
	    	%& = \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ - \lambda (1 - 2\mu_1) + \sqrt{2 \pi} / s\big]^2}\right\}  \ind \left( \mu_1 - \overline{R}_{1, s }\geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right) \ind \left(  \mu_1 < \frac{1}{2} \right).
	    %\end{aligned}
	%\]
	
	
	%(ii) \textit{If $R_{1, s} - \mu_1$ is not symmetric about $0$.} 
	We first note under the indicator $\ind\left(\overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right)$, we have
	\[
	    \overline{R}_{1, s} > \mu_1 + \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} > \mu_1.
	\]
	The basic idea is the fact that $\E X = \int_0^{\infty} \pr (X > r) \, \mathrm{d} r$ for any positive $X$. Hence, for any $r > 0$,  we consider set that 
	\[
	    \begin{aligned}
	    	E(r, s) & := \left\{ \overline{R}_{1, s} - \mu_1: \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} > r \right\} \\
	    	& = \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r\right\}.
	    \end{aligned}
	\]
	We need to divide the analysis into two cases: (i) $\overline{R}_{1, s} \geq \frac{\mu_1 + \lambda}{1 + 2 \lambda} $ and (ii)
	$\overline{R}_{1, s} < \frac{\mu_1 + \lambda}{1 + 2 \lambda} $ respectively. We first prove the case (i) since it is easier. Note that 
	\begin{equation}\label{a_k_constant_II_case1}
		\overline{R}_{1, s} > \frac{\mu_1 + \lambda}{1 + 2\lambda} > \mu_1
	\end{equation}
	when $\mu_1 < \frac{1}{2}$. Hence we can write $E(r, s)$ on condition \eqref{a_k_constant_II_case1} as
	\[
	    \begin{aligned}
	    	E(r, s) \alignedoverset{\text{by \eqref{a_k_constant_II_case1}}}{=} \left\{  \overline{R}_{1, s} - \mu_1 : \frac{\sqrt{3 s} (\overline{R}_{1, s} - \mu_1)}{\sqrt{2} \sigma_{\omega} \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)} > \sqrt{\log r}\right\} \\
	    	& = \left\{  \overline{R}_{1, s} - \mu_1 : \sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} > \left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right) (\overline{R}_{1, s} - \mu_1) \right\} \\
	    	& = \left\{ \begin{array}{ll}
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} > 0 >  \left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right) (\overline{R}_{1, s} - \mu_1) \right\}, & r \leq \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}, \\
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \frac{\sqrt{2 \log r} \sigma_{\omega} \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}}{\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} > (\overline{R}_{1, s} - \mu_1) \right\}, & r > \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} 
	    	\end{array}\right. \\
	    	\alignedoverset{\text{by \eqref{a_k_constant_II_case1} again}}{=} \left\{ \begin{array}{ll}
	    		\left\{ \overline{R}_{1, s} - \mu_1 \in \mathbb{R} \right\}, & r \leq \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}, \\
	    		\left\{  \overline{R}_{1, s} - \mu_1 : \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} > (\overline{R}_{1, s} - \mu_1) \right\}, & r > \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} 
	    	\end{array} \right. 
	    \end{aligned}
	\]
	Then,
	\[
	    \begin{aligned}
	    	II & = \int_0^{\infty} \pr \left( E(r, s) \, \cap \, \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& = \left[ \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} + \int_{\exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}}^{\infty} \right] \pr \left( E(r, s) \, \cap \, \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& = II_1 + II_2.
	    \end{aligned} 
	\]
	We first bound $II_2$. Write $II_2$ as
	\[
	    II_2 = \int_{\exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}}^{\infty} \pr \left( \frac{\lambda(1 - \mu_1)}{1 + 2 \lambda} < \overline{R}_{1,s} - \mu_1 <  \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} \right) \, \mathrm{d} r.
	\]
	By letting $s \longrightarrow \infty$,
	\[
	    \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\} \, \uparrow \, \infty, \qquad \left\{ \frac{\lambda(1 - \mu_1)}{1 + 2 \lambda} < \overline{R}_{1,s} - \mu_1 <  \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \frac{\sqrt{2 \log r} \sigma_{\omega}} {\left( \sqrt{2 \log r} \sigma_{\omega} - \sqrt{3 s}\right)} \right\}  \, \downarrow \, \varnothing,
	\]
	hence we have $II_2 \longrightarrow 0$. This implies  there exist $T_1 \in \mathbb{N}$ such that $II_2 \leq 1$ for any $s \geq T_1$. And for $II_1$, we take advantage of sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	II_1 & = \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( E(r, s) \ind \left\{ \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right\} \right) \, \mathrm{d} r \\
	    	& \leq \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( \overline{R}_{1,s} > \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right) \, \mathrm{d} r \\
	    	& \leq \int_0^{ \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}} \pr \left( \overline{R}_{1,s} - \mu_1 > \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda} \right) \, \mathrm{d} r \\
	    	\alignedoverset{\text{by sub-Gaussian inequality}}{\leq} \exp \left\{ \frac{3s}{2 \sigma_{\omega}^2}\right\}  \cdot \exp \left\{ - \frac{\lambda^2 (1 - 2 \mu_1)^2 s}{2 (1 + 2 \lambda)^2 \sigma_1^2}\right\} \\
	    	& = \exp \left\{ \left[ \frac{3}{2 \sigma_{\omega}^2} - \frac{\lambda^2 (1 - 2 \mu_1)^2}{2 (1 + 2 \lambda)^2 \sigma_1^2} \right] s \right\}.
	    \end{aligned}
	\]
	Therefore, for making $II_1$ have a upper a constant    free of $s$, a sufficient condition is
	\[
	    \frac{3}{2 \sigma_{\omega}^2} - \frac{\lambda^2 (1 - 2 \mu_1)^2}{2 (1 + 2 \lambda)^2 \sigma_1^2} \geq 0
	\]
	i.e.
	\begin{equation}\label{tuning_case_1}
		\lambda > \frac{\sqrt{3}\sigma_1}{(1 - 2\mu_1) \sigma_{\omega} - 2 \sqrt{3}\sigma_1} \qquad  \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{3} \sigma_1}{1 - 2\mu_1}.
	\end{equation}
	Combining these results, we conclude that if take \eqref{tuning_case_1}, we have $II \leq 2$ for any $s \geq T_1$. Now switching to case (ii). In case (ii), we will have:
	\begin{equation}\label{a_k_constant_II_fact1}
		\frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s} > 0 \qquad \text{ and } \qquad \frac{\sqrt{2 \pi}}{s(2 \lambda + 1)} < \overline{R}_{1, s} - \mu_1 < \frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}.
	\end{equation}
	\[
	    \begin{aligned}
	    	E(r, s) & = \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r\right\} \\
	    	(\text{use \eqref{a_k_constant_II_fact1}}) & \subseteq \left\{  \overline{R}_{1, s} - \mu_1 : \frac{3 s (\overline{R}_{1, s} - \mu_1)^{2 - \epsilon}}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2} > \log r \left[\frac{\lambda(1 - 2 \mu_1)}{1 + 2 \lambda}\right]^{-\epsilon}\right\} \\
	    	& =  \left\{  \overline{R}_{1, s} - \mu_1 : \left[ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r}\right]^{2 - \epsilon} > \left[ \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right]^2\right\} \\
	    	& =  \left\{  \overline{R}_{1, s} - \mu_1 : \left[ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r}\right]^{1 - \frac{\epsilon}{2}} > \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right\}
	    \end{aligned}
	\]
	For any $0 < \epsilon < 2$. Specially, we take $\epsilon = 1$, and 
	%We take $1 < \epsilon < \frac{4}{3}$, then $\frac{1}{3} < 1 - \frac{\epsilon}{2} < 1$ and $5 - 3\epsilon > 1$ . And denote the event
	\[
	    F(r, s) := \left\{ \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^{3} r} \geq 1 \right\},
	\]
	then
	\[
	    \begin{aligned}
	    	II & = \int_0^{\infty} \pr \left\{ E (r, s)  \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right) \right\} \, \mathrm{d} r \\
	    	& \leq \int_0^{\infty} \left[\pr \left\{ \big[ E (r, s) \, \cap  \, F(r, s) \big] \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right) \right\} + \pr \left\{ \big[ F(r, s)^c \big] \ind \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)\right\} \right]\, \mathrm{d} r \\
	    	& =: II_1 + II_2.
	    \end{aligned}
	\]
	For $II_2$, we write that
	\[
	    \begin{aligned}
	    	II_2 & \leq \int_0^{\infty} \pr \left\{ \big[ F(r, s)^c \big] \, \cap \, \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right)\right\}\, \mathrm{d} r  \\
	    	& = \int_0^{\infty} \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \left[ \int_0^{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}} + \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \right] \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, \mathrm{d}r.
	    \end{aligned}
	\]
	For $II_2$, we write that
	\[
	    \begin{aligned}
	    	II_2 & = \int_0^{\infty} \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \left[ \int_0^{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}} + \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \right] \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \, \mathrm{d}r \\
	    	& = \int_{\exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, \mathrm{d}r.
	    	%\\
	    	%& \leq \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty}  \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \log^{\frac{1}{2}} r  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{\frac{1}{2}} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right)  \, dr \\
	    	% & \leq \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\}}^{\infty} \exp \left\{ - \frac{\log r}{2 (3s)^{\frac{2}{2 - \epsilon}} \sigma_1^2}\right\} \, dr \\
	    	% & = 1 + \int_{\exp\left\{ \frac{2 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{- \frac{2(1 - \epsilon)}{2 - \epsilon}}\right\}}^{\infty} r^{- \frac{1}{2 (3s)^{\frac{2}{2 - \epsilon}} \sigma_1^2}} \, dr  
	    \end{aligned}
	\]
	By letting $s \longrightarrow \infty$, we have 
	\[
	    \exp\left\{ \frac{2 \cdot 3^{\frac{2}{2 - \epsilon}}}{(1 + 2 \lambda)} s^{\frac{2(\epsilon - 1)}{2 - \epsilon}}\right\} \longrightarrow \infty, \qquad \pr \left( \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  < \overline{R}_{1, s} - \mu_1 < \frac{\log^{3} r}{(3s)^{\frac{1}{2 - \epsilon}}}\right) \longrightarrow 0.
	\]
	Thus, $II_2$ shows we must have $II_2 \leq 1$ bounded by a constant free of $s$ for enough big $s$, say $s \geq T_2$.
	And for $II_1$, we take advantage that $x \geq x^{1 - \frac{\epsilon}{2}}$ for $x > 1$ and $0 < 1 - \frac{\epsilon}{2}< 1$, 
	\[
	    \begin{aligned}
	    	& E(r, s) \, \cap \, F(r, s) \\
	    	\subseteq & \left\{  \overline{R}_{1, s} - \mu_1 :  \frac{(3 s)^{\frac{1}{2 - \epsilon}} (\overline{R}_{1, s} - \mu_1)}{\log^3 r} > \frac{\sqrt{2} \sigma_{\omega}\left( \frac{1 + 2 \lambda}{\lambda(1 - 2 \mu_1)}\right)^{\frac{\epsilon}{2}}\left( \frac{\mu_1 + \lambda}{1 + 2 \lambda} - \overline{R}_{1, s}\right)}{\log^{\frac{5 - 3\epsilon}{2}} } \right\} \\
	    	= & \left\{  \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right\}.
	    \end{aligned}
	\]
	and in turn, we have
	\[
	    \begin{aligned}
	    	 & \big[ E(r, s) \, \cap \, F(r, s) \big] \ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \\
	    	 %\subseteq &  \left\{  \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}  \vee\frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right\} \\
	    	 \subseteq & \left\{ \begin{array}{ll}
	    	 	\varnothing, & r \leq \overline{r}_1 (s) \\
	    	 	\left\{ \overline{R}_{1, s} - \mu_1 : \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right\}, & r > \overline{r}_1(s) 
	    	 \end{array}\right..
	    \end{aligned}
	\]
	where
	\[
	    \overline{r}_1 (s) := \exp \left\{ \left[ \frac{\sqrt{2 \pi}}{\left[ \sqrt{2} \lambda (1 - 2 \mu_1) - 2 \sqrt{\pi} / s\right] \sigma_{\omega}}\right]^{\frac{2}{1 + 3 \epsilon}} \left( \frac{\lambda (1 - 2\mu_1)}{1 + 2\lambda} \right)^{\frac{\epsilon}{1 + 3 \epsilon}} (3s)^{\frac{2(\epsilon - 1)}{(2 - \epsilon)(1 + 3 \epsilon)}}  \right\}.
	\]
	Therefore, 
	\[
	    \begin{aligned}
	    	II_1 & = \left[ \int_{0}^{\overline{r}_1(s)} + \int_{\overline{r}_1(s)}^{\infty} \right] \pr \left( \big[ E(r, s) \, \cap \, F(r, s) \big] \ind \left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \right) \, \mathrm{d} r \\
	    	& \leq \int_{0}^{\overline{r}_1(s)} \pr \left(  \varnothing \right) \, \mathrm{d} r + \int_{\overline{r}_1(s)}^{\infty} \pr \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_1(s)}^{\infty} \pr \left( \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right) \, \mathrm{d} r.
	    \end{aligned}
	\]
	Then, by sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	II_1 & \leq \int_{\overline{r}_1(s)}^{\infty} \exp \left( - \frac{s}{2 \sigma_1^2} \left[ \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r} \right]^2\right) \, \mathrm{d} r \\
	    	\alignedoverset{\text{Cauchy inequality}}{\leq}\int_{\overline{r}_1(s)}^{\infty}  \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r\\ 
	    	& = \left[ \int_{\overline{r}_1(s)}^{\overline{r}_2(s)} + \int_{\overline{r}_2(s)}^{\infty} \right] \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& =: II_{11} + II_{12},
	    \end{aligned}
	\]
	where
	\[
	    \overline{r}_2(s) := \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}} s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}}\right\} 
	\]
	is a higher order of $\overline{r}_1(s)$ due to $0 < 2 (\epsilon - 1) < 2$. For $II_{12}$, 
	\[
	    \begin{aligned}
	    	II_{12} & \leq \int_{\overline{r}_2(s)}^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{2 \cdot 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_2(s)}^{\infty} \exp \left\{ - \frac{s}{8 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2} \right\} \, \mathrm{d} r \, \longrightarrow \, 0
	    \end{aligned}
	\]
	when $s \, \longrightarrow \, \infty$. Thus, there exists a $T_3$ such that, $II_{12} \leq 1$ whenever $s \geq T_3$. Finally, for $II_{11}$, 
	\[
	    \begin{aligned}
	    	II_{11} & \leq \int_{\overline{r}_1(s)}^{{\overline{r}_2(s)}} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{2 \cdot 3^{\frac{2}{2-\epsilon}} s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r}\right) \, \mathrm{d} r \\
	    	& = \int_{\overline{r}_1(s)}^{{\overline{r}_2(s)}} \exp \left\{  - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} r s^{\frac{- \epsilon}{2 - \epsilon}} \right\} \\
	    	& \leq \overline{r}_2(s) \exp \left\{  - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} s^{\frac{- \epsilon}{2 - \epsilon}} \big[ \log \overline{r}_2(s) \big]^{1 + 3\epsilon} \right\} \\
	    	& = \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}} s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}} - \frac{\sigma_{\omega}^2}{4 \cdot 3^{\frac{2}{2-\epsilon}}  \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} s^{\frac{- \epsilon}{2 - \epsilon}} \big[ \log \overline{r}_2(s) \big]^{1 + 3\epsilon}  \right\} \\
	    	& = \exp \left\{C_1 \cdot s^{\frac{2}{(2 - \epsilon)(1 + 3 \epsilon)}} - C_2 \cdot s \right\} \, \longrightarrow \, 0
	    \end{aligned}
	\]
	when $s \, \longrightarrow \, \infty$, where $C_1$ and $C_2$ are some positive constants free of $s$. Again, when $s \, \longrightarrow \, \infty$. Thus, there exists a $T_4$ such that, $II_{11} \leq 1$ whenever $s \geq T_4$.
	\iffalse
	\red{
	Therefore, by sub-Gaussian inequality,
	\[
	    \begin{aligned}
	    	& \pr \left( E(r, s) \, \cap \, F(r, s)  \, \cap \,\left\{ \overline{R}_{1, s} - \mu_1 > \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)} \right\} \right)\\
	    	& = \pr \\
	    	& \leq 1 + \int_1^{\infty} \exp \left( - \frac{s}{2 \sigma_1^2} \left[ \frac{\sqrt{2}\sigma_{\omega} \log^3 r\left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{1 - \frac{\epsilon}{2}}} {(3s)^{\frac{1}{2 - \epsilon}} \log^{\frac{5 - 3\epsilon}{2}} r + \sqrt{2}\sigma_{\omega} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{ - \frac{\epsilon}{2}} \log^3 r}\right]^2 \right) \, \mathrm{d}r \\
	    \alignedoverset{\text{Cauchy inequality}}{\leq} 1 + \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r\\
	    	& = 1 + \left[ \int_1^{\overline{r}(s)} +\int_{\overline{r}(s)}^{\infty}\right] \exp \left(  - \frac{\sigma_{\omega}^2}{2 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \frac{s \log^6 r}{3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r + 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}}\right) \, \mathrm{d} r \\
	    	& = : 1 + II_{21} + II_{22}:
	    \end{aligned}
	\]
	where $\overline{r}(s)$ is defined as 
	\[
	     \overline{r}(s) := \exp \left\{ \left[ \left( \frac{\lambda(1 - 2\mu)}{1 +2 \lambda} \right)^{\epsilon}\frac{3 s^{\frac{2}{2 - \epsilon}}}{2 \sigma_1^2}\right]^{\frac{1}{1 + 3 \epsilon}}\right\}.
	\]
	For $r \leq \overline{r}(s)$, we have $3 s^{\frac{2}{2-\epsilon}} \log^{5 - 3 \epsilon} r \geq 2 \sigma_{\omega}^2 \log^6 r \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{- \epsilon}$, hence
	\[
	    \begin{aligned}
	    	II_{21} & \leq \int_1^{\overline{r}(s)} \exp \left(  - \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} rs^{\frac{2(1 - \epsilon)}{2 - \epsilon}}\right) \, d r \\
	    	& \leq \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 + 3\epsilon} r s^{\frac{2(1 - \epsilon)}{2 - \epsilon}}\right) \, d r \\
	    	& \overset{\text{take } s = 1}{\leq}  \int_1^{\infty} \exp \left(  - \frac{\sigma_{\omega}^2}{6 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon} \log^{1 } r\right) \, d r \\
	    	& = \int_1^{\infty} r^{-  \frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2 - \epsilon}} \, d r
	    \end{aligned}
	\]
	Therefore, for making $II_{21}$ have a upper bound free of $s$, a sufficient condition is 
	\[
		\frac{\sigma_{\omega}^2}{12 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda} \right]^1 > 1
	\]
	i.e.
	\begin{equation}\label{tuning_sigma}
	    \lambda > \frac{12 \sigma_1^2}{(1 - 2\mu_1) \sigma_{\omega}^2 - 24 \sigma_1^2} \qquad \text{ and } \qquad \sigma_{\omega} > \frac{2 \sqrt{6} \sigma_1}{1 - 2\mu_1}
	\end{equation}	
	For $II_{22}$, we have
	\[
	    \begin{aligned}
	    	II_{22} \leq \int_{\overline{r}(s)}^{\infty} \exp \left\{ - \frac{1}{4 \sigma_1^2} \left[ \frac{\lambda (1 - 2 \mu_1)}{1 + 2\lambda}\right]^{2} s^2\right\} \, dr \longrightarrow 0
	    \end{aligned}
	\]
	when $s \longrightarrow \infty$, {there exist a $T_1$ such that $s \geq T_1$, $II_{22} < 1$.}}
	\fi
\end{itemize}
%Plug the above two bounds into \eqref{a_k_constant_2}, we obtain that
From the above expression, for proving $a_{k, s}$ is bounded by a constant free of $s$, it remains to show the expectation
\begin{equation}\label{a_k_constant_3}
	\E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \ind \left(  \mu_1 > \frac{1}{2} \right)
\end{equation}
%\begin{equation}\label{a_k_constant_3}
	%\begin{aligned}
		%a_{k, s} \leq \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \ind \left(\mu_1 \neq \frac{1}{2}\right) + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
	%\end{aligned}
%\end{equation}
%with $\mu_1 \neq \frac{1}{2}$ is bounded by a constant free of $s$.
%For bounding the expectation in \eqref{a_k_constant_3}, 
We need the following lemma.
%It can be seen that this upper bound consists {of} three parts: the first part is the moment generation function (MGF) of the square of the sample mean $\overline{R}_{1, s} - \mu_1$, the second part is a function of $(\mu_1, \lambda, \sigma_{\omega}^2)$, and the third part is just a constant $\big[ 1 - \Phi(\sqrt{2 \pi}) \big]^{-1} $. Note that as long as $\frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)}$ is not an integer, the second part must be a finite number free of $s$. It remains to deal with the first part, we use the following lemma.

%Now for $\mu_1 \neq 1 / 2$, notice that ${R}_{1, i} - \mu_1$ for $i \in [s]$ is sub-Gaussian. 
%For dealing with the expectation, we need the following lemma.
%\red{Same comment as above. The sentence is just too long. Imagine you are presenting. We need rests between sentences. }
% by the fact with the following lemma.
\begin{lemma}\label{lem_subGtosubE}
    Suppose $\{X_i\}_{i = 1}^n$ are i.i.d. zero-mean sub-Gaussian with variance proxy $\sigma^2$, and $\overline{X} = \frac{1}{n} \sum_{i = 1}^n X_i$, then
    \[
        \E \exp\left\{ \lambda\overline{X}^2 \right\} \leq e^{9 / 8}
        %\exp \left\{ \frac{64 \lambda^2 \sigma^4}{n^2} + \frac{\lambda \sigma^2}{n}\right\}, \qquad \forall \, |\lambda| \leq \frac{n}{8 \sqrt{2} \sigma^2}
    \]
    for any $|\lambda| \leq \frac{n}{8 \sigma^2}$.
\end{lemma}
Lemma \ref{lem_subGtosubE} ensures the expectation in \eqref{a_k_constant_3}
%\[
    %\begin{aligned}
    	%& \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2}\right\} \\
    	%= & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2} \cdot (\overline{R}_{1, s} - \mu_1)^2 \right\} \leq e^{9 / 8}.
    %\end{aligned}
%\]
\[
    \begin{aligned}
        & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2}\right\} \ind \left( \mu_1 > {1} / {2} \right) \\
        = & \E \exp \left\{ \frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2} \times(\overline{R}_{1, s} - \mu_1)^2 \right\} \ind \left( \mu_1 > {1} / {2} \right)  \leq e^{9/8} \times\ind \left( \mu_1 > {1} / {2} \right)
    \end{aligned}
\]
as long as we take
%\begin{equation}\label{cond.1}
    %\frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2} \leq \frac{s}{8 \sigma_1^2}.
%\end{equation}
\begin{equation}
\label{cond.1}
    \frac{3 s (1 + 2 \lambda)^2}{2 \sigma_{\omega}^2 \big[ \lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s\big]^2} \leq \frac{s}{8 \sigma_1^2}.
\end{equation}
%we will obtain $a_{k, s}$ is bounded by 
%\begin{equation}\label{a_k_constant}
    %a_{k, s} \leq e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
%\end{equation}
%\red{If time permits, we should polish the proof for several more times to address issues as raised above.}
%\begin{remark}
   %Lemma \ref{lem_subGtosubE} actually is a special case for the fact that the mean of iid sub-Weibull sample with sample size $n$ will have the local sub-Gaussian property in the interval up to $\sqrt{n}$.
%\end{remark}
%{\color{blue}{More details about the tuning parameters. }}
The condition \eqref{cond.1} is equal to 
%\begin{equation}\label{tuning_condition}
    %\frac{3 (2 \lambda + 1)^2 s }{2 \sigma_{\omega}^2 \big[ \lambda^2 (\mu_1 - 1 - \lambda)^2 + \lambda^2 (\lambda + \mu_1)^2\big]^2}  \leq \frac{\sigma_{\omega}}{2 \sigma_1}.
%\end{equation}

%for bound $a_{k, s}$ with a constant, we write the inequality with regarding $\lambda$ as
%\begin{equation}\label{tuning_condition}
    %\big[ (2 \mu_1 - 1)^2 \sigma_{\omega}^2 - 48 \sigma_1^2 \big] \lambda^2 - 2 \big[ 24 \sigma_1^2 - \sqrt{2 \pi} / s (2 \mu_1 - 1) \sigma_{\omega}^2\big] \lambda - \big[ 12 \sigma_1^2 - (2 \pi / s^2) \sigma_{\omega}^2 \big] \geq 0. 
%\end{equation}
%\begin{equation}\label{tuning_condition}
    %\big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big] \lambda \geq 2 \sigma_1.
%\end{equation}
\begin{equation}\label{tuning_condition}
    \frac{\sqrt{3} (1 + 2 \lambda)}{\lambda (2 \mu_1 - 1) + \sqrt{2 \pi} / s } \leq \frac{\sigma_{\omega}}{2 \sigma_1}.
\end{equation}
Hence it is enough to ask $\lambda (2 \mu_1 - 1) > {2 \sqrt{3} \sigma_1} (1 + 2 \lambda) / \sigma_{\omega}$, i.e.
    \[
        \lambda \left[ 2 \mu_1 - 1 - \frac{4 \sqrt{3} \sigma_1}{\sigma_{\omega}}\right] >  \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}}.
	\]
Solving the above inequality for positive $\lambda$ and $\sigma_{\omega}$ and we get that 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}.
	\]
\iffalse
\begin{itemize}
	\item If $\mu_1 > 1 / 2$, the above inequality is equal to 
	\[
	    \lambda (2 \mu_1 - 1) + \frac{\sqrt{2\pi}}{s} > \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}} (1 + 2 \lambda).
	\]
	And hence it is enough to ask $\lambda (2 \mu_1 - 1) > {2 \sqrt{3} \sigma_1} (1 + 2 \lambda) / \sigma_{\omega}$, i.e.
    \[
        \lambda \left[ 2 \mu_1 - 1 - \frac{4 \sqrt{3} \sigma_1}{\sigma_{\omega}}\right] >  \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}}.
	\]
	Solving the above inequality for positive $\lambda$ and $\sigma_{\omega}$ and we get that 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}.
	\]
	\item If $\mu_1 < 1 / 2$, the above inequality is equal to 
	\[
	    \lambda (1 - 2\mu_1) + \frac{\sqrt{2\pi}}{s} > \frac{2 \sqrt{3} \sigma_1}{\sigma_{\omega}} (1 + 2 \lambda).
	\]
	Similar to the case of $\mu_1 > 1 / 2$, the solution is 
	\[
	    \lambda > \frac{2 \sqrt{3} \sigma_1}{(1 - 2 \mu_1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {1 - 2 \mu_1}.
	\]
\end{itemize}
\fi
%Use the case $\mu_1 > 1 / 2$. 
%Since in this case, we already have $(2 \mu_1  - 1) > 0$ in the indicator, we can get the solution of \eqref{cond.1} as follows

%And solve it, and we can get regularity condition for tuning parameter $(\lambda, \sigma_{\omega}^2)$ is  
%\[
    %\sigma_{\omega}^2 > \frac{48 \sigma_1^2}{(2 \mu_1 - 1)^2}, \qquad \lambda \geq \frac{- \sqrt{2 \pi } \left(2 \mu _1-1\right) \sigma
   %_{\omega }^2 + 2 \sqrt{3} s \sqrt{\frac{\sigma _1^2 \left(4 \mu _1^2 s^2+s^2-4 \mu _1
   %\left(s+2 \sqrt{2 \pi }\right) s+4 \sqrt{2 \pi } s+8 \pi \right) \sigma _{\omega
   %}^2}{s^2}} + 24 s \sigma _1^2}{s \left(\left(1-2 \mu _1\right)^2 \sigma
   %_{\omega }^2 - 48 \sigma _1^2 \right)}
%\]
%i.e.
%\begin{equation}\label{tuning_condition_exact}
    %\sigma_{\omega}^2 > \frac{48 \sigma_1^2}{(2 \mu_1 - 1)^2}, \quad \lambda \geq  \frac{ - \sqrt{2 \pi } \left(2 \mu _1-1\right) \sigma _{\omega }^2+2 \sqrt{3}
    %\sqrt{\left(\left(4 \mu _1^2-\left(4+8 \sqrt{2 \pi }\right) \mu _1+4 \sqrt{2 \pi }+8
   %\pi +1\right) \sigma _1^2 \sigma _{\omega }^2\right)} + 24 \sigma _1^2}{\left(1-2 \mu _1\right){}^2 \sigma _{\omega }^2 - 48 \sigma
   %_1^2}.
%\end{equation}
Hence, in the case $\mu_1 \neq \frac{1}{2}$, we can take the tuning condition as 
\begin{equation}\label{tuning_condition_exact}
    \begin{aligned}
    	& \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1  - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1}, \qquad \text{ for } \qquad \mu_1 > \frac{1}{2} \\
    	& \lambda > \frac{\sqrt{3}\sigma_1}{(1 - 2\mu_1) \sigma_{\omega} - 2 \sqrt{3}\sigma_1} \qquad  \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{3} \sigma_1}{1 - 2\mu_1}, \qquad \text{ for } \qquad \mu_1 < \frac{1}{2}.
    \end{aligned}
\end{equation}	

\iffalse
\begin{equation}\label{tuning_condition_exact}
	\begin{aligned}
		 & \text{if the distribution of reward is symmetric:} \\
		 & ~~~~~~~~~~~~~~~~~~~~~ \lambda > \frac{2 \sqrt{3} \sigma_1}{|2 \mu_1 - 1| \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {|2 \mu_1 - 1|}  \\
	    & \text{if the distribution of reward is not symmetric} \\
	    & ~~~~~~~~~~~~~~~~~~~~~ \lambda > \frac{2 \sqrt{3} \sigma_1}{(2 \mu_1 - 1) \sigma_{\omega} - 4 \sqrt{3} \sigma_1} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sqrt{3} \sigma_1} {2 \mu_1 - 1} \qquad \text{ for } \mu_1 > \frac{1}{2} \\
	    & ~~~~~~~~~~~~~~~~~~~~~ \lambda >  \frac{12 \sigma_1^2}{(1 - 2\mu_1) \sigma_{\omega}^2 - 24 \sigma_1^2} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{2 \sqrt{6} \sigma_1}{1 - 2\mu_1} \qquad \text{ for } \mu_1 < \frac{1}{2}
	\end{aligned}
\end{equation}
\fi
%and \eqref{a_k_constant_3} will give $a_{k, s} \leq \Big[ e^{9 / 8} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \Big] \ind \left(\mu_1 \neq \frac{1}{2}\right)$.
%\begin{equation}\label{tuning_condition_exact}
    %\lambda \geq \frac{2 \sigma_1}{\big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big]} \qquad \text{ with } \qquad \sigma_{\omega} > \frac{4 \sigma_1}{2 \mu_1 - 1}.
%\end{equation}
%Directly, for the case $\mu_1 < 1 / 2$, we just need $\frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)} \in \mathbb{Z}$.
%This means under the case that $\mu_1 \neq 1 / 2$, if the tuning parameters $(\lambda, \sigma_{\omega}^2)$ satisfying \eqref{tuning_condition_exact}, the bound in \eqref{a_k_constant_2} will be further bounded by
%\begin{equation}\label{a_k_constant}
    %a_{k, s} \leq e^{9 / 8} 1 \{ \mu_1 > 1 / 2 \}  + \max_{s \in \mathbb{Z}} \exp \left\{ \frac{3 \pi}{\sigma_{\omega}^2 \big[  \sqrt{2 \pi} / s - \lambda (1 - 2 \mu_1) \big]^2} \right\} 1 \left\{ \mu_1 < {1} / {2}\right\} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
%\end{equation}

For the case $\mu_1 = \frac{1}{2}$, we analyze it separately, $Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right)$ will become
\[
    \begin{aligned}
        Q_{1, s} \left( \frac{\mu_1 + \lambda}{1 + 2 \lambda}\right) & = Q_{1, s} \left(\frac{1}{2}\right) \\
        & = \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \left( R_{1, i} - \frac{1}{2} \right) \omega_i > \frac{\lambda}{2} \sum_{i = 1}^s (\omega_i'' - \omega_i')  \right) \\
        & = \pr_{\omega, \omega', \omega''} \left( \sum_{i = 1}^s \big( R_{1, i} - \mu_1 \big) \omega_i > \frac{\lambda}{2} \sum_{i = 1}^s (\omega_i'' - \omega_i')  \right) \\
        & = \pr_Z \left( Z > \frac{- s(\overline{R}_{1, s} - \mu_1)}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right) \\
        & \geq \ind \left( \overline{R}_{1, s} - \mu_1 \geq 0 \right) \times\frac{1}{2} + \ind \left( \overline{R}_{1, s} - \mu_1 < 0 \right) \times\pr_Z \left( Z > \frac{ s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right).
    \end{aligned}
\]
where $Z \sim \mathcal{N}(0, 1)$ is the standard Gaussian variable. 
And then by the inequality $\pr (Z \geq x) \geq e^{-x^2} / 4$ for any $x > 0$ in \cite{zhang2022sharper}, we will have
\[
     \begin{aligned}
        & \pr_Z \left( Z > \frac{s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega}\sqrt{\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + \lambda^2 s  / 2}} \right) \\
        (\text{by Cauchy inequality})\geq & \pr \left( Z \geq \frac{s(\mu_1 - \overline{R}_{1, s})}{\sigma_{\omega} \sqrt{s (\mu_1 - \overline{R}_{1, s})^2 + \lambda^2 s  / 2}} \right)  \\
        \geq & \frac{1}{4} \exp\left\{ - \frac{s(\mu_1- \overline{R}_{1, s})^2}{4 (\mu_1- \overline{R}_{1, s})^2 + 2 \lambda^2} \right\}.
     \end{aligned}
\]
Therefore, by the fact \eqref{constant_bound} and Lemma \ref{lem_subGtosubE} again,
\[
    \begin{aligned}
        a_{k, s} & \leq Q_{1, s} \left(\frac{1}{2}\right) \\
        & \leq 2 \pr \left( \overline{R}_{1, s} - \mu_1 \geq 0 \right) + 4 \E \exp \left\{ \frac{s(\mu_1- \overline{R}_{1, s})^2}{4 (\mu_1- \overline{R}_{1, s})^2 + 2 \lambda^2} \right\} \\
        & \leq 2 + 4 \E \exp \left\{ \frac{s(\mu_1- \overline{R}_{1, s})^2}{ 2 \lambda^2} \right\} \\
        \alignedoverset{\text{apply Lemma \ref{lem_subGtosubE}}}{\leq} 2 \left( 1 + 2 e^{9 / 8} \right),
    \end{aligned}
\]
as long as we take
\[
    \frac{s}{2 \lambda^2} \leq \frac{s}{8 \sigma_1^2}
\]
which is equivalent to $\lambda \geq 2 \sigma_1$. 
%The result for $\mu_1 = \frac{1}{2}$ together with the results for the case $\mu_1 \neq \frac{1}{2}$, we get that for any $\mu_1 \in [0, 1]$, take 
%\begin{equation}\label{tuning_condition_exact_final}
    %\lambda \geq \frac{ 2 \sigma_1 1 (\mu_1 > 1 / 2) }{ \big[ (2 \mu_1 - 1) \sigma_{\omega} - 4 \sigma_1 \big]} + 2\sigma_1 1 (\mu_1 = 1 / 2) \quad \text{ and } \quad \frac{\sqrt{2 \pi}}{\lambda (1 - 2 \mu_1)} \not\in \mathbb{Z}_+ \quad \text{ with } \quad \sigma_{\omega} > \frac{4 \sigma_1}{2 \mu_1 - 1},
%\end{equation}

Combine the results for case of $\mu_1 \neq \frac{1}{2}$ and $\mu_1 = \frac{1}{2}$, $a_{k, s}$ has a constant upper bound as follows:
\begin{equation}\label{a_k_constant_final}
    \begin{aligned}
        a_{k, s} & \leq \big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) .
    \end{aligned}
\end{equation}

This step derives the restriction conditions of the tuning parameters in Theorem \ref{thm.MAB}. 
%The exact same situation appears in other papers of MAB theory: the condition of tuning parameters is derived and only used in the step of bounding $a_{k, s}$ with a constant free of $T$. See \cite{kveton2019garbage} and \cite{wu2022residual} for instance.

%which is the reason why we need the restriction of tuning parameters in the Theorem.
%with some $C \geq 0$. Hence, a sufficient condition for any tuning parameter $\lambda > 0$ is that $12 \sigma_1^2 / \sigma_{\omega}^2 \leq 1$ for any round $T \geq 2$. Or some bounded interval for $\lambda$ will be required when $12 \sigma_1^2 / \sigma_{\omega}^2 \geq 1$. To be specific, if $\sigma_1^2 = \sigma_{\omega}^2 = 1$, a sufficient condition for \eqref{tuning_condition} is $12 (2 \lambda + 1)^2 \leq C \left[ (\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2\right]$ for some $C \geq 0$. For instance, if $\mu_1 = 1$, we can take $C = 12$, then our theory will be valid if take the tuning parameter $\lambda \in (0, 1]$ whenever the total round $T \geq 12$.

%{$\sigma_k^2 \in (0, 1]$ for $k \in [K]$ and $\sigma_{\omega}^2 = 1$}

%\textbf{$\leq sth. \log T$ holds for $T \geq C$. When $T < C$, take $sth.$ large enough we can still get the order $\log T$.
%}

%{$\lambda$ cannot depend on unknown variable}

%For instance, if we just take $\mu_1 = 1/2$, we will need $\sigma_{\omega}^2 \geq 24 \sigma_1^2$ with any $\lambda > 0$.

%\textit{sub-Gaussian parameter can be assumed to in $[0, 1]$, then we can solve the bound off $\lambda$. }

%\begin{remark}
   %Different from the bounded rewards setting, here $\lambda$ together with the bound of $\mu_1$ as well as $\sigma_{\omega}^2$ and $\sigma_k^2$ establish the restriction condition for the tuning parameters. But \eqref{tuning_condition_exact} can be served as a sufficient condition.
%\end{remark}

%\begin{remark}
   %It can be shown that for bounded rewards, we can use any positive $\lambda$ and $\sigma_{\omega}^2$ to ensure that $a_{k, s}$ can be bounded by a constant free of $T$. 
%\end{remark}

Next, we decompose $a_{k, s}$ as $a_{k, s} = a_{k, s, 1} + a_{k, s, 2} + a_{k, s, 3}$, and we can focus on these simpler components $a_{k, s, j}$ for $j = 1, 2, 3$. 

Following the idea in \cite{kveton2019garbage}, we are going to try to bound 
\[
    s_{a, j} = \max \{ s: a_{k, s, j} \geq T^{-1}\}, \qquad j = 1, 2, 3
\]
with a constant times $\log T$. Indeed, if we successfully do so, then 
\[
    a_{k} \leq \max_{s \in [T]} a_{k, s} \times s_{a, j} + T^{-1} \times (T - s_{a, j}) \asymp O(1) \times O(\log T) + O(1) = O  (\log T),
\]
which does bound $a_{k} = \sum_{s = 0}^{T - 1} a_{k, s} \lesssim \log T$.
\todohw{I still need to go through the following part. I will get this done tonight and tomorrow.}
%giving an order $\log T$. 
%As we can see, decomposition will play an important role in this proof. 
For the decomposition, a common approach is using indicators on "good" events to decompose. Denote the shifted version mean reward defined as 
\[
    \overline{R}_{k, s}^* := \frac{\sum_{i = 1}^s R_{k, i} + \lambda s}{s(1 + 2 \lambda)} = \frac{\lambda}{1 + 2 \lambda} + \frac{1}{1 + 2 \lambda} \overline{R}_{k, s}.
\]
Then we can define the following "good" events for $k$-th arm as
\[
    A_{k, s} := \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  > - C_1 \Delta_k \right\}, \qquad A_{k, s}^{\prime} := \left\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2 \lambda}  < C_2 \Delta_k \right\},
\]
and
\[
    G_{k', s} := \left\{ - C_3 \Delta_k \leq \overline{Y}_{k', s} - \overline{R}_{k', s}^* \leq C_3 \Delta_k \right\}.
\]
The definitions of $A_{k, s}$ and $G_{k, s}$ are intuitive: $A_{k, s} \, \cap \, A_{k, s}'$ represent the sample mean does not derivative from the true mean too far; and events on $G_{k', s}$ means $\overline{Y}_{k', s}$ is not too far away from the scaled-shifted sample mean $\overline{R}_{k, s}^*$.

%It is worthy to note that $k'$ in $G_{k', s}$ is different from the fixed index $k$ in $\Delta_k$. And it is also easy to see that under two good events $A_{k', s} \cap G_{k', s}$, our target function $\overline{Y}_{k', s}$ is close to the shifted mean $\frac{\mu_{k'} + \lambda}{1 + 2\lambda}$, which means $\overline{Y}_{k', s}$ does remain the order of expected mean of each arm. 
Therefore, by using these good events, we decompose $a_{k, s}$ as the following three parts:
\[
    a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}^c)\Big],
\]
\[
    a_{k, s, 2} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}) \ind (G_{1, s}^c)\Big], \qquad a_{k, s, 3} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}) \ind (G_{1, s})\Big].
\]
As we can see, $a_{k, s, 1}$ and $a_{k, s, 2}$ are defined on complement sets of the good events or say "bad" events,
and we will bound them by bounding the probability $\pr (A_{1, s}^c)$ and $\pr (G_{1, s}^c)$; while $a_{k, s, 3}$ defined on the "good" events, we will need extra steps to bound them, which we will specify later. 

\subsubsection{Bounding $a_{k, s, 1}$ by analyzing $s_{a, 1}$}

We will bound $a_{k, s, 1}$ by bounding the probability of $A_{k, s}^c$. Write
\begin{equation}\label{a_k_1_bound}
    a_{k, s, 1} = \E \Big[ \big( N_{1, s} (\tau_k) \wedge T \big) \ind (A_{1, s}^c)\Big] \leq \E \Big[ T  \ind(A_{1, s}^c)\Big] = T \pr (A_{1, s}^c) 
\end{equation}
Since the summation of independent sub-Gaussian variables is still sub-Gaussian, \eqref{lem_subGtosubE_1} in Lemma \ref{lem_subGtosubE} gives $\overline{R}_{1, s} - \mu_1 \sim \subG (\sigma^2 /  s)$. And by the concentration inequality of the sub-Gaussian variable,
\[
    \begin{aligned}
        \pr (A_{1, s}^c) & = \pr \left( \mu_1 - \overline{R}_{1, s} \geq (1 + 2\lambda) C_1 \Delta_k \right) \\
        & \leq \exp \left\{ - \frac{(1 + 2\lambda)^2 C_1^2 \Delta_k^2 s}{2 \sigma_1^2}\right\} \\
        (\text{take} s \geq s_{a, 1} :=  \begin{matrix} \frac{\sigma_1^2}{C_1^2 (1 + 2 \lambda)^2 \Delta_k^2} \times\log T \end{matrix}) & \leq \frac{1}{T^2}
    \end{aligned}
\]
Hence, we obtain that
\[
    a_{k, s, 1} \leq  T \pr(A_{1, s}^c) \leq T^{-1}, \qquad \text{ for any } s \geq s_{a, 1} \asymp \log T.
\]

%\begin{remark}
   %For bounded rewards, there we can just use Hoeffding inequality and still have $s_{a, 1} \asymp \log T$.
%\end{remark}

\subsubsection{Tackling $a_{k, s, 2}$ with $s_{a, 2}$}

For bounding the probability of $G_{1, s}^c$ conditioning on $\his_{1, s}$, we use the fact that $\omega_i, \omega_i', \omega_i''$ is symmetric about $1$: 
%we use the fact $G_{k', s}^c = \{ |\overline{Y}_{k', s} - \overline{R}^*_{k', s}| > C_3 \Delta_k\}$ 
%Since a symmetric event. Hence, 
\[
    \begin{aligned}
        \pr (G_{1, s}^c \mid \his_{1, s}) & = \pr \big( |\overline{Y}_{k', s} - \overline{R}^*_{k', s}| > C_3 \Delta_k \mid \his_{1, s}\big)\\
        & = 2 \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) \omega_i + \lambda \sum_{i = 1}^s (2 R_{1, i} \omega_i - \overline{R}_{1, s} \omega_i' - \overline{R}_{1, s} \omega_i'') 
        \\
        & \qquad \qquad  + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega''_i) - C_3 (1 + 2\lambda) \Delta_k \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] > 0\Bigg\}.
    \end{aligned}
\]
To analyze the above probability, define the following functions of $\{ R_{1,i}\}_{i = 1}^s$:
\[
   f \big(\{ R_{1,i}\}_{i = 1}^s\big) := f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) + f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) - f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big)
\]
with 
\[
    f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) := \sum_{i = 1}^s \big[ (R_{1, i} - \overline{R}_{1, s}) + \lambda (2 \overline{R}_{1, i} - 1) - (1 + 2 \lambda ) C_3 \Delta_k  \big] \omega_i,
\]
%\[
    %f_1 \big(\{ R_{1,i}\}_{i = 1}^s \big) = \sum_{i = 1}^s \big[ (1 + 2 \lambda) R_{1, i} - \lambda - \overline{R}_{1, s} - C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i,
%\]
\[
    f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) := \sum_{i = 1}^s \big[ \lambda (\lambda + 1  - \overline{R}_{1, s}) - (1 + 2 \lambda ) C_3 \Delta_k  \big] \omega_i',
\]
%\[
    %f_2 \big(\{ R_{1,i}\}_{i = 1}^s \big) = \sum_{i = 1}^s \big[ \lambda (1 + 2 \lambda) - \lambda^2 - \overline{R}_{1, s} \lambda - \lambda C_3 (1 + 2 \lambda) \Delta_k \big] \omega_i',
%\] 
\[
    f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big) = \sum_{i = 1}^s \big[ \lambda (\overline{R}_{1, s} + \lambda) + (1 + 2 \lambda ) C_3 \Delta_k  \big] \omega_i''.
\]
%\[
    %f_3 \big(\{ R_{1,i}\}_{i = 1}^s \big) =  \sum_{i = 1}^s \big[ (\lambda^2 + \lambda \overline{R}_{1, s}) + \lambda C_3 (1 + 2\lambda) \Delta_k \big] \omega_i''.
%\]
Then we can write $\pr (G_{1, s}^c \mid \his_{1, s}) = 2 \pr_{\omega, \omega', \omega'} (f_1 + f_2 - f_3 > 0)$. Note that $f_1, f_2$, and $f_3$ are mutually independent. The expectation is
\[
    \E (f_1 + f_2 - f_3) = - 3 C_3 (1 + 2 \lambda) \Delta_k s,
\] 
and the variance is
\begin{equation}\label{bound_var_f}
    \begin{aligned}
        & \var(f_1 + f_2 - f_3) \\
        = & \sigma_{\omega}^2 \Bigg[ \overbrace{(1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 2 s \lambda (1 + 2 \lambda) (2 \overline{R}_{1, s} - 1 ) (\overline{R}_{1, i} - \overline{R}_{1, s}) + 2 s \lambda^2 \big(3 \overline{R}_{1, s}^2 - 3 \overline{R}_{1, s} + \lambda^2 + \lambda + 1 \big)}^{\text{the variance coming from the difference between $\overline{Y}_{k, s}$ and $\overline{R}_{k, s}$.}} \\
        & \qquad \qquad \qquad + \underbrace{3 s (1 + 2\lambda)^2 C_3^2 \Delta_k^2}_{\text{the maximal variance expansion allowed on the event $G_{1, k}^c$ (the cross term cancelling out).}} \Bigg] \\
        & = \sigma_{\omega}^2 \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 +  2 s \lambda^2 \big(3 \overline{R}_{1, s}^2 - 3 \overline{R}_{1, s} + \lambda^2 + \lambda + 1 \big) + 3 s (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \bigg] \\
        & =: \sigma_{\omega}^2 \bigg[ \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \bigg]
    \end{aligned}
\end{equation}
where we define
\[
    \mathbb{G}_1(s, \lambda) := (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2, \qquad \mathbb{G}_2 (s, \lambda) := 6 s \lambda^2 \overline{R}_{1, s} (\overline{R}_{1, s} - 1),
\]
and
\[
    g_3(s, \lambda) = s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2  \big].
\]
\iffalse
\[
    \begin{aligned}
        & \var(f_1 + f_2 - f_3) = \var f_1 + \var f_2 + \var f_3 \\
        = & \bigg\{ \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s})^2 + 4 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + 4 \lambda \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) (R_{1, i} - \mu_1) \\
        & \qquad + 2 \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \sum_{i = 1}^s (R_{1,i} - \overline{R}_{1, s}) \\
        & \qquad + 4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \sum_{ i =1}^s (R_{1, i} - \mu_1) + s \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big]^2 \bigg\} \\
        & + \lambda^2 \bigg\{ s^2 (\overline{R}_{1, s} - \mu_1)^2 + 2 \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big] s (\overline{R}_{1, s} - \mu_1) +  s \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \bigg\} \\
        & + \lambda^2 \bigg\{ s^2 (\overline{R}_{1, s} - \mu_1)^2 + 2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] s (\overline{R}_{1, s} - \mu_1) + s \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \bigg\} \\
        = & (1 + 4 \lambda^2 + 4 \lambda) \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + (-s - 4 \lambda s + \lambda^2 s^2 + \lambda^2 s^2) (\overline{R}_{1, s} - \mu_1)^2 + \Big\{ 4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big] \\
        & + 2 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] + 2 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big\} \sum_{i = 1}^s (R_{1, s} - \mu_1) \\
        & + \Big\{ s \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + 2\lambda) \Delta_k \big]^2 + s \lambda^2 \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \\
        & + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \Big\} \\
        =: & g_1(\lambda) \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + g_2(s, \lambda) (\overline{R}_{1, s} - \mu_1)^2 + g_3(\lambda) \sum_{i = 1}^s (R_{i, s} - \mu_1) + g_4(s, \lambda) \\
        =: & \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda).
    \end{aligned}
\]
\fi
%Here the hollow font $\mathbb{G}_{\cdot}$ represents random quantities whereas $g_{\cdot}$ is non-random.

The $\mathbb{G}_j$ for $j = 1, 2$ and $g_3$ have relatively complex expressions, so we want to give some simpler upper bounds of them. We calculate it as
%First, we note that $\var (f_1 + f_2 - f_3)$ is strictly positive, and it has the following upper bound,
\begin{equation}\label{G_function_bound}
    \begin{aligned}
        & \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \\
        = & (1 + 2 \lambda)^2 \bigg[ \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 - s (\overline{R}_{1, s} - \mu_1)^2\bigg] \\
        & \qquad + 6 s \lambda^2 \Big[ (\overline{R}_{1, s} - \mu_1)^2 + 2 (\mu_1 - 1) (\overline{R}_{1,  s} - \mu_1) + \mu_1 (\mu_1 - 1)\Big] + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) \\
        & \qquad + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2  \big] \\
        = & \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s (2 \lambda^2 - 4 \lambda - 1) (\overline{R}_{1, s} - \mu_1)^2 - 2s (1 - \mu_1) (\overline{R}_{1, s} - \mu_1) \bigg] \\
        & \qquad \qquad + s \big[ - 6 \lambda^2 \mu_1 (1 - \mu_1) + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        \overset{\text{dropping the negative terms}}{\leq} & \bigg[ (1 + 2 \lambda)^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s (2 \lambda^2 - 4 \lambda - 1) (\overline{R}_{1, s} - \mu_1)^2  \bigg]  \\
        & + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        \overset{\text{by Cauchy inequality}}{\leq} & \big[ (1 + 2 \lambda)^2 + (2 \lambda^2 - 4 \lambda - 1)  \big] \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 +  s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        = & 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]. 
    \end{aligned}
\end{equation}
As one can see, in this step, we bound $\mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda)$ by a sub-Exponential variable plus a strictly positive constant.
\iffalse
\begin{equation}\label{G_function_bound}
    \begin{aligned}
        & \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda) \\
        = & s^2 g_1(\lambda) (\overline{R}_{1, s} - \mu_1)^2 + g_2(s, \lambda) (\overline{R}_{1, s} - \mu_1)^2  + s g_3(\lambda) (\overline{R}_{1, s} - \mu_1) + g_4(s, \lambda) \\
        = & \big[ s^2 g_1(\lambda) + g_2(s, \lambda)\big](\overline{R}_{1, s} - \mu_1)^2 + s g_3(\lambda) (\overline{R}_{1, s} - \mu_1) + g_4(s, \lambda) \\
        \leq & \Big\{ s^2(2 \lambda + 1)^2 + (2 \lambda^2 s^2 - 4 \lambda s - 1)\Big\} (\overline{R}_{1, s} - \mu_1)^2 \\
        & \qquad + \Big\{ s \times4 \lambda \big[ \lambda(2 \mu_1 - 1) - C_3 (1 + \lambda) + \lambda (\lambda + \mu_1) + C_3 \lambda (1 + 2 \lambda) \Delta_k \big] \Big\} (\overline{R}_{1, s} - \mu_1) \\
        & \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \\
        & \qquad + s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\} \\
        \leq & 2 s^2 (6 \lambda^2 + 4 \lambda + 1) (\overline{R}_{1, s} - \mu_1)^2 + 4 s \lambda \big[ (2 C_3 \Delta_k + 1) \lambda^2 + (3 \mu_1 - 1 - C_3 + C_3 \Delta_k) \lambda - C_3 \big] (\overline{R}_{1, s} - \mu_1) \\
        & \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 \\
        & \qquad + s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\} \\
        \leq & 2s^2 (4 \lambda^2 + 4 \lambda + 1) (\overline{R}_{1, s} - \mu_1)^2  + 2 s \lambda (2 \lambda + 1) \times\lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \sqrt{s} (\overline{R}_{1, s} - \mu_1) \\
        & \qquad + s \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + g_5(s, \lambda)\\
        \leq & 2 s \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) +  \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2 + g_5(s, \lambda),
    \end{aligned}
\end{equation}
where the last two $\leq$ use the fact that $s \geq 1$ and $\mu_1, C_3 \in (0, 1]$. And furthermore, $g_5(s, \lambda) = s \lambda^2 \Big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \Big\}$ is a strict positive function for at least $\Delta_{k_1}, \ldots, \Delta_{k_{K - 3}}$, since
\[
    \frac{C_3 \Delta_k}{2(\mu_1 - C_3 \Delta_k) - 1} = \frac{1 - \mu_1 - C_3 \Delta_k}{2 C_3 \Delta_k - 1}.
\]
is a quadratic equation for $\Delta_k$ and cannot hold for all $k \in [K] / \{ 1\}$. And for $g_5(s, \lambda)$, it can be bounded by
\[
    \begin{aligned}
        g_5(s, \lambda) & \leq s \lambda^2 \Big( \big[ 1 + C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ 1 + C_3 (1 + 2 \lambda) \Delta_k + (1 + \lambda) \big]^2 \Big) \\
        & \leq 2 s \lambda^2 \left[ 1 + C_3^2 (\lambda^{-1} + 2)^2 \Delta_k^2 + (2 + \lambda)^2 + C_3^2 (1 + 2 \lambda)^2 \Delta_k^2\right] \\
        & \leq 2 s \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big].
    \end{aligned}
\]

%\textit{{Why the restriction will appears. Adding something to make the above strictly positive.}}

%Therefore, 
%\[
    %\begin{aligned}
        %& \frac{\var (f_1 + f_2 - f_3)}{|\E (f_1 + f_2 - f_3)} 1(\overline{R}_{1, s} - \mu_1 \leq 0)\\ 
        %= & \frac{ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + \mathbb{G}_{3}(s, \lambda) + g_4(s, \lambda)}{|\E (f_1 + f_2 - f_3)|} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & \frac{2 \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) + \sqrt{2} \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2}{C_3 (1 + 2 \lambda)^2 \Delta_k} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & \frac{2 \Big[\sqrt{2} \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2}{C_3 (1 + 2 \lambda)^2 \Delta_k} 1(\overline{R}_{1, s} - \mu_1 \leq 0) \\
        %\leq & 8 C_3 \lambda^2 \Delta_k 1(\overline{R}_{1, s} - \mu_1 \leq 0).
    %\end{aligned}
%\]
\fi

For the standard Gaussian variable $Z$, we have $\pr (Z \geq x)\leq \exp \{ - {x^2} / {2}\}$ for $x > 0$. Then
\[
    \begin{aligned}
        \pr (G_{1, s}^c \mid \his_{1, s}) & = 2 \pr \left(\frac{f_1 + f_2 - f_3 - \E (f_1 + f_2 - f_3)}{\sqrt{\var (f_1 + f_2 - f_3)}} > - \frac{\E (f_1 + f_2 - f_3)}{\sqrt{\var (f_1 + f_2 - f_3)}} \right) \\
        & \leq  2\exp \left\{ - \frac{\E^2 (f_1 + f_2 - f_3)}{2 \var (f_1 + f_2 - f_3)} \right\} \\
        (\text{by \eqref{bound_var_f}} )& \leq 2 \exp \left\{ - \frac{9 C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3(s, \lambda) \big]}\right\}.
    \end{aligned}
\]
Therefore, $a_{k, s, 2}$ will be bounded by 
\[
    \begin{aligned}
        a_{k, s, 2} & \leq \E \Big[ T  \ind(G_{1, s}^c)\Big] =  T \E \Big[ \pr(G_{1, s}^c \mid \his_{1, s}) \Big] \\
        & \leq 2 T \E \exp \left\{ - \frac{9 C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2 }{2\sigma_{\omega}^2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3(s, \lambda) \big]}\right\}.
    \end{aligned}
\]
%On the other hand, 
Recall $R_{1, i} - \mu_1 \sim \subG(\sigma_1^2)$, and then $(R_{1, i} - \mu_1)^2 - \var (R_{1, i}) \sim \subE(8 \sqrt{2} \sigma_1^2)$, hence by Corollary 4.2 (a) in \cite{zhang2020concentration},
\[
    \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 - s \var (R_{1, i}) \, \sim \, \subE (8 \sqrt{2 s} \sigma_1^2).
\]
Therefore, 
\begin{equation}\label{G_function_bound_2}
    \begin{aligned}
        2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3(s, \lambda) \big] & \overset{\text{by \eqref{G_function_bound}}}{\leq} 12 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        & \sim 12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + 12 \lambda s \var (R_{1, 1}) +  s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) \\
        & ~~~~~~~~~~~~~~ + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
        & \overset{\text{by } \var(R_{1, 1}) \leq \sigma_1^2}{\leq} 12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) \\
        & ~~~~~~~~~~~~~ + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big].
    \end{aligned}
\end{equation}
Here we use the $\subE(\lambda)$ to represent a random variable $Z \sim \subE(\lambda)$. And the distribution notation in the inequalities following will also have a similar meaning.

\iffalse
For tackling the expectation above, we first note that $\sqrt{s} (\overline{R}_{1, s} - \mu_1) \sim \subG (\sigma_1^2)$, then $\sqrt{s} (2\lambda + 1) (\overline{R}_{1, s} - \mu_1) \sim \subG \big((2\lambda + 1)^2\sigma_1^2 \big)$, and
hence
\[
    \begin{aligned}
        & \Big[ \sqrt{s} (2 \lambda + 1) (\overline{R}_{1, s} - \mu_1) + \lambda \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big] \Big]^2 \\
        & \quad - \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 - (2 \lambda + 1 )^2 \var (R_{1,s}) \,  \sim \, \subE \big(8\sqrt{2}(2\lambda + 1)^2\sigma_1^2, 8(2\lambda + 1)^2\sigma_1^2 \big),
    \end{aligned}
\]
\fi
Then applying Lemma \ref{lem_subE_ineq} in \eqref{G_function_bound} will furthermore give
\begin{equation}\label{a_2_bound}
    \begin{aligned}
        a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
        & \overset{\text{by \eqref{G_function_bound_2}}}{\leq} 2 T \E\exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        & \overset{\text{by } a \subE (\lambda) = \subE (a^2 \lambda)}{=} 2 T \E\exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{ \subE ( 1152 \sqrt{2} \lambda^4 \sigma_1^2) + \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        & \overset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} 2 T \Big[ 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s ( h_1 + h_2) \Big] \exp \left\{  - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\} \\
        & \overset{\text{by } s \leq T}{\leq} 2 T^2 \Big[ 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 ( h_1 + h_2) \Big] \exp \left\{  - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big]}\right\},
    \end{aligned}
\end{equation}
\iffalse
\begin{equation}\label{a_2_bound}
    \begin{aligned}
        a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s^2 }{2 \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
        & \leq 2 T \times \\
        & \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{4 \big[\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + (2 \lambda + 1 )^2 \var (R_{1,s})\big] + 2 s^{-1}g_5(s, \lambda)}\right\} \\
        & \leq 2 T \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 4 (2 \lambda + 1 )^2 \var (R_{1,s}) + 2 s^{-1} g_5(s, \lambda)}\right\} \\
        & \qquad \times \Big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s (h_1 + h_2) \Big]\\
        & \leq 2 T^2 \Big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1 + h_2) \Big] \\
        & \exp \left\{ - \frac{C_3^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 4 (2 \lambda + 1 )^2 \sigma_1^2 + 4 \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big]}\right\}.
    \end{aligned}
\end{equation}
\fi
where $h_1$ and $h_2$ are finite and free of $s$ by following Lemma \ref{lem_subE_ineq}. 
%And we use the fact that for $s$ big enough one must have $b \leq \sqrt{2 c a \cdot 8 \sigma_1^2}$ with $a := 4$, $b := 8 \lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 2 (2 \lambda + 1 )^2 \var (R_{1,s})\big] + 4 s^{-1}g_5(s, \lambda)$, and $c := C_3^2 (1 + 2 \lambda)^4 \Delta_k s$. 

\iffalse
\begin{lemma}[Need to be corrected!]\label{lem_subE_ineq}
    Suppose zero-mean random variable $X \sim \subE(\lambda, \alpha)$, and positive constants $a, b, c$ satisfying $a X + b > 0$,
    then
    \[
        \E \exp \left\{ - \frac{c}{a X + b}\right\}  \leq e^{- c / b} \big[1 + c h_1(a, b, \alpha) + c h_2(a, b, \lambda) \big]
    \]
    where $h_1$ and $h_2$ are finite positive functions.
\end{lemma}

\begin{proof}
    Note that differentiable $f$ is positive, we have $0 \leq \E f(X) \leq f(0) + \int_0^{\infty} \big[ f'(u) - f'(-u) \big]\pr (|X| > u) \, du$, then 
    \[ 
        \begin{aligned}
            & \E \exp \left\{ - \frac{c}{a X + b}\right\} \\
            \leq & e^{-c / b} + \int_0^{\infty} \bigg[ \exp \left\{ - \frac{c}{a u + b}\right\}  \frac{ca }{ (a u + b)^2} - \exp \left\{ - \frac{c}{ - a u + b}\right\}  \frac{ca }{ (- a u + b)^2} \bigg] \, \pr (|X| > u) \, du \\
            \leq & \int_0^{\infty} \bigg[ \exp \left\{ - \frac{c}{a u + b}\right\}  \frac{ca }{ (a u + b)^2} - \exp \left\{\frac{c}{ a u - b}\right\}  \frac{ca }{ (a u - b)^2} \bigg] \, \exp \left\{ - \frac{1}{2} \left( \frac{u^2}{\lambda^2} \wedge\frac{u}{\alpha} \right) \right\} \, du \\
            = & \int_0^{\infty} \exp \left\{ - \frac{c}{a u + b}\right\} \bigg[   \frac{ca }{ (a u + b)^2} - \exp \left\{\frac{b + au}{ b - au}\right\}  \frac{ca }{ (a u - b)^2} \bigg] \, \exp \left\{ - \frac{1}{2} \left( \frac{u^2}{\lambda^2} \wedge\frac{u}{\alpha} \right) \right\} \, du \\
            \leq & \exp (-c / b) \int_0^{\infty} \Bigg[ \frac{ca}{(a u + b)^2} \exp \left\{ - \frac{u}{2 \alpha}\right\} + \frac{ca}{(a u - b)^2} \exp \left\{ - \frac{1}{2}\frac{u^2}{ \lambda^2}  \wedge \frac{u}{ \alpha} + \frac{b + au}{b - au}\right\} \Bigg] \, du \\
            =: &  \exp (-c / b) \big[ I_1 + I_2 \big].
        \end{aligned}
    \]
    Denote $\Gamma(\cdot, \cdot)$ as incomplete gamma function, then one can calculate that
    \[
        I_1 = \frac{c}{b} - \frac{c e^{\frac{b}{2 a \alpha}}\Gamma(0, \frac{b}{2 a \alpha})}{2 a \alpha} =: c h_1 (a, b, \alpha),
    \]
    which is finite as long as $a, \alpha$ is positive.
    For calculating $I_2$, we write $I_2$ as
    \[
        \begin{aligned}
            I_2 = & c a \int_{0}^{\lambda^2 / \alpha} \frac{1}{(a u - b)^2} \exp \left\{ - \frac{u^2}{2 \lambda^2}  + \frac{b + a u}{b - au}\right\} \, du  + \int_{\lambda^2 / \alpha}^{\infty}  \frac{1}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + a u}{b - au}\right\} \, du \\
            =: & ca ( I_{21} + I_{22}).
        \end{aligned}
    \]
    As $I_{21}$ and $I_{22}$ are both free of $c$, we only need to care its irregular point $\frac{b}{a}$ and $\infty$. We separate it as the following two cases:
    \begin{itemize}
        \item[(i)] If $\frac{b}{a} \leq \frac{\lambda^2}{\alpha}$, then 
        \[
            \lim_{u \rightarrow \frac{b}{a}} (a u - b)^{1 / 2}\frac{1}{(a u - b)^2} \exp \left\{ - \frac{u^2}{2 \lambda^2} + \frac{b + au}{b - au}\right\} = 0,
        \]
        and 
        \[
            \lim_{u \rightarrow \infty} u^{3 / 2}\exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} = 0.
        \]
        \item[(ii)] If $\frac{b}{a} \geq \frac{\lambda^2}{\alpha}$, then $I_{21}$ will be strictly finite. And for $I_{22}$, it will be
        \[
            \lim_{u \rightarrow \frac{b}{a}} (a u - b)^{1 / 2}\frac{1}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} = \lim_{u \rightarrow \infty},
        \]
        
    \end{itemize}
    Hence, $\exists \, I_2 \in \mathbb{R}$, and then
    \[
        \exists \, I_2 = c \int_0^{\infty} \frac{a}{(a u - b)^2} \exp \left\{ - \frac{u}{2 \alpha} + \frac{b + au}{b - au}\right\} =: c h_2(a, b, \lambda) \in c \times (0, \infty)
    \]
    with $h_1$ and $h_2$ are finite positive functions.
\end{proof}
\fi


\begin{lemma}[sub-Exponential concentration]\label{lem_subE_ineq}
    Suppose zero-mean random variable $X \sim \subE(\lambda, \alpha)$, and positive constant $a, b, c$ satisfies $a X + b > 0$. If $b \leq 2 c a\lambda^2 \alpha^2 \wedge \sqrt{2 c a\alpha}$, then
    \[
        \E \exp \left\{ - \frac{c}{a X + b}\right\}  \leq e^{- c / b} \big[1 + c h_1(a, b, \alpha, \lambda) + c h_2(a, b, \alpha) \big] := e^{- c / b} [1 + ch_1 + ch_2],
    \]
    where $h_1$ and $h_2$ are finite positive functions free of $c$.
\end{lemma}

Let us take
\[
    \begin{aligned}
        s \geq s_{a, 2} := \frac{ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_3^2 \Delta_k^2}{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log \Big[ 2 T^3 \big( 1 + 9 \sigma_{\omega}^{-2} C_3^2 (1 + 2\lambda)^2 \Delta_k^2 ( h_1 + h_2) \big) \Big]
    \end{aligned}
\]
%\[
    %\begin{aligned}
        %s \geq s_{a, 2} := & \frac{12 \big(2\lambda^2 \big[ (\lambda + \mu_1) + C_3 (1 + 2 \lambda) \Delta_k \big]^2 + 6 (2 \lambda + 1 )^2 \sigma_1^2 + \big[ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 \big] \big)}{C_3^2 (1 + 2\lambda)^4 \Delta_k^2}\\
        %& \qquad \times \log \Big[  2 C_3^2 \lambda^2 (1 + 2\lambda)^4 \Delta_k^2 \big[ 1 + C_3^2 (1 + 2\lambda)^4 \Delta_k^2 (h_1 + h_2) \big] \Big] \log T
    %\end{aligned}
%\]
in the last step of \eqref{a_2_bound}, we will obtain $a_{k, s, 2} \leq T^{-1}$.

\subsubsection{Tackling $a_{k, s, 3}$ with $s_{a, 3}$}

In the previous section, we control the probability on bad events to bound $a_{k, s, 1}$ and $a_{k, s, 2}$. But since $a_{k, s, 3}$ is defined on good events, we need a different technique to deal with $a_{k, s, 3}$.

Different from dealing with $a_{k, s, 1}$ and $a_{k, s, 2}$, in which we control the probability of the bad events with $O(T^{-2})$,
$a_{k, s, 3}$ is defined on good events. Hence, 
We need a special technique to deal with $a_{k, s, 3}$ . Note that 
\begin{equation}\label{a_k_3_sw}
    \begin{aligned}
        \{N_{1, s}(\tau_{k})<T^{-1}\} & \supseteq \{N_{1, s}(\tau_{k}) < (T^{2}-1)^{-1}\} = \big\{Q_{1, s}\left(\tau_{k}\right)^{-1}<1+\left(T^{2}-1\right)^{-1}\big\} \\
        &=\big\{Q_{1, s}(\tau_{k})^{-1} < (1-T^{-2})^{-1}\big\} = \big\{\left[1-Q_{1, s}(\tau_{k})\right]<T^{-2}\big\},
    \end{aligned}
\end{equation}
and $a_{k, s, 3} \leq \E \big[ N_{1, s} (\tau_k) 1(A_{1, s} \cap G_{1, s}) \big]$. 
Thus, similar to 
\cite{wang2020residual}, it is sufficient to find $s \geq s_{a,3}$ satisfying $\big\{[1-Q_{1,s}(\tau_{k})]<T^{-2}\big\}$ on the event $\{A_{1, s} \cap G_{1, s}\}$.

We write 
\[
    \big[1-Q_{1, s}(\tau_{k})\big]  \ind (A_{1, s})\ind  (G_{1,s}) = \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, s} \big)  \ind (A_{1, s} \, \cap \, G_{1, s})
\]
with $\Gamma_1 := \Gamma_1(\tau_1) = \tau_1 - \overline{R}_{1, s}^*$ measuring the difference between $\overline{Y}_{1, s}$ and $\overline{R}_{1,s}^*$. And on the event $A_{1, s} \, \cap \, G_{1, s}$, $\Gamma_1$ can be bounded in an interval.
%It is not hard to see $\Gamma_1$ should be negative with a moderate value. And $\Gamma_1$ does have an appropriate on the event $A_{1, s} \, \cap \, G_{1, s}$, this can be true. 
To see this, we write 
\[
    A_{1, s} = \bigg\{ \overline{R}_{1, s}^* - \frac{\mu_1 + \lambda}{1 + 2\lambda} > - C_1 \Delta_k \bigg\} = \bigg\{ \Gamma_1 < C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} + \tau_1 \bigg\} 
\]
and
\[
    \begin{aligned}
        G_{1, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_1 -C_3 \Delta_k \leq \overline{Y}_{1, s} + \Gamma_1 \leq \tau_1 + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_1 - C_3 \Delta_k - \overline{Y}_{1, s} \leq \Gamma_1 \leq \tau_1 + C_3 \Delta_k - \overline{Y}_{1, s}\big\} \\
        (\text{by plugging in the inequality for } \overline{Y}_{1, s})& \subseteq \big\{ \tau_1 - 2 C_3 \Delta_k - \overline{R}_{1, s}^* \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \overline{R}_{1, s}^* \big\},
        % & \subseteq \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 \leq \tau_1 + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2 \lambda}\bigg\},
    \end{aligned}
\]
then
\[
    \begin{aligned}
        A_{1, s} \, \cap \, G_{1, s} \\
        % & = \bigg\{ \tau_1 -  2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2 \lambda} \leq \Gamma_1 < \tau_1 + C_1 \Delta_k - \frac{\mu_1 + \lambda}{1 + 2\lambda} \bigg\} \\
        (\text{by plugging the inequality for $\overline{R}_{1, s}^*$ in } A_{1, s})\subseteq & \bigg\{ \tau_1 -  2 C_3 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\} \\
        (\text{take } C_1 \geq 2 C_3 ) \subseteq & \bigg\{ \tau_1 -  C_1 \Delta_k - 1 \leq \Gamma_1 < C_1 \Delta_k + \tau_1 - \frac{\mu_1}{2}\bigg\}.
    \end{aligned}
\]
%It is easy to see that in the above derivation, we add the requirement that
Since $\tau_1 - C_1 \Delta_k - 1 < 0$, to control $\Gamma_1$ within a small interval, we add conditions: 
\begin{equation}\label{requirement_1}
     \Delta_k + \tau_1 - \frac{\mu_1}{2} \leq 0 \qquad \text{ together with }  \qquad C_1 \geq 2C_3.
\end{equation}
Hence, we obtain the range of the positive quantity $-\Gamma_1$ lies in
\[
    C_1 \Delta_k = \frac{\mu_1 }{2} - \tau_1 - C_1 \Delta_k <  - \Gamma_1 \leq 1 + C_1 \Delta_k  - \tau_k = 1 - \frac{\mu_1}{2} + 3 C_1 \Delta_k < 4.
\]
Now fix
\begin{equation}\label{requirement_2}
    \tau_1 = \frac{\mu_1}{2} - \Delta_k,
\end{equation}
we get $ (- \Gamma_1) \in (C_1 \Delta_k, 4) \subset (0, + \infty)$.

Returning to the quantity we care about, $ \big[ 1 - Q_{1,s} (\tau_k)\big] 1(A_{1, s}) 1(G_{1, s})$, we write it as 
\[
    \begin{aligned}
        & \big[ 1 - Q_{1,s} (\tau_k)\big] \ind (A_{1, s}) \ind (G_{1, s}) \\
        = & \pr \big(\overline{Y}_{1, s} - \overline{R}_{1, s}^* \leq \Gamma_1 \, | \, \his_{1, s} \big)  \ind (A_{1, s} \, \cap \, G_{1, s})\\
        = & \E \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s (R_{1, i} - \overline{R}_{1, s}) \omega_i + \lambda \sum_{i = 1}^s (2 R_{1, i} \omega_i - \overline{R}_{1, s} \omega_i' - \overline{R}_{1, s} \omega_i'') 
        \\
        & \qquad \qquad + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega''_i) - \Gamma_1 (1 + 2\lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] < 0\Bigg\} \ind (A_{1, s} \, \cap \, G_{1, s}).
    \end{aligned}
\]
Similar to the technique we use to bound conditional probability $\pr (G_{1, s}^c \mid \his_{1, s})$, we just need to replace $C_3 \Delta_k$ by $(-\Gamma_1)$ in \eqref{a_2_bound}. We get that 
\[
    \begin{aligned}
         & \big[ 1 - Q_{1,s} (\tau_k)\big] \ind (A_{1, s}) \ind(G_{1, s}) \\
         \overset{\text{apply steps in  \eqref{G_function_bound_2}}}{\leq} & \E \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 (- \Gamma_1)^2 s^2 }{12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_1^2) + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 (- \Gamma_1)^2  \big]}\right\} \\
         \overset{\text{by the bound of } \Gamma_1}{\leq} & \E \exp \left\{ - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 s }{12 \lambda^2 \subE (8 \sqrt{2} \sigma_1^2) + \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2  \big]}\right\}\\
         \overset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} & \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s ( h_1^* + h_2^*) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2 \big]}\right\} \\
         \overset{s \leq T}{\leq} & T \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 ( h_1^* + h_2^*) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2 \big]}\right\}.
    \end{aligned}
\]
%
%in the above section. By using the same technique, one can get that
\iffalse
\begin{footnotesize}
\[
    \begin{aligned}
        & \big[ 1 - Q_{1,s} (\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \\
        \leq & \E \exp \left\{ - \frac{\Gamma_1^2 (1 + 2\lambda)^4 s}{4 (\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) + (1 + 2 \lambda) \Gamma_1 \big]^2 + (2 \lambda + 1 )^2 \sigma_1^2 + 2 \lambda^2(\sqrt{5} + \lambda)^2 + 2 (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2 ) }\right\} \\
        \leq & \E \exp \left\{ - \frac{C_1^2 \Delta_k^2 (1 + 2\lambda)^4 s}{4 (\subE (8\sqrt{2}\sigma_1^2, 8\sigma_1^2) + 2\lambda^2 \big[ (\lambda + \mu_1) -  (1 + 2 \lambda) 4 \big]^2 + (2 \lambda + 1 )^2 \sigma_1^2 + \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2) }\right\} \\
        \leq &  T  \exp \left\{ - \frac{C_1^2 (1 + 2\lambda)^4 \Delta_k^2 s}{8 \lambda^2 (7 \lambda + 4 - \mu_1)^2 + 4 (2 \lambda + 1 )^2 \sigma_1^2 + 4 [ \lambda^2(\sqrt{5} + \lambda)^2 + (1 + \lambda^2)(1 + 2 \lambda)^2 C_3^2 \Delta_k^2]}\right\} \\
        & \times \big[1 + C_1^2 \Delta_k^2 (1 + 2\lambda)^4  (h_1^* + h_2^*)\big] 
    \end{aligned}
\]
\end{footnotesize}
\fi
Therefore, to find $s$ such that $[1 - Q_{1, s} (\tau_k)] < T^{-2}$ on $\{ A_{1, s} \, \cap \, G_{1, s}\}$, let
\[
   \begin{aligned}
       s \geq s_{a, 3} := \frac{ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2}{144 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \log \Big[ T^3 \big( 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 ( h_1^* + h_2^*) \big) \Big],
   \end{aligned}
\]
where $h_1^*$ and $h_2^*$ free of $s$ are $h_1(\cdot, \cdot, \cdot)$ and $h_2(\cdot, \cdot, \cdot)$ in Lemma \ref{lem_subE_ineq} by replacing the corresponding parameters. By the argument in \eqref{a_k_3_sw}, we have $a_{k, s, 3} \leq T^{-1}$ whenever $s \geq s_{a,3}$ defined above.

Now, combining all the results in Section C.2, we get that 
\[
    a_{k} \leq \underbrace{\max_{s = 0, \ldots, T -  1} a_{k, s}}_{\text{bound by a constant in \eqref{a_k_constant_3}}} \times\overbrace{\max _{j = 1, 2, 3} s_{a, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{a, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Here we do not give the explicit expression of the bound as it involves several complicated integrals, but its order is exactly $\log T$. However, for some explicit distributions, the expectation in Lemma \ref{lem_subE_ineq} can be bounded by some simpler displays, and hence we can get explicit expressions for the bounds in these cases. See Corollary \ref{cor_ber} and Corollary \ref{cor_gau} for instance.
\end{remark}

\subsection{Bounding $b_k$}

Similar to the previous sections, for bounding $b_k = \sum_{s = 0}^{T - 1} b_{k, s}$, we decompose $b_{k, s} = \pr \big( Q_{k, s} (\tau_k) > T^{-1}\big) + 1$ as $b_k = b_{k, s, 1} + b_{k, s, 2} + b_{k, s, 3} + 1$ with
\[
    b_{k, s, 1} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A_{k, s}^{\prime c} )\big],
\]
\[
    b_{k, s, 2} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A'_{k, s}) \ind (G_{k, s}^c)\big],
\]
and
\[
    b_{k, s, 3} := \E \big[ \ind ( Q_{k, s} (\tau_k) > T^{-1}) \ind (A'_{k, s}) \ind (G_{k, s})\big].
\]
Since $b_{k, s}$ is naturally bounded {the} constant $2$, it only needs to bound $s_{b, j}: = \max \{ s: b_{k, s, j} \geq T^{-1}\}$ with the $C \log T$ for $j = 1, 2, 3$ with some positive constant $C$.
%\hl{I would say "show xx is of order O(), or bound xx by c LogT where c is a constant. I am not familiar with "bound xx by order xx" - an order itself is not an upper bound.}

% \hl{the next sentence is not correct. Please carefully check every sentence to make sure they are readable, and then we can move to the proof logic. }


For any $\star \in \{ (a, j), (b, j): j \in 1, 2, 3\}$, we denote $s_{\star}'$ as the quantity where we {replaces} $C_2$ in $s_{\star}$  by $C_1$. 

It is easy to see that $\pr (A^{\prime c}_{k, s}) \leq T^{-2} $ when $s \geq s_{a, 2}' / 2$. Then by the results on bounding $a_{k, s, 2}$,
we have $\max\{ b_{k,s, 1}, \, b_{k, s, 2}\} \leq T^{-2} < T^{-1}$ as long as $s \geq \max \{ s'_{a, 1}  / 2 , \, s'_{a, 2} \} \asymp \log T$. 

It remains to deal with $b_{k, s, 3}$. We will first bound $\Gamma_k = \overline{Y}_{k, s}  - \overline{R}_{k, s}^*$ on the event $A_{k, s}' \, \cap \, G_{k, s}$. Write
\[
    A'_{k, s} = \bigg\{ \overline{R}_{k, s}^* - \frac{\mu_k + \lambda}{1 + 2\lambda} < C_2 \Delta_k \bigg\} = \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \bigg\},
\]
and
\[
    \begin{aligned}
        G_{k, s} = \big\{ -C_3 \Delta_k \leq \overline{Y}_{k, s} - \overline{R}_{k, s}^* \leq C_3 \Delta_k \big\} & = \big\{ \tau_k -C_3 \Delta_k \leq \overline{Y}_{k, s} + \Gamma_k \leq \tau_k + C_3 \Delta_k \big\} \\
        & = \big\{ \tau_k - 2 C_3 \Delta_k - \overline{R}_{k, s}^* \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \overline{R}_{k, s}^* \big\}.
        %& \subseteq \bigg\{ \tau_k - 2 C_3 \Delta_k - \frac{1 + \lambda}{1 + 2\lambda} \leq \Gamma_k \leq \tau_k + 2 C_3 \Delta_k - \frac{\lambda}{1 + 2\lambda}\bigg\}.
    \end{aligned}
\]
%\hl{2 sentences (a common observation)}
Hence, we conclude that 
\[
    \begin{aligned}
        A'_{k, s} \, \cap \, G_{k, s}\\
        (\text{by plugging the inequality for $\overline{R}_{k, s}^*$ in } A'_{k, s}) \subseteq & \bigg\{ \tau_k - \frac{\mu_k + \lambda}{1 + 2\lambda} - C_2 \Delta_k  < \Gamma_k \leq\tau_k + C_2 \Delta_k - \frac{\lambda}{1 + 2\lambda} \bigg\} \\
        (\text{let } 2 C_3 \geq C_2) \subseteq & \bigg\{ \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2}  < \Gamma_k < \tau_k + C_2 \Delta_k \bigg\}
    \end{aligned}
\]
% It is worthwhile to recall that the construction of $s_{a, 1, 2}$ is free of any $\tau_k$, hence this argument is valid. 
Exactly the same as before, we require $\tau_k - C_2 \Delta_k - \frac{\mu_k }{2} \leq 0$ to ensure $\Gamma_k$ falls in a relatively small interval. To achieve this, we can just take
\begin{equation}\label{requirement_4}
    \tau_k = 2 C_2 \Delta_k + \mu_k / 2
\end{equation}
together with
\begin{equation}\label{requirement_3}
    2 C_3 \geq C_2.
\end{equation}
Then we will obtain that a bound for $\Gamma_k$ is
\[
    C_2 \Delta_k = \tau_k  - C_2 \Delta_k - \frac{\mu_k}{2} < \Gamma_k < \tau_k + C_2 \Delta_k = 3 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{7}{2} < 4,
\]
%\hl{avoid notations like below.. $1 > 2 < 3$.}
i.e. $\Gamma_k \in (C_2 \Delta_k, 4) \subset (0, + \infty)$. Similar to the technique in \eqref{a_2_bound}, we have
% \hl{I understand that equations are part of the text, but I would still recommend at least putting one or two words in between (such as "we have" }
\[
    \begin{aligned}
        & Q_{k, s}\left(\tau_{k}\right) \ind\left(A_{k, s}^{\prime}\right) \ind\left(G_{k, s}\right) = \E \pr \left(\overline{Y}_{k, s}-\overline{R}_{k, s}^{*}>\Gamma_{k} \mid \mathcal{H}_{k, T}\right) \ind\left(A_{k, s}^{\prime}\right) \ind\left(G_{k, s}\right) \\
        = & \E \pr_{\omega, \omega', \omega''} \Bigg\{ \sum_{i = 1}^s (R_{k, i} - \overline{R}_{k, s}) \omega_i + \lambda \sum_{i = 1}^s (2 R_{k, i} \omega_i - \overline{R}_{k, s} \omega_i' - \overline{R}_{k, s} \omega_i'')
        \\
        & \qquad \qquad \qquad + \lambda \sum_{i = 1}^s (\omega_i' - \omega_i) + \lambda^2 \sum_{i = 1}^s (\omega_i' - \omega''_i) - \Gamma_k (1 + 2\lambda) \bigg[ \sum_{i = 1}^s \omega_i + \lambda \sum_{i = 1}^s \omega_i' + \lambda \sum_{i = 1}^s \omega_i''\bigg] < 0\Bigg\}\\
        \overset{\text{apply steps in  \eqref{G_function_bound_2}}}{\leq} & \E \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 \Gamma_k^2 s^2 }{12 \lambda^2 \subE (8 \sqrt{2 s} \sigma_k^2) + s \big[ 12 \lambda \sigma_1^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 \Gamma_k^2  \big]}\right\} \\
        \overset{\text{by the bound of } \Gamma_k}{\leq} & \E \exp \left\{ - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 s }{12 \lambda^2 \subE (8 \sqrt{2} \sigma_k^2) + \big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2  \big]}\right\}\\
        \overset{\text{Lemma \ref{lem_subE_ineq}}}{\leq} & \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s ( h_1^{**} + h_2^{**}) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2 \big]}\right\} \\
        \overset{\text{by }s \leq T}{\leq} & T \Big[ 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 ( h_1^{**} + h_2^{**}) \Big] \exp \left\{  - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2  s }{\big[ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2 \big]}\right\}.
    \end{aligned}
\]
%\hl{Not understandable.}
where $h_1^{**}$ and $h_2^{**}$ are defined in Lemma \ref{lem_subE_ineq} by replacing the corresponding parameters again. Therefore, one can just take 
\[
    \begin{aligned}
        s \geq s_{b, 3} & := \frac{ 12 \lambda \sigma_k^2 + 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 6  (1 + 2\lambda)^2 C_2^2 \Delta_k^2}{144 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \log \Big[ T^3 \big( 1 + 144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 ( h_1^{**} + h_2^{**}) \big) \Big]
    \end{aligned}
\]
to ensure $b_{k, s, 3} \leq T^{-1}$.
%\hl{The sentence break is weird, if not wrong..}
And then, by using a similar argument, we have 
\[
    b_{k} \leq 2 \times\overbrace{\max _{j = 1, 2, 3} s_{b, j}}^{\text{with order } \log T} + 3 T^{-1} \cdot\big(T - \underbrace{\max_{j = 1, 2, 3} s_{b, j}}_{\text{with order } \log T}\big) \lesssim \log T.
\]
\begin{remark}
   Similarly, for specific reward distributions, we can bound $b_k$ in $\log T$ with some simple and specific coefficients. See Corollary \ref{cor_ber} and Corollary \ref{cor_gau}.
\end{remark}

Finally, {what} remains is to show {that} the restrictions (\ref{requirement_0}), (\ref{requirement_1}), (\ref{requirement_2}), (\ref{requirement_3}), and (\ref{requirement_4}) are compatible. Indeed, they will build the following system of constraints,
\[
    \left\{ \begin{array}{l}
         \frac{\mu_1}{2} - 2 C_1 \Delta_k \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
         2 C_2 \Delta_k + \frac{\mu_k}{2} \leq \frac{\mu_1 + \lambda}{1 + 2 \lambda} \\
        \tau_k - \frac{\mu_1}{2} - C_1 \Delta_k  \leq \tau_k + C_2\Delta_k - \frac{\mu_k }{2} \\
        C_1 \geq 2C_3 \\
        2 C_3 \geq C_2 \\
        \frac{\mu_1}{2} - 2 C_1 \Delta_k = 2 C_2 \Delta_k + \frac{\mu_k}{2}
    \end{array}\right..
\]
We can see that 
\[
    C_1 = C_2 = \frac{1}{8}, \qquad C_3 = \frac{1}{16},
\]
is the unique solution of the above system. Up to now, we have finished the first part in Theorem \ref{thm.MAB}. For the second part, 
\begin{equation*}
    \begin{aligned}
        \operatorname{Reg}_T & = \sum_{\Delta_k : \Delta_k < \Delta} \Delta_k \E J_{k, T} + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k \E J_{k, T} \\
        & \lesssim T \Delta + \sum_{\Delta_k : \Delta_k \geq \Delta} \Delta_k  +  \sum_{\Delta_k : \Delta_k \geq \Delta} \frac{\log T}{\Delta_k} \\
        & \lesssim T \Delta + \frac{ K \log T}{\Delta} \lesssim \sqrt{K T \log T}.
    \end{aligned}
\end{equation*}
for any previously specified $\Delta \in (0, 1)$ by Cauchy inequality. Therefore, we finish the proof of Theorem \ref{thm.MAB}.



%\textit{{Bounded case need to separate to prove?}}

%As all the restrict conditions for $C_1, C_2, C_3$ are exactly the same as previous, we still take $C_1 = C_2 = \frac{1}{8}$ and $C_3 = \frac{1}{16}$. And the final bounds need to be doubled.

\section{Proof of Corollary \ref{cor_ber}}

The similar as stated in Section \ref{proof_thm}. Take advantage of Bernoulli rewards are bounded in $[0, 1]$, one can get that 
\[
    \begin{aligned}
        a_{k, s} & \leq \big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ).
    \end{aligned}
\]
\todohw{Need to revise later}
as long as the parameters satisfying the restrictions in Theorem \ref{thm.MAB}. Then we need to control $a_{k, s, j}$ with $\log T$ for $j \in \{ 1, 2, 3\}$. These steps will be completed in the following.
\begin{itemize}
    \item For $a_{k, s, 1}$, recall the inequality \eqref{a_k_1_bound}. We use the fact that the rewards are bounded in $[0,1]$, Hoeffding inequality will give
    \[
        \pr (A_{1, s}^c) = \pr (\mu_1 - \overline{R}_{1, s} \geq (1 +2  \lambda) C_1 \Delta_k) \leq \exp \left\{ - 2 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2 s\right\}.
    \]
    Hence, take
    \[
        s \geq s_{a, 1} := \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} \log T,
    \]
    we have $\pr (A_{1, s}^c) \leq T^{-2}$ , and $a_{k, s, 1} \leq T^{-1}$ then.
    
    \item For $a_{k, s, 2}$, one can {follow} the same steps as in the proof of Theorem \ref{thm.MAB}, while constants in the upper bound can be simpler and sharper due to the distribution of rewards being Bernoulli.
    To be specific, the variance $\sigma_{\omega}^{-2} \var(f_1 + f_2 - f_3)$ in \eqref{bound_var_f} can be bound by a deterministic quantity:
    
    % \hl{Can not find this one by one. We should make sure the writing is readable, and then discuss the proof.}
    \[
        \begin{aligned}
            & \mathbb{G}_1 (s, \lambda) + \mathbb{G}_2 (s, \lambda) + g_3 (s, \lambda) \\
            \overset{\text{by the same steps in} \eqref{G_function_bound_2}}{\leq} & 6 \lambda^2 \sum_{i = 1}^s (R_{1, i} - \mu_1)^2 + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big] \\
            \overset{\text{use the fact } R_{1, i} \in [0, 1]}{\leq} & 6 \lambda^2 s + s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 1 ) + 3  (1 + 2\lambda)^2 C_3^2 \Delta_k^2 \big].
        \end{aligned}
    \]
    Then use \eqref{a_2_bound} again, 
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T  \E \exp \left\{ - \frac{9 C_3^2 (1 + 2\lambda)^2 \Delta_k^2 s^2 }{2 \sigma_{\omega}^{2} \big[ \mathbb{G}_{1}(s, \lambda) + \mathbb{G}_{2}(s, \lambda) + g_3 (s, \lambda) \big]}\right\} \\
            & \leq 2 T \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s}{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }\right\}.
        \end{aligned}
    \]
    Hence, if we take 
    \[
        \begin{aligned}
            s \geq s_{a, 2} & := \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log T \\
            (
            \text{require } T \geq 2) & \geq \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{9\sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} \log (2 T^2)
        \end{aligned}
    \]
    and then $a_{k, s, 2} \leq T^{-1}$.
    \iffalse
    Then if we denote 
    \[
        f(x) := \exp \left\{ - \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k^2 s}{4 \Big[ s^{- 1 / 2} (2 \lambda + 1) (x - s \mu_1) + \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] \Big]^2 + 2 s^{-1} g_5(s, \lambda) \big]^2} \right\},
    \]
    then $f(x)$ is a decreasing function on $0 \leq x \leq s \mu_1$ and an increasing function on $x \geq s \mu_1$. By symmetric technique of Binomial distribution and Lemma 2 in \cite{kveton2019garbage}, we have
    \[
        a_{k, s, 2} \leq {\red{4}} T \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x ; s, \mu_1) f(x) \leq 4 T \left[ \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s})+\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \right].
    \]
    Similarly to \cite{kveton2019garbage}, we can show that 
    \[
        \begin{aligned}
            & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] f(\mu_1 s -(i+1) \sqrt{s}) +\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            \leq & \sum_{i=0}^{\lfloor s \mu_1 \rfloor} \exp \left[-2 i^{2}\right] \exp \left\{- \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k^2 s}{4 \left[ \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] - (2 \lambda + 1) (i + 1)\right]^2 + 2 s^{-1} g_5(s, \lambda)} \right\} \\
            & \qquad +\exp \left[-2 s^{2} \mu_1^2 \right] f(0) \\
            \leq & \int_1^{s \mu_1 + 1} \exp \{ - 2 (u - 1)^2 \} \exp \left\{ - \frac{c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3}\right\}  \, du \\
            = & \int_1^{s \mu_1 + 1} \exp \left\{ - \left[ 2 (u - 1)^2 + \frac{c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3} \right] \right\}  \, du \\
            \leq & \int_1^{s \mu_1 + 1} \exp \left\{- \left[ 2 s^2 \mu_1^2 + \frac{c_1 s}{4(c_2 - (2 \lambda + 1) (s \mu_1 + 1))^2}\right] \right\} \, du \\
            \leq & \int_1^{s \mu_1 + 1} \exp \left\{ - 2 s \mu_1^2 \right\} \, du \leq T \mu_1 \exp \left\{ - 2 s \mu_1^2 \right\}
            %\leq & s \mu_1 \exp \left\{ - s \mu_1 \right\} \leq T \mu_1 \exp \{ - s \mu_1 \}
            % \leq & \left[ \int_1^{s \mu_1 + 1} \exp \{- 4 (u - 1)^2 \} \, du \right]^{1 / 2} \left[\int_1^{s \mu_1 + 1} \exp \left\{ - \frac{2c_1 s}{4 (c_2 - (2 \lambda + 1) u )^2 + 2 c_3}\right\} \, du \right]^{1 / 2} \\
            %= & \left[ \right] \exp 
        \end{aligned}
    \]
    with $c_1 = 64^{-1} (1 + 2 \lambda)^4 \Delta_k^2$, $c_2 = \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big]$, and $c_3 = \lambda^2 \big\{ \big[ (2 \mu_1 - 1) - C_3 (\lambda^{-1} + 2) \Delta_k \big]^2 + \big[ \mu_1 + C_3 (1 + 2 \lambda) \Delta_k - (1 + \lambda) \big]^2 \big\}$. Therefore, if $T \geq 2$, by taking 
    \[
        \red{s_{a, 2} \geq \frac{5 \log T}{\mu_1^2}\geq \frac{\log 4 T^3 \mu_1}{\mu_1^2}}
    \]
    one will have 
    \[
        a_{k, s, 2} \leq T^{-1}
    \]
    \fi
    \item To deal with $a_{k, s, 3}$,
    %recall we have bound $s^{-1} \var(f_1 + f_2 - f_3)$ with a constant times $s$. Then, 
    by taking the same technique as $a_{k, s, 2}$, we have
    \[
        \begin{aligned}
             \big[ 1 - Q_{1,s} (\tau_k)\big] \ind(A_{1, s}) \ind(G_{1, s}) & \leq \E \exp \left\{ - \frac{9 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 (- \Gamma_1)^2 s^2 }{ s \big[ 4 \lambda^2 (\lambda^2 + \lambda + 4)  + 6  (1 + 2\lambda)^2 (- \Gamma_1)^2  \big]}\right\} \\
             & \leq \exp \left\{ - \frac{144 \sigma_{\omega}^{-2} (1 + 2\lambda)^2 s }{ 4 \lambda^2 (\lambda^2 + \lambda + 4)  + 6  (1 + 2\lambda)^2 C_1^2 \Delta_k^2 }\right\} \leq T^{-2}
        \end{aligned}
    \]
    as long as 
    \[
        s \geq s_{a, 3} := \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \log T.
    \]
    \iffalse
    \[
        g(x) = \exp \left\{ - \frac{64^{-1} (1 + 2 \lambda)^4 \Delta_k s}{4 \Big[ s^{- / 2} (2 \lambda + 1) (x - s \mu_1) + \lambda \big[ (\lambda + \mu_1) + 4 (1 + 2 \lambda)\big] \Big]^2 + 2 s^{-1} g_5(s, \lambda)}\right\}
    \]
    one can show that
    \[
        \begin{aligned}
            \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq 2 \sum_{x = 0}^{\lfloor s \mu_1 \rfloor} B(x; s, \mu_1) g(x) \leq 2 s \mu_1 \exp \{ - s \mu_1\} \leq T^{-1}
        \end{aligned}
    \]
    as long as $s \geq s_{a, 3} := s_{a, 2}$. And hence, in this case, one will have $a_{k, s, 3} \leq T^{-1}$.
    \fi
\end{itemize}

Combining these results above with 
\[
    \begin{aligned}
        &\max \left\{ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2}, \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3\sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \right\} \\
        \leq & \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{4 \lambda^2 (\lambda^2 + \lambda + 4) + 6 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{-2} C_3^2 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2}\\
        = & \frac{36 (1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} + \frac{32^2 \lambda^2 \sigma_{\omega}^{2}  (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2},
    \end{aligned}
\]
we obtain that 
\[
    \begin{aligned}
        a_k & \leq \max_{s = 0, \ldots, T -  1} a_{k, s} \times\max _{j = 1, 2, 3} s_{a, j} + 3 T^{-1} \cdot\big(T - \max_{j = 1, 2, 3} s_{a, j}\big) \\
        & \leq \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big] \\
        & \qquad \qquad \times \left[  \frac{36 (1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{- 2}  (1 + 2 \lambda)^2} + \frac{32^2 \lambda^2 \sigma_{\omega}^{2}  (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2} \right] 
        \log T + 3.
    \end{aligned}
\]
%Specially, if $\sigma_{\omega}^2 \geq 1$ and $\lambda \geq 1$, by using the fact that $\lambda^2\big[ (\lambda - 1)^2 + \lambda^2\big] \geq \lambda (\lambda + 1)$, one will have 
%\[
    %a_k \leq  \left[ e^{ 3 (2\lambda + 1)^2 / 2} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right] \left[ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2} + \red{\frac{5}{\mu_1^2}}\right] \log T + 3.
%\]
By using the same technique, one can show that 
\[
    \begin{aligned}
        b_k & \leq 2 \times\max _{j = 1, 2, 3} s_{b, j} + 3 T^{-1} \cdot\big(T - \max_{j = 1, 2, 3} s_{b, j}\big) \\
        & \leq 2 \times \left\{ \frac{4}{(1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2 }{3 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2}, \frac{2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_2^2 \Delta_k^2}{36 \sigma_{\omega}^{-2} (1 + 2 \lambda)^2} \right\} \log T + 3 \\
        & \leq  2 \left[  \frac{18(1 + 2 \lambda)^2 + \lambda^2 (\lambda^2 + \lambda + 4)}{18 \sigma_{\omega}^{- 2}  (1 + 2 \lambda)^2} + \frac{2 \times16^2  \sigma_{\omega}^{2}  \lambda^2 (\lambda^2 + \lambda + 4) + 12}{3 (1 + 2 \lambda)^2 \Delta_k^2} + \frac{\sigma_{\omega}^{2} \Delta_k^2}{3 \times 16^2} \right] 
        \log T + 3
    \end{aligned}
\]
These results together with Lemma \ref{lem.a.b} give Corollary \ref{cor_ber}.

\section{Proof of Corollary \ref{cor_gau}}

The basic proof idea is the same as the proof of Corollary \ref{cor_ber}. Since the Gaussian variable is still sub-Gaussian, the constant bound in \eqref{a_k_constant_3} is still available for this case. And next we will bound $s_{a,  j} :=  \min \{ s: a_{k, s, j} \leq T^{-1}\}$ with $\log T$ under the Gaussian case.
%except the constant bound of $a_{k, s}$ is simpler due to the nice property of Gaussian distribution. And we follow the steps below:
\iffalse
\begin{itemize}
    \item[1.] By using the fact that $s^2 (\overline{R}_{1, s} - \mu_1) \sim \chi^2(s)$,
    \[
        \begin{aligned}
            a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\} \\
            & \leq 
        \end{aligned}
    \]
    \[
        \begin{aligned}
            a_{k, s} & \leq \E \exp \left\{ \frac{3 s (\overline{R}_{1, s} - \mu_1)^2}{2 \sigma_{\omega}^2 \left(  \overline{R}_{1, s} - \frac{\mu_1 + \lambda}{1 + 2 \lambda} \right)^2 }\right\} \times1 \left\{ \overline{R}_{1, s} - \mu_1 \geq \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \times1 \left\{ \overline{R}_{1, s} - \mu_1 < \frac{\sqrt{2 \pi}}{s (2 \lambda + 1)}\right\}  \\
            (\text{by using the MGF of } \chi^2(s))& = \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]s^2}\right]^{- \frac{s}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
            (\text{take } s = 1) & \leq \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}.
        \end{aligned}
    \]
    since $s = 0$ naturally satisfies the above inequality. This further implies we will need
    \[
        \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 \lambda^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]} < 1
    \]
    with its sufficient condition as 
    \[
        \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \leq 1
    \]
    i.e. $\lambda \geq 1 + \sqrt{2}$. In a word, under the assumptions in Corollary \ref{cor_gau}, one will have
    \[
        \begin{aligned}
            a_{k, s} & \leq \left[ 1 - \frac{3 (2 \lambda + 1)^2}{\sigma_{\omega}^2 [(\lambda + 1 - \mu_1)^2 + (\lambda + \mu_1)^2]}\right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \\
            & \leq \left[ 1 - \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1}. 
        \end{aligned}
    \]
    with $\sigma_{\omega}^2 \geq 1$ for $s \in \{ 0, \ldots, T - 1\}$.
    
    \item[2.] For controlling $a_{k}$, one can easily show that 
    \[
        a_k \leq \left\{ \left[ 1 - \frac{3(2 \lambda + 1)^2}{\lambda^2[\lambda^2 + (\lambda + 1)^2]} \right]^{- \frac{1}{2}} + \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \right\} \left[ \frac{65}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{6}{\log 2} \right] \log T + 3.
    \]
    by the following statements.
    \begin{itemize}
        \item[2.1] Still use sub-Gaussian inequality to get that we have $a_{k, s, 1} \leq T^{-1}$ when
        \[
            s \geq s_{a, 1} = \frac{64 }{(1 + 2 \lambda)^2 \Delta_k^2} \log T.
        \]
        
        \item[2.2] For dealing with $a_{k, s, 2}$, we again use the fact that 
        \[
            \Big[ \sqrt{s} (\overline{R}_{1, s} - \mu_1) + \lambda \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big] \Big]^2 \, \sim \, \chi^2(s; s^{-1}\lambda^2 \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k \big]^2 )
        \]
        is a noncentral chi-squared distribution, then it will lead to the result that 
        \[
            \begin{aligned}
                a_{k, s, 2} & \leq 2 T \E \exp \left\{ - \frac{64^{-1}(1 + 2 \lambda)^4 \Delta_k^2 s}{4\big[ \chi^2(s; s^{-1}\lambda^2 \big[ (\lambda + \mu_1) + 16^{-1} (1 + 2 \lambda) \Delta_k) + 2 s^{-1}g_5(s, \lambda)\big]}\right\} \\
                & \leq 2 T \E \exp \left\{ - \frac{64^{-1} (1 + 2\lambda)^4 \Delta_k^2 s}{4  \big[ \chi^2(s) + s^{-1}g_5(s, \lambda)\big]}\right\} \\
                & \leq 2 T \int_0^{\infty} \frac{2^{- s / 2}}{\Gamma(s / 2)} u^{-s / 2-1} e^{-1 /(2 u)} e^ { - 256^{-1} (1 + 2\lambda)^4 \Delta_k^2 s u} \, du \\
                (\text{by Cauchy inequality})& \leq  2 T \frac{2^{- s / 2}}{\Gamma(s / 2)}  \int_0^{\infty} u^{- s / 2 - 1} e^{- 1 / u} e^{- 16 (1 + 2 \lambda)^4 \Delta_k \sqrt{s}} \, du  \\
                & =  2 T \frac{2^{- s / 2}}{\Gamma(s / 2)}  \Gamma(s /2 ) e^{- 16 (1 + \lambda)^2 \Delta_k \sqrt{s}} \\
                & \leq 2 T \exp \left\{ - \left[ \frac{\log 2}{2} s + 16 (1 + 2 \lambda)^2 \Delta_k \sqrt{s}\right]\right\} \leq T^{-1}
            \end{aligned} 
        \]
        if 
        \[
            s \geq s_{a, 2} :=  \left[ \frac{1}{8(1 + 2 \lambda)^2 \Delta_k} + \frac{4}{\log 2}\right] \log T
        \]
        \item[2.3] Just by replacing $C_3 \Delta_k$ by $(- \Gamma_1)$ which is bounded in $(C_1 \Delta_k, 4)$, and we will get that
        \[
            \begin{aligned}
                \big[ 1 - Q_{1, s}(\tau_k)\big] 1(A_{1, s}) 1(G_{1, s}) \leq  \exp \left\{ - \left[ \frac{\log 2}{2} s + 16 (1 + 2 \lambda)^2 \Delta_k \sqrt{s}\right]\right\} \leq T^{-1}
            \end{aligned}
        \]
        i.e. $a_{k, s, 3} \leq T^{-1}$ whenever 
        \[
            s \geq s_{a, 3} := \left[ \frac{1}{16(1 + 2 \lambda)^2 \Delta_k} + \frac{2}{\log 2}\right] \log T.
        \]
    \end{itemize}
    
    \item[3.] Exactly the same as 2., we can get that 
    \[
        b_{k} \leq 2 \left[ \frac{33}{(1 + 2 \lambda)^2 \Delta_k^2} + \frac{6}{\log 2}\right] \log T + 3.
    \]
\end{itemize}
These results give Corollary \ref{cor_gau}.
\fi

\begin{itemize}
    \item For $a_{k, s, 1}$, we still use the same steps of proof in Theorem \ref{thm.MAB} directly: take
    \[
        s \geq s_{a, 1} = \frac{\sigma_1^2}{C_1^2 (1 + 2 \lambda)^2 \Delta_k^2} \log T,
    \]
    we have $a_{k, s, 1} \leq T^{-1}$.
    
    \item For $a_{k, s, 2}$, we note that
    \begin{equation}\label{chi_square}
    	\sum_{i = 1}^s (R_{1, i} - \mu_1)^2 = \sigma_1^2 \sum_{i = 1}^s \left( \frac{R_{1, i} - \mu_1}{\sigma_1} \right)^2 \, \sim \, \sigma_1^2 \chi^2(s).
    \end{equation}
    is a chi-square distribution.
    By using the density of chi-square distribution, we have a bound of \eqref{a_2_bound} as
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T \E \exp \left\{ - \frac{9 C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2}{2 \sigma_{\omega}^{2} \big[ \mathbb{G}_{1} (s, \lambda) + \mathbb{G}_{2} (s, \lambda) + g_3(s, \lambda)\big]}\right\} \\
            & \overset{\text{use the bound in \eqref{G_function_bound_2} and \eqref{chi_square}}}{\leq} 2 T \E \exp \left\{ - \frac{9 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2 s^2}{12 \lambda^2 \sigma_1^2 \chi^2(s) + 2 s \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big] }\right\} \\
            & =  2 T \int_0^{\infty} \exp \left\{ - \frac{D_1 s^2}{D_2 u + D_3}\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u / 2} \, du \\
            & = 2 T \int_0^{\infty} \exp \left\{ - \left[ \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \right]\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u / 4} \, du
        \end{aligned}
    \]
    %{\color{blue}{
    with
    \[
        D_1 = 9 \sigma_{\omega}^{- 2}  C_3^2 (1 + 2 \lambda)^2 \Delta_k^2, \qquad D_2 = 12 \lambda^2 \sigma_1^2, \qquad D_3 = 2 \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big].
    \]
    Write 
    \[
        \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} = D_4 s^2 + \frac{D_2 u^2 + (D_3 - 4 D_2 D_4 s^2) u + 4 (D_1 - D_3 D_4) s^2}{4 (D_2 u + D_3) }
    \]
    with $D_4 > 0$ is a constant making
    \begin{equation}\label{gau_D_4}
        D_2 u^2 + (D_3 - 4 D_2 D_4 s^2) u + 4 (D_1 - D_3 D_4) s^2 \geq 0
    \end{equation}
    strictly holds on $u \in (0, \infty)$. A sufficient condition for \eqref{gau_D_4} is
    \[
         \begin{aligned}
             \boldsymbol\Delta & = (D_3 - 4 D_2 D_4 s^2)^2 - 4 D_2 \big[ 4 (D_1 - D_3 D_4) s^2 \big] \\
             & = 16 D_2^2 D_4^2 s^4 + 8 D_2 (D_3 D_4 - 2) s^2 + D_3^2 > 0, \qquad s \in [T].
         \end{aligned}
    \]
    For ensuring the above holds, one only needs to ask
    \[
        D_3 D_4 -  2 \geq 0.
    \]
    Therefore, we choose 
    \[
        D_4 := \frac{2}{D_3} = \frac{1}{\big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big]}.
    \]
    and hence 
    \[
        \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \geq \frac{2}{D_3} s^2, \qquad \forall \, u > 0.
    \]
    It will furthermore give
    \[
        \begin{aligned}
            a_{k, s, 2} & \leq 2 T \int_0^{\infty} \exp \left\{ - \left[ \frac{D_1 s^2}{D_2 u + D_3} + \frac{u}{4} \right]\right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u  / 4}\, du \\
            & \leq 2 T \int_0^{\infty} \exp \left\{ - \frac{2 s^2 }{D_3} \right\} \frac{1}{2^{s / 2} \Gamma(s / 2)} u^{{s} / {2} - 1} e^{- u /4} \, du \\
            (\text{use the density of Gamma distribution})& = 2 T \exp \left\{ - \frac{2 s^2}{D_3} \right\} 2^{s / 2} \\
            & = 2 T \exp \left\{ -  \frac{2 s^2}{D_3} + \frac{s \log 2} {2} \right\} \leq 2 T \exp \left\{ -  \frac{2 s^2}{D_3} \right\} .
        \end{aligned}
    \]
    Hence, we can take
    \[
        s \geq s_{a, 2} := \frac{3 D_3 \log T}{2} = 3 \sigma_{\omega}^{2} \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_3^2 \Delta_k^2\big] \log T.
    \]
    to guarantee $a_{k, s, 2} \leq T^{-1}$ for any $T \geq 2$.
    \item The approach to deal with $a_{k, s, 3}$ is the same as above, and we can get we have $a_{k, s, 3} \leq T^{-1}$ whenever
    \[
        s \geq s_{a, 3} = 3  \sigma_{\omega}^{2}  \big[ 2 \lambda^2 (\lambda^2 + \lambda + 4) + 3 (1 + 2 \lambda)^2 C_1^2 \Delta_k^2\big] \log T.
    \]

    %}}
\end{itemize}

Combining the expressions of $a_{k, s, j}$, $j \in 1, 2, 3$, we obtain 
    \[
        \begin{aligned}
            a_{k} & \leq \Big[\big( e^{9 / 8} +  \big[ 1 - \Phi(\sqrt{2 \pi})\big]^{-1} \big) \ind ( \mu_1 \neq 1 / 2 )  + 2 \big( 1 + 2 e^{9 / 8} \big) \ind ( \mu_1 = 1/ 2 ) \Big] \\
            & \qquad \qquad \times \left[  \frac{16 \sigma_1^2}{(1 + 2 \lambda)^2 \Delta_k^2} + 12 \lambda^2  \sigma_{\omega}^{2} (\lambda^2 + \lambda + 4)  + \frac{153}{256} (1 + 2 \lambda)^2  \sigma_{\omega}^{2}  \Delta_k^2 \right] 
        \log T + 3.
        \end{aligned}
    \]
And similarly the bound of $b_k$ can be also proven as follows:
\[
     b_k \leq 2 \left[  \frac{16 \sigma_k^2}{(1 + 2 \lambda)^2 \Delta_k^2} + 9 \lambda^2  \sigma_{\omega}^2 (\lambda^2 + \lambda + 4)  + \frac{297}{512} (1 + 2 \lambda)^2 \sigma_{\omega}^{2} \Delta_k^2 \right] \log T + 3.
\]

==> ARCHIVE/advances.tex <==
% \cite{vaswani2018new} throw an insight for how to theoretically analyze the cumulative regret under nonasymptotic sense at Bootstrap framework. Here the nonasymptotic means we can get the relationship of the regret and the round $T$ exactly. 


% In summary
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \todorw{These approaches are bootstrapping-based TS/UCB-type algorithms. They are very different from TS/UCB themselves. Besides, the argument below is unclear why Bootstrapping-UCB is more restricted. E.g., is is only applicable to some problem? Does it rely on some tuning parameter that is unknown to the user?}

% It is worthy to note that for a specific problem, i.e. MAB with some particular type of random rewards, the UCB method is partly restricted. This is by the fact that once we got the Bootstrap upper bound with weights $\mathbf{w}_n = (w_1, \ldots, w_n)^{\top} \in \mathbb{R}^n$ such that
% \begin{equation*}
%     \pr_{\mathbf{R}_{k, n}} \left[ \frac{1}{n} \sum_{i = 1}^n R_{k, i} - \mu_k > q_{\alpha} (\mathbf{R}_{k, n}, \mathbf{w}_n)\right] \leq \alpha,
% \end{equation*}
% then that the algorithm will be exactly become $I_t = \arg \max_{k \in [K]}  \left[ \frac{1}{n} \sum_{i = 1}^n R_{k, i} + q_{\alpha} (\mathbf{R}_{k, n}, \mathbf{w}_n) \right]$ with some pre-specific $\alpha \asymp o(T^{-1})$. In the contrast, TS method can vary widely since there are many choices of the Bayesian posterior $P_{\omega_k}$, we conclude the existing literature is listed in chronological order as follows

% \begin{itemize}
    % \item pioneers this line of research and proposes ensemble sampling, where we maintain $M$ models  is the first one to that put TS and try to theoretically analyze the regret in the Bandit problem. However, their results are neither nonasymptotic and problem specific.
    % \item \cite{vaswani2018new} throw an insight for how to theoretically analyze the cumulative regret under nonasymptotic sense at Bootstrap framework. Here the nonasymptotic means we can get the relationship of the regret and the round $T$ exactly. 
    % \item \cite{kveton2019garbage} is the pioneer, which exactly use the TS to achieve the optimal rate. It adds $a$ pseudo rewards from $(0, 1)$ with tuning parameter $a$ on each arm's history, and prove this method guarantees an $\log T$ under Bernoulli rewards on $\{ 0, 1\}$;
    
    % \item is the pioneer, which exactly use the TS to achieve the optimal rate. It adds $a$ pseudo rewards from $(0, 1)$ with tuning parameter $a$ on each arm's history, and prove this method guarantees an $\log T$ under Bernoulli rewards on $\{ 0, 1\}$;

    % \item \cite{kveton2019perturbed} again uses another Bayesian posterior to deal with the same problem with \cite{kveton2019perturbed}: it adds $a$ Bernoulli perturbation at each reward step, the $a$ is again the tuning parameter. It is worthy to note that this method is quite similar to \cite{kveton2019garbage} sharing with the same condition (under some transformation);
    
    % \item \cite{wang2020residual} construct another Bayesian posterior based on the residuals $R_{k, i} - \overline{R}_{k}$, extended the existent theory and the optimal rate $\log T$ to a specific unbound reward, Gaussian setting. Their theory is exactly based on the exact tail of Gaussian distribution.
% \end{itemize}

% Another essential aspect for an algorithm is computation cost and storage cost. Hence, we have to study these costs of the existent literature which achieves the optimal convergence rates. As we can see, \cite{kveton2019garbage} and \cite{kveton2019perturbed} need to add $a$ pseudo random quantile at each round, their storage cost and computation cost are $\mathcal{O}(T), \mathcal{O} (T^2)$ and $\mathcal{O}(T), \mathcal{O} (KT)$ representatively. While \cite{wang2020residual} achieves the rate $\mathcal{O}(T), \mathcal{O} (KT)$, while they need some extra steps to compute the residuals. 



% \textbf{Advances of our proposed method. }
% Compared with the existing methods, our main advantages include
% \begin{itemize}
%      \item[1.] Our method is directly base on TS method, no other transformation like in \cite{wang2020residual} is required. And our storage cost and computation cost are also $\mathcal{O}(T), \mathcal{O} (KT)$, exactly the same as the existent best storage and computation cost talked in \cite{wang2020residual}.
    
%     \item[2.] Our theoretical analysis is mainly dependent on the tail probability of the Bootstrap weights $\boldsymbol\omega$, as long as the rewards are bounded, our method can be applied while other literature require the rewards satisfies the specific distribution which is hard to verify in practice.
    
%     \item[3.] Our method can be easily extended to linear bandit and more complex setting, while \cite{wang2020residual}'s method requires extra techniques (ridge tuning will be introduced) to apply in linear bandit problem. \blue{ridge is part of linear regression, not an additional step. }
    
%     \item[4.] The tuning parameter in our method is only required to be positive, i.e. any positive parameter can guarantee the optimal rate. However, other algorithms need the tuning parameter satisfies some specific restriction that related to the underling distribution of the rewards.
%      \blue{This is just a difference, not advantage. E.g., if one algorithm requires $\lambda = 1$ to be optimal, it is fine, as long as this requirement is known to the user a priori. }
% \end{itemize}




==> Alg/alg_expert.tex <==
\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
Function class $\Pi$, 
loss function $\mathcal{L}$, 
multiplier weight distribution $\rho(\omega)$, 
tuning parameter $\lambda$
}

\todorw{Wrong yet. }

Set $\his = \{\}$ be the history and $\his' = \{\}$ be the pseudo-history

Initialize $\hat{f}$  in an optimistic way
% of the arm $k$, $c_k = 0$ ,and $\overline{Y}_{k} = +\infty, \forall k \in [K]$

\For{$t = 1, \dots, T$}{

    Observe context $\vx_t$ and action set $\mathcal{A}_t$

    Offer $A_t = \hat{\pi}(\vx_t)$ (break tie randomly)

    Observe reward $R_t$
    
    Update $\his = \his \cup \{(\vx_t, A_t, R_t)\}$
    
    Update $\his' = \his' \cup \{(\vx_t, A_t, 0), (\vx_t, A_t, 1)\}$

    
    Sample the multiplier weights $\{\omega_l, \omega'_l, \omega''_l\}_{l=1}^t \sim \rho(\omega)$
    
    Solve the weighted loss minimization problem to update $\hat{\pi}$ as
    \begin{align*}
        \hat{\pi} = \argmin_{\pi \in \Pi} \mathcal{L}\big( \{ 
        (\vx_l, A_l, R_l, \omega_l)
        , (\vx_l, A_l, 0, \lambda \omega'_l)
        , (\vx_l, A_l, 1, \lambda \omega''_l)
        \}_{l=1}^t \big)
    \end{align*}
} 
% Multiplier Bootstrap-based Thompson Sampling
\caption{General Template for \name{MBTS} (expert-version) }\label{alg:MBTS-expert}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Alg/main_alg_GP.tex <==
\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
number of bootstrap repetitions $B$,
number of arms $K$, 
multiplier weight distribution $\rho(\omega)$
}

Sample 
$\boldsymbol{\omega}^{b}_k \sim \rho(\omega), \forall k \in [K], b \in [B]$ 

Initialize $\mD^b = \{(\vx_k, \boldsymbol{\omega}^{b}_k)\}_{k \in [K]}, \forall k \in [K]$

Train a kernel function $\mathcal{f}^b$ based on $\mD^b$



\For{t = 1, \dots, T}{
    Observe the candidate arms $\mA_t$

    Sample the index $b_t$ uniformly from $\{1, \dots, B\}$
    
    Offer $\vx_t = \argmax_{\vx \in \mA_t} \hat{\vthe}^T_b \vx$

    Observe reward $R_t$

    \For{b = 1, \dots, B}{
    Sample the multiplier weight $\omega_b \sim \rho(\omega)$
    
    Update $\textbf{G}_b = \textbf{G}_b + \omega_b \vx_t \vx^T_t$ 
    and $\textbf{Z}_b = \textbf{Z}_b + \omega_b \vx_t R_t$
    % the empirical covariance matrix as 
    
    Update $\hat{\vthe}^T_b = \textbf{G}_b^{-1} \textbf{Z}_b$
    }

}
% a fixed set of arms and 
 \caption{Multiplier Bootstrap-based Thompson Sampling for kernel bandits with 
 a fixed set of arms and 
 with 
 reward in $[0, 1]$ }\label{alg:MBTS-LB}
\end{algorithm}


==> Alg/main_alg_MAB.tex <==
\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
number of arms $K$, 
multiplier weight distribution $\rho(\omega)$
}

Set $\mH_{a, s}$ is the history of the arm $a$ up to round $s$. and $\Bar{Y}_a = 1, \forall a \in [K]$

\For{t = 1, \dots, T}{

    Offer $A_t = \argmax_{a \in [K]} \Bar{Y}_a$ (break tie randomly)

    Observe reward $R_t$

    \For{a = 1, \dots, K}{
    Sample the multiplier weights $\{\omega_l\}_{l=0}^{|\mH_a|} \sim \rho(\omega)$. {\color{blue}{Note that $\E \omega_{\ell}$ should be equal to one to ensure the consistency.}}
    
    Update the mean reward $\Bar{Y}_{a} = (0 + \omega_0 * \lambda_1 + \sum_{l=1}^{|\mH_a|} \omega_l R_a^l
    ) / (\sum_{l=0}^{|\mH_a|} \omega_l + \lambda_2)$, where $R_a^l$ is the $l$th element of $\mH_a$
    }
    
}

 \caption{Exact Version: Multiplier Bootstrap-based Thompson Sampling for MAB with $[0, 1]$ rewards}\label{alg:MBTS-MAB}
\end{algorithm}

\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
number of bootstrap repetitions $B$,
number of arms $K$, 
multiplier weight distribution $\rho(\omega)$
}
\For{b = 1, \dots, B}{
    \For{k = 1, \dots, K}{
        Sample a multiplier weight $\omega_{b,k} \sim \rho(\omega)$

        Add two pseudo rewards $0$ and $1 \times \omega_{b,k}$ to initialize the counter as $\Bar{Y}^{b}_{k} = (0 + \omega_{b,k}) / 2$
    }
}

Initialize the counter as $c_{k} = 2, \forall k \in [K]$

\For{t = 1, \dots, T}{
    Sample the index $b_t$ uniformly from $\{1, \dots, B\}$
    
    Offer $A_t = \argmax_{a \in [K]} \Bar{Y}^{b_t}_a$

    Observe reward $R_t$

    \For{b = 1, \dots, B}{
    Sample the multiplier weight $\omega_b \sim \rho(\omega)$
    
    Update the mean reward $\Bar{Y}^{b}_{A_t} = (\Bar{Y}^{b}_{A_t} * c_{A_t} + R_t * \omega_b) / (c_{A_t} + 1)$
    
    }

    Update the counter as $c_{A_t} = c_{A_t} + 1$

}

 \caption{Multiplier Bootstrap-based Thompson Sampling for MAB with $[0, 1]$ rewards}\label{alg:MBTS-MAB}
\end{algorithm}

\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
number of bootstrap repetitions $B$,
number of arms $K$, 
multiplier weight distribution $\rho(\omega)$
}
\For{b = 1, \dots, B}{
    \For{k = 1, \dots, K}{
        Sample a multiplier weight $\omega_{b,k} \sim \rho(\omega)$

        Add two pseudo rewards $0$ and $1 \times \omega_{b,k}$ to initialize the counter as $\Bar{Y}^{b}_{k} = (0 + \omega_{b,k}) / 2$
        
        Initialize the counter as $c^b_{k} = 1 + \omega_{b,k}$
    }
}



\For{t = 1, \dots, T}{
    Sample the index $b_t$ uniformly from $\{1, \dots, B\}$
    
    Offer $A_t = \argmax_{a \in [K]} \Bar{Y}^{b_t}_a$

    Observe reward $R_t$

    \For{b = 1, \dots, B}{
    Sample the multiplier weight $\omega_b \sim \rho(\omega)$
    
    Update the mean reward $\Bar{Y}^{b}_{A_t} = (\Bar{Y}^{b}_{A_t} * c^b_{A_t}  + R_t * \omega_b) / (c^b_{A_t}  + \omega_b)$
    
    Update the counter as $c^b_{A_t} = c^b_{A_t} + \omega_{b}$

    }
    

}

 \caption{Multiplier Bootstrap-based Thompson Sampling for MAB with $[0, 1]$ rewards}\label{alg:MBTS-MAB}
\end{algorithm}





==> Fig/fig_MAB.tex <==
\begin{figure*}[t]
 \centering
 \includegraphics[width=\textwidth, height = 4cm]{Fig/MAB.pdf}
%  \vspace{-.5cm}
 \caption{Simulation results with a fixed and finite set of arms. (TBD: linear Gaussian)}
\label{fig:MAB}
\end{figure*}


% \begin{figure*}[t]
%      \centering
%  \begin{subfigure}[b]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, height = 3cm]{Fig/Bernoulli.png}
%         %   \vspace{-.5cm}
%      \caption{Bernoulli MAB.}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, height = 3cm]{Fig/Gaussian.png}
%         %   \vspace{-.5cm}
%      \caption{Gaussian MAB.}
%  \end{subfigure}
%   \begin{subfigure}[b]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, height = 3cm]{Fig/Bernoulli_LB.png}
%         %   \vspace{-.5cm}
%      \caption{Bernoulli linear bandits.}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, height = 3cm]{Fig/Gaussian_LB.png}
%         %   \vspace{-.5cm}
%      \caption{Gaussian linear bandits.}
%  \end{subfigure}
% %  \vspace{-.5cm}
%  \caption{Simulation results with a fixed and finite set of arms.}
% \label{fig:MAB}
% \end{figure*}


==> Mis/new_commands.tex <==
\newcommand{\lam}{\lambda}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\vlam}{\boldsymbol{\lam}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\vM}{\boldsymbol{M}}
%%%%%%%%%%%%%%%%%%%%
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vY}{\boldsymbol{Y}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vgamma}{\boldsymbol{\gamma}}

\newcommand{\hRI}{\widehat{RI}}
\newcommand{\vthe}{\boldsymbol{\theta}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\mR}{\mathcal{R}}

\newcommand{\TO}{\tilde{O}}

\newcommand{\indep}{\perp \!\!\! \perp}
% \newcommand{\Y}[1]{Y^*(#1)}
\newcommand{\Yz}{Y^*(0)}
\newcommand{\Yzi}{Y_i^*(0)}

\newcommand{\Yo}{Y^*(1)}
\newcommand{\Yoi}{Y_i^*(1)}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mE}{\mathbb{E}} 
\newcommand{\vxi}{\mathbf{x}_i} 
\newcommand{\vxj}{\mathbf{x}_j} 
\newcommand{\vc}{\mathbf{c}}
\newcommand{\veps}{\mathbf{\epsilon}}
\newcommand{\vdelta}{\boldsymbol{\delta}}


\newcommand{\dopt}{d^{opt}} 

\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vJ}{\boldsymbol{J}}


\newcommand{\E}{{\mathbb{E}}}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\his}{\mathcal{H}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\neigh}{\mathcal{N}}
\newcommand{\ber}{\operatorname{ber}}

\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\vS}{\boldsymbol{S}}
\usepackage{soul}
\usepackage{xcolor}
\newcommand{\tH}{\tilde{H}}
\newcommand{\Mean}{{\mathbb{E}}}
\newcommand{\Var}{{\mathbb{VAR}}}
% \newcommand{\Cov}{{\mathbb{COV}}}
\newcommand{\Cov}{\boldsymbol{\Sigma}}

\newcommand{\prob}{\mathbb{P}}

\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vPhi}{\boldsymbol{\Phi}}
\newcommand{\vR}{\boldsymbol{R}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vone}{\boldsymbol{1}}
\newcommand{\vzero}{\boldsymbol{0}}
\newcommand{\vI}{\boldsymbol{I}}
\newcommand{\vmu}{\boldsymbol{\mu}}

\newcommand{\mX}{\boldsymbol{X}}
\newcommand{\mK}{\boldsymbol{K}}
\newcommand{\mZ}{\boldsymbol{Z}}
\newcommand{\mU}{\boldsymbol{U}}
\newcommand{\mW}{\boldsymbol{W}}
\newcommand{\mV}{\boldsymbol{V}}



\usepackage{amsthm}
\usepackage[amsmath]{ntheorem}
\makeatletter
\renewtheoremstyle{plain}%
  {\item[\hskip\labelsep \theorem@headerfont ##1\ ##2\theorem@separator]}%
  {\item[\hskip\labelsep \theorem@headerfont ##1\ ##2, ##3\theorem@separator]}
\makeatother
\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{asmp}{Assumption}
% \newtheorem*{remark}{Remark}
\newtheorem{remark}{Remark}


==> cb_table.tex <==
\begin{table*}[t!]
\caption{Contextual bandits. 
}
\label{tab:comparison}
\centering
\begin{tabular}{lllll}
\hline
& Mushroom
& Mushroom
& Mushroom
& Mushroom 
\\ \hline
\name{MBE} ($\sigma_\omega = 0.1$, $\lambda = 0.1$)  &   &  &   &  \\ 
\name{MBE} ($\sigma_\omega = 0.1$, $\lambda = 0.1$)  &   &  &   &  \\ 
\name{MBE} ($\sigma_\omega = 0.1$, $\lambda = 0.1$)  &   &  &   &  \\ 
\hline
LinearTS  &   &  &   &  \\ 
GP  &   &  &   &  \\ 
% \hline
\hline % finite-arm (x)         
%(\cite{jin2022finite} \cite{jin2021mots})
\end{tabular}

% TODO: add more without theoretical guarantee, o.w., our advantage on this is limited. 
% Hopefully, we can get more advantage in reward assumption.}

\end{table*}

